Breakdown of homoclinic orbits to L3 in the RPC3BP (I). Complex singularities and the inner equation

The Restricted 3-Body Problem models the motion of a body of negligible mass under the gravitational influence of two massive bodies, called the primaries. If the primaries perform circular motions and the massless body is coplanar with them, one has the Restricted Planar Circular 3-Body Problem (RPC3BP). In synodic coordinates, it is a two degrees of freedom Hamiltonian system with five critical points, L1,..,L5, called the Lagrange points. The Lagrange point L3 is a saddle-center critical point which is collinear with the primaries and is located beyond the largest of the two. In this paper and its sequel, we provide an asymptotic formula for the distance between the one dimensional stable and unstable invariant manifolds of L3 when the ratio between the masses of the primaries $\mu$ is small. It implies that L3 cannot have one-round homoclinic orbits. If the mass ratio $\mu$ is small, the hyperbolic eigenvalues are weaker than the elliptic ones by factor of order $\sqrt{\mu}$. This implies that the distance between the invariant manifolds is exponentially small with respect to $\mu$ and, therefore, the classical Poincar\'e--Melnikov method cannot be applied. In this first paper, we approximate the RPC3BP by an averaged integrable Hamiltonian system which possesses a saddle center with a homoclinic orbit and we analyze the complex singularities of its time parameterization. We also derive and study the inner equation associated to the original perturbed problem. The difference between certain solutions of the inner equation gives the leading term of the distance between the stable and unstable manifolds of L3. In the sequel we complete the proof of the asymptotic formula for the distance between the invariant manifolds.

==> Article Inner/PoincareCoordinates.tex <==
\paragraph{Delaunay coordinates.}

The Delaunay elements,
denoted $(\ell,L,\hat{g},G)$,
are action--angle variables for the $2$-Body Problem (for negative energy) in non-rotating coordinates.
%
The variable $\ell$ is the mean anomaly, 
$\hat{g}$ is the argument of the pericenter,
$L$ is the square root of the semi major axis and $G$ is the angular momentum,
(see~\cite{MeyerHallOffin}).
%

Let us introduce some formulae to describe these elements from the non-rotating polar coordinates $(r,\hat{\tht},R,G)$, namely $\hat{\tht}={\tht}+t$. 
%
The action $L$ is defined by
\begin{equation*}
-\frac{1}{2L^2} =
\frac{1}{2} \paren{ R^2 + \frac{G^2}{r^2} } - \frac{1}{r},
\end{equation*}
%However, since $\phi_{\Del}$ does not have an explicit expression, the perturbation term $\mu \wt{H}_1$,as defined in~\eqref{eq:RShamiltonianInitial1}, does not have an explicit form.
%
and the (osculating) eccentricity of the body is expressed as 
\begin{equation}\label{def:eccentricityDelaunay}
e = \sqrt{1-\frac{G^2}{L^2}}
= \frac{\sqrt{(L-G)(L+G)}}{L}.
\end{equation} 
%
Let us recall now the ``anomalies'': the three angular parameters that define a position at the (osculating) ellipse. These are the mean anomaly $\ell$,  the eccentric anomaly $u$, and the true anomaly $f$, which satisfy
\begin{equation}\label{eq:rthetaDefinition}
r = L^2(1-e\cos u) \qquad
\text{ and } \qquad 
\hat{\tht} = f + \hat{g}.
\end{equation}
%
To use these elements in a rotating frame, we consider rotating Delaunay coordinates $(\ell,L,g,G)$, where the new
angle is defined as $g=\hat{g}-t$ (the argument of the pericenter with respect to the line defined by the primaries $S$ and $J$).
%
As a result, %the argument on rotating coordinates is given by  
\begin{equation}\label{eq:thetaDefinition}
{\tht} = f + {g},
\end{equation}
and the unperturbed Hamiltonian $H_0^{\pol}$ becomes
\[
H_0^{\pol} = -\frac{1}{2L^2} - G.
\]
%
The eccentric and true anomalies are related by 
\begin{equation}\label{eq:fTrigDefinition}
\cos f=\frac{\cos u-e}{1-e\cos u}, 
\qquad
\sin f=\frac{\sqrt{1-e^2}\sin u}{1-e\cos u},
\end{equation}
and the mean anomaly $u$ is given by Kepler's equation
\begin{equation}\label{eq:uImplicitDefinition}
u-e \sin u = \ell.
\end{equation}
%
The critical point $L_3$ (see~\eqref{def:pointL3}) satisfies $\tht = \ell + g = 0$ and
\begin{equation}\label{eq:pointL3Delaunay}
%\ell+g=0, \quad 
%
L = \sqrt{\frac{d_{\mu}}{2-d^3_{\mu}}}
= 1 + \OO(\mu), \qquad
%
G = d^2_{\mu}
= 1  + \OO(\mu), \qquad
%
L- G = \OO(\mu^2).
\end{equation}
Note that the Delaunay coordinates are not well defined for circular orbits ($e=0$), since the pericenter, and as a consequence the angle $g$, are not well defined.

%and the resonant zone takes place at $(L,G)\sim (1,1)$, as $\mu \to 0$.
%
%Our study focuses on a particular region of the resonance $1:1$, the one that includes $L_3$, which corresponds to orbits close to circular, such that $0 < \vabs{L-G} \ll 1$. 
%Thus, taking e = 0, we see that L3 takes place at (L;G) = (1; 1). 
%

%see~\cite{MeyerHallOffin}. 
%Thus, this means that we focus on the orbits close to circular, $0 < e \ll 1$.
%
%The planar Delaunay elements, denoted by $(\ell,L,\hat{g},G)$, are defined as
%\begin{itemize}
%	\item[--] The mean anomaly $\ell$: It can be defined as the ratio of the area sector swept to the total area, and normalized by $2\pi$.
%	\item[--] The argument of the pericenter $g$: 
%	Since we are in rotating coordinates, this argument is with respect to the line between the primaries: $S$ and $J$. 
%	%It can expressed as $g=\tht - f$, where $f$ is the true anomaly.
%	\item[--] The square root of the semi-major axis $L$. %of the elliptic orbit,
%	\item[--] \textcolor{red}{The angular momentum $G$.}
%\end{itemize}
%
%This set of variables defines a symplectic change of variables from polar coordinates:
%\begin{equation*}
%\phi_{\Del}: (\ell,L,g,G) \mapsto (r,\tht,R,G).
%\end{equation*}
%with symplectic normal form $d\ell \wedge dL + dg \wedge dG$. 
%
%, see Figure~\ref{fig:Delaunay}.
%\begin{figure}
%	\centering
%	\begin{overpic}[scale=0.7]{delaunay.png}
%		\put(45,43){{\color{blue} $S$ }}
%		\put(42,68){{\color{myGreen} $\ell$ }}
%		\put(19,58){{\color{blue} $q(t)$ }}
%		\put(62,52){{\color{myOrange} $g$ }}	
%		\put(76,68){{\footnotesize \color{myOrange} pericenter}}
%		\put(-13,11){{\footnotesize \color{myOrange} apocenter }}	
%		\put(102,48){$\Re(q)$}
%		\put(45,88){$\Im(q)$}	
%	\end{overpic}
%	\caption{Representation of the Delaunay planar elements for the unperturbed system, $\mu=0$, on Cartesian coordinates. }
%	\label{fig:Delaunay}
%\end{figure}
%

\paragraph{Poincar\'e coordinates.}

To ``blow-down'' the singularity of the Delaunay coordinates at circular motions,
we use the classical Poincar\'e coordinates, which can be expressed  by means of (rotating) Delaunay variables.
%
Let us define
\begin{equation}\label{def:changePoincare}
\phi_{\Poi}: (\la, L, \eta, \xi) \mapsto
(r, \tht, R,G) ,
\end{equation}
given by
\begin{equation}\label{def:changePoincare2}
\begin{aligned}
\la=\ell+g, \qquad  
\eta=\sqrt{L-G} e^{i g}, \qquad
\xi= \sqrt{L-G} e^{-i g}.
\end{aligned}
\end{equation}
% where $(\ell,g,L,G)$ are the Delaunay variables.
%
These coordinates are symplectic and analytic. 
%
Moreover, even though they are defined through the Delaunay variables, they are also analytic when the eccentricity tends to zero (i.e at $L=G$), see~\cite{MeyerHallOffin, Fejoz2013}.
%
%Roughly speaking, this change of variables assumes that $(\sqrt{L-G}, g)$ acts similarly to polar coordinates, where the angle $g$ is not defined when the ``radius'' is $\sqrt{L-G} = 0$. To solve the issue, it applies a change back to the corresponding ``Cartesian'' coordinates.

The Hamiltonian equation associated to~\eqref{def:hamiltonianPolars}, expressed in Poincar\'e coordinates, defines a Hamiltonian system with respect to the symplectic form $d\la \wedge dL + i \h d\eta \wedge d\xi$ and
\begin{equation*} %\label{def:hamiltonianPoincare}
H^{\Poi} = H_0^{\Poi}
+ \mu H_1^{\Poi},
\end{equation*}
where
\begin{equation}\label{def:hamiltonianPoincareSplitting}
\begin{split}
H_0^{\Poi}(L,\eta,\xi) = -\frac{1}{2L^2} - L +  \eta \xi 
%
\qquad \text{and} \qquad
%
H_1^{\Poi} = H_1^{\pol} \circ \phi_{\Poi}.
\end{split}
\end{equation}
%
%Since Delaunay variables are not explicit, neither is the Poincar\'e change of coordinates: $\phi_{\Poi}$. As a result, $H^{\Poi}_1$ does not have an explicit expression. 
%
%However, we can obtain a series expression on an appropriate domain. See Lemma~\ref{lemma:seriesH1Poi}.
%
%Let us consider the equilibrium point $L_3^{\mu}$, as expressed in~\eqref{def:pointL3} then, applying the formulae in Section~\ref{section:proofB-poincareFormulas}, it can be seen that
%\begin{equation}\label{eq:fixedPointL3Poi}
%\phi_{\Poi}(L_3^{0}) = (0,1,0,0).
%\end{equation}
%
In Poincar\'e coordinates, the critical point $L_3$, as given in~\eqref{eq:pointL3Delaunay}, satisfies
\[
\la=0, \qquad
(L,\eta,\xi) = (1,0,0) + 
\OO(\mu).
\]
%
%The unperturbed Hamiltonian $H_0^{\Poi}$ has a circle of equilibrium point at $(\la,1,0,0)$. 
%
The linearized part of the vector field associated to this point has, at first order, an uncoupled nilpotent and center blocks,
\begin{equation*}
\begin{pmatrix}
0 & -3 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & i & 0 \\
0 & 0 & 0 & -i
\end{pmatrix} + \OO(\mu).
\end{equation*}
%
The center is found on the projection to coordinates $(\eta,\xi)$ and the degenerate behavior on the projection to $(\la,L)$. 
%
%Moreover, the degeneracy is found on the component $L$ of the vector field.
%
%Therefore, we scale the coordinates to obtain a suitable first order with a non-degenerate saddle.

The perturbative term $\mu H_1^{\Poi}$ is not explicit. 
%
We overcome this problem by computing the first terms of the series of $\mu H_1^{\Poi}$ in powers of $(\eta,\xi)$, (see Lemma~\ref{lemma:seriesH1Poi}).
%
%We use this result extensively through this document and~\cite{?}.

Notice that, on the original coordinates, Hamiltonian $h$ (see~\eqref{def:hamiltonianInitialNotSplit}) is analytic at points away from collision with the primaries.
%
However, the collisions are not as easily defined in Poincar\'e coordinates. %(See Remark~\ref{remark:seriesH1Poi}).


%In particular, for $(L,\eta,\xi)\sim(1,0,0)$, $\vabs{\Im \la}$ bounded and $\mu \geq 0$ small enough, we can see that 
%%
%there exists a constant $\cttInnPoiA=\cttInnPoiA(\mu)>0$ such that 
%%
%the Hamiltonian $H^{\Poi}$ is analytic
%%
%for $\vabs{\la-\pi}>\cttInnPoiA$.
%%
%See Corollary~\ref{corollary:HPoiAnalytic} for the details.


%In particular, we consider the Poincar\'e complex change of coordinates $\phi_{\Poi}:(r,\tht,R,G)  \to (\la, L, \eta, \xi) \in \torus \times \reals^3$ given by
%\begin{align}\label{def:changePoincare}
%%\left\{ \begin{array}{ll}
%\la=\ell+g, \hh  
%\eta=\sqrt{L-G} e^{i g}, \hh
% \xi= \sqrt{L-G} e^{-i g},
%%\end{array} \right.
%\end{align}
%we analyze the resonance where the asteroid and the primaries have the same period (mean motion resonance $1:1$), specifically at the $L_3$ point. 
%\begin{align*}
%\phi_{\Poi}: \wt{D}_s \subset \reals^2 \times \reals^2 &\to \torus \times \reals^3  \\
%(q,p) &\mapsto (\la, L, \eta, \xi)
%\end{align*}
%where $\ell$ is the mean anomaly, $g$ the argument of the perihelion, $L$ the mean longitude and $G$ the angular momentum.  
%See Section~\ref{section:proofB-poincareFormulas} for further details on these coordinates. 


==> Article Inner/commands.tex <==
%%%%%%%%%%%%%%%%%%%
% LATEX SHORTCUTS %
%%%%%%%%%%%%%%%%%%%

% EDITION
\def\singlespace{ \renewcommand{\baselinestretch}{1.0}\normalsize }
\def\middlespace{ \renewcommand{\baselinestretch}{1.3}\normalsize }
\def\doublespace{ \renewcommand{\baselinestretch}{2.0}\normalsize }
%\newcommand{\st}{\text{ : }}
\newcommand{\st}{\h:\h}
\newcommand{\stb}{\text{ }\big\rvert \text{ }}
\newcommand{\h}{\hspace{1mm}}
\newcommand{\hh}{\hspace{5mm}}
\newcommand{\pp}{\\[0.6em]}
\newcommand{\dps}{\displaystyle}
\newcommand{\coma}{\text{, \h }}
\newcommand{\dpf}[2]{\left( \frac{#1}{#2} \right)}
\newcommand{\idk}[1]{\mathbf{1}_{\{k=#1\}}}
\newcommand{\efr}[2]{^{\frac{#1}{#2}}}
\newcommand{\mefr}[2]{^{-\frac{#1}{#2}}}

% THEOREMS
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{theorem}[lemma]{Theorem}
%\theoremstyle{remark}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{example}[lemma]{Example}
%\theoremstyle{definition}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{notation}[lemma]{Notation}
\newtheorem{comentary}[lemma]{Comentary}
\def\figlabel#1{\label{#1}}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\beal{\begin{aligned}}
\def\enal{\end{aligned}}

% BASICS
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\normf}[1]{\llbracket#1\rrbracket}
\newcommand{\vabs}[1]{\left| #1 \right|}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\claus}[1]{\left\{#1\right\}}
\newcommand{\boxClaus}[1]{\left[#1\right]}
\newcommand{\ii}{^{-1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\tl}{\tilde}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\renewcommand{\Re}{\mathrm{Re\, }}
\renewcommand{\Im}{\mathrm{Im\,}}
\renewcommand{\arg}{\mathrm{arg\,}}
\renewcommand{\inf}{\mathrm{inf\,}}

% SPACES
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\complexs}{\mathbb{C}}
\newcommand{\torus}{\mathbb{T}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\field}{\mathbb{F}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\scalarField}{\mathbb{K}}
\newcommand{\disc}{\mathbb{D}}

% TRIGONOMETRY
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\arccsc}{arcCsc}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arcsech}{arcsech}
\DeclareMathOperator{\arccsch}{arcCsch}
\DeclareMathOperator{\arccoth}{arcCoth} 

% GREEK ALPHABET
\newcommand{\al}{\alpha}
\newcommand{\bet}{\beta}
\newcommand{\de}{\delta}
\newcommand{\D}{\Delta}
\newcommand{\e}{\varepsilon}
\newcommand{\ph}{\varphi}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\s}{\sigma}
\newcommand{\Si}{\Sigma}
\newcommand{\tht}{\theta}
\newcommand{\Tht}{\Theta}
% \newcommand{\kk}{\kappa}
% \newcommand{\rr}{\rho}
% \newcommand{\ups}{\Upsilon}
%\newcommand{\be}{\beta}
% \newcommand{\om}{\omega}
% \newcommand{\lo}{\gamma}
% \newcommand{\Xxi}{\Xi}
% \newcommand{\ppi}{\phi}
% \newcommand{\Ppi}{\Phi}

% VECTORS
\newcommand{\vect}[1]{{\bm #1}}
\newcommand{\fb}{{\bm f}}
\newcommand{\nb}{{\bm n}}
\newcommand{\sbb}{{\bm s}}
\newcommand{\xb}{{\bm x}}
\newcommand{\zb}{{\bm z}}

% POINT DERIVATIVES
\newcommand{\qd}{\dot{q}}
\newcommand{\pd}{\dot{p}} 
\newcommand{\rd}{\dot{r}}
\newcommand{\ud}{\dot{u}}
\newcommand{\xd}{\dot{x}}
\newcommand{\yd}{\dot{y}}
\newcommand{\zd}{\dot{z}}
\newcommand{\zbd}{\dot{\bm z}}
\newcommand{\ttd}{\dot{\tau}}
\newcommand{\td}{\dot{\theta}}
\newcommand{\Rd}{\dot{R}}
\newcommand{\xdd}{\ddot{x}}
\newcommand{\udd}{\ddot{u}}
\newcommand{\rdd}{\ddot{r}}
\newcommand{\lad}{\dot{\lambda}}
\newcommand{\Lad}{\dot{\Lambda}} 

% OVERLINE VARIABLES
\newcommand{\xl}{\tilde{x}}
\newcommand{\yl}{\tilde{y}} 
\newcommand{\lal}{\tilde{\la}} 
\newcommand{\Lal}{\tilde{\La}} 

% DERIVATIVES
\newcommand{\pa}{\partial}
\newcommand{\Dt}[2]{\dfrac{d #1}{d {#2}}}
\newcommand{\Dx}[2]{\dfrac{\partial #1}{\partial {#2}}}
\newcommand{\Dxx}[2]{\dfrac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\Dxy}[3]{\dfrac{\partial^2 #1}{\partial {#2} \partial {#3}}}
\newcommand{\diff}[2]{\frac{d {#1}}{d {#2}}}
\newcommand{\dx}[2]{\frac{\partial #1}{\partial {#2}}}
\newcommand{\dt}[1]{\frac{d {#1}}{dt}}

% CALIGRAPHIC FONTS
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NNN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\RRR}{\mathcal{R}}
\newcommand{\SSS}{\mathcal{S}}
\newcommand{\TTT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\ZZZ}{\mathcal{Z}}
\newcommand{\tEE}{\widetilde{\mathcal{E}}}


% OPERATORS
%\newcommand{\vect}{\mathrm{vec}}
\newcommand{\trace}{\text{Trace}}
\newcommand{\sgn}{\text{sgn}}
\newcommand{\Lip}{\mathrm{Lip}}
%\newcommand{\El}{\mathrm{El}}
%\newcommand{\Par}{\mathrm{Par}}
%\newcommand{\hyp}{\mathrm{hyp}}
%\newcommand{\el}{\mathrm{ell}}
\newcommand{\mix}{\mathrm{mix}}
\newcommand{\adj}{\mathrm{adj}}
\newcommand{\unc}{\mathrm{unc}}
\newcommand{\coup}{\mathrm{coup}}
\newcommand{\mi}{\mathrm{min}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\glob}{\mathrm{glob}}
\newcommand{\inte}{\mathrm{int}}
\newcommand{\fut}{\mathrm{f}}
\newcommand{\past}{\mathrm{p}}
%\newcommand{\h}{\mathrm{h}}
\newcommand{\ex}{\mathrm{e}}

% COLORS
\definecolor{myGreen}{RGB}{0, 200, 0}
\definecolor{myOrange}{RGB}{255, 100, 0}
\definecolor{myYellow}{RGB}{255, 200, 0}
\definecolor{myBlue}{RGB}{0, 200, 255}
\definecolor{myPurple}{RGB}{200, 0, 200}

% ARROWS
\newcommand{\SAParrow}{\hspace{0.2cm} \makebox[-0.25cm][l]{$\Bumpeq$}\longrightarrow}

% OTHER EXPRESSIONS
\newcommand{\Res}{\mathrm{Res\,}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\lln}{\llfloor}
\newcommand{\rrn}{\rrfloor}




==> Article Inner/innerComputations.tex <==
We devote this section to study two special solutions of the inner equation given by the Hamiltonian $\HH$ in~\eqref{def:hamiltonianInner}. 
%
%In particular, we study the solutions of the inner equation which approximate $\zuOut$ and $\zsOut$, as given by~\eqref{eq:invariantManifoldsExpression}, near the singularities, after the inner change of variables, $\phi_{\Inner}$. 
%
We introduce $Z=(W,X,Y)$ and the matrix
\begin{equation}\label{def:matrixAAA}
\AAA= \begin{pmatrix}
0 & 0 & 0 \\
0 & i & 0 \\
0 & 0 & -i
\end{pmatrix}.
\end{equation}
Then, the equation associated to the Hamiltonian $\HH$ can be written as
\begin{equation}\label{eq:systemEDOsInner}
\left\{ \begin{array}{l}
\dot{U} = 1 + g(U,Z),\\
\dot{Z} = \AAA Z + f(U,Z),
\end{array} \right.
\end{equation}
where 
$f = \paren{-\partial_U \KK, 
	i \partial_Y \KK, -i\partial_X \KK }^T$ 
and
$g = \partial_{W} \KK$.
%where $f^{\Inner}=(f^{\Inner}_1,f^{\Inner}_2,f^{\Inner}_3)$ and
%\begin{equation}\label{eq:definitionfgInner}
%\begin{split}
%g^{\Inner}(U,Z) = \Dx{\KK}{W}, \quad
%f_1^{\Inner}(U,Z) = -\Dx{\KK}{U}, \quad
%f_2^{\Inner}(U,Z) = i\Dx{\KK}{Y}, \quad 
%f_3^{\Inner}(U,Z) =-i\Dx{\KK}{X}.
%\end{split}
%\end{equation}

We look for solutions of this equation parametrized as graphs with respect to $U$,
namely we look for functions
\begin{equation*}%\label{def:graphInner}
\ZdInn(U) = \big(\WdInn(U),\XdInn(U),\YdInn(U)\big)^T,
\qquad
\text{for } \diamond=\unstable,\stable,
\end{equation*}
satisfying the invariance condition given by~\eqref{eq:systemEDOsInner}, that is
\begin{equation}\label{eq:invariantEquationInner}
\partial_U \ZdInn = 
\AAA \ZdInn + \RRR[\ZdInn],
\qquad
\text{for } \diamond=\unstable,\stable,
\end{equation}
where
\begin{equation}\label{def:operatorRRRInner}
\RRR[\varphi](U)= 
\frac{f(U,\varphi)- g(U,\varphi) \AAA \varphi }{1+g(U,\varphi)}.
% \begin{pmatrix}
%f_1(U,\ZInn) \\
%f_2(U,\ZInn)-i\XInn g(U,\ZInn) \\
%f_3(U,\ZInn)+i\YInn g(U,\ZInn)
%\end{pmatrix},
\end{equation}


In order to ``select'' the solutions we are interested in, we point out that, since we need some uniformity with respect to $\de$
%
and $U=\de^{-2}(u-iA)$, then $\Re U \to \pm \infty$ as $\de \to 0$, depending on the sign of $\Re U$.
%
Then, according to~\eqref{eq:approxInnerw} and~\eqref{eq:approxInnerxy}, we deduce that $(W,X,Y) \to 0$ as $\Re U \to \pm \infty$.
%
For that reason, we look for $\ZdInn$ satisfying the asymptotic conditions
\begin{equation}\label{eq:asymptoticConditionsInner}
\begin{split}
\lim_{\Re U \to -\infty} \ZuInn(U) = 0, 
\qquad 
\lim_{\Re U \to +\infty} \ZsInn(U) = 0. 
\end{split}
\end{equation}
%
%Therefore, applying the inner change of coordinates $\phi_{\Inner}$, $\ZuInn$ and $\ZsInn$ give the first order nearby the singularity $iA$ of the invariant manifolds  $W^\unstable$ and $W^\stable$, as given in~\eqref{eq:invariantManifoldsExpression}. 
%
In fact, for a fixed $\beta_0 \in \paren{0,\frac{\pi}{2}}$, we look for functions $\ZuInn$ and $\ZsInn$ satisfying~\eqref{eq:invariantEquationInner},
\eqref{eq:asymptoticConditionsInner}  defined in the domains
\begin{equation}\label{def:domainInnner}
\begin{split}
&\DuInn = \claus{ U \in \complexs \text{ : }
|\Im U | \geq \tan \beta_0 \,\Re U + \rhoInn}, 
\qquad 
\DsInn = -\DuInn,
\end{split}
\end{equation}
respectively, for some $\rhoInn>0$ big enough (see Figure~\ref{fig:dominiInnerUnstable}).
\begin{figure}[t] 
	\centering
	\vspace{5mm}
	\begin{overpic}[scale=0.8]{dominiInnerUnstable.png}
		\put(10,60){$\DuInn$}
		\put(32.5,44){{$\beta_0$}}
		\put(45,55){{$\rhoInn$}}
		\put(102,41){$\Re U$}
		\put(47,87){$\Im U$}
	\end{overpic}
	\bigskip
	\caption{The inner domain, $\DuInn$, for the unstable case.}
	\label{fig:dominiInnerUnstable}
\end{figure} 
%
We analyze the  the difference $\DZInn=\ZuInn-\ZsInn$ in the overlapping domain
\begin{equation}\label{def:domainInnnerDiff}
\EInn = \DuInn \cap \DsInn \cap 
\claus{ U \in \complexs \st \Im U< 0}.
\end{equation}

%\begin{remark}
%	Let us remark that for $U \in \DdInn$, where $\diamond=\unstable,\stable$, the distance to $U=0$ in this domain is bounded and
%	\begin{equation}\label{eq:UBounds} 
%		\vabs{U} \geq {\rhoInn}{\cos(\beta_0)}.
%	\end{equation}
%\end{remark}

%On the following Theorem, we state the two main results of the document. In particular, we state the existence of the solutions of the inner equation associated with the unstable and stable manifold of $L_3$ nearby the singularities of the separatrix. We also state the asymptotic expression for the difference between these two solutions.

\begin{theorem}\label{theorem:innerComputations}
	There exist $\rhoInn_0, \cttInnExist>0$
	such that for any $\rhoInn\geq\rhoInn_0$,	
	the equation~\eqref{eq:invariantEquationInner} has analytic solutions
	$
	\ZdInn(U) =(\WdInn(U),\XdInn(U),\YdInn(U))^T, 
	$ for $U \in \DdInn$, $\diamond=\unstable,\stable$, satisfying
	\begin{equation}\label{result:innerExistence}
	| U^{\frac{8}{3}} \WdInn(U)| \leq \cttInnExist, \qquad
	| U^{\frac{4}{3}} \XdInn(U) | \leq \cttInnExist, \qquad
	| U^{\frac{4}{3}} \YdInn(U) | \leq \cttInnExist.
	%\text{for }	U \in \DdInn.
	\end{equation}
	In addition, there exist $\CInn \in \complexs$ and $\cttInnDiff>0$ independent of $\rhoInn$, and a function $\chi=(\chi_1,\chi_2,\chi_3)^T$ 
	such that
	\begin{equation}\label{result:innerDifference}
	\DZInn(U) = \ZuInn(U)-\ZsInn(U) =
	\CInn e^{-iU} \Big(
	(0,0,1)^T + \chi(U) \Big),
	\end{equation}
	and, for $U \in \EInn$,
	\begin{align*}
	| U^{\frac{7}{3}} \chi_1(U)| \leq \cttInnDiff, \qquad
	| U^{2} \chi_2(U) | \leq \cttInnDiff, \qquad
	| U \chi_3(U) | \leq \cttInnDiff.
	%\text{for } U \in \EInn.
	\end{align*}
	%Moreover, $K \neq 0$ if and only if $\DZInn \neq 0$.
\end{theorem}

%\begin{remark}\label{remark:innerComputationConjugats}
%	The change~\eqref{def:changeInner} allows us to study an approximation of the invariant manifolds $\zusOut(u)$ near the singularity $u=iA$. However, to obtain an approximation near $u=-iA$ we have to consider the change
%	\begin{equation*}\label{def:changeInnerNegatiu}
%	V=\frac{u+iA}{\de^2}, \hh
%	\widehat{W}=\de^{\frac{4}{3}}\frac{w}{2 \al_-^2}, \hh
%	\widehat{X}=\frac{x}{\de^{\frac{1}{3}} \sqrt{2} \al_- } , \hh
%	\widehat{Y}=\frac{y}{\de^{\frac{1}{3}}\sqrt{2} {\al_-}},
%	\end{equation*}
%	where  $\al_- \in \complexs$ was defined on Theorem \ref{theorem:singularities}, such that $\conj{\al_-} = \al_+$. 
%	In this case, for $V \in \conj{\DdInn}$, one can prove the existence of the solutions 
%	\[
%	\ZdInnN(V)=(\WdInnN(V),\XdInnN(V),\YdInnN(V)), \h
%	\text{ where } \diamond = \mathrm{u, s}.
%	\]
%	Notice that, since $x=\conj{y}$ by its definition on~\eqref{def:changeOuter} , then $\widehat{X} = \conj{Y}$. 
%	Therefore, the difference between these two solutions $\DZInnN = \ZuInnN - \ZsInnN$, is given asymptotically for $V \in \conj{\EInn}$ by
%	\begin{equation}\label{result:innerDifferenceNegative}
%	\DZInnN(V) = \conj{\CInn} e^{iV} \Big(
%	(0,1,0) + \zeta(V) \Big),
%	\end{equation}
%	where $\conj{\CInn}$ is the conjugate of the constant $\CInn$ given in Theorem~\ref{theorem:innerComputations} and $\zeta=(\zeta_1,\zeta_2,\zeta_3)$ satisfies 
%	$\vabs{V^{\frac{7}{3}} \zeta_1(V)} \leq C$,
%	$\vabs{V \zeta_2(V)} \leq C$ and
%	$\vabs{V^{2} \zeta_3(V)} \leq C$.
%\end{remark}


\begin{remark}\label{remark:CInnNumerics}
This theorem implies that ${\CInn} = \lim_{\Im U \to - \infty}{\DYInn(U) e^{iU}}$. Thus, we can obtain a numerical approximation of the constant $\CInn$. 
%Indeed, for $U \in \EInn$, we have
%\begin{align*}
%{\CInn} \approx {\DYInn(U) e^{iU}}.
%\end{align*}
Indeed, for $\rho>\kappa_0$, we can define
\begin{equation}\label{def:CInnrho}
\CInn_{\rho} = \vabs{ \DYInn(-i\rho)} e^{\rho},
%\quad \text{for} \quad \rho>0.
\end{equation} 
which, for $\rho$ big enough, satisfies $\CInn_{\rho} \approx \vabs{\CInn}$.

To compute $\DYInn(-i\rho)=\YuInn(-i\rho)-\YsInn(-i\rho)$,
we first look for good approximations of $\ZuInn(U)$ for $\Re U\ll -1$ and of $\ZsInn(U)$ for $\Re U \gg 1$, as power series in $U^{-\frac13}$.
%
One can easily check that $\ZuInn(U)$ as $\Re U \to -\infty$  and $\ZsInn(U)$ as $\Re U \to +\infty$ have the same asymptotics expansion:
\begin{align*}
\WdInn(U) &= 
\frac{4}{243 \, U^{\frac{8}{3}} } 
- \frac{172}{2187 \, U^{\frac{14}{3}}}
+ \OO \paren{U^{-\frac{20}{3}}}, \\
%
\XdInn(U) &= -\frac{2i}{9 \, U^{\frac{4}{3}} } 
+\frac{28}{81 \, U^{\frac{7}{3}} }
+ \frac{20i}{27 \, U^{\frac{10}{3}} }
- \frac{16424}{6561 \, U^{\frac{13}{3}} }
+ \OO \paren{U^{-\frac{16}{3}}}, \\
%
\YdInn(U) &= \frac{2i}{9 \, U^{\frac{4}{3}} } 
+\frac{28}{81 \, U^{\frac{7}{3}} }
- \frac{20i}{27 \, U^{\frac{10}{3}} }
- \frac{16424}{6561 \, U^{\frac{13}{3}} }
+ \OO \paren{U^{-\frac{16}{3}}}.
\end{align*}	
We use these expressions to set up the  initial conditions for the numerical integration  for computing $\DYInn(-i\rho)$.
%
We take as initial points  the value of the truncated power series at order $U^{-\frac{13}{3}}$ at $U= 1000 -i\rho$ (for $\diamond=\stable$) and $U= -1000 -i\rho$ (for $\diamond=\unstable$).
% , and compute $\YdInn(-i\rho)$ by numerical integration. 
%
(See Table~\ref{table:CInnrho}). 
%we perform numerical integration on the equation in~\eqref{eq:systemEDOsInner} to obtain approximations for $\ZuInn$ and $\ZsInn$ on $U=-i\rho$.
%To compute them, we look for good approximations of $\ZuInn$ for $\Re(U)\ll -1$ and for $\ZsInn$ for $\Re(U) \gg 1$.
%We use them to set up initial conditions for the numerical integration.
%
%Then, as initial condition, we truncate $\DZInn(\pm 1000 - i\rho)$ at order $U^{-\frac{13}{3}}$, and we integrate numerically to compute $\DZInn(-i\rho)$ (see Table~\ref{table:CInnrho}). 
%
We perform the numerical integration for different values of  $\rho\leq 23$ and an  integration solver with tolerance $10^{-12}$.
 
 
Table~\ref{table:CInnrho} shows that the constant $\Theta$ is approximately 1.63 which indicates that it is not zero. We expect that this computation method can be implemented rigorously \cite{BCGS21}.

\begin{table}[H]
\begin{equation*}
\begin{array}{|c||c|c|c|}
	\hline
	\rho & \vabs{\DYInn(-i\rho)} & e^{\rho} & \CInn_{\rho}\\
	\hline 
	\hline
	13 & 3.7 \cdot 10^{-6} & 4.4 \cdot 10^{5} & 1.6373 \\
	\hline
	14 & 1.4 \cdot 10^{-6} & 1.2 \cdot 10^{6} & 1.6361 \\
	\hline
	15 & 5.0 \cdot 10^{-7} & 3.3 \cdot 10^{6} & 1.6351 \\
	\hline
	16 & 1.8 \cdot 10^{-7} & 8.9 \cdot 10^{6} & 1.6341 \\
	\hline
	17 & 3.7 \cdot 10^{-8} & 2.4 \cdot 10^{7} & 1.6333 \\
	\hline
	18 & 6.8 \cdot 10^{-8} & 6.6 \cdot 10^{7} & 1.6326 \\
	\hline
	19 & 9.1 \cdot 10^{-9} & 1.8 \cdot 10^{8} & 1.6320 \\
	\hline
	20 & 3.4 \cdot 10^{-9} & 4.9 \cdot 10^{8} & 1.6315 \\
	\hline
	21 & 1.2 \cdot 10^{-9} & 1.3 \cdot 10^{9} & 1.6312 \\
	\hline
	22 & 4.6 \cdot 10^{-10} & 3.6 \cdot 10^{9} & 1.6313 \\
	\hline
	23 & 1.7 \cdot 10^{-10} & 9.7 \cdot 10^{9} & 1.6323 \\
	\hline
\end{array}
\end{equation*}
\caption{Computation of $\CInn_{\rho}$, as defined in~\eqref{def:CInnrho}, for different values of $\rho\leq 23$.}
\label{table:CInnrho}
\end{table}

\end{remark}


==> Article Inner/innerDerivation.tex <==

Due to the slow-fast character of the system, to capture the asymptotic first order of the difference $\dzOut = \zuOut-\zsOut$, we need to give the main terms of this difference close to the singularities, concretely, up to distance of order $\de^2$. 
%
%To compute the splitting of separatrices of this problem, we must detect the asymptotic first order of the difference $\dzOut$.
%where  $\zuOut$ and $\zsOut$ are the graphs of the unstable and unstable manifolds respectively.%, introduced on Proposition~\ref{proposition:existenceOuter}.
%As we mentioned before, our study requires the knowledge of the asymptotics of the parameterizations $\zuOut$ and $\zsOut$, introduced in Proposition~\ref{proposition:existenceOuter}, for $u$ near the singularities $\pm iA$.
%As we mentioned before, the difference $\dzOut(u)$ is exponentially small for real values of $u$.
%
%The main idea is that functions which are of algebraic order with respect to $\de$ near the singularities $\pm iA$, are exponentially small
%for real values of $u$. 
%
%As we mentioned before, the difference $\dzOut$ is exponentially small for real values of $u$. Thus, we want to compute the difference and capture the asymptotic first
%order close to the singularities.
%%, concretely, up to distance of order $\de^2$.
%
To this end, we derive the inner equation, see~\cite{Bal06, BalSea08}, which  contains the first order of the Hamiltonian $H^{\out}$ (see~\eqref{def:hamiltonianOuter}) close to (one of) the singularities and is independent of the small parameter $\de$.
% 
That is, we look, for instance, for a Hamiltonian which is a good approximations of $H^{\out}$ in a neighborhood of $u=iA$. 
%
Here, we focus on a domain near the singularity $u=iA$, but a similar analysys  can be done near $u=-iA$. 

Since we need to control the difference up to distance of order $\de^2$ of the singularity $u=iA$, we consider $U$ such that
\[
u-iA = \de^2 U.
\] 
Notice that we can take $\vabs{U}\gg 1$ independent of $\de$.
%
Close to the singularity $u=iA$, the homoclinic connection is not the dominant term of the perturbed invariant manifolds anymore.
%
Let us be more precise, take $\La=\La_h(u)-\frac{w}{3\La_h(u)}$, and recall that, by Theorem~\ref{theorem:singularities}, we have
\[
\La_h(u) \sim -\frac{2\al_+}{3} (u-iA)^{-\frac{1}{3}}, \quad
\text{for}  \quad \vabs{u-iA} \leq \nu,
\]
or equivalently,
\[
\La_h(iA + \de^2 U) \sim 
-\frac{2\al_+}{3 \de^{\frac{2}{3}} U^{\frac{1}{3}}} \sim
\OO\paren{\frac{1}{\de^{\frac{2}{3}} U^{\frac{1}{3}} }}.
%\text{ for } \quad U \sim \OO(1).
\]
Then,
\begin{equation}\label{eq:approxInnerw}
\wdOut(iA + \de^2 U) \sim 
3 \La_h^2(iA + \de^2 U) \sim
\OO\paren{\frac{1}{\de^{\frac{4}{3}} U^{\frac{2}{3}}}}.
\end{equation}
In addition,  the unperturbed Hamiltonian must have all of its terms of the same order. Therefore,
\begin{equation}\label{eq:approxInnerxy}
\frac{\xdOut(iA + \de^2U) \, \ydOut(iA+\de^2 U)}{\de^2}
\sim \OO\paren{\frac{1}{\de^{\frac{4}{3}}
		U^{\frac{2}{3}}}}.
\end{equation}
By symmetry, $\xdOut(iA + \de^2U)$, $\ydOut(iA + \de^2U) \sim \OO(\de^{\frac{1}{3}} U\mefr{1}{3})$.
%


To avoid the dependence on the inner equation with respect to $\al_+$ (see Theorem~\ref{theorem:singularities}) and to keep the symplectic character, we perform the scaling
%For the other variables $(w,x,y)$, we consider scaled coordinates $(W,X,Y)$, so that the components of the unperturbed problem, $H^{\out}_0$, are all of the same order with respect to $\de$. That is
%\[
%H^{\out}_0 \sim \de^{p}
%\big( W + XY + \OO(1) \big),
%\]
%for a certain $p\in \reals$.
%% 
%Additionally, we set the scaling of coordinates to be symplectic with respect to the normal form ${dU \wedge dW} + i {dX \wedge dY}$.
\begin{equation}\label{def:changeInner}
\phi_{\Inner}:(U,W,X,Y) \to (u,w,x,y),
\end{equation}
given by
\begin{equation*}
U=\frac{u-iA}{\de^2}, 
\qquad
W=\de^{\frac{4}{3}}\frac{w}{2 \al_+^2}, 
\qquad
X=\frac{x}{\de^{\frac{1}{3}} \sqrt{2} \al_+ }, \qquad
Y=\frac{y}{\de^{\frac{1}{3}}\sqrt{2} {\al_+}},
%
%T = \frac{\tau}{\de^2}.
\end{equation*}
and the time scaling $\tau=\de^2 t$. 
%where  $\al_+ \in \complexs$ was introduced on Theorem~\ref{theorem:singularities}.
%This change has constant determinant and therefore the new system is also Hamiltonian.
%
The heuristics above lead us to assume that $(U,W,X,Y) = \OO(1)$ when $u-iA=\OO(\de^2)$.
%
In the following proposition, by applying the change of coordinates $\phi_{\Inner}$,  we obtain the inner equation of the Hamiltonian $H^{\out}$.


\begin{proposition}\label{proposition:innerDerivation}
%	Let us consider the inner change of variables $\phi_{\Inner}$ as defined on~\eqref{def:changeInner} and
%	a scaling in time by a factor of ${\de^{-2}}$.
	The Hamiltonian equations associated to~\eqref{def:hamiltonianOuter} expressed in inner coordinates (see~\eqref{def:changeInner}) are Hamiltonian with respect to
	\begin{equation*}%\label{def:hamiltonianInnerComplete}
	H^{\Inner} = \HH + H_1^{\Inner},
	\end{equation*}
	where 
	\begin{equation}\label{def:hamiltonianInner}
	\HH(U,W,X,Y) =\left. H^{\Inner}(U,W,X,Y;\de)\right|_{\de=0} = W + XY + \KK(U,W,X,Y),
	\end{equation}
	with
	\begin{align}
	\KK(U,W,X,Y) &= 
	-\frac{3}{4}U^{\frac{2}{3}} W^2 
	- \frac{1}{3 U^{\frac{2}{3}}}
	\paren{\frac{1}{\sqrt{1+\JJ(U,W,X,Y)}} - 1 } \label{def:hamiltonianK}
	\end{align}
	and
	\begin{equation}\label{def:hFunction}
	\begin{split}
	\JJ(U,W,X,Y) =& \,  
	\frac{4 W^2}{9 U^{\frac{2}{3}} } 
	-\frac{16 W}{27 U^{\frac{4}{3}}}  
	+\frac{16}{81 U^{2}}
	%\nonumber \\
	%
	+\frac{4(X+Y)}{9 U}
	\paren{W -\frac{2}{3 U^{\frac{2}{3}}}} \\[0.5em]
	&- \frac{4i(X-Y)}{3 U^{\frac{2}{3}}}
	%
	-\frac{X^2+Y^2}{3 U^{\frac{4}{3}}}
	+\frac{10 XY}{9 U^{\frac{4}{3}}}. 	
	\end{split}
	\end{equation}
	Moreover, if 
	$\cttInnDerA^{-1} \leq \vabs{U} \leq \cttInnDerA$ and 
	$\vabs{(W,X,Y)} \leq \cttInnDerB$ 
	for some $\cttInnDerA>1$ and $0<\cttInnDerB<1$,
	we have that there exist $\cttInnDerC, \cttInnDerAA, \cttInnDerBB>0$ independent of $\de, \cttInnDerA, \cttInnDerB$ such that
	\[
	\vabs{H_1^{\Inner}(U,W,X,Y;\de)} \leq 
	\cttInnDerC \cttInnDerA^{\cttInnDerAA} \cttInnDerB^{\cttInnDerBB}\de^{\frac{4}{3}}.
	\] 
%	where $\cttInnDerC>0$ is a constant depending {potentially} on $\cttInnDerA$ and $\cttInnDerB$, i.e. there exists $\g_2, \g_3 \geq 0$ such that
%	$\cttInnDerC\leq \cttInnDerA^{\g_2} \cttInnDerB^{\g_3}$.
	%\[
	%\HH^{\Inner}(U,W,X,Y,\de) := \frac{\de^{4/3}}{2\al^2} \HH(\phi^{-1}_{\Inner}(U,W,X,Y);\de).
	%\]
	%such that $\Omega = \left(2\al^2 \de^{2/3} \right) \Omega_{\Inner}$
\end{proposition}

\begin{remark}\label{remark:innerComputationConjugats}
The change of coordinates \eqref{def:changeInner} allows us to study an approximation of the invariant manifolds $\zusOut(u)$ near the singularity $u=iA$. %Since $x=\conj{y}$ by its definition on~\eqref{def:changeOuter}, 
To obtain an approximation near $u=-iA$, one can proceed analogously by
\begin{equation*}\label{def:changeInnerNegatiu}
U=\frac{u+iA}{\de^2}, 
\qquad
W=\de^{\frac{4}{3}}\frac{w}{2 \al_-^2}, 
\qquad
X=\frac{x}{\de^{\frac{1}{3}} \sqrt{2} \al_-}, \qquad
Y=\frac{y}{\de^{\frac{1}{3}}\sqrt{2} \al_-},
\end{equation*}
where $\al_- = \conj{\al_+}$ (see Theorem \ref{theorem:singularities}). 
\end{remark}


==> Article Inner/introMainResults.tex <==
%In this section, we introduce the rigourous statement of the results in this work and give the main ideas to obtain them.

We devote this section to state the main results concerning the Steps A, B, C and D explained in Section \ref{sec:schemeproof}. 
First, in Section~\ref{subsection:reformulation}, we present the changes of coordinates involved  to rewrite the Hamiltonian $h$ in~\eqref{def:hamiltonianInitialNotSplit} as a singular perturbation problem given by a  fast oscillator weakly coupled with a one degree of freedom Hamiltonian with a saddle point and a separatrix (Step A).
%such that, the new Hamiltonian becomes a fast oscillator weakly coupled with a pendulum-like Hamiltonian with a saddle and an homoclinic connection.
%
In Section~\ref{subsection:singularities}, we consider the  time-parametrization of the separatrix and analyze the properties of its analytical continuation (Step B).
%
In Section~\ref{subsection:innerDerivation} we give some heuristic ideas regarding the parametrization of the perturbed manifolds on certain complex domains (Step E) and deduce the singular change of variables which leads to the inner equation (Step C).
%
Finally, in Section~\ref{subsection:innerComputations}, we present the study of certain solutions of the inner equation and give an asymptotic formula for their difference (Step D).


==> Article Inner/introduction.tex <==
The understanding of the motions of the $3$-Body Problem has been of deep interest  in the last centuries. Since Poincar\'e, see \cite{Poincare1890}, one of the fundamental problems is to understand how the invariant manifolds of its different invariant objects (periodic orbits, invariant tori) structure its global dynamics.
%
% Its significance lies in that, unlike the $2$-Body Problem, no general closed-form solution exists, leading to the existence of chaotic behaviors.
%
Assume that one of the bodies (say the third) has mass zero. Then, one has the Restricted  $3$-Body Problem. In this model, the two first bodies, called the primaries, are not influenced by the massless one. As a result, their motions are governed by the classical Kepler laws. If one further assumes that the primaries perform circular motion and that the third body is coplanar with them, one has the Restricted Planar Circular 3-Body Problem (RPC$3$BP).
% 
% (RPC$3$BP), which is a useful simplification of the $3$-Body Problem while maintaining its complexity.
% 
% The RPC$3$BP models the motion of a body of negligible mass under the gravitational influence of two massive bodies, called the primaries. 
% %
% Since the third body is assumed massless, it does not influence the motion of the two primaries and, 
%
%As a consequence, it is only necessary to study the motion of the body with negligible mass.
%
% In addition, we consider the circular and planar case;
% % 
% namely, that the primaries perform circular motions and that the third body moves on the same plane as the primaries.

Let us name the two primaries $S$ (star) and $P$ (planet).
%
Normalizing their masses, we can assume that $m_S=1-\mu$ and $m_P=\mu$, with $\mu \in \left( 0, \frac{1}{2} \right]$. 
%
Since the primaries follow circular orbits, in rotating (usually also called synodic) coordinates, their positions can be fixed at $q_S=(\mu,0)$ and  $q_P=(\mu-1, 0)$.
%
Then, denoting by $(q,p) \in \reals^2 \times \reals^2$ the position and momenta of the third body and  taking appropriate units, the RPC$3$BP is a $2$-degrees of freedom Hamiltonian system with respect to
%
\begin{equation}\label{def:hamiltonianInitialNotSplit} 
	\begin{split}
		\HInicial(q,p;\mu) &= \frac{||p||^2}{2} 
		- q^t \left( \begin{matrix} 0 & 1 \\ -1 & 0 \end{matrix} \right) p 
		-\frac{(1-\mu)}{||q-(\mu,0)||} 
		- \frac{\mu}{||q-(\mu-1,0)||}.
	\end{split}
\end{equation}
% Notice that this Hamiltonian is analytic away from $q=q_S$ and $q=q_P$, which correspond to collision with the primaries.

For $\mu>0$, it is a well known fact that $\HInicial$ has five equilibrium points: $L_1$, $L_2$, $L_3$, $L_4$ and $L_5$, called Lagrange points\footnote{
	For $\mu=0$, the system has a circle of critical points $(q,p)$ with $\norm{q}=1$ and $p=(p_1,p_2)=(-q_2,q_1)$.
}
%
(see Figure~\ref{fig:L3perturbed}(a)). 
%
On an inertial (non-rotating) system of coordinates, the Lagrange points correspond to periodic orbits with the same period as the two primaries, i.e they lie on a 1:1 mean motion resonance. 
%
%In this work, we focus on the $L_3$ point. 
%
The three collinear points with the primaries, $L_1$, $L_2$ and $L_3$, are of center-saddle type and, for small $\mu$, the triangular ones, $L_4$ and $L_5$, are of center-center type (see for instance \cite{Szebehely}). 

% The invariant manifolds of $L_1$ and $L_2$ have been widely studied 
% due to their proximity to the primaries, the invariant manifolds of  $L_1$ and $L_2$ have been heavily studied for its interest in astrodynamics applications, \textcolor{red}{(see \cite{KLMR00, GLMS01v1, Canalias07})}.
%

Since the points $L_1$ and $L_2$ are rather close to the small primary, their invariant manifolds  have been widely studied 
 for their interest in astrodynamics applications, (see \cite{KLMR00, GLMS01v1, CGMM04}).
%
The dynamics around the points $L_4$ and $L_5$ have also been considerably studied since, due to its stability, it is common to find objects orbiting around these points (for instance the Trojan and Greek Asteroids associated to the pair Sun-Jupiter, see \cite{GDFGS89,CelGio90, RobGab06}).

On the contrary, the invariant manifolds of the Lagrange point $L_3$ have received somewhat less attention. Still, they  structure the dynamics in regions of the phase space of the RPC3BP. In particular, the horseshoe-shapped  orbits that explain the orbits of Saturn satellites Janus and Epimetheus lie ``close'' to the invariant manifolds of $L_3$ (see \cite{NPR20}). Moreover, the invariant manifolds of  $L_3$ (more precisely its center-stable and center-unstable manifolds) act as effective boundaries of the stability domains around $L_{4,5}$ (see in \cite{SSST13}). See the companion paper \cite{articleOuter} for more references about the dynamics of the RPC3BP in a neighborhood of $L_3$ and its invariant manifolds.
%
% In particular, for small values of $\mu$, the dynamics are rather similar to that of other mean motion resonances, which play an important role in creating instabilities in the Solar system, see \cite{formulesRPC3BP}.


The purpose of this paper and its sequel \cite{articleOuter} is to study the invariant manifolds of $L_3$ and, particularly, show that they do not intersect  for $0< \mu\ll 1$ (at their first round). 



\begin{figure}
	\subfloat[$\mu>0$]{%
		\begin{overpic}[scale=0.7]{lagrangePointsPerturbedEsquema.png}
			\put(43,38){{\color{blue} $q_S$ }}
			\put(14,38){{\color{blue} $q_P$ }}
			\put(23,45){{\color{red} $L_1$ }}
			\put(10,45){{\color{red} $L_2$ }}
			\put(63.5,45){{\color{red} $L_3$ }}
			\put(27,69){{\color{red} $L_5$ }}	
			\put(27,14){{\color{red} $L_4$ }}
			\put(89,42){$q_1$}
			\put(37.5,82.5){$q_2$}
		\end{overpic}
		\vspace{1cm}	
	}\hfill
	\subfloat[$\mu=0.003$]{%
		\begin{overpic}[width=7.5cm]{L3manifoldsm003.png}
			\put(50,1){$q_1$}
			\put(12,38){$q_2$}
			\put(71.5,37.5){{\color{red} $ L_3 \h \bullet$ }}
			\put(37,58){{\color{red} $\bullet$ }}
			\put(28,61){{\color{red} $L_5$ }}
			\put(37,17){{\color{red} $\bullet$ }}	
			\put(28,12){{\color{red} $L_4$ }}
			\put(50.5,37.5){{\color{blue} $\bullet$ }}
			\put(50.5,34){{\color{blue} $q_S$ }}
			\put(23,37.5){{\color{blue} $\bullet$ }}
			\put(23,34){{\color{blue} $q_P$ }}
		\end{overpic}
	}
	\caption{(a) Projection onto the $q$-plane of the equilibrium points for the RPC$3$BP on rotating coordinates. (b) Plot of the stable (green) and unstable (blue) manifolds of $L_3$ projected onto the $q$-plane for $\mu=0.003$. }
	\label{fig:L3perturbed}
\end{figure}

\subsection{The unstable and stable invariant manifolds of \texorpdfstring{$L_3$}{L3}}

The eigenvalues of the  the Lagrange point $L_3$
% is a center-saddle critical point, it posseses possesses $1$-dimensional stable and unstable manifolds %(which we denote by $W^{\stable}$ and $W^{\unstable}$, respectively) 
% and a $2$-dimensional center manifold.
%
% Moreover,  its eigenvalues 
satisfy that
%
\begin{equation}\label{eq:specRot}
	\mathrm{Spec}  = \claus{\pm \sqrt{\mu} \, \rho(\mu), \pm i  \, \omega(\mu) },
	\quad
	\text{with} \quad \left\{
	\begin{array}{l}
		\rho(\mu)=\sqrt{\frac{21}{8}}  + \OO(\mu),\\[0.4em]
		\omega(\mu)=1 + \frac{7}{8}\mu + \OO(\mu^2),
	\end{array}\right.
\end{equation}
%
as $\mu \to 0$ (see \cite{Szebehely}). Notice that, due to the different size in the eigenvalues, the system posseses two time scales, which translates to rapidly rotating dynamics coupled with a slow hyperbolic behavior around the critical point $L_3$.

The one dimensional unstable and stable invariant manifolds have two branches each (see Figure~\ref{fig:L3perturbed}(b)).
% 
One pair, which we denote  by $W^{\unstable,+}(\mu)$ and $W^{\stable,+}(\mu)$ circumvents $L_5$ whereas the other, denoted as  $W^{\unstable,-}(\mu)$ and $W^{\stable,-}(\mu)$,  circumvents $L_4$.
%
%Due to the symmetry of the system given by Hamiltonian $\HInicial$, we can restrict our study to the positive branches $W^{\unstable,+}$ and $W^{\stable,+}$, since the negative branches are symmetric.
%
Since the Hamiltonian system associated to  $\HInicial$ in \eqref{def:hamiltonianInitialNotSplit} is reversible with respect to the involution
\begin{equation}
	\label{def:involutionCartesians}
	\Phi(q,p;t)=(q_1,-q_2,-p_1,p_2;-t),
\end{equation}
the $+$ branches are symmetric to the $-$ ones. Thus, one can restrict the study to the first ones.
% $+$ branches, since the $-$ branches are symmetric.

As already mentioned, the aim of this paper (and its sequel \cite{articleOuter}) is to give an asymptotic formula for the distance between $W^{\unstable,+}(\mu)$ and $W^{\stable,+}(\mu)$, for $0<\mu\ll 1$ (in an appropriate transverse section). 
%
However, due to the rapidly rotating dynamics of the system (see \eqref{eq:specRot}), the stable and unstable manifolds of $L_3$ are exponentially close to each other with respect to $\sqrt{\mu}$. This implies that the classical Melnikov Theory \cite{Melnikov1963} cannot be applied and that obtaining the asymptotic formula is a rather involved problem.

The precise statement for the asymptotic formula for the distance is properly stated in the  sequel of this paper \cite{articleOuter}. Let us give here a more informal statement.
%
Consider the classical symplectic polar coordinates $(r,\theta,R, G)$, where $R$ is the radial momentum and $G$ the angular momentum, and  the section $\Sigma=\{\theta=\pi/2, r>1\}$. Then, if one denotes by $P^\unstable$ and $P^\stable$ the first intersections of the invariant manifolds $W^{\unstable,+}(\mu)$,$W^{\stable,+}(\mu)$ with $\Sigma$,  the distance between these points, is 
% stable and unstable manifolds of $L_3$ in section $\Sigma$ is 
given by
%
\begin{equation}\label{eq:dist}
	\mathrm{dist}_{\Sigma}(P^\unstable,P^\stable) = \sqrt[3]{4} \, \mu^{\frac13}
	e^{-\frac{A}{\sqrt\mu}} \boxClaus{\vabs{\CInn}
			+ \OO\paren{\frac1{\vabs{\log\mu}}}},
\end{equation}
for $0<\mu\ll1$ and certain constants $A>0$ and $\CInn \in \complexs$.
%
%Broadly speaking, by studying the complex singularities of an homoclinic connection of the system and the so-called inner equation, we are able to obtain expressions for the constants $A$ and $\CInn$ (see Section \ref{subsection:introSplittin}).
%
The proof of this asymptotic formula spans both the present paper and the sequel \cite{articleOuter}. In this first paper, we perform the first steps towards the proof (see Section \ref{sec:schemeproof} below). In particular, we obtain and describe the constants $A$ and $\CInn$ appearing in \eqref{eq:dist}.  
%
% Meanwhile, the sequel paper \cite{articleOuter} is concerned with the obtention of the asymptotic formula \eqref{eq:dist}.

%%%%%%%%%%%

A fundamental problem in dynamical systems is to prove that a model has chaotic dynamics (for instance a Smale Horseshoe). 
%
For many physically relevant problems, like those in Celestial Mechanics, this is usually a remarkably difficult problem.
%
% One of the methods used is to rely on the Smale-Birkhoff homoclinic theorem (see \cite{Arrowsmith1990}) which, by proving the existence of transverse homoclinic orbits to invariant objects, proves the existence of chaotic dynamics.
%
% Notice that, since the Hamiltonian $h$ in \eqref{def:hamiltonianInitialNotSplit} is autonomous, its unstable and stable manifolds either coincide or do not intersect.
%
% Therefore, \eqref{eq:dist} does not directly implies the existence of chaotic orbits.
%
Certainly, the fact that the invariant manifolds of $L_3$ do not coincide does not lead to chaotic dynamics. However, one should expect the existence of Lyapunov periodic orbits which are exponentially close (with respect to $\sqrt{\mu}$) to $L_3$ and whose stable and unstable invariant manifolds intersect transversally. If so, the Smale-Birkhoff Theorem 
%(see \cite{GuckenheimerHolmes}) 
would imply the existence of a hyperbolic set whose dynamics is conjugated to that of the Bernoulli shift (in particular, with positive topological entropy) exponentially close to the invariant manifolds of $L_3$. 
%
% We plan to prove this result in a forthcoming paper (see \cite{articleChaos}).
% , implying the existence of chaotic dynamics. \textbf{(Posar cites)}.
%
%This would imply the existence of chaotic motions which pass ``exponentially close'' to $L_3$.


\subsection{Exponentially small splitting of separatrices}
\label{subsection:introSplittin}

Even though there is a standard theory to analyze the breakdown of homoclinic and heteroclinic connections, the so called Poincar\'e-Melnikov Theory (see \cite{Melnikov1963} and \cite{GuckenheimerHolmes} for a more
modern exposition),
it cannot be applied to obtain \eqref{eq:dist} due to its exponential smallness.
%
% Indeed, notice that, in \eqref{eq:dist} the difference between manifolds cannot be detected in the truncation of their normal form at any finite order.
%
% It is, what is usually called, a \emph{beyond all orders} phenomenon.
%
Indeed, the breakdown of homoclinic connections to $L_3$ fits into what is usually  referred to as exponentially small splitting of separatrices problems. 
%
This \emph{beyond all orders} phenomenon was first detected by Poincar\'e in~\cite{Poincare1890} when he  studied the non integrability of the $3$-Body Problem. 

The first obtention of an asymptotic formula for an exponentially small splitting of separatrices did not appear until the 1980's with the pioneering work  by Lazutkin for the \emph{standard map}~\cite{Laz84, Laz05}.
%
% There, the author studied the splitting of separatrices for the standard map, and gave the main tools to obtain an asymptotic formula for it.
%
Even if Lazutkin's work was not complete (the complete proof was achieved by
Gelfreich in~\cite{Gel99}), the ideas he developed have been very influential and  have been the basis of many of the works in the field (and in particular of this paper and the sequel \cite{articleOuter}). Other methods to deal with exponentially small splitting of separatrices are Treschev's \emph{continuous averaging}  (see \cite{Tre97}) or ``direct'' series methods (see \cite{GGM99}).


Usually, the exponentially small splitting of separatrices problems are classified as \emph{regular} or \emph{singular}.

In the regular cases, even if  Melnikov theory cannot be straightforwardly applied, the Melnikov function  gives the leading term for the distance between the perturbed invariant manifolds. That is,   Melnikov theory provides the  first order for the distance but leads to too crude estimates for the higher order terms.
% asymptotic expression of the difference, but is not able to provide small enough estimates for the remainder terms.
%
% Therefore, the relevance of these cases lie in proving that the asymptotic formula is indeed correct. 
%
This phenomenon has been studied in rapidly forced periodic or quasi-periodic perturbations of $1$-degree of freedom Hamiltonian systems, see 
\cite{HMS88, DelSea92, DelSea97, Gel97a, Gel00, BF04, BF05, GGS20}, 
%\cite{HMS88, DelSea92, Fon93, Gel94, Fon95, DelSea97, Gel97a, Tre97, Gel00, BF04, BF05, GOS10}, 
in close to the identity area preserving  maps, see \cite{DelRRR98}, and in Hamiltonian systems with two or more degrees of freedom which have hyperbolic tori with  fast quasiperiodic dynamics \cite{Sau01}.
%
In particular, \cite{GMS16} provides  the first  prove of exponentially small splitting of separatrices in a Celestial Mechanics problem (see also \cite{GMSS17,GPSV21}).

In the singular cases, the exponentially small   first order for the distance between the invariant manifolds is no longer given by the Melnikov function. Instead, one has to consider an auxiliary equation, usually called  \emph{inner equation}, which does not depend on the perturbative parameter and  provides the first order for the distance. Some results on inner equations can be found on \cite{Gel97b, GS01, OSS03, Bal06, BalSea08, BM12} and
%
the application of  the inner equation analysis to the original problem can be  found in  \cite{BFGS12, Lom00, GOS10, GaiGel10, MSS11, BCS13,BCS18a, BCS18b}.
%
% In particular, in \cite{} the authors present one of the most general results for rapidly forced $1$-degree of freedom Hamiltonians.


Due to the extreme sensitivity of the exponentially small splitting of separatrices phenomenon on the features of each particular model, most of the available results apply  under quite restrictive hypothesis and,  therefore, cannot be applied to analyze the invariant manifolds of $L_3$.
% are not suitable to be applied to our system.

\subsection{Strategy to obtain an asymptotic formula for the breakdown of the invariant manifolds of \texorpdfstring{$L_3$}{L3}}\label{sec:schemeproof}

For the limit problem $h$ in \eqref{def:hamiltonianInitialNotSplit} with $\mu=0$, the five Lagrange point ``disappear'' into the circle of (degenerate) critical points  $\norm{q}=1$ and $p=(p_1,p_2)=(-q_2,q_1)$. As a consequence, the one-dimensional invariant manifolds of $L_3$ disappear when $\mu=0$ too. 
%
For this reason, to analyze perturbatively these invariant manifolds, the first step is to perform a singular change of coordinates to obtain a ``new first order'' Hamiltonian which  has a center saddle equilibrium point (close to $L_3$) with stable and unstable manifolds that coincide along a separatrix.
% 
% One of the first issues we face is the degeneracy of the unperturbed system. 
% %
% Indeed, for $\mu=0$, let us recall that the stable and unstable manifolds of $L_3$ become a circle of critical points (see also \eqref{eq:specRot}).
% %
% Therefore, before properly beginning the analysis of their breakdown, 
% %
% we have to reformulate the system in order to obtain a ``good enough'' first order of the Hamiltonian $h$ in \eqref{def:hamiltonianInitialNotSplit}.
% %
% The aim is for this first order to have a saddle and an homoclinic connection, also know as separatrix.
To perform the change of coordinates  we use the Poincar\'e planar elements (see~\cite{MeyerHallOffin}) plus a singular (with respect to $\mu$) scaling.
% which are action-angle variables for the $2$-Body Problem. 
%
% However, they do not have an explicit expression, 
%
% which adds difficulties to our analysis later on (see Section \ref{subsection:reformulation} for the details).
%This new first order is integrable and, therefore, the stable and unstable manifolds of $L_3$ coincide along a separatrix. 

%One of the difficulties faced during this study is that the first order of the difference is not correctly given by the Melnikov function (i.e  singular case, see Section \ref{subsection:introSplittin}).
%%
%Therefore, it is necessary to derive and study the associated inner equation.

In the following list, we present the main steps of our strategy to prove  formula \eqref{eq:dist}.
%
%The strategy to proof the breakdown of the invariant manifolds of $L_3$ is as follows.
%
We split the list in two. First we explain the steps performed in this paper and later those carried out in its sequel \cite{articleOuter}.
%


In this paper, we complete the following steps: 
\begin{enumerate}[label*=\Alph*.]
	\item We perform a change of coordinates which captures the slow-fast dynamics of the system.
	%
	The new Hamiltonian becomes a (fast) oscillator weakly coupled to a $1$-degree of freedom Hamiltonian with a saddle point and a separatrix associated to it.
	%
	\item We analyze the analytical continuation of a time-parametrization of the separatrix.
	%
	In particular, we obtain its maximal strip of analyticity (centered at the real line).
	%
	We also describe the character and location of the singularities  at the boundaries of this region.
	%
	
	%Finally, for technical reasons, we also analyze the zeros of the derivative of the first component of the separatrix. In this points, the separatrix fails to be a graph over its first component. 
	%
	%This is not necessary for the analysis of the splitting of separatrices. However, since later in Item D we parameterize the perturbed invariant manifolds as graphs, the analysis of the zeros is necessary to control when the graph property breaks down.
	% 	
	
	\item We derive the inner equation, which gives the first order of the original system close to the singularities of the separatrix described in Step B.
	%
	This equation is independent of the perturbative parameter $\mu$.
	
	\item We study two special solutions of the inner equation which are approximations of the perturbed invariant manifolds near the singularities.
	%
	Moreover, we provide an asymptotic formula for the difference between these two solutions of the inner equation.
	%
	We follow the approach presented in~\cite{BalSea08}.
\end{enumerate}

%Roughly speaking, in this article we perform the preliminary change of coordinates  and deal with the results  concerning the analysis of the invariant manifolds near their singularities: the singularity analysis of the separatrix and the derivation and analysis of the inner equation. 
%
%To finish the proof, in \cite{articleOuter}, we prove the existence of the invariant manifolds in a suitable domain, match this results with the ones obtained by the inner equation and compute the distance between the manifolds.

In \cite{articleOuter} we complete the following steps:

\begin{enumerate}
\item[E.] We prove the existence of the analytic continuation of suitable parametrizations of $W^{\unstable,+}(\de)$ and $W^{\stable,+}(\de)$ in appropriate complex domains (and as graphs).
%
These domains contain a segment of
the real line and intersect a neighborhood sufficiently close to the singularities of the  separatrix.
%
\item[F.] By using complex matching techniques, we compare the solutions of the inner equation with the graph parametrizations of the perturbed invariant manifolds.
%
\item[G.] Finally, we prove that the dominant term of the difference between manifolds is given by the term obtained from the difference of the solutions of the inner equation.
\end{enumerate}

The structure of this paper goes as follows. 
%
In Section \ref{section:mainResults}, we present the main results for the Steps A to D and introduce some heuristics to contextualize them.
%
Sections \ref{section:proofA-singularities}-\ref{section:proofD-AnalysisInner} are devoted to the proof of the results in Section~\ref{section:mainResults}.

\paragraph{The constants in the asymptotic formula for the distance.}

The constant $A$ in \eqref{eq:dist} is given by the height of the maximal strip of analyticity of the unperturbed separatrix (see Step B).
%
Therefore, to obtain its value, one has to compute the imaginary part of the singularities of the separatrix which are closer to the real line.

On all the previous mentioned works on splitting of separatrices, either the separatrix of the unperturbed model has an analytic expression (see for example~\cite{DelSea92,GaiGel10,GOS10,BCS13,GMS16}) or otherwise certain properties of its analytic continuation are given as assumptions (see~\cite{DelSea97,Gel97b,BF04, BFGS12}).
%
%From a numerical point of view, in~\cite{SimoGelf08} the authors presented a numerical method to study the singularities of the separatrices of different area preserving maps.
%
In this case, we do not have an explicit expression for the time-parameterization of the separatrix and, to obtain its complex singularities, we need to rely on techniques of analytical continuation to analyze them (see Section \ref{subsection:singularities}). In particular, we describe the parametrization of the separatrix in terms of a multivalued function involving a complex integral and (see Theorem \ref{theorem:singularities} below) we obtain 
%
% Then, by analyzing and classifying all the possible integration paths, we are able to show that the singularities of the unperturbed separatrix which are closest to the real axis have imaginary part obtain an expression for the constant $A$.
% 
\begin{equation*}
	A= \int_0^{\frac{\sqrt{2}-1}{2}} \frac{2}{1-x}\sqrt\frac{x}{3(x+1)(1-4x-4x^2)}  dx\approx 0.177744.
\end{equation*}	
%
This value agrees with the numerical computations of the distance between the invariant manifolds given in \cite{FontPhD, SSST13}.

Since we are in a singular case, the constant $\CInn$ in \eqref{eq:dist} is not correctly given by the Melnikov function but by the analysis of the  inner equation of the system (see Step C above and also  Sections \ref{subsection:innerDerivation} and \ref{subsection:innerComputations}).
%
In particular, $\CInn$ corresponds to a Stokes constant 
% that depends on the full jet of the Hamiltonian and, as a result, it
and does not have a closed formula.
%
% Thus, the correct value of $\CInn$ is obtained by the study of the inner equation of the system (see Sections \ref{subsection:innerDerivation} and \ref{subsection:innerComputations}).
%
By a numerical computation,  we see that $\vabs{\CInn}\approx 1.63$ (see Remark \ref{remark:CInnNumerics}). 
%
% Unfortunately, the accuracy of this computation is quite poor due to the exponentially small behavior between the manifolds.
%
We expect that, by means of a computer assisted proof, it would be possible to obtain rigorous estimates and verify that $\vabs{\CInn}\neq 0$, see \cite{BCGS21}. 





%%%%%%%%%%%%%%%%%%%%%%%%

%The $N$-body problem (the study of the motions of a group of $N$ bodies interacting with each other gravitationally) has been and is currently being one of the most important  problem studied in celestial mechanics.
%%
%The techniques developed by the dynamical systems field are crucial to understand the different types of behaviors that take place. 
%%
%The general $N$-body problem in $\reals^3$ is far from being understood in its entirety (for $N\geq3$), yet different simplified models can give us more information.
%%
%One of these simplified models is the famous restricted $3$-body problem.
%
%The restricted $3$-body problem models the motion of a body of negligible mass under the gravitational influence of two massive bodies, called the primaries. 
%%
%Since the third body has no mass, it does not influence the motion of the two primaries and, as a result, their motions are governed by the classical Kepler laws.
%%
%Assume that the primaries perform a circular motion and that the third body moves on the same plane as the primaries.
%%
%This is the so-called Restricted Planar Circular $3$-Body Problem (RPC$3$BP). 
%
%\subsection{The RPC3BP and the Lagrange point}
%
%%%%% THE MODEL %%%%%
%
%%We briefly present the equations of the motions we study, see~\cite{Szebehely} for the details.
%
%Let us name the two primaries $S$ (star) and $P$ (planet). Normalizing their masses, we can assume that $m_S=1-\mu$ and $m_P=\mu$, with $\mu \in \left( 0, \frac{1}{2} \right]$. 
%%
%%We consider a synodic reference system. 
%%
%Since the primaries follow circular orbits, choosing a suitable rotating coordinate system, their positions can be fixed at $q_S=(\mu,0)$ and  $q_P=(\mu-1, 0)$.
%
%Let us denote by $(q,p) \in \reals^2 \times \reals^2$ the position and momenta of the third body.
%%
%Then, taking appropriate units, the RPC$3$BP is a $2$-degrees of freedom Hamiltonian system with Hamiltonian
%\begin{equation}\label{def:hamiltonianInitial}
%\HInicial(q,p;\mu) = \HInicial_0(q,p) + \mu \HInicial_1(q;\mu),
%\end{equation}
%where
%\begin{equation}\label{def:hamiltonianInitial01} 
%\begin{split}
%\HInicial_0(q,p) &= \frac{||p||^2}{2} - q^t K p - \frac{1}{||q||}, 
%\qquad \text{with} \qquad 
%K= \left( \begin{smallmatrix} 0 & 1 \\ -1 & 0 \end{smallmatrix} \right). \\
%%\end{equation}
%%and 
%%\begin{equation}\label{eq:RShamiltonianInitial1}
%\mu \HInicial_1(q;\mu) &= \frac{1}{||q||} - \frac{(1-\mu)}{||q-(\mu,0)||} 
%- \frac{\mu}{||q-(\mu-1,0)||}.
%\end{split}
%\end{equation}
%%
%%Notice that, in the rotating reference system, the Hamiltonian system modeling the RPC$3$BP is autonomous. 
%%
%Notice that the system has a symmetry with respect to the involution 
%\begin{equation}
%\label{def:involutionCartesians}
%\Phi_h(q,p;t)=(q_1,-q_2,-p_1,p_2;-t).
%\end{equation}
%
%%%%% EQUILIBRIUM POINTS %%%%%
%
%%When $\mu=0$, the system becomes a $2$-body problem between the third body and the largest primary, $S$. Therefore, it is integrate  
%%
%For $\mu>0$, it is a well known fact that the system has five equilibrium points: $L_1$, $L_2$, $L_3$, $L_4$ and $L_5$, called Lagrange points\footnote{
%For $\mu=0$, the system has critical points $(q,p)$ with $\norm{q}=1$ and $p=K q$.
%},
%%
%(see Figure~\ref{fig:L3perturbed}(a)). 
%%
%On an inertial (non-rotating) system of coordinates, the Lagrange points move with the same period as the two primaries, i.e on a 1:1 mean motion resonance.
%
%\begin{figure}
%\subfloat[$\mu>0$]{%
%	\begin{overpic}[scale=0.7]{lagrangePointsPerturbedEsquema.png}
%		\put(43,38){{\color{blue} $q_S$ }}
%		\put(14,38){{\color{blue} $q_P$ }}
%		\put(23,45){{\color{red} $L_1$ }}
%		\put(10,45){{\color{red} $L_2$ }}
%		\put(63.5,45){{\color{red} $L_3$ }}
%		\put(27,69){{\color{red} $L_4$ }}	
%		\put(27,14){{\color{red} $L_5$ }}
%		\put(89,42){$q_2$}
%		\put(37.5,82.5){$q_1$}
%	\end{overpic}
%	\vspace{1cm}	
%}\hfill
%\subfloat[$\mu=0.003$]{%
%	\begin{overpic}[width=7.5cm]{L3manifoldsm003.png}
%		\put(50,1){$q_1$}
%		\put(12,38){$q_2$}
%		\put(71.5,37.5){{\color{red} $ L_3 \h \bullet$ }}
%		\put(37,58){{\color{red} $\bullet$ }}
%		\put(28,61){{\color{red} $L_4$ }}
%		\put(37,17){{\color{red} $\bullet$ }}	
%		\put(28,12){{\color{red} $L_5$ }}
%		\put(50.5,37.5){{\color{blue} $\bullet$ }}
%		\put(50.5,34){{\color{blue} $q_S$ }}
%		\put(23,37.5){{\color{blue} $\bullet$ }}
%		\put(23,34){{\color{blue} $q_P$ }}
%	\end{overpic}
%}
%\caption{(a) Projection onto the $q$-plane of the equilibrium points for the RPC$3$BP on rotating coordinates. (b) Plot of the stable (green) and unstable (blue) manifolds of $L_3$ projected onto the $q$-plane for $\mu=0.003$. }
%\label{fig:L3perturbed}
%\end{figure}
%
%%%%% THE POINT L3 %%%%%
%
%The Lagrange point $L_3$ is collinear with the primaries and it is on the ``opposite side'' of the primary $P$ with respect to $S$.
%%
%It is a center-saddle critical point and, hence, it has $1$-dimensional stable and unstable manifolds (which we denote by $W^{\stable}$ and $W^{\unstable}$, respectively) and a $2$-dimensional center manifold.
%
%The stable and unstable invariant manifolds have two branches each (see Figure~\ref{fig:L3perturbed}(b)).
%% 
%One pair circumvents $L_4$ 
%%(that is with $\claus{q_2>0}$), 
%we denote them by $W^{\stable,+}$ and $W^{\unstable,+}$, respectively. 
%%
%Accordingly, $W^{\stable,-}$ and $W^{\unstable,-}$ are the symmetric (see~\eqref{def:involutionCartesians}) pair of branches that circumvent $L_5$.
%%
%%Notice that, by the involution $\wt{\Phi}$, it is only necessary to compute the upper branches since the inferior branches are symmetric.
% 
%%%%% HOMOCLINIC CONNECTIONS %%%%%
%
%Since the Hamiltonian $\HInicial$ is autonomous, the invariant manifolds $W^{\unstable}$ and $W^{\stable}$ of $L_3$ may coincide (forming primary homoclinic connections) or not, but they cannot intersect transversally. 
%%
%%On a first sight, it may seem that they coincide forming a primary homoclinic connection (a connection between the branches $W^{\unstable,\pm}$ and $W^{\stable,\pm}$).
%%
%%However, it has been seen numerically that this is not the case, see~\cite{algo}.
%%
%
%
%
%%%%% HORSESHOE ORBITS %%%%%%%
%
%Over the past decades, one of the main focus of study of dynamics associated to the Lagrange point $L_3$ has been about the so called ``horseshoe-shaped orbits'', first considered in~\cite{Brown1911},
%which are quasi-periodic orbits that encompass the critical points $L_4$, $L_3$ and $L_5$.
%%
%The interest on these types of orbits arose when modeling the motion of co-orbital satellites, the most famous being Saturn’s satellites Janus and Epimetheus. 
%%
%Recently, in~\cite{NPR20}, the authors proved the existence of $2$-dimensional elliptic invariant tori on which the trajectories mimic the motions followed by these satellites.
%%
%See the references in \cite{NPR20} for more information on these type of orbits.
%
%
%%%%%%%  L4-L5 RELATION %%%%%%%%%
%
%On an averaged first order, the stable and unstable manifolds of $L_3$ coincide and separate the region of the phase space where the horseshoe-shaped orbits take place with the region where ``tadpole orbits'' occur (trajectories surrounding $L_4$ or $L_5$).
%%
%However, since the stable and unstable manifolds are $1$-dimensional, on the RPC$3$BP, the center-stable and center-unstable manifolds are the objects that separate the two different behaviors.
%
%%However, in~\cite{Chris00} the author showed that the region containing the tadpole orbits is not disconnected from the horseshoe one and that there exist transitions between these two domains. 
%%(Aixo nomes en 3D).
%
%%
%Indeed, an important question is understanding how the stable and unstable manifolds of the objects on the center manifold of $L_3$ confine regions of effective stability around $L_4$ and $L_5$ on the general restricted $3$ body problem, see \cite{SSST13}.
%%for numerical evidence
%
%
%%%%%%%% CHAOS %%%%%%%%
%
%A fundamental problem in dynamical systems is to prove that a model has chaotic motions.
%%
%In particular, in celestial mechanics models, proving the existence of chaotic motions is a notably difficult problem with very few results.
%%
%The majority of the results are found using collision orbits, see for example \cite{Moe81, BolMac06, Bol06}, or parabolic orbits (which allows to construct chaotic/oscillatory motions), see~\cite{Sitnikov1960, Alekseev1976, Moser2001, GMS16}.
%%
%Notice that, these results are found on regions where the $2$-body problem already presents some form of ``hyperbolicity''.
%%
%However, the case for the critical point $L_3$ is different. Since, though $L_3$ remains for the unperturbed problem, it does not maintain its hyperbolic character.
%%
%%As a consequence, the chaotic motions that may result from the invariant manifolds of $L_3$ will be confined to a small region of the phase-space. %\textcolor{red}{The size of this region, $\OO(\sqrt{\mu})$, is given by the two time scales of the system (see~\eqref{eq:specRot})}. 
%%
%
%%
%%Recently, on~\cite{NPR20}, the authors provided a rigorous proof of existence of 2-dimensional elliptic invariant tori on which the trajectories are similar to those followed by Janus and Epimetheus on the planar $3$-body problem.
%%%
%%(See the references therein, for more information on this type of trajectories).
%
%%Furthermore, there is numerical evidence, see \cite{SSST13}, on the fact that the stable and unstable manifolds of the objects (Lyapunov periodic orbits and 2D tori) of the center manifold of $L_3$ in the $3$-dimensional restricted $3$ body problem confine regions of effective stability around the triangular points $L_4$ and $L_5$.
%
%
%\subsection{Beyond all orders breakdown of the stable and unstable manifolds}
%
%The goal of this paper (and its companion~\cite{?}) is to prove the breakdown of the $1$-dimensional invariant manifolds of $L_3$ for $0<\mu\ll 1$.
%%
%To this end, we compute an asymptotic formula for the distance between the invariant manifolds $W^{\unstable,+}$ and $W^{\stable,+}$.
%%
%
%%
%%A perturbative analysis is convenient since it allows us to apply perturbative methods and has relevant physical interpretations \textcolor{red}{(Sun-Earth system, for example)}.
%
%%%%%% L3 FORMULAS %%%%%
%
%%We present expressions for the critical point $L_3$ for small values of $\mu$, see~\cite{Szebehely} for the details.
%%
%As $\mu \to 0$, the critical point $L_3$ satisfies that
%\begin{equation}\label{def:pointL3}
%(q,p)=(d_{\mu}, 0, 0, d_{\mu}), 
%\quad \text{with} \quad
%d_{\mu} = 1 + \frac{5}{12} \mu + \OO(\mu^3),
%\end{equation}
%%
%Moreover, the associated eigenvalues are
%\begin{equation}\label{eq:specRot}
%\mathrm{Spec}  = \claus{\pm \sqrt{\mu} \, \rho(\mu), \pm i  \, \omega(\mu) },
%\quad
%\text{with} \quad \left\{
%\begin{array}{l}
%		\rho(\mu)=\sqrt{\frac{21}{8}}  + \OO(\mu),\\[0.4em]
%		\omega(\mu)=1 + \frac{7}{8}\mu + \OO(\mu^2).
%\end{array}\right.
%\end{equation}
%%
%and the eigenvectors of the real eigenvalues are \begin{equation}\label{def:eigenvectorsL3}
%v^{\unstable} = \paren{
%- \sqrt{\frac{7\mu}{6}} ,	1 ,	-1 ,
%\sqrt{\frac{7\mu}{24}}
%}(1+\OO(\mu)), \, \,
%v^{\stable} = \paren{
%		\sqrt{\frac{7\mu}{6}} , 1 , -1 , 
%		-\sqrt{\frac{7\mu}{24}}	}(1+\OO(\mu)).
%\end{equation}
%Note that, due to the different size in the eigenvalues, the system possesses two time scales.
%%Notice that the $q_2$ component of both $v^{\unstable}$ and $v^{\stable}$ is positive, so we are considering the ``upper'' branches of the one-dimensional stable and unstable manifolds.
%%
%%(See Figure~\ref{fig:L3perturbed}(b)).
%%
%%
%%Moreover, for $\mu=0$, the saddle degenerates and~\eqref{eq:RShamiltonianInitial} posses a circle of critical points.
%%
%%From these expressions we see that, for $\mu>0$, the point $L_3$ is a center-saddle equilibrium point, with a one-dimensional stable and unstable manifold and a two-dimensional center manifold.
%%
%%(See Figure~\ref{fig:L3perturbed}(b)).
%%
%%
%%As well, if we write the differential equations of the system as $\zd = F_{\wt{H}}(z)$, then the spectrum of the linear part of the vector field for $L_3$ is
%%
%%where
%%\[
%%\rho(\mu)=\sqrt{\frac{21}{8}}  + \OO(\mu), \hh \omega(\mu)=1 + \frac{7}{8}\mu + \OO(\mu^2),
%%\]
%%\paragraph{The resonant zone.}
%%\begin{itemize}
%%	\item[--] In particular, we study the dynamics of a specific resonant region of the phase space.
%%	\item[--] On the unperturbed case ($\mu=0$), the resonance $1:1$ is the region of the phase space where the third body has the same period as the primaries.
%%	\item[--] This region includes orbits with different eccentricities. We focus on the case where, on a non-rotating framework, the third body follows a circular orbit.
%%	\item[--] On rotating coordinates, the circular orbits on 1:1 resonance correspond with the fixed points (of the unperturbed) system.
%%	\item[--] \textcolor{red}{Valdria la pena introduir el model en non-rotating per parlar m\'es f\`acilment de la resonancia 1:1?}
%%	\item[--] These fixed points satisfy
%%	\[
%%	\norm{q}=1, \quad p+Kq = (0,0).
%%	\]
%%	\item[--] We define the \emph{resonant zone} as the region close to the $1:1$ resonance and circular orbits, when $\mu \to 0$.
%%	\item[--] That is
%%	\[
%%	\norm{q}\sim 1, \quad p+Kq \sim (0,0) \text{ as } \mu \to 0.
%%	\]
%%	\item[--] \textcolor{red}{Modificar Fig 1a per incloure the resonant zone.}
%%	\item[--] On the perturbed case ($\mu>0$), the system has five equilibrium points: $L_1$, $L_2$, $L_3$, $L_4$ and $L_5$, called Lagrange points, represented in Figure~\ref{fig:L3perturbed}(a).
%%	\item[--] The five Lagrange points are found on the resonant zone.
%%	\item[--] We focus our study on $L_3$. 
%%	\item[--] \textcolor{red}{Citar~\cite{Gua13} per splitting near resonances?}
%%\end{itemize}
%%
%
%
%%%%%% OUR BREAKDOWN %%%%%
%
%Even though there is a standard theory to analyze the breakdown of stable and unstable invariant manifolds, the so called Melnikov Theory (see~\cite{Melnikov1963} and~\cite{GuckenheimerHolmes} for a more
%modern exposition),
%they cannot be applied to this setting
%due to the rapidly rotating dynamics of the system (see~\eqref{eq:specRot}).
%% we will prove through this paper and its companion \cite{?} that classical perturbative techniques are not useful when studying the breakdown of the invariant manifolds of $L_3$.
%%
%Therefore, the invariant manifolds of $L_3$ are exponentially close to each other with respect to the parameter ${\mu}$.
%%
%Namely, its difference cannot be detected in the truncation of their normal form at any finite order and, as it is usually called, it is a \emph{beyond all orders} phenomenon.
%
%
%%%%% EXPONENTIALLY SMALL SPLITTING  %%%%%
%
%%The first tool to study this phenomenon was given by Melnikov (developing some ideas by Poincar\'e) on~\cite{Melnikov1963} (see~\cite{GuckenheimerHolmes} for a more
%%modern exposition). 
%%%
%%The Poincar\'e– Melnikov method provides asymptotic expressions of the distance (and other related quantities) between the perturbed invariant manifolds, when the perturbative parameter tends to zero.
%%%
%%The first order of the difference is given by a function called the Melnikov function. 
%%
%%However, a difficult question arises when the Melnikov function turns out to be exponentially small with respect to the perturbative parameter and hence is not a priori the dominant term. 
%%
%%
%%This setting is usually referred to as the {exponentially small splitting of separatrices} phenomenon.
%%
%This situation is nowadays referred to as the exponentially small splitting of separatrices phenomenon and was first pointed out by Poincar\'e in~\cite{Poincare1890}.
%%
%The first work that dealt with this kind of
%problem was by Lazutkin in~\cite{Laz84, Laz05}.
%%
%There, the author studied the splitting of separatrices for the standard map, and gave the main tools to obtain an asymptotic formula for it.
%%
%Even if Lazutkin's work was not complete (the complete proof was achieved by
%Gelfreich in~\cite{Gel99}), the ideas in this paper established the basis of the methods used later.
%%
%%A new approach that avoids some complications of
%%Lazutkin's method and that has had much influence in posterior studies of exponentially
%%small splitting was introduced in~\cite{Sau01, LMS03}.
%
%The exponentially small splitting of separatrices has been studied in rapidly forced periodic or quasi-periodic perturbations of $1$-degree of freedom Hamiltonian systems, \cite{HMS88, DelSea92, Fon93, Gel94, Fon95, DelSea97, Gel97a, Tre97, Gel00, BF04, BF05, GOS10, BFGS12}, in nearly integrable symplectic mappings that are close to the identity, see \cite{FS90a, FS90b, DelRRR98, MSS11}, and in Hamiltonian systems with two or more degrees of freedom which have hyperbolic tori with some fast frequencies \cite{Sau01, GaiGel10,Lom00, BCS13,BCS18a, BCS18b, GGS20}, among
%others.
%%
%%These singular cases are also known as rapidly forced systems.
%%
%
%%
%%Later on, asymptotic formulas for several examples were obtained (see~\cite{KruSeg91, DelSea92, DelSea97, Gel97a, Sau01, LMS03, BF04, BF05}).
%%
%%A new approach that has had much influence in posterior studies of exponentially small splitting was introduced in~\cite{Sau01, LMS03}.
%%
%%Note that, besides~\cite{Laz05} and~\cite{KruSeg91}, all the examples cited above deal with the regular case, namely when the Melnikov method gives the correct size of the splitting.
%
%The singular cases are those where the splitting of separatrices is still exponentially small but its asymptotic first order is no longer given by the Melnikov function.
%%
%On this case, one often has to study a certain equation, called the \emph{inner equation}. Some results corresponding inner equations can be found on \cite{Gel97b, GS01, OSS03, Bal06, BalSea08, BM12}.
%%
%
%%%% CONCLUSION %%%%
%
%In conclusion, one of the interests behind the study of the breakdown of the $1$-dimensional invariant manifolds of $L_3$ is to prove the none existence of primary homoclinic connections of $L_3$.
%%
%Additionally, it make sense to claim that this result would be an important first step to understand some of the dynamic motions and chaotic phenomena surrounding different objects of $L_3$ (Lyapunov periodic orbits, for example).
%
%Regarding secondary homoclinic connections (connections between the opposed branches $W^{\unstable,\pm}$ and $W^{\stable,\mp}$) for $L_3$,
%in~\cite{BMO09}, the authors conjecture (based on numerics) their existence for a sequence of values $\claus{\mu_k}_{k \in \naturals}$ such that $\mu_k\to 0$ as $k \to \infty$. 
%
%\textcolor{red}{Parlar dels future goals: chaos and secondary homoclinic.}
%
%%There are very few works with rigorous proofs in the singular case, see for instance \cite{Tre97, Gel00, GOS10,MSS11}.
%%
%%In particular, the most general
%%result dealing with Hamiltonian systems with a periodic perturbation in time is given in~\cite{BFGS12, Gua13}.
%
%%for Hamiltonian systems of two degrees of freedom
%%Moreover, in~\cite{BCS13,BCS18a, BCS18b} the authors study the breakdown of a one-dimensional and two-dimensional heteroclinic connection in the generic Hopf-zero singularity, respectively. 
%%%
%%In~\cite{GGS20}, the authors study a partial differential equation by considering the heteroclinic breakdowns of a finite-dimensional reduction of the equation given by a two degrees of freedom Hamiltonian.
%
%\subsection{Outline}
%
%%The tools used in the splitting of separatrices methods to compute the distance between manifolds rely on the existence of a (primary) homoclinic connection or separatrix for the unperturbed case.
%%
%%This connection is usually referred to as the \emph{separatrix} of the system.
%%
%%However, the critical point $L_3$ is nilpotent when $\mu=0$ (see~\eqref{eq:specRot}) and, as a consequence, it does not have stable nor unstable manifolds, but a circle of fixed points.
%
%%Traditionally, the splitting of separatrices method is used with the aim of finding transversal intersections of the manifolds.
%%%
%%Since, as it is well known, the transversal intersection of invariant manifolds is one of the main causes of the appearance of chaos.
%%
%%However, for the splitting of separatrices of $L_3$, transversal intersection do not exist. 
%%%
%%Nevertheless, in other instances, the computing of the splitting on autonomous systems has been used to prove different chaotic phenomena, see~\cite{BIS20}.
%%\textcolor{red}{(Comentar)}
%
%
%%This difficulty, has been noticed to take place in different settings. 
%%%
%%This happens, for instance, in rapidly forced periodic or quasi-periodic perturbations of one-degree-of-freedom Hamiltonian systems \textcolor{red}{(see ...)}, 
%%nearly integrable symplectic mappings that are close to the identity	\textcolor{red}{(See ...)} or Hamiltonian systems with two or more degrees of freedom which have hyperbolic tori with some fast frequencies \textcolor{red}{(see ...)}.
%
%%\begin{itemize}
%%	\item[--] Melnikov~\cite{Melnikov1963} (developing some ideas by Poincar\'e) gave a tool, which is called Poincar\'e–Melnikov function, to provide asymptotic expressions of the distance (and other related quantities) between the perturbed invariant manifolds, when $\mu \to 0$.
%%	\item[--] The Poincar\'e--Melnikov method gives us an asymptotic formula for the distance
%%between the stable and unstable invariant manifolds, on the parameter $\mu$. 
%%See, for
%%instance,~\cite{Melnikov1963, GuckenheimerHolmes, WigginsGlobalBifurcations}. The first order is given by a function, called the Melnikov function. 
%%	\item[--] The classical perturbative techniques theory to analyze the intersection of stable and unstable invariant manifolds, such as Poincaré–Melnikov, do not work in this setting. (Frase de GMS16)
%%	\item[--] This implies that there is no hope that classical perturbative techniques, such as
%%Melnikov Theory, will allow to study the possible intersection of these manifolds. (frase Gua13)
%%	\item[--] Melnikov~\cite{Melnikov1963} (developing some ideas by Poincar\'e) gave a tool, which is called Poincar\'e–Melnikov method, to provide asymptotic expressions of the distance (and other related quantities) between the perturbed invariant manifolds, when the perturbative parameter $\mu \to 0$.
%%	\item[--] The first order is given by a 	function, called the Melnikov function.  
%%	See, for instance,~\cite{GuckenheimerHolmes}.
%%	\item[--] The phenomenon of splitting of separatrices has been widely studied by several authors, see for instance~\cite{GuckenheimerHolmes, WigginsGlobalBifurcations}. 
%%	\item[--] A difficult question arises when the Melnikov function turns out to be exponentially small with respect to $\mu$ and hence is not a priori the dominant term. (frase BalSea06)
%%	%\item[--] Fast rotating term lead us to a exponentially small splitting.
%%	\item[--] This situation is nowadays referred to as the exponentially small	splitting of separatrices phenomenon.
%%	\item[--] This difficulty, has been noticed to take place in different settings. This happens, for instance, in
%%	\begin{itemize}
%%		\item Rapidly forced periodic or quasi-periodic perturbations of one-degree-of-freedom Hamiltonian systems. \textcolor{red}{(See ...)}
%%		\item Nearly integrable symplectic 	mappings that are close to the identity
%%		\textcolor{red}{(See ...)}
%%		\item Hamiltonian systems with two or
%%		more degrees of freedom which have hyperbolic tori with some fast frequencies. \textcolor{red}{(See ...)}
%%	\end{itemize}
%%	\item[--] Moreover, there are two types of cases depending on the validity of the Melnikov function.
%%	\begin{itemize}
%%		\item The regular cases are those were assuming some condition about the smallness of the perturbation, the Melnikov method gives the correct size of the splitting.
%%		\item The singular cases are those where the splitting of separatrices is still exponentially small but its asymptotic first order is no longer given by the Melnikov function.
%%	\end{itemize}
%%	\item[--] During the development of the problem it was seen that is singular.
%%	\item[--] To study the singular case one needs to study the inner equation and use matching techniques to relate different approximations for the invariant manifolds.
%%	\item[--] The first author who dealt with this singular case was Lazutkin in [Laz84, Laz03]. He studied the splitting of separatrices of the Chirikov standard map, and gave the main idea that inspired most of the works in the subject: one needs to deal with suitable complex parameterizations
%%	of the invariant manifolds.
%%	\item[--] Examples of Inner equations. \textcolor{red}{(See ...)}
%%\end{itemize}
%
%
%In this work and~\cite{?} we 
%analyze the distance between the $1$-dimensional invariant manifolds of $L_3$ and give an asymptotic formula for its difference.
%%
%%Indeed, in~\cite{?} we give asymptotic formulas for the distance between the stable and unstable manifolds of $L_3$.
%%
%\textcolor{red}{The method we use follows the approaches described, for example, in~\cite{BFGS12, BCS13}.}
%%
%Roughly speaking, the method is as follows:
%\begin{enumerate}[label*=\Alph*.]
%	\item We perform a change of coordinates which captures the slow-fast dynamics of the system.
%	%
%	The new Hamiltonian becomes a (fast) oscillator weakly coupled to a $1$-degree of freedom Hamiltonian with a saddle and an homoclinic connection (also know as separatrix).
%	%
%	To obtain this new system, we use the Poincar\'e planar elements (see~\cite{MeyerHallOffin}).
%	%These variables do not have an explicit expression, which difficult the analysis of the new Hamiltonian.
%	%
%	\item We analyze the analytical continuation of the time-parametrization of the unperturbed separatrix.
%	%
%	In particular, we obtain the maximal strip of analyticity (centered at the real line) for the parametrization.
%	%
%	We also describe the singularities and its character at the boundaries of this region.
%	%
%	
%	Finally, for technical reasons, we also have to analyze the zeros of the derivative of the first component of the separatrix, where the parameterization of the perturbed invariant manifold fails to be a graph over the first component of the separatrix.
%% 	. This is not necessary for the analysis of the splitting of separatrices. However, since later in Item D we parameterize the perturbed invariant manifolds as graphs, the analysis of the zeros is necessary to control when the graph property breaks down.
%% 	
%	
%	\item We derive the inner equation, which gives the first order of the original system close to the singularities.
%	%
%	This equation is independent of the perturbative parameter and possesses two special solutions which are approximations of the perturbed invariant manifolds near the singularities.
%	%
%	Moreover, we provide an asymptotic formula for the difference between the two solutions of the inner equation.
%	%
%	We follow the approach presented in~\cite{BalSea08}.
%	%
%	\item We prove the existence of the analytic continuation of suitable (graph) parametrizations of the invariant manifolds of $L_3$, $W^{\unstable}$ and $W^{\stable}$, in appropriate complex domains, the so called outer domains.
%	%
%	These domains contain a segment of
%	the real line and intersects a neighborhood sufficiently close to the singularities of the separatrix.
%	%
%	\item By using complex matching techniques, we compare the solutions of the inner equation with the perturbed invariant manifolds on the outer domain.
%	%
%	\item Finally, we prove that the dominant term of the difference between manifolds is given by the term obtained from the difference of the solutions of the inner equation.
%\end{enumerate}
%
%In this work, we perform the preliminary change of coordinates (Step A) and deal with the results  concerning the analysis of the invariant manifolds near their singularities: the singularity analysis of the separatrix (Step B) and the derivation and analysis of the inner equation (Step C). 
%%
%The final result for the distance between invariant manifolds and the remaining of the proof (Steps D, E and F) is found on~\cite{?}.
%
%
%%In order to introduce a singular change of coordinates, we use the Poincar\'e planar elements (see~\cite{MeyerHallOffin}).
%%
%%These variables do not have an explicit expression, this complicates the definition of the singular change of coordinates and later the derivation of the inner equation.
%%
%%To analyze the inner equation, we follow the approach presented in~\cite{BalSea08}.
%
%On all the previous mentioned works on splitting of separatrices, either the separatrix has an analytic expression (see for example~\cite{DelSea92,GaiGel10,GOS10,BCS13,GMS16}) or otherwise certain properties of its analytic continuation are given as assumptions (see~\cite{DelSea97,Gel97b,BF04, BFGS12}).
%%
%%From a numerical point of view, in~\cite{SimoGelf08} the authors presented a numerical method to study the singularities of the separatrices of different area preserving maps.
%%
%In this paper, we do not have an explicit expression for the separatrix and we obtain its singularities by performing a detailed analysis of the first order Hamiltonian obtained in Step A.
%%
%In particular, we describe the parametrization of the separatrix in terms of a multivalued function involving a complex integral.
%%
%Then, by analyzing and classifying all the possible integration paths, we are able to characterize and locate certain singularities of the unperturbed separatrix.
%
%%obtain the information necessary of the separatrix to proceed with the study.
%
%
%%present an alternative analytic method (applied to the case of $L_3$) to compute the singularities of a non-explicit separatrix.
%%%
%%This method requires the use of complex integration techniques and Riemann surfaces.
%%%
%%As far as the authors are aware, this is the only result where the explicit parametrization of the homoclinic connection is unknown.
%%
%%To be able to apply the tools of splitting of separatrices, we apply a singular change of coordinates to the system.
%%%
%%This change of coordinates ``blows-up'' the singularity of the unperturbed system in $L_3$ to capture its slow-dynamics. 
%%%
%%(See Section~\ref{subsection:reformulation}).
%%
%%As a result, we obtain an equivalent Hamiltonian with a new ``unperturbed'' or first order part, which possesses a saddle-center equilibrium point (corresponding with $L_3$) with a separatrix.
%%
%
%The structure of this paper goes as follows. 
%%
%In Section \ref{section:mainResults} we present the main result for the Steps A, B and C above and introduce some heuristics to contextualize them.
%%
%Sections \ref{section:proofA-singularities}-\ref{section:proofD-AnalysisInner} are devoted to the proof of the results in Section~\ref{section:mainResults}.
%
%In particular, in Section \ref{subsection:reformulation}, we detail the singular change of coordinates that allow us to obtain a new Hamiltonian (Step A).
%%
%In Section \ref{subsection:singularities} (see also Section \ref{section:proofA-singularities}), we study the analytic continuation of the separatrix and its singularities (Step B).
%%
%In Section \ref{subsection:innerDerivation} (see also Section \ref{section:proofBC-poincareFormulasInnerDerivation}), we introduce the ideas behind the inner change of coordinates and use it to derive the inner equation (first part of Step C).
%%
%Finally, in Section \ref{subsection:innerComputations} (see also Section \ref{section:proofD-AnalysisInner}), we study special solutions of the inner equation and give asymptotics for its difference (second part of Step C).
%%
%%Sections~\ref{section:proofA-singularities}-\ref{section:proofD-AnalysisInner} are devoted to the proof of the results in Section~\ref{section:mainResults}.
%
%
%
%
%
%%Consider the projection of Hamiltonian~\eqref{eq:RShamiltonianFinal} to $(\la,\La)$ with $\mu=0$. Then, it can be seen that the stable and unstable manifolds of the saddle coincide and form two homoclinic connections, as represented in Figure~\ref{fig:L3unperturbed}(b). A fundamental question is whether do they persist if the full problem with $\mu>0$ is considered. It is believed that the separatrices break down. However, traditional methods can not be applied, as the center is of order $\OO(\frac{1}{\sqrt{\mu}})$. This indicates that the perturbation has fast rotation which implies that the splitting is exponentially small. Accordingly, the primary objective of this thesis is to compute the distance between the stable and unstable manifolds by means of exponentially small splitting of separatrices techniques. 
%%
%%It is worth noticing that there can not exist transverse homoclinic points, as in the traditional Poincar\'e--Melnikov method setting. This is because the problem considered is an autonomous $4$-dimensional system with one-dimensional stable and unstable \mbox{manifolds}. Therefore they either coincide or are have empty intersection.
%


==> Article Inner/outerHeuristics.tex <==
%\section{Heursitics of the perturbed manifolds} \label{section:outer}

% In this section we present the so-called inner equation associated to the Hamiltonian $H$ in \eqref{def:hamiltonianScaling}.
%
The inner equation  associated to the Hamiltonian $H$ in \eqref{def:hamiltonianScaling} describes the dominant behavior of suitable complex parametrizations of the invariant manifolds  close to (one of) the singularities $\pm iA$ of the unperturbed separatrix. %See~\cite{Bal06, BalSea08}.
%The inner equation provides good approximations of the invariant manifolds near the singularities of the unperturbed problem: in our case $\pm iA$ as given in Theorem~\ref{theorem:singularities}.
Let us explain how this equation arises from the Hamiltonian $H$. 
%
%The study of this inner equation will allow us to capture the asymptotic first order of the difference between the invariant manifolds of critical point $\Ltres(\de)$. See Proposition~\ref{proposition:HamiltonianScaling}.
%
%First, we consider the critical points of Hamiltonian $H$ in~\eqref{def:hamiltonianScaling}.
%fixed point $L_3$ on the set of coordinates $(\la,\La,x,y)$ introduced in~\eqref{def:changeScaling}.
%
%\begin{lemma}
%	For $\de\geq 0$ small enough, the Hamiltonian system associated with $H$, see~\eqref{def:hamiltonianScaling}, has a critical point at
%	\begin{equation}\label{def:PfixPoint}
%		P^*(\de)= \Big(\de^2 \la^*(\de), \de^2 \La^*(\de),
%		\de^3 x^*(\de), \de^3 y^*(\de) \Big) ,
%	\end{equation}
%	with
%	$\vabs{\la^*(\de)},  \vabs{\La^*(\de)} , \vabs{x^*(\de)},  \vabs{y^*(\de)} \leq C
%	$,
%	for some constant $C>0$ independent of $\de$.
%\end{lemma}
%The critical point $P^*(\de)$ is just the $L_3$ point expressed on the set of coordinates $(\la,\La,x,y)$, introduced in~\eqref{def:changeScaling}.
%
%The first step is to study the stable and unstable invariant manifolds of $\Ltres(\de)$ for the complete system given by Hamiltonian $H$ in~\eqref{def:hamiltonianScaling}.
%


First, we consider the translation of the equilibrium point $\Ltres(\de)$ to the origin, 
\begin{equation}\label{def:changeEqui}
	\phi_{\equi}:(\la,\La,x,y) \mapsto (\la,\La,x,y) + \Ltres(\de).
\end{equation}
Second, to measure the distance of the stable and unstable manifolds, we parameterize them as graphs.
%
In the unperturbed case, we know that the invariant manifolds coincide along the separatrix $(\la_h(t),\La_h(t),0,0)$.
%
Since we need to involve, in some sense, the time; we consider as a new independent variable $u$ such that $\la_h(u)=\la$. 
%
Notice that $\dot{u}=1$ for the unperturbed system.
%
To this end, we consider the symplectic change of coordinates 
\begin{equation}\label{def:changeOuter}
\phi_{\out}:(u,w,\xp,\yp) \to (\la,\La,\xh,\yh),
\qquad 
{\la}= \la_h(u), 
\quad
 {\La}= \La_h(u) - \frac{w}{3\La_h(u)},
\end{equation}
where $\s=(\la_h,\La_h)$ is the parametrization of the separatrix studied in Theorem~\ref{theorem:singularities}. 
%This change is symplectic and therefore the system given by $H \circ \phi_h^{-1}$ is also Hamiltonian.
%
Notice that, except for $u=0$ (see Proposition~\ref{proposition:domainSeparatrix}), the perturbed manifolds can be expressed as a graph and the change \eqref{def:changeOuter} is well defined. 

The Hamiltonian $H$, written in these coordinates and after the translation $\phi_{\equi}$ in~\eqref{def:changeEqui}, becomes
%with respect to the symplectic form ${d u \wedge d w} + i \h {d\xp \wedge d\yp}$ with Hamiltonian
\begin{equation}\label{def:hamiltonianOuter}
H^{\out} =  H^{\out}_0 +  H^{\out}_1,
\end{equation}
with 
\begin{equation*}%\label{def:hamiltonianOuterSplit}
\begin{split}
H^{\out}_0(w,x,y) &= 
w + \frac{xy}{\de^2}, \qquad
%- \frac{w^2}{6 \La_h^2(u)} 
%
H^{\out}_1 =
{H} \circ \paren{\phi_{\equi} \circ \phi_{\out}} -H^{\out}_0.
\end{split}
\end{equation*}
%After all these consideration it seems a good strategy to 
Since we look for the perturbed manifolds as graphs with respect to $u$, we consider
 parametrizations
\[
\zdOut(u) = \left(\wdOut(u),\xdOut(u),\ydOut(u)\right)^T,
\quad \text{ for } \diamond=\unstable,\stable,
\]
such that the unstable  and stable invariant manifolds of $H$ associated to $\Ltres(\de)$ can be expressed as
\begin{equation*}%\label{eq:invariantManifoldsExpression}
W^{\diamond}= \left\{ \paren{\la_h(u), \La_h(u)-\frac{\wdOut(u)}{3\La_h(u)}, \xdOut(u), \ydOut(u)} + \Ltres(\de)\right\}, \quad \text{for } \diamond=\unstable,\stable,
\end{equation*}
%\footnote{In these coordinates, the unperturbed separatrix is  $\{(w,x,y)=(0,0,0)\}$.}
with $u$ belonging to appropriate domains.
%
The proof of existence of $\zuOut$ and $\zsOut$ defined in appropriate (complex) domains requires a significant amount of technicalities. 
%
We present this result in the companion paper, see~\cite{articleOuter}.

%
%Therefore, we look for solutions satisfying  the asymptotic conditions 
%\begin{equation}\label{eq:asymptoticConditionsOuter}
%\begin{split}
%\lim_{\Re(u) \to -\infty} \left(\frac{\wuOut(u)}{\La_h(u)},\xuOut(u), \yuOut(u) \right) = %0, \hh
%\lim_{\Re(u) \to +\infty} \left(\frac{\wsOut(u)}{\La_h(u)},\xsOut(u), \ysOut(u) \right) = 0.
%\end{split}
%\end{equation}
%
%Notice that, by Proposition~\ref{proposition:domainSeparatrix}, the invariant manifolds can not be written as a graph globally, as the change of variables $\phi_{\out}$ is not defined for  $u= 0$.

%The difference $\dzOut=\zuOut-\zsOut$ is exponentially small in $\de$. 
%
%To obtain an asymptotic formula for $\dzOut=\zuOut-\zsOut$, we need to analyze $\zuOut$ and $\zsOut$ in a suitable domain of the complex plane. 
%
%These domains must contain a segment of the real line and must intersect a neighborhood sufficiently close to the singularities $\pm iA$ of $(\la_h(u),\La_h(u))$, see~\cite{BFGS12}. 




==> Article Inner/polarCoordinates.tex <==

When studying a close to integrable Hamiltonian system at a resonance, it is usual to ``blow-up'' the ``resonant zone'' to capture the slow-fast time scales.
%
In this section we present the singular change of coordinates which transforms the Hamiltonian $h$ in \eqref{def:hamiltonianInitialNotSplit} into a pendulum-like Hamiltonian plus a fast oscillator with a small coupling, namely
\[
H(\la,\La,x,y) = 
-\frac{3}{2}\La^2 + V(\la) +
\frac{x y}{\sqrt{\mu}} + o(1),
\]
with respect to the symplectic form $d\la \wedge d\La + i dx \wedge dy$.
%
In these coordinates, the first order of the  Hamiltonian has a saddle in the $(\la,\La)$--plane and a center in the $(x,y)$--plane.
%
Notice that the system possesses two time scales ($\sim 1$ and $\sim1/{\sqrt{\mu}}$). Recall that this two time scales are also present in the eigenvalues of $L_3$ in~\eqref{eq:specRot}.

We consider Poincar\'e coordinates for the RPC$3$BP (see~\eqref{def:hamiltonianInitialNotSplit}) in order to write the system as a close to integrable Hamiltonian system and decouple (at first order) the saddle and the center behaviour.
%
To this end, we first consider the symplectic polar and Delaunay coordinates.
%
%Finally, we perform a singular scaling.


\paragraph{Polar Coordinates.}
%
%Let us consider first Hamiltonian \eqref{eq:RShamiltonianInitial} on polar coordinates. 
%
Let us consider the change of coordinates: 
\[
\phi_{\pol}:(r,\tht,R,G) \mapsto (q,p),
\]
where $r$ is the radius, $\tht$ the argument of $q$, $R$ the linear momentum in the $r$ direction and $G$ is the angular momentum.
%
Then, the Hamiltonian~\eqref{def:hamiltonianInitialNotSplit}, becomes %defines a Hamiltonian system, with respect to the symplectic form $dr \wedge dR + d\tht \wedge dG$, with Hamiltonian:
\begin{equation}\label{def:hamiltonianPolars}
	H^{\pol} = H_0^{\pol} + \mu H_1^{\pol},
\end{equation}
where
\begin{equation} \label{def:hamiltonianPolarsSplitting}
\begin{split}
H^{\pol}_0(r,R,G) &= \frac{1}{2} \paren{ R^2 + \frac{G^2}{r^2} } - \frac{1}{r} - G,  \\
%
\mu H^{\pol}_1(r,\theta;\mu) &= 
\frac{1}{r} -
\frac{ 1-\mu}{\sqrt{r^2-2\mu r\cos \tht + \mu^2}}
- \frac{\mu}{\sqrt{r^2+2(1-\mu) r\cos\tht +(1-\mu)^2}}.
\end{split}
\end{equation}
%
The critical point $L_3$ (see~\cite{Szebehely} for the details) satisfies that, as $\mu \to 0$,
\begin{equation}\label{def:pointL3}
(r,\tht,R,G) = (d_{\mu},0,0,d_{\mu}^2), 
\qquad \text{with} \quad
d_{\mu} = 1 + \frac{5}{12} \mu + \OO(\mu^3).
\end{equation}

%In polar coordinates, the critical point $L_3$ (see~\eqref{def:pointL3}) satisfies
%\begin{equation}\label{eq:pointL3polars}
%(r,\tht,R,G) = (d_{\mu},0,0,d_{\mu}^2) 
%= \big(1+\OO(\mu),0,0,1+\OO(\mu)\big),
%\quad \text{as } \mu \to 0.
%\end{equation}

%\begin{equation} \label{def:hamiltonianPolarsSplitting}
%	\begin{split}
%		H^{\pol}_0(r,R,G) &= \frac{1}{2} \left\{ R^2 + \frac{G^2}{r^2} \right\} - \frac{1}{r} - G,  \\
%		%
%		\mu H^{\pol}_1(r,\theta;\mu) &= D^{\pol}[0] + \left( \mu- 1 \right) D^{\pol}[\mu]
%		- \mu D^{\pol}[\mu-1], 
%	\end{split}
%\end{equation}
%with 
%\begin{equation}\label{def:functionD}
%	D^{\pol}[\zeta](r,\tht)=(r^2-2\zeta r\cos \tht + \zeta^2)^{-1/2}.
%\end{equation}
%Notice that $\mu H_1^{\pol,S}+\mu H_1^{\pol,J}$ is a perturbation of size $\OO(\mu)$ when the third body is ``far'' from the primaries, situation that it includes $L_3$. 
%Notice that we have split the perturbation on two: the $\mu H_1^{\pol,S}$ term concerns the perturbation given by the big primary, and the $\mu H_1^{\pol,J}$ term relates to the perturbation given by the small primary.


==> Article Inner/proofA-ClassificationSingularities.tex <==
\subsection{Classification of the singularities of \texorpdfstring{$q(t)$}{q(t)}} \label{subsection:classificationSingularities}

Equation~\eqref{eq:odeSeparatrixQ} with initial condition $q(0)= a_+ =-\frac{1}{2}+\frac{\sqrt{2}}{2}$ is equivalent to 
\begin{align*}
t = \int_{a_+}^{q(t)} f(s) ds, 
\qquad \text{for }  t\in \reals, 
\end{align*}
%To extend $q(t)$ to the complex plane, we define the real-valued function
where
\begin{equation*}%\label{def:functionf}
 f(q)=\frac{1}{q-1}\sqrt{\frac{q}{3(q+1)(q-a_+)(q-a_-)}},
\end{equation*}
is defined in $\reals \setminus \{ [a_-,-1] \cup (0,a_+] \cup \{1\} \} $
with $a_{\pm}=-\frac{1}{2}\pm\frac{\sqrt{2}}{2}$.
%
%Since we are studying the parametrization $q(t)$ such that $q(0)=a_+$, equation~\eqref{eq:odeSeparatrixQ} for $q(t)$ is equivalent to
%\begin{align*}
%t = \int_{a_+}^{q(t)} f(s) ds.
%\end{align*}
From~\cite{Fon95}, we know that there exist $\upsilon>0$ such that $q(t)$ can be extended to the open complex strip 
\begin{equation*}%\label{def:PiXi}
\Pi_{\upsilon} = \{ t \in \complexs \st  |\Im t|< \upsilon \},
\end{equation*}
and  $q(t)$ has singularities in $\partial \Pi_{\upsilon}$. Namely,
\begin{align}\label{proof:integralReals}
t = \int_{a_+}^{q(t)} f(q) dq, 
\qquad \text{for }  t\in \Pi_{\upsilon}.
\end{align}

Since $f$ is a multi-valued function in the complex plane, in order to analyze the possible values of $\int_{a_+}^{q(t)} f(s) ds$, we consider its complete analytic continuation. That is,
\begin{align}\label{eq:fcompleteanalytic}
\begin{array}{rl}
\fh: \mathscr{R}_f &\to \complexs  \\
\Big(q;\arg \argf(q)\Big) &\mapsto
%q &\to 
\displaystyle \frac{\sqrt{\argf(q)}}{q-1},
\end{array}
\quad \text{where} \quad 
\argf(q)=\frac{q}{3 (q+1)(q-a_+)(q-a_-)},
\end{align}
and $\mathscr{R}_f$ is the Riemann surface associated to $f$.
%see~\cite{Conway}. 
%
We define ${\proj:\mathscr{R}_f \to \complexs}$ as the projection to the complex plane.
%
We choose the first Riemann sheet to correspond to ${\arg \argf(q) \in (-\pi,\pi]}$. Accordingly the second Riemann sheet corresponds to $(\pi, 3\pi]$. 


To integrate $\fh$ along a path $\g \subset \mathscr{R}_f$, we introduce the notation
% \[
% \int_{q_{\ini}}^{q_{\fin}} \fh(s) d\g(s) = \int_{\g} \fh(q) dq,
% \]	
\[
\int_{\g} \fh(q) dq=\int_{q_{\ini}}^{q_{\fin}} \fh d\g =\int_{s_{\ini}}^{s_{\fin}} \fh(\g(s)) \g'(s)ds ,
\]	
such that $\g:(s_{\ini},s_{\fin}) \to \mathscr{R}_f$ where $\lim_{s \to s_{\ini}} \proj \g(s)=q_{\ini}$ and $\lim_{s \to s_{\fin}} \proj \g(s)=q_{\fin}$.
%
Moreover, we assume that the paths $\g \subset \mathscr{R}_f$ are $\CC^0$ and $\CC^1\text{-piecewise}$.
%
Therefore, by~\eqref{proof:integralReals}, we have that
\begin{equation}\label{eq:lemmaIntegralEquationGeneral}
t = \int_{a_+}^{q(t)} \fh d \g,
\qquad \text{for }  t\in \Pi_{\upsilon}.
\end{equation}
%
Now, for $q\in\mathscr{R}_f$ and an integration path $\g \subset \mathscr{R}_f$,  we define the function $G$ as the right hand side of~\eqref{eq:lemmaIntegralEquationGeneral},
\[
G(q)= \int_{a_+}^{q} \hat{f} \h d\g.
\]
%
Notice that for a given $q\in\mathscr{R}_f$, $G(q)$ may depend on the integration path, and therefore,  $G$ may be multi-valued on $\mathscr{R}_f$.
%
However, by~\eqref{eq:lemmaIntegralEquationGeneral}, $G$ is single-valued when 
\[
t=G(q(t)), \qquad \text{for } t \in \Pi_{\upsilon}.
\]
%
We use $G$ to characterize and locate the singularities of $q(t)$.
%
Indeed, if function $G(q)$ is biholomorphic at $q=q^*$, then $q(t)$ is analytic at a neighborhood of all values of $t$ such that $q(t)=q^*$.
%
Therefore, $q(t)$ may have singularities at $t=t^*$ when the hypothesis of the Inverse Function Theorem are not satisfied for $G$.
%
That is, for $q(t^*)=q^*$ such that either
\begin{align}\label{eq:conditionsInverseTheo}
G'(q^*)= 0, \qquad
%
G \notin \CC^1 \text{ at }
q=q^*, 
%
\qquad \text{or} \quad
%
\vabs{q^*} \to \infty.
\end{align}
%
Namely, when there exist $q^*$ and $\g \subset \mathscr{R}_f$ satisfying~\eqref{eq:conditionsInverseTheo},
 such that 
\begin{equation}\label{eq:lemmaIntegralEquationSingularities}
t^* = G(q^*) = \int_{a_+}^{q^*} \hat{f} \h  d\g.
\end{equation}
%
Since $G$ is a multivalued function, the values of $t^*$ can, and in fact will, depend on the integration path on $\g \subset \mathscr{R}_f$.
%
From \eqref{eq:fcompleteanalytic} and \eqref{eq:conditionsInverseTheo}, one deduces that the singularities may take place only if $q(t^*)=q^*$ with
\begin{equation}\label{eq:candidatesSingularities}
q^*=0,1,-1, a_+, a_- 
\qquad \text{and} \qquad 
\vabs{q^*} \to \infty.
\end{equation}
The following proposition proves that we only need to consider $\vabs{q^*} \to \infty$ and $q^*=0$ .

\begin{proposition} \label{proposition:singularitiesSeparatrix}
 Let $q(t)$ be a solution of equation~\eqref{eq:odeSeparatrixQ} with initial condition $q(0)=a_+$. Then, the singularities $t^* \in \complexs$ of the analytic extension of $q(t)$ are characterized by  either
\begin{equation*} %\label{eq:integralPolesSection}
 t^* = \int_{a_+}^{0} \hat{f} \h d\g, 
 \hh  \text{ or } \hh
 t^* = \int_{a_+}^{\infty} \hat{f} \h d\g,
\end{equation*}
for some path $\g \subset \mathscr{R}_f$.

%where $\g\subset \mathscr{R}_f$ is a path from $q=a_+$ to $q=0$ or $\vabs{q} \to \infty$.
Moreover:
\begin{itemize}
%\item If $t^*=t^*_{0}(\g)$, then 
\item If $t^*=\int_{a_+}^0 \fh d\g$
and $\Im t^*>0$ with 
$\arg \paren{t-t^*} \in \paren{-\frac{3\pi}{2},\frac{\pi}{2}}$, then
\begin{equation}
\label{eq:singularitatExpressio}
q(t) = -\frac{3\al}{2}  (t-t^*)^{\frac{2}{3}} + \OO(t-t^*)^{\frac{4}{3}}, \qquad
\text{for } \h 0<|t-t^*|\ll 1,
\end{equation}
where  $\al \in \complexs$ satisfies $\al^3=\frac{1}{2}$. 
%
If $\Im t^*<0$ and
$\arg\paren{t-t^*} \in \paren{-\frac{\pi}{2},\frac{3\pi}{2}}$, the same holds true.
%
\item If $t^*=\int_{a_+}^{\infty} \fh d\g$, 
then
\begin{equation}
\label{eq:singularitatExpressioInfinit}
q(t) = - \frac{1}{\sqrt{3}(t-t^*)}\left( 1 + \OO(t-t^*)\right),
 \qquad
 \text{for } \h 0<|t-t^*|\ll 1.
\end{equation}
%where $\beta \in \complexs$ such that $\beta^2=\frac{1}{3}$ and 
\end{itemize}
\end{proposition}
%\begin{remark}
%it is worth noticing that, for $q^*=\infty$, the corresponding singularities $t^*$ of $(q(t),\qd(t))$ are singularities for both $q(t)$ and $\qd(t)$. However, for $q^*=0$, the corresponding singularities of $(q(t),\qd(t))$ are only singularities for $\qd(t)$ and are zeroes for $q(t)$.
%\end{remark}

%\begin{proof}
%From differential equation~\eqref{eq:odeSeparatrixQ}, we have
%\[
% t-t_0 =\int_{q_0}^q \frac{1}{s-1}\sqrt{\frac{s}{3(s+1)(s-a_-)(s-a_+)}} d\g(s).
%\]
%for some initial condition $q(t_0)=q_0$. To compute this integral we use the Riemann surface $\mathscr{R}_f$ and the complete analytic continuation of $f$ as defined on~\eqref{eq:fcompleteanalytic}. Thus
%\begin{equation} \label{eq:lemmaIntegralEquationGeneral}
%t-t_0= \int_{q_0}^{q} \hat{f}(s) \h d\g(s),
%\end{equation}
%where $\g \subset \mathscr{R}_f$ is an integration path from $q_0$ to $q$ such that the integral is convergent.  Notice that, though the domain of $\hat{f}$ is on the Riemann surface $\mathscr{R}_f$, the result of the integral,  $t-t_0 \in \complexs$. 
%We consider  $q_0, q \in\complexs$ and the choice of path $\g$ will specify the Riemann sheet the initial and final points of the path belong to. 
%%We postpone an accurate definition of the integration paths until Section~\ref{section:complexpaths}. 
%Singularities $t^* \in \complexs$ of $q(t)$ with initial condition $q(0)=a_+$ satisfy
%\[
% t^* = \int_{a_+}^{q^*} \hat{f}(s) \h  d\g(s), 
%\]
%for some $q^*\in \complexs$. Moreover, $\lim_{t \to t^*} q(t) = q^*$.
%%for $q^* \in \complexs$. Notice, that we do not consider $q^*$ in the Riemmann surface $\mathscr{R}_f$  that the choice of path $\g$ will specify the Riemann sheet $q^*$ belongs to.  
%To find the possible values of $q^*$, we define function
%\[
% G(q):= \int_{a_+}^{q} \hat{f}(s) \h d\g(s).
%\]
%Then, $q(t)= G^{-1}(t)$ for $t \in D \subset \complexs$, an unknown domain. Note that is not a ``correct'' inverse, as the solution depends on the integration paths as well, and $G$ may be multi-valued. However, this points out that the singularities $t=t^*$ of $q(t)$ arise on the points $q=q^*$ where is not possible to apply the inverse function theorem on function $G(q)$. There are three possibilities:
%\begin{enumerate}
% \item $|q^*| \to + \infty$.
% \item $G(q)$ not $\CC^1$ on a neighbourhood of $q^*$.
% \item $G'(q^*)= 0$.
%\end{enumerate}
\begin{proof}
To prove this result first we need to analyze all the possible values of $q^*$ that may lead to singularities, (see~\eqref{eq:candidatesSingularities}).
%
We will use the expressions of $t$ and $t^*$ given in~\eqref{eq:lemmaIntegralEquationGeneral} and~\eqref{eq:lemmaIntegralEquationSingularities}, respectively.

\begin{enumerate}
%	
\item If $|q^*| \to  \infty$, we have
\[
t - t^* = \int^{q(t)}_{\infty} \hat{f} \h d\g.
\]
Then, since
\[
\fh(q) = \frac{1}{\sqrt{3} q^2} + \OO\paren{\frac{1}{q^3}}, \qquad \text{ for }\quad |q|\gg 1,
\]
we obtain
\[
t-t^* = -\frac{1}{\sqrt{3}q} + \OO\paren{\frac{1}{q^2}},
\]
which implies~\eqref{eq:singularitatExpressioInfinit}.
%\begin{equation*}%\label{proof:classificationInfty}
%  q(t) = \pm\frac{1}{\sqrt{3}(t-t^*)}\left( 1 + \OO(t-t^*)^{\beta} \right), \h
%  \text{ for } 0<\vabs{t-t^*} \ll 1.
%\end{equation*}
%
\item If $q^*=a_+$, we have that 
\begin{equation*}\label{proof:integralames}
t - t^* = \int^{q}_{a_+} \fh d\g.
\end{equation*}
The function $\fh$ can be written as 
\[
\hat{f}(q)= \frac{h_{a_+}(q)}{\sqrt{q-a_+}},
\]
%
for some function $h_{a_+}$ which is analytic and non-zero in a neighborhood of $a_+$. Then,  $h_{a_+}$ can be written as 
$h_{a_+}(q) = \sum_{k=0}^{\infty} c_k (q-a_+)^k$, with $c_0 \neq 0$
%
and,  for 
$0< \vabs{q-a_+} \ll 1$, we obtain from \eqref{proof:integralames}
\[
t-t^*=\sqrt{q-a_+} \sum_{k=0}^{\infty} \frac{c_k}{k+\frac{1}{2}} (q-a_+)^k,
\]
which implies $(t-t^*)^2=g_{a_+}(q)$ with 
\[
g_{a_+}(q)=(q-a_+)\left( \sum_{k=0}^{\infty} \frac{c_k}{k+\frac{1}{2}} (q-a_+)^{k} \right)^2.
\]
%
The function $g_{a_+}(q)$ is analytic on a neighborhood of $a_+$ and satisfies $g_{a_+}(a_+)=0$, $g'_{a_+}(a_+)=4 c_0^2 \neq 0$. 
%
Thus, applying the Inverse Function Theorem, 
\begin{equation}\label{proof:qexpressionZeroes}
q(t)=g_{a_+}^{-1}\left((t-t^*)^{2}\right),\qquad \text{for}\quad 0<\vabs{t-t^*}\ll 1.
\end{equation}
Therefore, $q(t)$ is analytic for $\vabs{t-t^*}\ll 1$.
%
%Therefore, taking $q^*=a_+$ does not produce any singularities. 
%
One can analogously prove that the same happens at $q^*=a_-$ and $q^*=-1$. 

\item The value $q^*=1$ corresponds to the saddle point $(\la,\La)=(0,0)$ of $H_{\pend}$ (see~\eqref{def:HpendHosc}). Indeed, 
\begin{equation}\label{proof:classificationSaddle}
 \int^{q}_{1} \fh d\g\quad \text{is divergent.}
\end{equation}
This implies that $q(t)\neq 1$ for any complex $t$.
% 
% %
% Therefore, 
% \begin{equation}\label{proof:classificationSaddle}
%  \lim_{t \to \pm \infty} q(t) = 1, 
%  \qquad \text{for } t \in \reals,
% \end{equation}
%for $t \in \reals$ and $q(t)$ can be expressed as
%\[
% q(t) \sim \OO(e^{\pm \vap t}) , \h \text{ as } |t| \to +\infty,
%\]
%for $\vap= \sqrt{\frac{21}{8}}$. 
% and the analytic extension to the complex plane of $q(t)$ does not have a singularity when $q(t)=q^*=1$. 

%We have that $G'(q) = \hat{f}(q)$. Then, $G'(q^*)= 0$ only for $q^*=0$.
%For the third case, we have that
%\[
% G'(q) = f(q) = \frac{1}{q-1}\sqrt\frac{q}{3(q+1)(q-a_-)(q-a_+)} = 0 \iff q=0.
%\]
%Thus, we consider the case $q^*=0$. 
\item If $q^*=0$, 
\begin{equation*}%\label{proof:integralZero}
t - t^* = \int^{q}_{0} \fh \h d\g.
\end{equation*}
We can introduce $h_0(q)= \frac{1}{\sqrt{q}} \fh(q)$ which is analytic and of the form $h_0(q)=\sum_{k=0}^{\infty}c_k q^k$ with $c_0 \neq 0$. 
%
Then, for $0<\vabs{q} \ll 1$, 
we obtain
% \[
% t - t^* = q^{\frac{3}{2}} \sum_{k=0}^{\infty} \frac{c_k}{k+\frac{3}{2}} q^k.
% \]
% Introducing
\begin{equation*}
%\label{proog:functiongZero}
(t-t^*)^{\frac{2}{3}} =g_0(q) = q \left(\sum_{k=0}^{\infty} \frac{c_k}{k+\frac{3}{2}} q^k \right)^{\frac{2}{3}}
= q \paren{\frac{2 c_0}{3} + \OO(q) }^{\frac{2}{3}},
\end{equation*}
% we have that $(t-t^*)^{\frac{2}{3}} = g_0(q)$,
%
where $g_0(q)$ is analytic in a neighborhood of $q=0$ and satisfies $g_0(0)=0$, $g'_0(0) = \paren{\frac{2}{3} c_0}^{\frac{2}{3}} \neq 0$.
%
Thus, applying the Inverse Function Theorem, 
\begin{equation}
\label{proof:seriesqEnZero}
q(t) = g_0^{-1}\paren{(t-t^*)^{\frac{2}{3}}}
= \sum_{k=1}^{\infty} C_k (t-t^*)^{\frac{2k}{3}},\quad \text{for } 0<|t-t^*|<\ll 1,
\end{equation}
for some $C_k \in \complexs$ and choosing  the Riemann sheet $\arg \paren{t-t^*} \in \paren{-\frac{3\pi}{2},\frac{\pi}{2}}$ for $\Im t^*>0$
%
and  $\arg \paren{t-t^*} \in \paren{-\frac{\pi}{2},\frac{3\pi}{2}}$
for $\Im t^*<0$.
%
%Then, taking into account that $\lim_{t \to t^*} q(t) = 0$, we have that
%\[
%q(t) = \sum_{k=1}^{\infty} C_k (t-t^*)^{\frac{2k}{3}}, \h \text{ for } 0<\vabs{t-t^*}\ll 1,
%\]
%for some $C_k \in \complexs$. 
Replacing~\eqref{proof:seriesqEnZero} in equation~\eqref{eq:odeSeparatrixQ} we obtain
$
C_1 = -\frac{3\al}{2},
$
where $\al \in \complexs$ satisfies $\al^3=\frac{1}{2}$, which implies~\eqref{eq:singularitatExpressio}.
\end{enumerate}
\end{proof}

%Applying integration by parts and the triangle inequalities, we obtain
%\[
%% C_1 |q|^{3/2} \leq |t-t^*| \leq C_2 |q|^{3/2} \implies 
%(t-t^*) \sim \OO \left( q^{3/2} \right),
% \text{ as } |q| \to 0.
%\]
%Then, for some $C \in \complexs$ and $\beta>0$ the inverse satisfies
%\[
% q(t) \sim \OO \left( (t-t^*)^{2/3} \right), \h \text{ as } |t - t^*| \to 0.
% \] 
%From this computations it can be inferred that in the case $q^*=0$, if there exist singularities for $q(t)$, are only singularities for $\qd(t)$. Specifically, nearby $t^*$, $q(t)$ will behave as a zero of order $\frac{2}{3}$, and $\qd(t)$ as a branching point of order $\frac{1}{3}$. 
%Hence, there exists $\nu>0$ such that for $t\in \complexs$ where $|t-t^*|<\nu$, $q(t)$ can be expressed as 
%\[
%  q(t) = C(t-t^*)^{2/3}\left( 1 + \OO(t-t^*)^{\beta} \right),
%\]
%with $\beta>0$ and $C \in \complexs$ constant. Then, replacing this expression on equation~\eqref{eq:odeSeparatrixQpolynomial} nearby the singularity we obtain
%\begin{align*}
%  &\frac{4}{9} \frac{C^2 }{(t-t^*)^{\frac{2}{3}}} \left( 1 + \OO(t-t^*)^{\beta} \right) = \\
%  &=\frac{3}{4} \left( 4 C^4 (t-t^*)^{\frac{8}{3}} 
%  - 9 C^2 (t-t^*)^{\frac{4}{3}} 
%  + C (t-t^*)^{\frac{2}{3}} 
%  + 5 - \frac{1}{C (t-t^*)^{\frac{2}{3}}} + \OO(t-t^*)^{\beta} \right).
%\end{align*}
%Now, we can proceed by computing constant $C \in \complexs$: equating orders on the previous equation,
%\[
%\frac{4}{9} C^2 = -\frac{3}{4 C} \implies C^3 = - \frac{27}{16} \implies C = -\frac{3\al}{2},
%\]
%where $\al \in \complexs$ such that $\al^3=1/2$.


%\begin{remark}
%When performing the analytical continuation to the complex of $q(t)$, it is important to chose an initial condition on the original real-valued separatrix of the problem, which are
% \[ q(t)  \in [a_+,1) \text{ for } t \in \reals,\]
%as seen on Lemma~\ref{lemma:separatrixChangeCoordinates}. This is because there can exist multiple analytical continuations, and we are interested in the one, that for $t\in \reals$, $q(t)$ correspond with our original separatrix. Choosing a different initial condition could not guarantee this attribute.
%\end{remark}

% \begin{remark}
% It is worth noticing that for each $q^*$ could exist more than one (or none) singularity $t^*$, depending on the path $\g$ chosen on~\eqref{eq:integralPolesSection}. 
% \end{remark}



==> Article Inner/proofA-ComplexPathsCrossingR.tex <==
\subsubsection{Paths first crossing the real axis at \texorpdfstring{$\reals \setminus [0,1]$}{outside [0,1]}}
\label{subsubsection:pathsB}

In this section, we continue the proof of Proposition~\ref{proposition:camins} by checking that
the singularities generated by paths B.1 to B.4 (see the list in Section~\ref{subsection:computationSingularities}) are not visible.

First, we introduce some concepts. Let us consider a path $\g \in \PP_{0}\cup \PP_{\infty}$. 
%
We define the \emph{parameter of the first crossing} of the real line as
\[
 s_1(\g)= \inf \{s \in(s_{\ini},s_{\fin}) \st \Im \proj \g(s)=0 \},
\]
the \emph{location of the first crossing} as
\[
q_1(\g)= \proj \g(s_1(\g)) \in \reals \setminus \{ a_-, -1, 0, a_+, 1\},
\]
%Therefore, paths $\g$ can be classified depending on the region of the first crossing $q_1(\g)$.
%
the \emph{piece of the path} before the first crossing of the real line as
\[
\g_1(\g) = \claus{\g(s) \st s \in (s_{\ini},s_1(\g))},
\]
and the \emph{time of the first crossing} as
\begin{equation*}
%\label{def:t1FirstCrossing}
t_1(\g) = \int_{\g_1(\g)} \fh(q) dq.
\end{equation*}
In the following lemmas, we focus on the paths that stay in $\complexs^+$ until the first crossing of the real line, that is $\proj \g_1(\g) \subset \complexs^+$
%
(see~\eqref{eq:reflection} for the conjugate paths, i.e.  $\proj \g_1(\g) \subset \complexs^-$). 
%
%Notice that, if $t^*(\g)$ is not visible, neither is $\conj{t^*(\g)}$.
%
%
\begin{remark}\label{remark:pathsCrossingReals}
	To prove that a singularity $t^*(\g)$ is not visible (see Definition~\ref{definition:visibleSingularity}) it is sufficient to check that $\vabs{\Im t_1(\g)} \geq A$.
	%
%	We use this fact extensively in the proofs of the following lemmas.
\end{remark}

\begin{lemma} \label{lemma:caminsPol}
The singularities $t^*(\g)$ given by paths $\g \in \PP_{0} \cup \PP_{\infty}$ such that 
$q_1(\g) \in (1,+\infty)$ are not visible.
\end{lemma}

\begin{proof}
%Let us fix $q_1 \in (1,+\infty)$ and 
Consider a path $\g \in \PP_{0} \cup 
\PP_{\infty}$ with $q_1=q_1(\g) \in (1,+\infty)$ and $\proj \g_1(\g)\subset \complexs^+$. 
%
%We impose that $\g_1(\g) \subset \complexs^+$ since, by Lemma~\ref{lemma:reflection}, we obtain analogous results for the negative complex plane.
%
% We compute $t_1(\g)$ (see~\eqref{def:t1FirstCrossing}).
%
%Then, we define the auxiliary path
%\[
%\wt{\g}:= \{ \g(\tau) \st  \tau \in (\tau_0,\tau_1(\g))\}.
%\]
%Then
%\begin{equation}\label{proof:equivalentIntegrals1}
%t_1(\g)=\int_{\wt{\g}} \fh.
%\end{equation}
%Notice that path $\g_1(\g)$ does not cross $\reals$, and stays on the first Riemann sheet. 
%
Integrating the function $\fh$ along the path $\g_1(\g)$ is equivalent to integrate $\fh$ along the path
 $ {\eta}={\eta}^{1} \vee {\eta}^{2} \vee \eta^{3}$ where
\begin{equation}\label{proof:pathEtaPol}
\begin{cases}
 {\eta}^{1}(q) = (q,0) & \text{ with } q \in (a_+,1-\e], \\
\proj{\eta}^{2}(\phi) = 1 + \e e^{i\phi} & \text{ with } \phi \in [\pi,0], \\
\proj{\eta}^{3}(q) = q  & \text{ with } q \in [1+\e,q_1),
\end{cases}
\end{equation}
for  $\e>0$ small enough,
%
(see Figure~\ref{fig:caminsVoltesPol}).
%
\begin{figure}[b]
\centering
\begin{overpic}[scale=0.8]{caminsVoltesPol.png}
	\put(8,14){{\color{red} $0$ }}
	\put(51,14){{\color{blue} $1$ }}	
	\put(18,14.5){{\color{red} $a_+$ }}
	\put(77,22){{\color{myPurple} $q_1(\g)$ }}
	\put(24,31){{\color{myGreen} $\proj \g$ }}
	\put(40,22){{\color{myBlue} $\proj \eta$ }}
	\put(101,18){$\Re q$}
	\put(7,44.5){$\Im q$}
\end{overpic}
	\caption{Example of a path $\g \in \HH_{q,\infty}$  such that ${q_1(\g) \in (1,+\infty)}$
	and $\proj \g_1(\g)\subset \complexs^+$. 
	The path $\eta$ has been defined in~\eqref{proof:pathEtaPol}.}
	\label{fig:caminsVoltesPol}
\end{figure}
%
Then,
\[
t_1(\g) = \int_{\eta} \fh(q) dq 
= \sum_{j=1}^3 \int_{\eta^j} \fh(q) dq,
\]
%
and the integrals on ${\eta}^{1}$ and ${\eta}^{3}$ take real values since $\fh(q)\in \reals$ when $\proj(q) \in (a_+,1)\cup(1,+\infty) \subset \reals$. Analogously to the proof of Lemma~\ref{lemma:caminsInfinitSimple}, we have that
\[
|\Im t_1 (\g)| = \left|\Im \int_{{\eta}^{2}} \fh(q) dq \right|=
 \pi \left|\Res\paren{\fh,(1,0)}\right| =
 \pi \sqrt{\frac{2}{21}} > A.
\]
Therefore, $t^*(\g)$ is not visible (see Remark~\ref{remark:pathsCrossingReals}).
% since
% \[
% |\Im t_1 (\g)| = 
% \vabs{ \Im {\int_{\eta^2} \fh(q) dq}} =
%  \pi \sqrt{\frac{2}{21}} > A.
% \]
\end{proof}

\begin{lemma} \label{lemma:caminsNegatius2}
The singularities $t^*(\g)$ given by paths $\g \in \PP_{0} \cup \PP_{\infty}$ such that 
$q_1(\g) \in (-\infty,a_-)$ are not visible.
\end{lemma}

\begin{proof}
Consider a path $\g \in \PP_{0} \cup \PP_{\infty}$ with $q_1=q_1(\g) \in (-\infty,a_-)$ and $\proj \g_1(\g) \subset \complexs^+$. 
%
% We compute $t_1(\g)$ (see~\eqref{def:t1FirstCrossing}).
%
To compute $t_1(\g)$ we introduce the auxiliary path
$
{\eta}_{\infty} = \g_1(\g) \vee \wt{\eta} 
$,
where
\begin{equation}\label{proof:pathEtaWT}
\proj \wt{\eta}(q)=q \qquad
\text{with }
q \in [q_1, -\infty),
\end{equation}
(see Figure~\ref{fig:caminsNegatius2}).
\begin{figure}
\centering
\begin{overpic}[scale=0.8]{caminsNegatius2.png}
	\put(71,12){{\color{red} $0$ }}	
	\put(76.5,12){{\color{red} $a_+$ }}
	\put(35,12){{\color{red} $-1$ }}
	\put(28,12){{\color{red} $a_-$ }}
	\put(89,15){$\Re q$}
	\put(66,37){$\Im q$}
	\put(41,29){{\color{myGreen} $\proj \g$ }}
	\put(16.5,12){{\color{myPurple} $q_1(\g)$ }}
	\put(16,19){{\color{myBlue} $\proj \wt{\eta}$ }}
\end{overpic}
\caption{Example of a path $\g \in \PP_{0}$  	
	such that ${q_1(\g) \in (-\infty,a_-)}$ 
	and $\proj \g_1(\g)\subset \complexs^+$. 
	The path $\wt{\eta}$ has been defined in~\eqref{proof:pathEtaWT}.}
\label{fig:caminsNegatius2}
\end{figure}
Then, taking into account that $\fh|_{\wt{\eta}} \subset \reals$,
% Now, we consider the path  $\g^*$ as defined on~\eqref{proof:pathgamma2}. By Cauchy's Integral Theorem and Lemma~\ref{lemma:caminsInfinitSimple}, we have
\begin{equation*}
\vabs{\Im  t_1(\g)}=\left|
\Im \int_{\eta_{\infty}} \fh(q) dq \right|= 
\left|\Im \int_{\g_*} \fh(q) dq \right|=
 \pi \sqrt{\frac{2}{21}}>A,
\end{equation*}
where   $\g^*$ is the path  defined in~\eqref{proof:pathgamma2}.
%path $\eta_{\infty}$ ${\g}_{\infty} \in \HH_{q,\infty}$ and 
%${\g}_{\infty} \subset \complexs^+$. Then, by Lemma~\ref{lemma:caminsInfinitSimple}, we have that
%\[
%\Im \paren{\int_{{\g}_{\infty}} \fh(q) dq} = 
%\Im \paren{ t^*({\g}_{\infty}) } = -\pi \sqrt{\frac{2}{21}},
%\]
%Function $f(q)$ is holomorphic for $q \in \complexs^+$ considered on the same Riemann sheet as path $\wt{\g}_{\infty}$. Furthermore, it decays with a rate of $1/q^2$ as $|q| \to \infty$. Then, by Cauchy integral's theorem,  we have that path $\wt{\g}_{\infty}$  gives the same result for integral~\eqref{eq:integralEquationPole} as path $\g_1$ defined on the proof Lemma~\ref{lemma:caminsInfinitSimple}.
% This implies that
% \begin{align*}
% \vabs{\Im  t_1(\g)} 
%
%= \vabs{\Im  \int_{\eta} \fh(q) dq } 
%
% =\vabs{\Im  \int_{{\eta}_{\infty}}\fh(q) dq } 
% > A,
% \end{align*}
Therefore $t^*(\g)$ is not visible.
\end{proof}

\begin{lemma} \label{lemma:caminsNegatius1}
The singularities $t^*(\g)$ given by paths $\g \in \PP_{0} \cup \PP_{\infty}$ such that 
$q_1(\g) \in (-1,0)$ are not visible.
\end{lemma}

\begin{proof}
Let $\g \in \PP_{0} \cup \PP_{\infty}$ be a path such that $q_1 = q_1(\g) \in (-1,0)$ and $\proj \g_1(\g) \subset \complexs^+$.
%
% We compute $t_1(\g)$ (see~\eqref{def:t1FirstCrossing}).
%
Integrating the function $\fh$ along the path $\g_1(\g)$ is equivalent to integrating  $\fh$ along
% \begin{equation}\label{proof:pathEtaNegatius1}
${\eta}={\eta}^1 \vee {\eta}^2 \vee \eta^3
\vee \eta^4 \vee \eta^5$
% \end{equation}
where
\begin{equation}\label{proof:pathEtaNegatius1}
\begin{cases}
\eta^1(q) = (q,0) & 
\text{ with } q \in (a_+,a_+ + \e], \\
%
\proj \eta^2(\phi) = a_+ + \e e^{i\phi} & 
\text{ with } \phi \in [0,\pi], \\	
%	
\proj \eta^3(q) = q & 
\text{ with } q \in [a_+-\e,\e], \\
%
\proj \eta^4(\phi) = \e e^{i\phi} & 
\text{ with } \phi\in [0,\pi], \\
%
\proj \eta^5(q) = q & \text{ with } q \in [-\e,q_1), 
\end{cases}
\end{equation}
for $\e>0$ small enough,
%
(see Figure~\ref{fig:caminsNegatius1}).
%
\begin{figure}
\centering
\begin{overpic}[scale=0.8]{caminsNegatius1.png}
	\put(53,9.5){{\color{red} $0$ }}	
	\put(61,9.5){{\color{red} $a_+$ }}
	\put(29,9.5){{\color{red} $-1$ }}
	\put(22,9.5){{\color{red} $a_-$ }}
	\put(75,12){$\Re q$}
	\put(52,30){$\Im q$}
	\put(48,23.5){{\color{myGreen} $\proj \g$ }}
	\put(45,15){{\color{myBlue} $\proj \eta$ }}
	\put(37,9.5){{\color{myPurple} $q_1(\g)$ }}
\end{overpic}
\caption{Example of a path $\g \in 	\PP_{\infty}$  such that ${q_1(\g) \in (-1,0)}$ and $\proj \g_1(\g)\subset \complexs^+$. 
The path $\eta$ has been defined in~\eqref{proof:pathEtaNegatius1}.}
\label{fig:caminsNegatius1}
\end{figure}
%
% \[
% t_1(\g) = \int_{\eta} \fh(q) dq
% = \sum_{j=1}^5 \int_{\eta^j} \fh(q) dq.
% \]
% %
Using that $\int_{\eta^j} \fh(q) dq = \OO(\sqrt{\e})$ for $j=1,2,4$, that  $\fh|_{\eta^5} \subset \reals$, and~\eqref{proof:singularityt1mes}, one has that  $t^*(\g)$ is not visible since
\[
\vabs{\Im t_1(\g)}= 
\lim_{\e \to 0} 
\vabs{\int_{{\eta^3}} \fh(q) dq} = A.
\]
\end{proof}

\begin{lemma} \label{lemma:caminsBranca2}
The singularities $t^*(\g)$ given by paths $\g \in \PP_{0} \cup \PP_{\infty}$ such that 
$q_1(\g) \in (a_-,-1)$ are not visible.
\end{lemma}
\begin{proof}
Take a path $\g \in \PP_{0} \cup \PP_{\infty}$ with $q_1=q_1(\g)\in (a_-,-1)$ and $\proj \g_1(\g) \subset \complexs^+$.	
%
The integral of  the function $\fh$ along the path $\g_1(\g)$ coincides with the integral along the path
\begin{equation}\label{proof:pathEtaBranca2}
\eta = \bigvee_{j=1}^7 \eta^j,
\end{equation}
where the paths $\eta^j$, $j=1,2,3,4$, are defined in~\eqref{proof:pathEtaNegatius1} and
\[
\begin{cases}
\proj \eta^5(q) = q & 
\text{ with } q \in [-\e,-1+\e], \\
%
\proj \eta^6(\phi) = -1 + \e e^{i\phi} & 
\text{ with } \phi \in [0,\pi], \\
%
\proj \eta^7(q) = q & 
\text{ with } q \in [-1-\e,q_1), \\
\end{cases}
\]
for small enough $\e>0$,
%
(see Figure~\ref{fig:caminsBranca2}).
%
\begin{figure}
	\centering
	\begin{overpic}[scale=0.8]{caminsBranca2.png}
		\put(64,12){{\color{red} $0$ }}	
		\put(71,12){{\color{red} $a_+$ }}
		\put(30,12){{\color{red} $-1$ }}
		\put(20,12){{\color{red} $a_-$ }}
		\put(83,15){$\Re q$}
		\put(60,37){$\Im q$}
		\put(45,32){{\color{myGreen} $\proj \g$ }}
		\put(50,19){{\color{myBlue} $\proj \eta$ }}
		\put(18,19){{\color{myPurple} $q_1(\g)$ }}
	\end{overpic}
	\caption{Example of a path $\g \in 	\PP_{\infty}$  such that ${q_1(\g) \in (a_-,-1)}$ and $\proj \g_1(\g)\subset \complexs^+$. 
	Path $\eta$ as defined in~\eqref{proof:pathEtaBranca2}.}
	\label{fig:caminsBranca2}
\end{figure}
%
Then, proceeding analogously to the proof of Lemma \ref{lemma:caminsNegatius1},
\begin{equation}\label{def:eta5to7}
\Im t_1(\g) = \lim_{\e\to 0 }\Im \int_{\eta} \fh(q) dq
= -A+\sum_{j=5}^7\lim_{\e\to 0 } \Im  \int_{\eta^j} \fh(q) dq.
\end{equation}
% 
Since $\fh|_{\eta^5} \subset \reals$ and $\int_{\eta^6} \fh(q) dq = \OO(\sqrt{\e})$,
%
%Moreover, by~\eqref{proof:singularityt1mes}, we have that
%\[
%\lim_{\e \to 0} \int_{{\eta}^3} \fh(q) dq = 
%t^*_{1,+} = - iA.
%\]
it only remains to compute the integral on $\eta^7$.
%
Following the natural arguments of the path $\eta$, we obtain
\[
\begin{array}{llll}
\arg(\eta^7) = \pi, & 
\arg(\eta^7-a_+) = \pi, &
\arg(\eta^7+1) = \pi, & 
\arg(\eta^7-a_-) = 0
\end{array} 
\]
%
and, as a consequence,
\begin{align*}
\lim_{\e \to 0} \int_{\eta^7} \fh(q) dq 
&= \int_{-1}^{q_1}  \frac{1}{q-1}\sqrt{\frac{|q|e^{i \pi}}{3|q+1|e^{i \pi}|q-a_+| e^{i\pi}(q-a_-)}} dq 
=- i B(q_1),
\end{align*}
where  $B(q_1)$ a real-valued, positive and strictly decreasing  function for $q_1 \in (a_-,-1)$.
% Notice that, in addition, $B(q_1)$ is for $q_1 \in (a_-,-1)$. 
%
Then, $t^*(\g)$ is not visible since,  by \eqref{def:eta5to7},
% \begin{align*}
$\vabs{\Im t_1(\g)} = 
%
% \lim_{\e \to 0}
% \vabs{\int_{{\eta^3}} \fh(q) dq  
% + \int_{{\eta^7}} \fh(q) dq} =
A + B(q_1)> A$.
%
% \end{align*}
% As a consequence, $t^*(\g)$ is not visible.
\end{proof}



==> Article Inner/proofA-ComplexPathsNotCrossingR.tex <==
\subsubsection{Paths not crossing the real axis}
In this section, we check the singularities resulting from the paths A.1 and A.2. 
% (on the list in Section~\ref{subsection:computationSingularities}).


\begin{lemma} \label{lemma:caminsZeroSimple}
There exist only two singularities, $t^*_{1,\pm}$, given by the paths $\g \in \PP_{0}$ not crossing the real axis. These singularities are  visible and
\[
 t^*_{1,\pm} = \mp iA,
\]
with $A$  defined in~\eqref{def:integralA} and satisfying $A \in  \left[\frac{3}{50}, \frac{3}{10}\right]$.
%as
%\begin{equation}\label{def:integralALemma}
%A= \int_0^{a_+} \frac{1}{1-x}\sqrt\frac{x}{3(x+1)(a_+-x)(x-a_-)}  dx
%\in \left[\frac{3}{50}, \frac{3}{10}\right].
%%\text{ with } a_{\pm}=-\frac{1}{2}\pm\frac{\sqrt{2}}{2}.
%\end{equation}
%Moreover, there are visible singularities.
%exist a path $\g_2 \in  \HH_{q,0}$ such that $T[\g_2] \in \HH_{t}$.
%As well, there exist a specific integration path ${\g_{2,\pm} \in \HH_{q,0}}$ such that $T[\g_{2,\pm}] \in \HH_t$  is a visible path.
\end{lemma}

\begin{proof}
Let us consider paths $\g \in \mathcal{P}_0$ such that $\proj \g \subset \complexs^+ = \claus{\Im z>0}$. 
%
Notice that, since $\g$ does not cross the real axis, it does not encircle any singularity of $\fh$ and, by Cauchy's Integral Theorem, all the paths considered generate the same singularity $t_{1,+}^*$. 
%
The singularity $t^*_{1,-}$ is given by the conjugated paths (see~\eqref{eq:reflection}).
%

Let us consider the path $\g_*=\g_{*}^1 \vee \g_{*}^2 \vee \g_{*}^3$ with
\begin{equation}\label{proof:pathgamma1}
\begin{cases}
\g_{*}^1(q) = (q,0) & \text{ with } q \in (a_+,a_+ + \e], \\
%
\proj \g_{*}^2(\phi) = a_+ + \e e^{i\phi} & \text{ with } \phi \in [0,\pi], \\
%
\proj \g_{*}^3(q) = q  & \text{ with } q \in [a_+ -\e,0), \\
\end{cases}
\end{equation}
for $\e>0$ small enough,
%
(see Figure~\ref{fig:caminsZeroSimpleSuperior}).
%
\begin{figure}
	\centering
	\begin{overpic}[scale=0.8]{caminsZeroSimpleSuperior.png}
		\put(48,9.5){{\color{red} $0$ }}	
		\put(56,9.5){{\color{red} $a_+$ }}
		\put(75,9.5){{\color{blue} $1$ }}
		\put(25,9.5){{\color{red} $-1$ }}
		\put(17,9.5){{\color{red} $a_-$ }}
		\put(93,12){$\Re q$}
		\put(47,30){$\Im q$}
		\put(39,26){{\color{myGreen} $\proj \g$ }}	
		\put(52,16){{\color{myBlue} $\proj \g_*$ }}
	\end{overpic}
	\caption{Example of a path $\g \in \PP_{0}$ such that $\proj \g \subset \complexs^+$. Path $\g_*$ as defined in~\eqref{proof:pathgamma1}.}
	\label{fig:caminsZeroSimpleSuperior}
\end{figure}
%
%Integrating $\fh$ along path $\g$ is equivalent to integrating along $\g_*$.
%
Then, the resulting singularity is
\[
t^*_{1,+} 
= t^*(\g_*) 
= \int_{\g_*} \fh(q) dq
= \sum_{j=1}^3 \int_{\g_{*}^j} \fh(q) dq.
\]
%for all values of $\e>0$. 
%
%We perform an analysis of the arguments of $\g_{*}$ with respect the remaining three branching points.
%We have that
%
Since $\int_{\g_*^j} \fh(q) dq = \OO(\sqrt{\e})$ for $j=1,2$,  taking the limit $\e \to 0$, we have
\[
t_{1,+}^* = \lim_{\e \to 0} \int_{\g_*^3} \fh(q) dq.
\]
%Since $\g_*\in \mathcal{P}_0$, the initial point of the path is $(a_+,0)$.
Then, by following the natural arguments of the path $\g_*$, we obtain
\[
\begin{array}{llll}
\arg(\g_{*}^3) = 0, & 
\arg(\g_{*}^3-a_+) = \pi, &
\arg(\g_{*}^3+1) = 0, & 
\arg(\g_{*}^3-a_-) = 0,
\end{array} 
 \]
and, as  a consequence, by the definition of $A$ in~\eqref{def:integralA}, we have
\begin{equation}\label{proof:singularityt1mes}
 t^*_{1,+}  = 
  \lim_{\e \to 0} \int_{\g_*^3} \fh(q) dq =
 \int_{a_+}^0 \frac{1}{x-1}\sqrt\frac{x}{3(x+1) \vabs{x-a_+} e^{i\pi}(x-a_-)} dq  = -iA.
\end{equation}
%where $A$ is the real-valued integral defined on~\eqref{def:integralALemma}. 
%
Moreover,
\begin{align*}
	A \leq & \frac{\sqrt{a_+}}{(1-a_+)\sqrt{3\vabs{a_-}}} 
	\int_0^{a_+} \frac{dx}{\sqrt{a_+-x}}
	%
	= \frac{4\sqrt{3}}{3}\frac{a_+^{3/2}}{1-a_+}
	%
	\leq \frac{3}{10}, \\
	%
	A \geq & \frac{1}{\sqrt{3a_+(a_+ + 1)(a_+ -a_-)}}
	\int_0^{a_+} \sqrt{x} \, dx 
	%
	= \frac{2 \sqrt[4]{74}}{9} {a_+^{3/2}}
	% 
	\geq \frac{3}{50}.
\end{align*}
%
Now, it just remains to see that $t_{1,+}^*$ is visible, namely, we check that $T[\g_*] \subset \Pi_A$. 
%That is, we need to see that $\vabs{\Im T[\g^2_{*}](\tau)} < A$ for $\tau \in (0,a_+)$. 
Indeed, for $s \in (0,a_+]$, we have that
\[
\vabs{\Im T[\g_*](s)} =  
\int_{s}^{a_+} \frac{1}{1-x}\sqrt\frac{x}{3(x+1)(a_+-x)(x-a_-)} dx
< A.
\]
\end{proof}

% As before, applying this theorem is not entirely correct, as paths $\g$ begin at  singularity $q=a_+$. However, as it was seen in Remark~\ref{remark:initialConditionConvergent}, the choice of initial condition does not affect the convergence of the integral.
% \[
%   \g_{2}:=\g_{2,a} \cup \g_{2,b} \cup \g_{2,c},
% \]
%where
%\[
%\begin{cases}
% \g_{2,a}(x) = a_+ + iy & \text{ with } y \in (0,\de], \\
% \g_{2,b}(x) = x + i\de & \text{ with } x \in [a_+,0], \\
% \g_{2,c}(x) = iy & \text{ with } y \in [\de,0),
%\end{cases}
%\]
%for $\de>0$ small enough. %This path is a representation of a path in $\HH_{q,\infty}$.
%It is worth noticing that $\g_2 \notin \HH_{q,0}$, because its domain is not $(0,1)$. However, because $\g_2$ is homotopic to the paths $\g \in \HH_{q,0}$ defined in the statement, it can be used to perform the necessary computations. As well, if necessary, it could be easily adapted to have the appropriate domain. \\
%For every $\de>0$,  integrating on paths $\g_2$ give the same result. Hence, we chose $\de \to 0$ to perform the computations. 
 %\[
% t^*_{2,+}:=t^*(\g) = \int_{\g_2} f = \lim_{\de \to 0} \int_{\g_2} f.
%\]
%In this case, the integrals of both $\g_{2,a}$ and $\g_{2,c}$ tend to $0$. So, the only path contributing towards the integral is $\g_{2,b}$,
%\begin{align*}
% t^*_{2,+} 
% %&=\lim_{\de \to 0} \int_{\g_{2,b}} f  = 
% %\lim_{\de \to 0} \int_{\g_{2,b}} \frac{1}{q-1}\sqrt\frac{q}{3(q+1)(q-a_-)(q-a_+)} dq  \\
% & =  \lim_{\de \to 0}  \int_{a_+}^0 \frac{1}{x-1+i\de}\sqrt\frac{x+i\de}{3(x+1+i\de)(x-a_-+i\de)(x-a_++i\de)} dx.
%\end{align*}
% in the square root of $f$ for path $\g_{2,b}$. Taking into account that $\g_2$ stays above the logarithm branch $B_1=(0,a_+)$ and that the arguments are in $(-\pi,\pi)$. Then, for $\de \to 0$,
%\[ \begin{array}{ll}
%q=x+i\de  & \arg{q} \to 0 \\
%q-a_+ = (x-a_+)+i\de \text{ \hspace{5mm} }& \arg{q-a_+} \to \pi \\
%q-a_- = (x-a_-)+i\de & \arg{q-a_-} \to 0 \\
%q+1 = (x+1)+i\de  & \arg{q+1} \to 0 \\
%\end{array} \]
%where $x \in [0,a_+]$. 
%On the conjugated path $\ol{\g_2} \subset \complexs^-$ all the arguments will be the same except for $\arg(q-a_+) \to -\pi$. In both cases $q-a_+$ tends to the negative real line, but for paths in $\complexs^+$ it does so above the logarithm branch $B_1$ and for paths in $\complexs^-$  below the logarithm branch. 
%Then
%\begin{align*}
% t^*_{2,+} 
% &= \int_{a_+}^0 \frac{1}{x-1}\sqrt\frac{|x|}{3|x+1||x-a_-||x-a_+| e^{i\pi}} dx 
% %&= e^{-i\pi/2}\int_{a_+}^0 \frac{1}{x-1}\sqrt\frac{x}{3(x+1)(x-a_-)(a_+-x)}  dx  \\
%  %&= -i\int_0^{a_+} \frac{-1}{x-1}\sqrt\frac{x}{3(x+1)(x-a_-)(a_+-x)} dx 
%  = -iA,
%\end{align*}
%where
%\begin{equation}\label{eq:definitionA}
%A:= \int_0^{a_+} \frac{1}{1-x}\sqrt\frac{x}{3(x+1)(x-a_-)(a_+-x)}  dx ,
%\end{equation}
%which is a real and positive integral. %By applying Lemma~\ref{lemma:reflection}, we obtain the result for the negative complex path
%\[
% t^*_{2,-} = +iA.
%\]
%This result can also be obtained by reproducing the previous computations and changing the argument $\arg(q-a_+) \to -\pi$. 

%%Now, it just remains to check that $t_{2,+}$ is a visible singularity. % First, we proceed with $t_{2,+}$. That is we need to find a visible path $\g \in \HH_{q,0}$ and $\g \subset \complexs^+$ such that $t_{2,+}=T[\g]$. It would be convenient to choose the previous path $\g_2$ and check if it is a visible path. However, $\g_2 \notin \HH_{q,0}$, because its domain is not $(0,1)$. Still, it can be easily adapted as
%Let us take
% \[
%   \eta_{2}:=\eta_{2,a} \cup \eta_{2,b} \cup \eta_{2,c},
% \]
%where
%\[
%\begin{cases}
% \eta_{2,a}(x) := \g_{2,a}(\tau) & \text{ with } \tau \in (0,\de], \\
% \eta_{2,b}(x) := \g_{2,b}(\frac{a_+}{2\de -1} (\tau-1+\de)) & \text{ with } \tau \in [\de,1-\de], \\
% \eta_{2,c}(x) := \g_{2,c}(a_+(1-\tau)) & \text{ with } \tau \in [1-\de,1).
%\end{cases}
%\] 
%with $\de>0$ small enough. Now, following an analogous procedure at the one done previously, we choose $\de \to 0$ and consequently the only integral that contributes to the path is $\eta_{2,b}$. Then
%\begin{align*}
%T[\eta_{2}](\tau) &= 
%\int_0^\tau f d\eta_2 = 
%\lim_{\de \to 0} \int_0^\tau f d\eta_2 = 
%\lim_{\de \to 0} \int_{\de}^\tau f d\eta_{2,b} \\
%&= \lim_{\de \to 0}\int_{\de}^{\tau} f\left(\frac{a_+}{2\de -1} (\nu-1+\de) + i\de\right) \frac{a_+}{2\de -1}  d\nu,
%\end{align*}
%for $\tau \in [0,1]$. Applying the change of variables $x=\frac{a_+}{2\de -1} (\nu-1+\de)$,
%\[
% T[\eta_2](\tau) = \lim_{\de \to 0} \int^{\frac{a_+}{2\de -1} (\tau-1+\de)}_{a_+} f(x + i\de) dx.
%\]
%This integral (with different integration limits) was already solved in the previous part of the proof. Then, adapting it we obtain
%\[
% T[\eta_2](\tau) = -i \int_{a_+(1-\tau)}^{a_+} \frac{1}{1-x}\sqrt\frac{x}{3(x+1)(x-a_-)(a_+-x)}  dx = -i A(\tau),
%\]
%where $A(\tau):[0,1] \to \reals$. Then, $\eta_{2}$ is a visible path if the follow inequality holds
%\[
% |A(\tau)|=|\Im(T[\eta_2](\tau))| < |\Im(T[\eta_{2}](1)|= |A(1)|,
%\]
%for $\tau \in [0,1)$. Because $A(0)=0$, if we check that $A(\tau)$ is a strictly monotonous function, then the inequality holds. Consequently, we need to check that $A'(\tau) \neq 0$ for all $\tau \in (0,1)$. Taking
%\[
% A(\tau) = \int_{a_+(1-\tau)}^{a_+} g(x)  dx,
%\]
%where
%\[
%g(x):=\frac{1}{1-x}\sqrt\frac{x}{3(x+1)(x-a_-)(a_+-x)},
%\]
%it can be seen that $g(x)>0$ for $x \in (0,a_+)$. Then
%\[
%A'(\tau) = g(a_+)\cdot 0 - g\left(a_+(1-\tau)\right)(-a_+) = a_+ g(a_+(1-\tau))>0,
%\]
%for $\tau \in (0,1)$, as we wanted to prove. %And applying Lemma~\ref{lemma:reflection}, $\ol{\eta_{2}}\subset  \complexs^-$ is a visible path generating the conjugated singularity $t^*_{2,-}$.


%\begin{remark}
% Using mathematical software to compute $A$ as defined on~\ref{eq:integralA} we obtain:
%\[
% A \approx 0.177744.
%\]
%% Then,
%% \[
%% t_{2}^* \approx -i 0.177744.
%% \]
%%\[
%%t_{2,-} \approx +i 0.177744.
%%\]
%%By Lemma~\ref{lemma:quatreSingularities}, if $t^*$ is a singularity of the separatrix, then 
%%$-t^*, \conj{t^*}, -\conj{t^*}$ are singularities as well. In this case, $t_{2,+}$ and $t_{2,-}$ are all the singularities that can be found from this result, as they are purely imaginary.
%\end{remark}
%
%\begin{remark}
%It is possible to bound the value of integral  $A$,
%\begin{align*}
%A \leq & \frac{\sqrt{a_+}}{(1-a_+)\sqrt{3\vabs{a_-}}} 
%\int_0^{a_+} \frac{dx}{\sqrt{a_+-x}}
%%
%= \frac{4\sqrt{3}}{3}\frac{a_+^{3/2}}{1-a_+}
%%
%\leq \frac{3}{10}.
% \end{align*}
%And, for the lower bound:
%\begin{align*}
% A \geq & \frac{1}{\sqrt{3(a_+ + 1)(a_+ -a_-)(a_+)}}
% \int_0^{a_+} \sqrt{x} dx 
% %
%= \frac{2 \sqrt[4]{74}}{9} {a_+^{3/2}}
%% 
% \geq \frac{3}{50}.
%\end{align*}
%\end{remark}

%\begin{lemma}  \label{lemma:caminsZeroSimpleInferior}
% The complex paths $\hat{\g_2} \in \HH_q$ from $q_0=a_+$ to $q_l=0$ that do not cross the real axis and stay on $\complexs^-$ (as represented in Figure~\ref{fig:caminsZeroSimpleInferior}) are homotopic.
% 
%The pole resulting from this paths is
% \[
% \hat{t}_2^* = T[\hat{\g_2}(\tau_l)] = t_0 + iA
%\]
%where $A \in \left[\frac{1}{10}, \frac{1}{2}\right]$. As well, there exists a specific integration path such that $T[\hat{\g_2}]$  is a direct path.
%\end{lemma}
%
%
%\begin{figure}[H] 
%   \centering
%   \includegraphics[scale=0.8]{caminsZeroSimpleInferior.png}
%   \caption{Paths on $\HH_q$ towards $q_l=0$ on $\complexs^-$.}
%   \label{fig:caminsZeroSimpleInferior}
%\end{figure}
%
%\begin{proof}
% This result can be proved by aplying the results in Lemma~\ref{lemma:reflection} and \ref{lemma:caminsZeroSimpleSuperior}. 
%\end{proof}

%On this part we have found two different sets of singularities, $\pm t_{1,\pm}$ and $t_{2,\pm}$. Of the two sets, the one with smaller imaginary part in module is $t^*_{2,\pm}$:
%\[
%|\Im(t_{2,\pm}^*)| =  A \in \left[\frac{3}{50},\frac{3}{10}\right],
%\]
%which are visible singularities as well. 
%Thus $A$ is a candidate to define the wide $\de$ of the strip of analyticity $\Pi_{\de}$ defined on equation~\eqref{eq:deltaAnalicity}. Hence, from now on, we focus on looking for singularities with a smaller or equal imaginary module than $A$. In the case we find singularities with imaginary module exactly $A$, then we will be interested in knowing if that singularity is exactly $t_{2,\pm}=\mp iA$ or a new one.

\begin{lemma} \label{lemma:caminsInfinitSimple}
	There exist only two singularities, $t_{2,\pm}^*$, resulting from the paths ${\g \in \PP_{\infty}}$ not crossing the real axis. These singularities are not visible and have imaginary part
	\[
	\Im (t_{2,\pm}^*) = \mp \pi \sqrt{\frac{2}{21}}.
	\]
\end{lemma}

\begin{proof}
Let us consider paths $\g \in \PP_{\infty}$ such that $\proj \g \subset \complexs^+$. Then, since $\fh(q)$ decays with a rate of $\vabs{q}^{-2}$ as $|q| \to \infty$,  all paths considered generate the same singularity, $t^*_{2,+}$.
%
The singularity $t^*_{2,-}$ is given by the conjugated paths.


%
Let us consider the path $\g_*=\g_{*}^1 \vee \g_{*}^2 \vee \g_{*}^3$ where
\begin{equation}\label{proof:pathgamma2}
\begin{cases}
\g_{*}^1(q) = (q,0) & \text{ with } q \in (a_+,1-\e], \\
\proj \g_{*}^2(\phi) = 1 + \e e^{i\phi} & \text{ with } \phi \in [\pi,0], \\
\proj \g_{*}^3(q) = q  & \text{ with } q \in [1+\e,+\infty), \\
\end{cases}
\end{equation}
for any small enough $\e>0$. (See Figure~\ref{fig:caminsInfinitSimpleSuperior}).
%
Then, the resulting singularity is
\[
t_{2,+}^* = t^*(\g_*) 
= \sum_{j=1}^3
\int_{\g_{*}^j} \fh(q) dq .
\]
\begin{figure}[H] 
	\centering
	\begin{overpic}[scale=0.8]{caminsInfinitSimpleSuperior.png}
		\put(48,9.5){{\color{red} $0$ }}	
		\put(56,9.5){{\color{red} $a_+$ }}
		\put(75,9.5){{\color{blue} $1$ }}
		\put(25,9.5){{\color{red} $-1$ }}
		\put(17,9.5){{\color{red} $a_-$ }}
		\put(93,12){$\Re q$}
		\put(47,30){$\Im q$}
		\put(56,20){{\color{myGreen} $\proj\g$ }}	
		\put(66,16){{\color{myBlue} $\proj \g_*$ }}
	\end{overpic}
	\caption{Example of a path $\g \in \PP_{\infty}$ such that $\proj \g \subset \complexs^+$. Path $\g_*$ as defined in~\eqref{proof:pathgamma2}.}
	\label{fig:caminsInfinitSimpleSuperior}
\end{figure}
%
Since $\fh(q)\in \reals$ when $\proj(q) \in (a_+,1)\cup(1,+\infty) \subset \reals$, the integrals on $\g_{*}^1$ and $\g_{*}^3$ take real values.
Therefore, $\g_{*}^2$ is the only path that contributes to the imaginary part to the singularity.
%
Notice that the path $\g_*^2$ partially encircles the pole $q=(1,0)$ of $\fh(q)$. Then, one has
\[
\Im (t_{2,+}^*)  = 
\Im \int_{\g_{*}^2} \fh(q) dq = 
- \pi \Res \paren{\fh,(1,0)} =
-\pi \sqrt{\frac{2}{21}}.
\]
%Seeing that, $\Res\paren{\fh,(1,0)}=\sqrt{\frac{2}{21}}$, one deduce
%	\[
%	\Im (t_{2,+}^*)  = 
%	\Im  \int_{\g_{*}} \fh(q) dq  = 
%	%\int_{\g_{1,b}} f = 
%	- \pi \sqrt{\frac{2}{21}}.
%	\]
Since, by Lemma \ref{lemma:caminsZeroSimple},  $|\Im(t^*_{2,+})|>A$, the singularity $t^*_{2,+}$ is not visible.
\end{proof}

\begin{remark} \label{remark:quatreSingularitiest1}
Using mathematical software, one can see that the singularities $t^*_{2,\pm}$ in Lemma~\ref{lemma:caminsInfinitSimple} satisfy
$t^*_{2,\pm} \approx -0.086697 \mp 0.969516i$.
\end{remark}


==> Article Inner/proofA-ComplexPathsSecondSheet.tex <==
\subsubsection{Paths first crossing the real axis at \texorpdfstring{$[0,1]$}{[0,1]}}
\label{subsubsection:pathsC}
In this section, we check that
the singularities generated by paths C.1 to C.3 (see the list in Section~\ref{subsection:computationSingularities}) are either not visible or $\pm iA$. 

\begin{lemma} \label{lemma:caminsBranca1a}
The singularities $t^*(\g)$ given by paths $\g \in \PP_{0}$ only crossing $\reals$ at $(0,1)$ are either $t^*(\g)=iA$ or $t^*(\g)=-iA$.
\end{lemma}


\begin{proof}
The paths considered in this lemma can turn around the branching point $q=a_+$, but not around the other branching points nor the pole. 
%
Therefore, we classify these paths depending on how many turns they perform around $q=a_+$.
%
In order to do so, we define
\begin{equation}\label{proof:finalArgumentDef}
 \tht_{\fin}(\g) = \lim_{s \to s_{\fin}} \arg(\g(s)-a_+).
\end{equation}
%
%An example of paths classified on relation to $\tht_f(\g)$ is found on Figure~\ref{fig:caminsBranca1zero}.
%
The considered paths satisfy
$\tht_{\fin}(\g)=(2k+1)\pi$
for some $k \in \integers$ (see Figure~\ref{fig:caminsBranca1zero}).
 \begin{figure}
    \centering
        \begin{overpic}[scale=0.68]{caminsBranca1zero.png}
		\put(8,10){{\color{red} $0$ }}
		\put(57,10){{\color{red} $0$ }}	
		\put(35,9.5){{\color{blue} $1$ }}
		\put(84,9.5){{\color{blue} $1$ }}
		\put(19.5,10){{\color{red} $a_+$ }}
		\put(69,10){{\color{red} $a_+$ }}
		\put(19,20){{\color{myGreen} $\proj \g$ }}
		\put(75,17){{\color{myGreen} $\proj \g$ }}
		\put(43.5,12){$\Re q$}
		\put(93,12){$\Re q$}
		\put(8,26){$\Im q$}
		\put(57,26){$\Im q$}
    \end{overpic}
    \caption{Example of paths $\g \in \PP_{0}$ only crossing $\reals$ at $(0,1)$. Left: $\tht_{\fin}(\g)=\pi$. Right: $\tht_{\fin}(\g)=3\pi$.}
    \label{fig:caminsBranca1zero}
 \end{figure}
%
% We compute now
% \begin{equation*}
% 	%\label{proof:operatorSingularities}
% 	t^*(\g)=  \int_{\g} \fh(q) dq,.
% \end{equation*}
%as defined on~\eqref{def:operatorSingularities}.
%
% By Cauchy's Integral Theorem, i
Integrating the function $\fh$ along the path $\g$ is equivalent to integrating along ${\eta}={\eta}^1 \vee {\eta}^2 \vee \eta^3$ with 
\begin{equation}\label{proof:pathsEtaB}
\begin{cases}
\eta^1(q) = (q,0) & 
\text{ with } q \in 
(a_+,a_+ - \e], \\
%	
\proj \eta^2(\phi) = a_+ + \e e^{i\phi} & 
\text{ with } \phi \in [\pi,(2k+1)\pi], \\
%
\proj \eta^3(q) = q & 
\text{ with } q \in [a_+-\e,0),
\end{cases}
\end{equation}
for  small enough $\e>0$. Since
$\int_{\eta^j} \fh(q) dq = \OO(\sqrt{\e})$ for $j=1,2$,
% Then,
\begin{equation*}
t^*(\g) =
\lim_{\e \to 0} \int_{\eta^3} \fh(q) dq = 
\int_{a_+}^0 \frac{1}{q-1}\sqrt\frac{q}{3(q+1) \vabs{q-a_+} e^{i(2k+1)\pi}(q-a_-)} dq  = (-1)^{k+1} iA.
\end{equation*}
% where $A$ is the constant given in~\eqref{def:integralA}. 
\end{proof}
% \begin{figure}[t] 
%	\centering
%	\begin{overpic}[scale=0.68]{caminsBranca1zeroMal.png}
%		\put(7,10){{\color{red} $0$ }}
%		\put(40,10){{\color{red} $0$ }}
%		\put(73,10){{\color{red} $0$ }}	
%		\put(19,10){{\color{red} $a_+$ }}
%		\put(52,15){{\color{red} $a_+$ }}
%		\put(85,11){{\color{red} $a_+$ }}
%		\put(27,12){$\Re(q)$}
%		\put(60,12){$\Re(q)$}
%		\put(94,12){$\Re(q)$}
%		\put(7,24){$\Im(q)$}
%		\put(40,24){$\Im(q)$}
%		\put(73,24){$\Im(q)$}
%	\end{overpic}
%	\caption{Example of paths $\g \in \PP_{0}$ such that $q_1(\g)\in(0,a_+)\cup(a_+,1)$ and $\tht(\g)=\pi$ (left), $\tht(\g)=-\pi$ (center) and $\tht(\g)=3\pi$ (right).}
%	\label{fig:caminsBranca1zeroMal}
%\end{figure}
%
%% Sense considerar multiples.
%
%Let us consider first a path such that $\tht(\g)=\pi$. 
%%
%By Cauchy's integral theorem, integrating function $\fh(q)$ over path $\g$ would be equivalent to integrating over a path $\eta \in \PP_{0}$ such that $\eta \subset \complexs^+$.  
%%
%Therefore, by~\eqref{proof:operatorSingularities} and Lemma~\ref{lemma:caminsZeroSimple}, we have
%\[
%t^*(\g)= t^*(\eta)=-iA.
%\]
%
% $\tht(\g)=3\pi$: \\
% The path $\g$ ends on the second Riemann sheet. Since $q=a_+$ is a branching point  of order $1/2$, ``turning around'' does not add to the integral, just changes the argument of the path. Thus there exists a path $\eta \in \PP_{0}$ completely on the second Riemann sheet (including the initial point) such that $\g$ and $\eta$ give the same result for integral~\eqref{proof:operatorSingularities}. Then,
% \[
%  t^*(\g) = \int_{\g} \fh = \int_{\eta} \fh.
% \]
% Let us consider $\wt{\eta}$ as a projection of path $\eta$ on the first Riemann sheet. That means, selecting the same path but subtracting $2\pi$ to the argument of $\eta$ with respect to the branching point $a_+$. On the function $\fh$, changing Riemann sheet means a change in sign. 
%%Indeed
%%\begin{equation}\label{eq:changeSign}
%% \begin{split}
%%  &f(q;\arg(q), \arg(q-a_+)+2\pi,\arg(q-a_-), \arg(q+1)) =\\
%%&=\frac{1}{q-1}\sqrt{\frac{|q|e^{i\arg(q)}}
%%{3|q-a_+|e^{i\arg(q-a_+)+i2\pi}|q-a_-|e^{i\arg(q-a_-)}|q+1|e^{i\arg(q+1)} }} = \\
%%&= -f(q;\arg(q),\arg(q-a_+),\arg(q-a_-),\arg(q+1)).
%% \end{split}
%%\end{equation}
%Therefore
%\[
% t^*(\g) = %\int_{\eta} \fh = 
% - \int_{\wt{\eta}} \fh.
%\]
%Since the result of the integral for path $\wt{\eta}$ is considered on Lemma~\ref{lemma:caminsZeroSimple}, we have that $t^*(\g)=-t^*_{2,+}=iA$. 
%
%
%Let us recall that we are defining the first Riemann sheet for arguments in $(-\pi,\pi]$ and the second one for arguments in $(\pi,3\pi]$. Therefore, we only need to consider two cases:



\begin{lemma} \label{lemma:caminsBranca1b}
The singularities $t^*(\g)$ given by paths $\g \in \PP_{\infty}$ only crossing $\reals$ at $(0,1)$ are not visible.
\end{lemma}
\begin{proof}
%
We analyze the paths $\g \in \PP_{\infty}$ such that $\proj \g$ goes to infinity on $\complexs^+$
%
(by~\eqref{eq:reflection}, the paths on $\complexs^-$ give conjugated results).
%
Following the proof of Lemma~\ref{lemma:caminsBranca1a}, we classify the paths $\g$ depending on $\tht_{\fin}(\g)$, the final argument with respect to $a_+$ (see~\eqref{proof:finalArgumentDef} and Figure~\ref{fig:caminsBranca1infty}). 
%
\begin{figure}
\centering
\begin{overpic}[scale=0.7]{caminsBranca1Infty.png}
	\put(8,10){{\color{red} $0$ }}
	\put(57,10){{\color{red} $0$ }}	
	\put(30,9.5){{\color{blue} $1$ }}
	\put(79,9.5){{\color{blue} $1$ }}
	\put(15,10){{\color{red} $a_+$ }}
	\put(63,9){{\color{red} $a_+$ }}
	\put(25,18){{\color{myGreen} $\proj \g$ }}
	\put(71,18){{\color{myGreen} $\proj \g$ }}
	\put(44,12){$\Re q$}
	\put(93,12){$\Re q$}
	\put(8,26){$\Im q$}
	\put(58,26){$\Im q$}
\end{overpic}
\caption{
	Example of paths $\g \in \PP_{\infty}$ only crossing $\reals$ at $(0,1)$ such that $\proj \g$ ends on the positive complex plane.
	Left: $\tht_{\fin}(\g)\in(0,\pi)$.
	Right: $\tht_{\fin}(\g)\in(2\pi,3\pi)$.
	}
\label{fig:caminsBranca1infty}
\end{figure}
The paths considered satisfy 
\[
\tht_{\fin}(\g)\in \big(2\pi k,(2k+1)\pi \big),
\quad \text{ for some } k \in \integers.
\]
We compute $t^*(\g)$ using  the path  ${\eta}={\eta}^1 \vee {\eta}^2 \vee \eta^3 \vee \eta^4
\vee \eta^5$ where the paths $\eta^1$, $\eta^2$ are defined in~\eqref{proof:pathsEtaB} and
\[
\begin{cases}
%\eta^1(q) = (q,0) & 
%\text{ with } q \in (a_+,a_+ +\e], \\
%%
%\proj \eta^2(\phi) = a_+ + \e e^{i\phi} & 
%\text{ with } \phi \in [0,2\pi k], \\
%
\proj \eta^3(q) = q & 
\text{ with } q \in [a_+ + \e,1-\e],\\
%
\proj \eta^4(\phi) = 1 + \e  e^{i\phi} & 
\text{ with } \phi \in [\pi,0], \\
%
\proj \eta^5(q) = q &
\text{ with } q \in [1+\e,+\infty),
\end{cases}
\]
for small enough $\e>0$. 
%
Since the integrals on $\eta^3$ and $\eta^5$ take real values and applying the results in Lemma~\ref{lemma:caminsBranca1a} for $\eta^1$ and $\eta^2$, we obtain
%
\[
\Im {t^*(\g)} = \Im \int_{\eta^4} \fh(q) dq.
\]
%
Proceeding as in the proof of Lemma~\ref{lemma:caminsInfinitSimple} and following the natural arguments of the path $\eta$, one deduces that
\[
\Im {t^*(\g)} = -\pi \Res \paren{\fh,(1,2\pi k)} =(-1)^{k+1} \pi \sqrt{\frac{2}{21}}.
\]
Therefore, since $\vabs{\Im t^*(\g)}>A$, the singularity is not visible.
\end{proof}


\begin{lemma} \label{lemma:caminsBranca1c}
	The singularities $t^*(\g)$ given by paths $\g \in \PP_{0} \cup \PP_{\infty}$ 
	both crossing $(0,1)$ and $\reals \setminus [0,1]$
	are not visible.
\end{lemma}

\begin{proof}
Let us define the parameter of the first crossing at $\reals \setminus [0,1]$ as 
\[
 s_2(\g)= \inf \{s \in(s_0,s_{\fin}) \st \Im \proj \g(s)=0, \, \Re \proj \g(s) \notin [0,1] \}
\]
and the corresponding point
\[
q_2(\g)=  \proj \g(s_2(\g)) \in 
\reals \setminus \left\{ [0,1], a_-, -1 \right\}.
\]
%
We consider paths $\g$ with $q_2= q_2(\g) \in (1,+\infty)$ and such that $\proj \g$ approaches $q_2(\g)$ from $\complexs^+$ (see~\ref{eq:reflection}). The cases $q_2 \in (-\infty,a_-)$,  $q_2 \in(a_-,-1)$ and $q_2 \in (-1,0)$ are proved analogously.
% by applying Lemmas~\ref{lemma:caminsNegatius2}, \ref{lemma:caminsNegatius1} and~\ref{lemma:caminsBranca2}, respectively.


%
The strategy is to classify the paths $\g$ depending on how many turns they perform around $q=a_+$ before crossing $\reals \setminus [0,1]$.
%
To this end, we define $\tht_2(\g) = \arg(q_2(\g)-a_+)$ (see Figure~\ref{fig:caminsBranca1creuament}).
% we can  
 \begin{figure}[t] 
    \centering
    \begin{overpic}[scale=0.7]{caminsBranca1creuament.png}
    	\put(7.5,9.5){{\color{red} $0$ }}
    	\put(57.5,9.5){{\color{red} $0$ }}	
    	\put(27.5,9){{\color{blue} $1$ }}
    	\put(77.5,9){{\color{blue} $1$ }}
    	\put(13,9.5){{\color{red} $a_+$ }}
    	\put(63,9.5){{\color{red} $a_+$ }}
    	\put(40,11){$\Re q$}
    	\put(90,11){$\Re q$}
    	\put(8,24){$\Im q$}
    	\put(58,24){$\Im q$}
    	\put(28,18){{\color{myGreen} $\proj \g$ }}
    	\put(78,18){{\color{myGreen} $\proj \g$ }}
    	\put(34,14){{\color{myOrange} $q_2(\g)$ }}
    	\put(84,14){{\color{myOrange} $q_2(\g)$ }}
    \end{overpic}
    \caption{
    Example of paths $\g \in \PP_{\infty}$ crossing both $(0,1)$ and $\reals \setminus[0,1]$ with $q_2(\g) \in (1,+\infty)$ and such that $\proj \g$ approaches $q_2(\g)$ from $\complexs^+$.
    Left: $\tht_2(\g)=0$.
    Right: $\tht_2(\g)=2\pi$.
    }
    \label{fig:caminsBranca1creuament}
 \end{figure}
The paths we are considering satisfy  $\tht_2(\g)=2\pi k$ for some $k \in \integers$.
%
We also define the piece of  path before the crossing as
$
\g_2(\g) = \claus{\g(s) \st s \in (s_{\ini},s_2(\g))}
$
and the corresponding time
\begin{equation*}
	%\label{def:t2FirstCrossing}
	t_2(\g) = \int_{\g_2(\g)} \fh(q) dq.
\end{equation*}
To prove that a singularity $t^*(\g)$ is not visible, it is sufficient to check that $\vabs{\Im t_2(\g)} \geq A$.
%
\begin{enumerate}
\item Consider $\theta_2(\g)=2\pi k$ with $k$ an even number. 
%
Let us consider the path $\eta$ as defined in~\eqref{proof:pathEtaPol} replacing $q_1$ by $q_2$ in its definition.
%
This path $\eta$ lies entirely on the first Riemann sheet, that is $\arg \argf(\eta) \in (-\pi,\pi]$. 
% 
%Thus, we rename it $\eta^{1st}=\eta$.
%
Integrating the function $\fh$ along ${\g_2(\g)}$ is equivalent to integrating it along
\[
\xi= \widetilde{\eta}^1 \vee 
\widetilde{\eta}^2 \vee
\widetilde{\eta}^3 \vee
{\eta},
\]
where
\begin{equation}\label{proof:pathsEtaTilde}
\begin{cases}
\widetilde{\eta}^1(q) = (q,0) & 
\text{ with } q \in (a_+,a_+ +\e], \\
%
\proj \widetilde{\eta}^2(\phi)=a_+ + \e e^{i\phi} &
\text{ with } \phi \in [0,2\pi k], \\
%
\proj \widetilde{\eta}^3(q) = q & 
\text{ with } q \in [a_+ + \e,a_+),
\end{cases}
\end{equation}
for $\e>0$ small enough. 
%
Notice that this construction makes sense since the path $\widetilde{\eta}^3$ has argument 
$\arg \argf(\widetilde{\eta}^3)=2\pi k$ (which belongs to the first Riemann sheet).

Then, since
$\int_{\wt{\eta}^j} \fh(q) dq = \OO(\sqrt{\e})$ for $j=1,2,3$ and
applying Lemma~\ref{lemma:caminsPol}, we have
\[
\vabs{\Im t_2(\g)} = 
\lim_{\e \to 0}
\vabs{\Im \int_{\xi} \fh(q)dq} =
\vabs{\Im \int_{\eta} \fh(q)dq} > A.
\]

\item Consider $\theta_2(k)=2\pi k$ with $k$ an odd integer.
%
We define the  path $\eta^*$, lying on  the second Riemann sheet, as
\[
\eta^* = (\proj \eta, \arg \argf(\eta)+2\pi)\in \mathbb{C}\times (\pi,3\pi],
\]
where $\eta$ is the path introduced in~\eqref{proof:pathEtaPol} (replacing $q_1$ by $q_2$ in its definition).
%
Note that the path $\eta$ lies on the first Riemann sheet ($\arg \argf(\eta) \in (-\pi,\pi]$). 
%
%

It can be easily checked that switching the Riemann sheet implies a change in sign. That is,
\begin{equation}\label{proof:changeSheet}
\int_{\eta^*} \fh(q) dq = - \int_{\eta} \fh(q)dq.
\end{equation}
Then, integrating the function $\fh$ along the path ${\g_2(\g)}$ is equivalent to integrating it over 
\[
{\xi}=\widetilde{\eta}^1 \vee 
\widetilde{\eta}^2 \vee
\widetilde{\eta}^3 \vee
{\eta}^{*},
\]
where paths $\wt{\eta}^j$ for $j=1,2,3,$ are defined on~\eqref{proof:pathsEtaTilde}. 
%
This construction makes sense since the path $\widetilde{\eta}^3$ has argument $\arg \argf(\wt{\eta}^3)=2\pi k$ (which belongs to the second Riemann sheet).

Then, since
$\int_{\wt{\eta}^j} \fh(q) dq = \OO(\sqrt{\e})$ for $j=1,2,3$ and
applying Lemma~\ref{lemma:caminsPol} and formula~\eqref{proof:changeSheet}, we have
\[
\vabs{\Im t_2(\g)} = 
\lim_{\e \to 0}
\vabs{\Im \int_{\xi} \fh(q)dq} =
\vabs{\Im \int_{\eta} \fh(q)dq} > A.
\]
\end{enumerate}
\end{proof}


==> Article Inner/proofA-ComputationSingularities.tex <==
\subsection{Singularities closest to the real axis}
\label{subsection:computationSingularities}

Proposition~\ref{proposition:singularitiesSeparatrix} provides the type of singularities that $q(t)$ may posses in its first Riemann sheet.
%
Then, to prove Theorem~\ref{theorem:singularitiesChangeq}, we look for those singularities which are closest to the real axis. 
%
To do so, we analyze
\begin{equation}\label{eq:integralsIniciSeccio}
\int_{a_+}^{0} \fh  d\g, \qquad
\int_{a_+}^{\infty} \fh  d\g,
\end{equation}
along all paths $\g \subset \mathscr{R}_f$ with such endpoints
%
and prove that, for all possible paths, the only singularities in the complex strip $\overline{\Pi_A}$ (see~\eqref{def:PiA})  are $t=\pm iA$.
%
% which implies that $q(t)$ can be extended to .

We introduce the following paths
\begin{equation*}
%\label{def:spacesHq}
\begin{split}
&\PP_0 = \claus{ \g: (s_{\ini},s_{\fin}) \to \mathscr{R}_f \st
\lim_{s \to s_{\ini}} (\proj \g(s), \arg \argf( \g(s)))=(a_+,0), \,
\lim_{s \to s_{\fin}} \proj \g(s)= 0}, \\
%
&\PP_{\infty} = \claus{ \g: (s_{\ini},s_{\fin}) \to \mathscr{R}_f \st
\lim_{s \to s_{\ini}} (\proj \g(s), \arg \argf( \g(s)))=(a_+,0), \h
\lim_{s \to s_{\fin}}\vabs{\proj \g(s)}= \infty},
\end{split}
\end{equation*}
%where $(*) = \CC^0, \CC^1\text{-piecewise}$ and
with the natural projection $\proj:\mathscr{R}_f\to \complexs$.


We have chosen $\tht_{\ini} := \lim_{s \to s_{\ini}} 
\arg \argf( \g(s)) = 0$ without loss of generality. Indeed, since $q(t) \in [a_+,1)$ for $t \in \reals$ (see~\eqref{eq:basicsAboutq}), it could be either $0$ or $2\pi$. The paths with asymptotic argument $2\pi$ can be analyzed analogously and lead to singularities with opposed signed with respect to those given by paths in $\PP_0$, $\PP_\infty$.
% 
% \textcolor{red}{
% Notice that we have specified the asymptotic argument of the paths at the starting point as
% %
% $\tht_{\ini} := \lim_{s \to s_{\ini}} 
% \arg \argf( \g(s)) = 0.$
% %
% Indeed, since $q(t)$ is the analytic continuation of a real function with $q(t) \in [a_+,1)$ for $t \in \reals$ (see~\eqref{eq:basicsAboutq}), the argument $\tht_{\ini}$ must be either $\tht_0=0$ or $\tht_0=2\pi$.
% %
% However, due to the real-analyticity of $q(t)$ in the interval $[a_+,1)$ both arguments lead to the same results for Theorem~\ref{theorem:singularitiesChangeq}.
% %
% Thus, we assume $\tht_0=0$.}

Furthermore, the asymptotic argument of the paths at its endpoints is not specified since it is given by the path itself.

For a given path $\g \in \PP_0 \cup \PP_{\infty}$,
we can define a path $T[\g]:[s_{\ini},s_{\fin}) \to \complexs$ in the $t$-plane (or, more precisely, on the Riemann surface of $q(t)$) as 
\begin{equation}\label{def:operatorT}
T[\g](s)=  
\int_{s_{\ini}}^{s} \fh(\g(\tau)) \g'(\tau) d \tau, \quad
\text{ for } s \in [s_{\ini},s_{\fin}).
\end{equation}
%
Note that then the value of the integrals in~\eqref{eq:integralsIniciSeccio} is just
% , we use the following notation  
\begin{equation}\label{def:operatorSingularities}
t^*(\g) =
\lim_{s \to s_{\fin}} T[\g](s) =
\int_{\g} \fh(q) dq.
%\int_{s_0}^{s_f} \fh(\g(z)) \g'(z) dz.
\end{equation}
%
% Notice that, $T[\g]:[s_{\ini},s_{\fin}) \to \complexs$ defines a path in the complex $t$-plane or, more precisely, on the Riemann surface of $q(t)$.
%
Since we are interested in the singularities of $q(t)$ on its first Riemann sheet, we only consider the paths $T[\g]$ which belong to the complex strip $\Pi_A$
(Except, of course, the endpoint of the path $t^*(\g)\in\partial \Pi_A$). 
%
See Figure~\ref{fig:admisiblePaths}.

%Notice that, from \eqref{eq:lemmaIntegralEquationGeneral}, $T[\g]$ could be multivalued outside the region of analyticity of $q(t)$, yielding to different results. 
%%
%Therefore, we need to impose that the path $T[\g]$ stays on the complex strip $\Pi_A$. (Except, of course, the endpoint of the path, the singularity $t^*(\g)$, which should belong to $\partial \Pi_A$). See Figure~\ref{fig:admisiblePaths}.

\begin{figure}[H] 
	\centering
	\begin{overpic}[scale=0.7]{admisiblePaths.png}
		\put(21,13){{\color{myGreen} $0$ }}
		\put(74,13){{\color{myGreen} $0$ }}
		\put(15,27){{\color{myOrange} $iA$ }}
		\put(69,27){{\color{myOrange} $iA$ }}
		\put(21,28){{\color{myGreen} $t^*(\g)$ }}
		\put(82,28){{\color{myGreen} $t^*(\g)$ }}
		\put(12,3){{\color{myOrange} $-iA$ }}
		\put(66,3){{\color{myOrange} $-iA$ }}
		\put(30,17.5){{\color{myOrange} $\Pi_A$ }}
		\put(84,17.5){{\color{myOrange} $\Pi_A$ }}
		\put(39,15){$\Re t$}
		\put(94,15){$\Re t$}	
		\put(15,38){$\Im t$}		
		\put(70,38){$\Im t$}
		\put(7,20){{\color{myGreen} $T[\g]$ }}
		\put(58,22){{\color{myGreen} $T[\g]$ }}	
	\end{overpic}
	\caption{Example of paths $\g \in \PP_{0}\cup \PP_{\infty} $. 
	Left: $T[\g]\subset \Pi_A$ and $t^*(\g)=iA$.  
	Right: $T[\g] \not\subset {\Pi_A}$.}
% 	gives rise to an additional singularity $t^*(\g) \in \partial \Pi_A$ by encircling singularity $iA$.}
	\label{fig:admisiblePaths}
\end{figure}

The following definition  characterizes the paths that we consider.
\begin{definition}\label{definition:visibleSingularity}
We say that a singularity $t^*$ of $q(t)$ is \emph{visible} if there exists a path $\g \in \PP_{0} \cup \PP_{\infty}$ such that
\begin{itemize}
	\item $t^*=t^*(\g)$,
	\item $T[\g](s) \in \Pi_A, \,$ for  $s\in[s_{\ini},s_{\fin})$.
\end{itemize}
\end{definition}

\begin{remark}
	In~\cite{SimoGelf08}, the authors use a different definition of visible singularity: $t^* \in \complexs$ is considered a visible singularity if $q(t)$ can be continued from the real axis and then along the vertical line with a path of the form
	\[
	\zeta(t) = \Re t^* + i t, \qquad \text{for} \quad  t \in [0,\Im{t^*}).
	\]
	This condition on the paths is more restrictive than merely imposing that $T[\g] \subset \Pi_{\upsilon}$ for $\upsilon=\Im t^*$. 
	%
	However, to compute $t^*(\g)$, they are equivalent since both paths belong to $\Pi_{\upsilon}$.
	%
	%Nonetheless, we have opted for a less strict condition as it facilitates the task of checking that the paths selected are admissible.
\end{remark}

Theorem~\ref{theorem:singularitiesChangeq} is a consequence of Proposition~\ref{proposition:singularitiesSeparatrix} and the following result.
\begin{proposition}\label{proposition:camins}
There exist two paths $\g_{\pm} \in \PP_{0}$ yielding the visible singularities  $t^*(\g_{\pm})=\pm iA$.
Moreover, these are the only two visible singularities of $q(t)$.
\end{proposition}

We devote the rest of this section to prove Proposition~\ref{proposition:camins}. 
%
Let us introduce some tools and considerations to simplify  the analysis of the integrals in~\eqref{eq:integralsIniciSeccio}.
%
\begin{itemize}
\item If $\g \subset \mathscr{R}_f$ is an integration path then, defining $\eta=\conj{\g}$\footnote{
We define the conjugation on a Riemann surface as the natural continuation of the conjugation in the complex plane. That is, for $z=(x,\tht) \in \mathscr{R}_f$, its conjugated is  $\conj{z}=(\conj{x},-\tht)\in \mathscr{R}_f$.}
, we have that
\begin{equation}\label{eq:reflection}
\int_{\eta} \fh(q) dq = \conj{\int_{\g} \fh(q) dq}.
\end{equation}
%
\item Notice that the paths considered cannot contain the singularities of $\fh$ (except in their endpoints) since $0 ,a_{\pm}, \pm 1 \notin \mathscr{R}_f$.
%
\item When saying that a path $\g \in \PP_{0} \cup \PP_{\infty}$ crosses $\reals$, we refer to the two lines whose complex projection onto $\mathscr{R}_f$ coincide with $\reals$. Analogously for any other interval.
%
\item Instead of detailing the paths $\g  \in \PP_{0} \cup \PP_{\infty}$, 
%
we only describe their projections $\proj \g \subset \complexs$.
%
This omission makes sense since paths $\g$ are continuous on $\mathscr{R}_f$ and, as a result, $\arg \argf(\g)$ must be continuous as well (see~\eqref{eq:fcompleteanalytic}).
%
Therefore, we can let the natural arguments of $\proj \g$ and the initial point $(a_+,0)$ of the path define $\arg \argf(\g)$. 
\end{itemize}

To prove Proposition~\ref{proposition:camins}, we classify the paths as follows.
\begin{enumerate}[label*=\Alph*.]
	\item Paths not crossing $\reals$:
	\begin{enumerate}[label*=\arabic*.]
		\item Paths in $\PP_{0}$ not crossing $\reals$: Lemma~\ref{lemma:caminsZeroSimple}.
		\item Paths in $\PP_{\infty}$ not crossing $\reals$: Lemma~\ref{lemma:caminsInfinitSimple}.
	\end{enumerate}
	\item Paths first crossing the real axis at $\reals \setminus [0,1]$:
	\begin{enumerate}[label*=\arabic*.]
		\item First crossing of $\reals$ at $(1,+\infty)$:  Lemma~\ref{lemma:caminsPol}.
		\item First crossing of $\reals$ at $(-\infty,a_-)$: Lemma~\ref{lemma:caminsNegatius2}.
		\item First crossing of $\reals$ at $(-1,0)$: Lemma~\ref{lemma:caminsNegatius1}.
		\item First crossing of $\reals$ at $(a_-,-1)$: Lemma~\ref{lemma:caminsBranca2}.
	\end{enumerate}
	\item Paths first crossing the real axis at $(0,1)$: 
	\begin{enumerate}[label*=\arabic*.]
		\item Paths in $\PP_{0}$ only crossing $\reals$ at $(0,1)$: Lemma~\ref{lemma:caminsBranca1a}.
		\item Paths in $\PP_{\infty}$  only crossing $\reals$ at $(0,1)$: Lemma~\ref{lemma:caminsBranca1b}.
		\item Paths also crossing $\reals \setminus [0,1]$: Lemma~\ref{lemma:caminsBranca1c}.
	\end{enumerate}
\end{enumerate}

%	
%Furthermore, note that one can consider integrals on the real line of as uniform limits of integrals on $\complexs^+ = \claus{\Im(z)>0}$. We use this fact without mentioning along the following sections.

%Before, settling in which paths should be taken to compute the integrals on equation \eqref{eq:integralPolesSection}, we analyses function $\fh$.
%\begin{remark}
%	The function $\fh$, as defined on~\eqref{eq:fcompleteanalytic}, has one pole corresponding to the saddle point at $q=1$ and four branching points at $q=0,-1,a_+, a_-$. When taking $q \in \reals$ there are two possibilities:
%	\begin{align*}
%	& \fh(q) \in \reals \text{ when } q \in (-\infty, a_-) \cup (-1,0] \cup (a_+,1) \cup (1, +\infty), \\
%	& \fh(q) \in i \reals \text{ when } q \in (a_-,-1) \cup (0,a_+).
%	\end{align*}
%	See Figure~\ref{fig:integralConfiguration}.
%	%Hence, we decide to consider logarithm branches $(0,a_+)$ and $(a_-,-1)$ which correspond with the intervals such that when $q\in \reals$ the integrand is purely imaginary. And the arguments for this logarithm branches are defined to be in $(-\pi,\pi)$. 
%	%From now on, we consider the first Riemann sheet, with respect one of the four branching points of $f$ to take place when $\arg \in (-\pi,\pi)$. Respectively, the second Riemann sheet is considered to place when $\arg \in (\pi, 3\pi)$. Further sheets do not need to be considered, as we are dealing with square roots, and the third sheet is the same as the first. 
%	%Then, to analyse the complex integral on~\eqref{eq:integralPolesSection}, we have to take into account the characteristics of $f$ as represented in Figure~\ref{fig:integralConfiguration}.
%	\begin{figure}[H] 
%		\centering
%		\begin{overpic}[scale=0.8]{settingq.png}
%		\put(48,9.5){{\color{red} $0$ }}	
%		\put(56,9.5){{\color{red} $a_+$ }}
%		\put(75,9.5){{\color{blue} $1$ }}
%		\put(25,9.5){{\color{red} $-1$ }}
%		\put(17,9.5){{\color{red} $a_-$ }}
%		\put(93,12){$\Re(q)$}
%		\put(45,30){$\Im(q)$}
%		\put(35,18){{\color{myGreen} $q \to 0$ }}	
%		\put(66,18){{\color{myGreen} $q \to \infty$ }}
%		\end{overpic}
%		\caption{Setting for integrals~\eqref{eq:integralPolesSection}.
%		On blue the pole $q=1$ and on red the branching points and the intervals of the real line where $\fh$ is not real-valued. 
%		The two possible ending points of the integration paths are represented in green. }
%		\label{fig:integralConfiguration}
%	\end{figure}
%	%\begin{align*}
%	%& P_1 := \{1\}, & & \RRR_f^0:= \{z \in \RRR_f \st \Im(z)=0\}, \\
%	%& B_1 := (0,a_+), & & \RRR_f^+ := \{z \in \RRR_f \st \Im(z)>0\}, \\
%	%& B_2 := (a_-,-1), & & \RRR_f^- := \{z \in \RRR_f \st \Im(z)<0\}.
%	%\end{align*}
%\end{remark}




%This is explain with more detail on the following section. \\
%
%On this document, we are only interested in evaluating contour integrals of $f: \RRR_f \to \complexs$ on different paths $\g$. Thus, when performing computations, we will define paths on the complex plane,  $\g \subset \complexs$, and let the natural arguments of the integration paths define on which Riemann sheet the function is being evaluated.
%On this section, we are only interested in evaluating contour integrals of $f$ on different paths. Thus, we will let the natural arguments of the integration paths to define on which Riemann sheet the function is being evaluated.
%As seen on the previous section, our aim is to find the constant $\de$ of the analyticity strip $\Pi_{\de}$, defined on Lemma~\ref{lemma:FontichPols} as
%\[  \Pi_{\de} := \{ t \in \complexs \st  |\Im(t)|< \de \}, \]
%such that separatrix $\s(t)$ is analytic on it. That is, we have to find the singularity (or singularities) $t^*  \in \complexs$  of separatrix $\s(t)$ with smaller imaginary part.  And by Lemma~\ref{lemma:separatrixChangeCoordinates}, this will be equivalent to look for the singularities $t^* \in \complexs$ of  $(q(t),\qd(t))$. To simplify the notation, in this section, we are using indistinctly the name  separatrix to refer to $\s(t)$ and $(q(t),\qd(t))$. 
%By following the results from Lemma~\ref{lemma:singularitiesSeparatrix}, and recalling that we are selecting $t_0=0$ and $q_0=a_+$, we have that the singularities $t^*$ of $q(t)$ satisfy
%\begin{equation} \label{eq:integralEquationPole}
%  t^*= \int_{a_+}^{q^*} f(q) \h d \g(q),
%\end{equation}
%where $q^*=0$ or $q^*=\infty$ and $\g \subset \complexs$ an integration path from $a_+$ to $q^*$. 
%\begin{remark}
%It is not correct to define the integration paths $\g$ on the complex plane. Instead they should be defined on the Riemann surface $\RRR_f$. However, to simplify the notation, we are considering them on the complex plane, and letting the natural arguments of the path to define the argument of $g(q)$, as defined on~\eqref{eq:fcompleteanalytic}.
%\end{remark}
%As well, we are selecting $B_1=(0,a_+)$ and $B_2=(a_-,-1)$ as logarithm branches with arguments on $(-\pi,\pi)$.  \\
%Different paths $\g$ and different choices of $q^*$ will result in different singularities $t^*$. 

%Hence, the aim of this section is to find the  singularities of the separatrix that have smaller imaginary part in module and that are visible, as these singularities will define the analyticity strip of the separatrix, $\Pi_{\de^*}$ as follows  
%\begin{equation} \label{eq:deltaAnalicity}
%\de^* = \min\left\{ |\Im(t^*(\g))| \text{ s.t.} \g  \in \HH_{q,0} \cup \HH_{q,\infty} \text{ and } t^*(\g) \text{ is visible}\right\}.
%\end{equation}
%We say that a singularity $t^*$ is a {\em leading singularity} if $|\Im(t^*)|= \de^*$. \\

%Hence, we proceed by checking all possible paths $\g \in \HH_{q,0} \cup \HH_{q,\infty}$ that are visible, and select the ones where $t^*(\g)$ has the smaller imaginary module, which will give us the value $\de$. Additionally, in prevision of following work, it will be useful to compute as well how many leading visible singularities there are and where they are situated. \\

%Before beginning to check all possible paths, let us introduce an example of visible and non-visible paths and some remarks on the previously defined terms.
% We are not only interested in finding $\de$, but we will be interested as well in knowing how many singularities are on the border of $\Pi_{\de}$ and its position. That is, how many singularities are on the border of $\Pi_{\de}$.
%\begin{example} 
%We assume that, using three different paths on $\g_1,\g_2,\g_3 \in \HH_{q,0}  \cup \HH_{q,\infty}$, three different poles have been found
%\begin{align*}
%t_1^* =t^*(\g_1), \\
%t_2^* = t^*(\g_2), \\
%t_3^* = t^*(\g_3),
%\end{align*}
%with their corresponding paths $T[\g_1], T[\g_2], T[\g_3] \in \HH_t$. This paths are represented in Figure~\ref{fig:directpath}.
%\begin{figure}[H] 
%   \centering
%   \includegraphics[scale=0.6]{directpath.png}
%   \caption{Possible paths on $\HH_t$ for three different singularities. }
%   \label{fig:directpath}
%\end{figure}
%We notice that, a priori, it seems that $t_3^*$ is the leading singularity, as it has the smallest imaginary part in module. However, $\g_3$ is not visible because the imaginary part of $T[\g_3]$ goes past $t^*_3$ (where it may be encircling an unknown singularity of the problem, for example). Hence, if we are able to find a visible path $\hat{\g_3} \in \HH_q$ such that  $t^*_3=T[\hat{\g_3}]$, then we will take $\de^*=|\Im(t_3^*)|$. On the contrary, if such path does not exist, then we will take $\de^*=|\Im(t_2^*)|$ as $T[\g_2]$ is a visible path.
%\end{example}

%\begin{figure}[H] 
%   \centering
%   \includegraphics[scale=0.8]{SimoGelfreichPaths.png}
%   \caption{Representation of visible paths as defined by Sim\'o and Gelfreich (left). Representation of paths $\zeta \in \HH_{t}$ used in this document (right). }
%   \label{fig:SimoGelfreichPaths}
%\end{figure}

%\begin{remark}
%It is important to stress that on the definition of visible path~\eqref{eq:visiblePathInequality} the inequality is strict. That is because the analyticity of the separatrix can be only guaranteed on
% \[ \Pi_{\de^*} := \{ t \in \complexs \st  |\Im(t)|< \de^* \}.\]
%This means that the path to a leading singularity must be defined on $\Pi_{\de^*}$. Otherwise, if it is defined on $\ol{\Pi}_{\de^*}$, could be unknowingly crossing a singularity as, by definition, there exists at least one singularity on $\ol{\Pi}_{\de^*}$.\\
%In fact, on Remark~\ref{remark:nonVisiblePath}, we present a set of paths on $\ol{\Pi^*}_{\de}$ that produce countably infinite singularities on the border of this region by crossing other singularities. Specifically, we have constructed a set of paths $\g \in \HH_{q,0}$ that satisfy a ``$\leq$''-version of inequality~\eqref{eq:visiblePathInequality} and that by crossing a leading visible singularity can generate infinitely-countable non-visible leading singularities.
%\end{remark}
% We are not only interested in finding $\de$, but we will be interested as well in knowing how many singularities are on the border of $\Pi_{\de}$ and its position. That is, how many singularities are on the border of $\Pi_{\de}$.

%\begin{lemma} \label{lemma:quatreSingularities}
%If $t^*$ is a singularity of the separatrix $(q(t),\qd(t))$, then $-t^*, \ol{t^*}$ and $-\ol{t^*}$ are singularities as well.
%\end{lemma}
%
%
%\begin{proof}
%From Lemma~\ref{lemma:separatrixChangeCoordinates}, $q(t)$ satisfies
%\[ \qd^2 = \frac{3}{q} (q-1)^2(q+1)(q-a_-)(q-a_+), \]
%with initial condition $q(0)=a_+$. Then, $\tilde{q}(t):=q(-t)$  is a solution of the differential equation as well, because
%\[ \dot{\tilde{q}}^2=(-\tilde{\qd})^2 = \frac{3}{\tilde{q}} (\tilde{q}-1)^2(\tilde{q}+1)(\tilde{q}-a_-)(\tilde{q}-a_+), \]
%and the initial conditions hold
%\[ \tilde{q}(0) = q(0) = a_+.\]
%Consequently, by Picard theorem, $q=\tilde{q}$. This means that the separatrix is symmetric, i.e $q(t)=q(-t)$.
%Hence, if $t^*$ is a singularity of $(q(t),\qd(t))$, then $-t^*$ will be as well. 
%
%Now, let $\g \in \HH_{q,0} \cup \HH_{q,\infty}$ such that $t^*=t^*(\g)$ is a singularity of the separatrix. Then the conjugate path $\ol{\g} \in \HH_{q,0} \cup \HH_{q,\infty}$ generates a singularity as well. Then, by Lemma~\ref{lemma:reflection}, this singularity is
%\[ 
%t^*(\ol{\g}) = \int_{\ol{\g}} f =  \ol{\int_{\g} f} = \ol{t^*(\g)} = \ol{t^*} .
%\]
%Hence, if $t^*$ is a singularity of the separatrix $\ol{t^*}$ is one as well.
%\end{proof}




%With all this results, it just remains to check the singularities $t^*(\g)$ resulting from all the paths $\g \in \HH_{q,0} \cup  \HH_{q,\infty}$ and to find the ones that are visible and have smaller imaginary module, that is the leading visible singularities. To do so, we divide the different paths by the following scheme:
%\begin{enumerate}
%\item Paths $\g$ not crossing the real axis:
%\begin{enumerate}[label*=\arabic*.]
%\item Paths $\g \in \HH_{q,\infty}$ not crossing the real axis. Lemma~\ref{lemma:caminsInfinitSimple}.
%\item Paths $\g \in \HH_{q,0}$ not crossing the real axis.  Lemma~\ref{lemma:caminsZeroSimple}.
%\end{enumerate}
%\item Paths $\g$ not crossing $\reals^-$:
%\begin{enumerate}[label*=\arabic*.]
%\item Paths $\g$ not crossing $\reals^- \cup (0,a_+)$. Lemma~\ref{lemma:caminsVoltesPol}.
%\item Paths $\g$ not crossing $\reals^- \cup (1,\infty)$. Lemma~\ref{lemma:caminsVoltesBranca}.
%\item Paths $\g$ not crossing $\reals^-$. Lemma~\ref{lemma:caminsBranca1}.
%\end{enumerate}
%\item Paths $\g$ crossing $\reals^-$:
%\begin{enumerate}[label*=\arabic*.]
%\item First crossing of $\reals^-$ at $(-1,0)$. Lemma~\ref{lemma:caminsNegatius1}.
%\item First crossing of $\reals^-$ at $(a_-,-1)$. Lemma~\ref{lemma:caminsBranca2}.
%\item First crossing of $\reals^-$ at $(-\infty,a_-)$. Lemma~\ref{lemma:caminsNegatius2}.
%\end{enumerate}
%\end{enumerate}
%
%
%Therefore, taking into account the initial condition $q_0=(a_+,3\pi)$, these paths $\g$ have argument $\arg{g(\g)} \in [0,\pi]$, as defined on~\eqref{eq:fcompleteanalytic}, until their first crossing of $\reals$.
%



==> Article Inner/proofA-IntroductionSingularities.tex <==

In this section we prove Theorem~\ref{theorem:singularities} and Proposition~\ref{proposition:domainSeparatrix},  which deal with the study of the complex singularities and zeroes of the analytic extension of the time-parametrization $\s(t)=(\la_h(t),\La_h(t))$ of the homoclinic connection given in~\eqref{eq:separatrixParametrization}.

Let us recall that $\s(t)$ is a solution of the Hamiltonian system $H_{\pend}$ in~\eqref{def:HpendHosc} and it is found at the energy level ${H}_{\pend}=-\frac{1}{2}$. 
%
Therefore, 
%considering the trigonometric identity $1+\cos(\la)=2\cos^2(\frac{\la}{2})$, it satisfies
\begin{equation}\label{eq:odeSeparatrix}
(\dot{\la})^2 = 
%\paren{\Dt{\la}{t}}^2= 
15 - 12\cos^2\paren{\frac{\la}{2}}
- \frac{3}{\cos\paren{\frac{\la}{2}}}.
\end{equation}
%
Equation~\eqref{eq:odeSeparatrix} can be solved as
$t=F(\la)$,
where $F$ is a function defined by means of an integral.
%
Prove Theorem~\ref{theorem:singularities} and Proposition~\ref{proposition:domainSeparatrix} boils down to studying the analytic continuation of $F^{-1}$.

We divide the proof of Theorem~\ref{theorem:singularities} into three main steps. 
%
First, in Section~\ref{subsection:changeq}, we perform the change of variables $q=\cos(\frac{\la}{2})$ and
rephrase Theorem~\ref{theorem:singularities} in terms of $q(t)$ (Theorem~\ref{theorem:singularitiesChangeq}).
%
Then, in Section~\ref{subsection:classificationSingularities}, we analyze all the possibles types of singularities that $q(t)$ may have  (Proposition~\ref{proposition:singularitiesSeparatrix}), which turn out to be poles or branching points.
%
In addition we prove that all the singularities have to be given by integrals along suitable complex paths.
%
Finally, in Section~\ref{subsection:computationSingularities},
taking into account all complex paths leading to  singularities, we prove that the singularities of $q(t)$ with smaller imaginary part (in the first Riemann sheet of $q(t)$) are $t=\pm iA$.
%

Finally, in Section~\ref{subsection:propZeroes}, we use the results obtained in the previous sections, to
analyze the zeroes of $\La_h(t)$ in the strip of analyticity $\Pi_A$ (see \eqref{def:PiA}), thus proving Proposition~\ref{proposition:domainSeparatrix}.

In order to simplify the notation, through the rest of the section we denote by $C$ any positive constant independent of $t$.

\subsection{Reformulation of Theorem~\ref{theorem:singularities}}
\label{subsection:changeq}

To prove Theorem~\ref{theorem:singularities}, it is more convenient to work with the variable $q=\cos\paren{\frac{\la}{2}}$ instead of $\la$.
%
Notice that this change of coordinates, when restricted to $\la \in (0,\pi)$, is a diffeomorphism. 
%
%Then, proving Theorem~\ref{theorem:singularities} is a consequence to proving the following result.

\begin{theorem} \label{theorem:singularitiesChangeq}
	Consider the real-analytic time parametrization $\s(t)=(\la_h(t),\La_h(t))$ introduced in~\eqref{eq:separatrixParametrization} and denote $a_\pm =-\frac{1}{2}\pm \frac{\sqrt{2}}{2}$.
	%
	Then, $q(t)=\cos \paren{\frac{\la_h(t)}{2}}$ satisfies
	\begin{equation}\label{eq:basicsAboutq}
	q(t) \in [a_+,1) 
	\quad \text{for} \quad t \in  \reals, \qquad
	q(0) = a_+, 
	\end{equation}
	and the differential equation
	\begin{equation} \label{eq:odeSeparatrixQ}
	\qd^2 = \frac{3}{q} (q-1)^2 (q+1)(q-a_-)(q-a_+).
	\end{equation}
	
	Moreover, we have that:
	\begin{itemize}
	\item The function $q(t)$ extends analytically to the strip $\Pi_A$ defined in~\eqref{def:PiA}.
	\item The function $q(t)$ has only two singularities on $\partial \Pi_A$ at $t=\pm iA$. 
	\item There exists $\nu>0$ such that, for $t \in \complexs$ with $\vabs{t -iA}<\nu$ and $\arg(t-iA) \in (-\frac{3\pi}{2},\frac{\pi}{2})$,  we have
	\begin{align}\label{eq:expressionqSingularities}
		q(t) = - \frac{3\al_{+}}{2} (t -  iA)^{\frac{2}{3}} + 
		\OO(t - iA)^{\frac{4}{3}}, 
	\end{align}
	with $\al_{+} \in \complexs$ such that $\al_{+}^3=\frac{1}{2}$.
	%
	
	
	An analogous result holds for
	$\vabs{t+iA}<\nu$ and $\arg(t + iA) \in (-\frac{\pi}{2},\frac{3\pi}{2})$
	with $\al_{-}=\conj{\al_+}$.
	\end{itemize} 
\end{theorem}

% \begin{remark}
% Since $q(t)$ is the analytic continuation of a real function, if $t^*$ is a singularity of $q(t)$, its conjugate $\conj{t^*}$ is as well. 
% %
% In addition, if $q(t) \sim -\frac{3\al}{2}(t-\conj{t^*})^{\frac{2}{3}}$
% for $\vabs{t-t^*}\ll 1$, then
% $q(t) \sim -\frac{3\conj{\al}}{2}  (t-\conj{t^*})^{\frac{2}{3}}$
% when $|t-\conj{t^*}|\ll 1$.
% \end{remark}

Theorem~\ref{theorem:singularities} is a corollary of Theorem~\ref{theorem:singularitiesChangeq}.

\begin{proof}[Proof of Theorem~\ref{theorem:singularities}]

To obtain Theorem~\ref{theorem:singularities} from Theorem~\ref{theorem:singularitiesChangeq} it is enough to prove that $\La_h(t)$ has no singularities in $\ol{\Pi_A} \setminus \claus{\pm iA}$ and that $(\la_h(t),\La_h(t))$ can be expressed as in~\eqref{eq:homoclinicaSingularities} close to $t=\pm iA$.
	
Since $\dot{\la}_h = -3\La_h$ and using the change of coordinates $q=\cos (\frac{\la}{2})$, we have that
\begin{equation}\label{proof:LahSquared}
\La_h^2(t) = \frac{4}{9}\frac{\dot{q}^2(t)}{\paren{1-q^2(t)}}.
\end{equation}	
%
We claim that, if $\La_h(t)$ has a singularity at $t=t^*$, then $\La_h^2(t)$ has a singularity at $t=t^*$ as well. 
%
Indeed, the only case when the previous affirmation could be false is if $t^*$ is a branching point of order $\frac{k}{2}$ with $k\geq 1$ an odd natural number. 
%
In this case,
\begin{align*}
\la_h(t) = \la_h(t^*) + C (t-t^*)^{\frac{k}{2}-1} \paren{1 + \OO(t-t^*)^{\beta}}, \quad
\text{ when } 0<\vabs{t-t^*} \ll 1,
\end{align*}
for some $\beta>0$.
%
Replacing this expression in~\eqref{eq:odeSeparatrix} and comparing orders we see that this case is not possible.

Thus, we proceed to prove that $\La_h(t)$ has no singularities in $\ol{\Pi_A} \setminus \claus{\pm iA}$. Let us assume it has. That is, there exists $t^* \in \ol{\Pi_A} \setminus \claus{\pm iA}$ such that $\La_h(t)$ is singular at $t=t^*$. Note that Theorem \ref{theorem:singularitiesChangeq} implies that $q(t)$ and $\dot q(t)$  are analytic in a neighborhood of $t^* \in \ol{\Pi_A} \setminus \claus{\pm iA}$.

\begin{enumerate}
	\item If $q^2(t^*)\neq 1$, $1/(1-q^2(t))$ is analytic for $0<\vabs{t-t^*} \ll 1$. Since $\dot q(t)$ is also analytic in this neighborhood, \eqref{proof:LahSquared} implies that $\La^2_h(t)$ has no singularity at $t=t^*$ and we reach a contradiction.
% 	if an only if $\dot{q}^2(t)$ does.
% 	equation~\eqref{proof:LahSquared}, we have
% 	\begin{align*}
% 		\La^2_h(t) \approx C \qd^2(t),  \quad
% 		\text{ for } 0<\vabs{t-t^*} \ll 1.
% 	\end{align*}
% 	However, by Theorem~\ref{theorem:singularitiesChangeq} this is not possible
% 	, $\qd^2(t)$ has no singularities in $\ol{\Pi_A} \setminus \claus{\pm iA}$ and, as a result, neither does $\La^2_h(t)$ nor $\La_h(t)$. 
	%
% and we have a contradiction.
	
	\item If $q^2(t^*)=1$, by \eqref{eq:odeSeparatrixQ} and~\eqref{proof:LahSquared}, we deduce that
	\begin{align}\label{eq:equationLahSimplified}
		\La_h^2 = \frac{4}{3 q} (1-q)(q-a_+)(q-a_-).
	\end{align}
	Since by Theorem~\ref{theorem:singularitiesChangeq} $q$ is analytic in $\ol{\Pi_A} \setminus \claus{\pm iA}$, then $\La^2_h$ must be as well. 
% 	As a result, $\La_h$ does not have singularities in this region.  
\end{enumerate}
%
Finally, we notice that, by  equations~\eqref{eq:expressionqSingularities} and~\eqref{proof:LahSquared}, we have
\begin{align*}
\La_h^2(t) = \frac{4}{9}\al^2_{\pm} (t\mp iA)^{-\frac{2}{3}} + \OO(1), \quad
\text{ when } 0<\vabs{t\mp iA} \ll 1.
\end{align*}
Therefore, $\La_h(t)$ has branching points of order $-\frac{1}{3}$ in $t=\pm iA$.
%
Moreover, integrating the expression for $\La_h(t)$ and 
applying that $q(t)=\cos (\frac{\la_h(t)}{2})$ (and \eqref{eq:expressionqSingularities}), it is immediate to see that $\la_h(t)$ has branching points of order $\frac{2}{3}$ at $t=\pm iA$ and can be expressed as in~\eqref{eq:homoclinicaSingularities} close to $t=\pm iA$.
\end{proof}

We devote Sections \ref{subsection:classificationSingularities} and \ref{subsection:computationSingularities} to prove Theorem~\ref{theorem:singularitiesChangeq}. 
%
The statements~\eqref{eq:basicsAboutq} and~\eqref{eq:odeSeparatrixQ} are straightforward by applying the change of coordinates $q=\cos(\frac{\la}{2})$ to equation~\eqref{eq:odeSeparatrix}. 

We divide the rest of the proof of Theorem~\ref{theorem:singularitiesChangeq} into two parts. 
%
In Section~\ref{subsection:classificationSingularities} we classify the singularities of $q(t)$ and introduce a way to compute them using integration in complex paths. 
%
Finally, in Section~\ref{subsection:computationSingularities} we prove that the singularities of $q(t)$ with smallest imaginary part are $t=\pm iA$ and are branching points of order $\frac{2}{3}$.


==> Article Inner/proofB-poincareFormulas.tex <==
This section is devoted to prove Proposition~\ref{proposition:innerDerivation}. That  is we perform the suitable changes of coordinates, described in Section \ref{subsection:innerDerivation}, to Hamiltonian $H$ obtained in Theorem~\ref{theorem:HamiltonianScaling} (see~\eqref{def:hamiltonianScaling}) to obtain the inner Hamiltonian $\mathcal{H}$.
%
% To this end, we need to apply the changes of coordinates introduced in Section~\ref{subsection:reformulation} to the Hamiltonian $H$ obtained in Theorem~\ref{theorem:HamiltonianScaling} (see~\eqref{def:hamiltonianScaling}).
%
%To this end, we need to analyze the changes of coordinates introduced in Sections~\ref{subsection:reformulation} and \ref{subsection:innerDerivation} 
%that are applied to Hamiltonian~\eqref{def:hamiltonianPolars}.
%%
%These changes lead to the Hamiltonian $H^{\Inn}=\HH + H^{\Inn}_1$ where $H^{\Inn}_1 = \OO(\de^{\frac{4}{3}})$.
%%
%Note that, since the Poincar\'e change of coordinates $\phi_{\Poi}$, as defined in~\eqref{def:changePoincare},
%is not explicit, neither is $H_1^{\Poi}$, (see~\eqref{def:hamiltonianPoincareSplitting}).
%
However, recall  that the Hamiltonian $H$ is defined by means of $H_1^{\Poi}$ (see~\eqref{def:hamiltonianPoincareSplitting}) which does not have a closed form.
%
For this reason, a preliminary step to to prove Proposition~\ref{proposition:innerDerivation} is to provide suitable expansions for $H_1^{\Poi}$ in an appropriate domain. This is done in  Section~\ref{subsection:proofB-poincareFormulas}.
%
Then, in Section~\ref{subsection:proofC-innerDerivation}, we apply the changes of coordinates introduced in Section~\ref{subsection:innerDerivation} to conclude the proof of the proposition.

\subsection{The Hamiltonian in Poincar\'e variables}
\label{subsection:proofB-poincareFormulas}

%First, we give some classical formulas for the Poincar\'e planar elements.
%and we analyze the Hamiltonian $H_1^{\Poi}$ (given in~\eqref{def:hamiltonianPoincareSplitting}) on an appropiate domain, (see Lemma~\ref{lemma:seriesH1Poi} below).

%%%  POINCARE ELEMENTS FORMULAE %%%

First, we give some formulae to translate the Delaunay variables and other orbital elements into Poincar\'e coordinates (see \eqref{def:changePoincare}). %We apply this set of coordinates, as defined in~\eqref{def:changePoincare}, without mentioning it throughout this section.
\begin{itemize}
	\item[--] \textbf{Eccentricity $e$} (see~\eqref{def:eccentricityDelaunay}):
	It can be written as
	\begin{equation}\label{eq:ePoincare}
	e = 2 \, \tilde{e}(L,\eta,\xi) \sqrt{\eta \xi}, 
	\quad \text{where} \quad
	\tilde{e}(L,\eta,\xi) = \frac{\sqrt{2L-\eta\xi}}{2L}
	= \frac{1}{\sqrt{2L}} + \OO(\eta \xi).
	\end{equation}
%	where
%	\begin{equation}\label{eq:eResta}
%	\tilde{e}(L,\eta,\xi) = \frac{\sqrt{2L-\eta\xi}}{2L}
%	= \frac{1}{\sqrt{2L}} + \OO(\eta \xi).
%	\end{equation}
	Notice that $\tl{e}$ is analytic for $(L,\eta,\xi)\sim(1,0,0)$\footnote{
	This expansion is valid as long as $L\neq 0$.	
	%
	However, since our analysis focuses on $L \sim 1$, to simplify notation we use this more restrictive domain.}.
	%
%	To avoid cumbersome notation, we omit the dependence of the function $\tl{e}$ on its corresponding variables. 
	%
	\item[--] \textbf{Argument of the perihelion $g$:} From the expression of $\eta$ and $\xi$ in \eqref{def:changePoincare2},
	\begin{equation}\label{eq:gTrigPoincare}
	\cos g = \frac{\eta + \xi}{2 \sqrt{\eta \xi}}, \qquad
	\sin g = -i \frac{\eta - \xi}{2 \sqrt{\eta \xi}}. 
	\end{equation}
	%
	\item[--] \textbf{Mean anomaly $\ell$:}
	Since $\la=\ell+g$, we have that 
	\begin{equation*}
	\cos \ell = \frac{1}{2 \sqrt{\eta \xi}} \left( e^{-i \la} \eta + e^{i \la} \xi  \right), \qquad
	\sin \ell = \frac{i}{2 \sqrt{\eta \xi}} \left( e^{-i \la} \eta - e^{i \la} \xi  \right).
	\end{equation*}
	These expressions are not analytic at $(\eta,\xi)=(0,0)$. However, by~\eqref{eq:ePoincare},
	\begin{equation}\label{eq:eTriglPoincare}
	\begin{split}
	e\cos \ell = \tl{e}(L,\eta,\xi)\left( e^{-i \la} \eta + e^{i \la} \xi  \right), \quad
	e\sin \ell = i \tl{e}(L,\eta,\xi) \left( e^{-i \la} \eta - e^{i \la} \xi  \right),
	\end{split}
	\end{equation}
	are analytic for $(L,\eta,\xi) \sim (1,0,0)$.
	%
	\item[--] \textbf{Eccentric anomaly $u$:}
	It can be implicitly defined by $u=\ell+e\sin u$ (see~\eqref{eq:uImplicitDefinition}),
	which implies
	\begin{align*}\label{eq:uSeriesDefinition}
	u = \ell + e\sin \ell + e^2 \cos\ell\sin\ell + 
	\OO(e\sin\ell,e\cos\ell)^3.
	\end{align*}
	Then, by~\eqref{eq:ePoincare} and \eqref{eq:eTriglPoincare},
	\begin{equation}\label{eq:trigoU}
	\begin{split}
	&e\cos u = \frac{1}{\sqrt{2L}}
	\paren{e^{-i\la}\eta+e^{i\la}\xi} 
	+ \frac{1}{2L} \paren{e^{-i\la}\eta-e^{i\la}\xi}^2 
	+ \OO(e^{-i\la}\eta,e^{i\la}\xi)^3, \\
	&e\sin u = 
	\frac{i}{\sqrt{2L}} \paren{e^{-i\la}\eta-e^{i\la}\xi}
	+\frac{i}{2L} \paren{e^{-2i\la}\eta^2-e^{2i\la}\xi^2} 
	+\OO(e^{-i\la}\eta,e^{i\la}\xi)^3,
	\end{split}
	\end{equation}
	which are also analytic for $(L,\eta,\xi)\sim(1,0,0)$.
\end{itemize}
%
For any  $\zeta \in [-1,1]$,  we define the function
\begin{equation}\label{def:functionD}
D[\zeta] = 
\paren{r^2 -2\zeta r\cos\tht + \zeta^2}
\circ \phi_{\Poi}.
\end{equation}
By the definition of $\mu H_1^{\Poi}$ in~\eqref{def:hamiltonianPoincareSplitting}, we have that
\begin{equation}\label{eq:decompositionH1PoiA}
\mu H_1^{\Poi} = \frac{1}{\sqrt{D[0]}} -\frac{1-\mu}{\sqrt{D[\mu]}}
-\frac{\mu}{\sqrt{D[\mu-1]}}.
\end{equation}
%Thus, we introduce a series expression of function $D[\zeta]$ on an appropriate domain.

\begin{lemma}\label{lemma:seriesH1Poi}
	For $\vabs{(L-1,\eta, \xi)} \ll 1$ and any  $\zeta \in [-1,1]$, one can split $D[\zeta]$ as 
	\begin{align*}
		D[\zeta] =  D_0[\zeta] + D_1[\zeta] + D_2[\zeta] + D_{\geq 3}[\zeta],
	\end{align*}
	where 
	\begin{align*}%\label{def:D0}
	D_0[\zeta](\la,L) =& \, 
	L^4 - 2\zeta L^2 \cos \la  +\zeta^2,  \\
	%%%
	\begin{split}%\label{def:D1}
	D_1[\zeta](\la,L,\eta,\xi) =& \,
	\eta  \frac{\sqrt{2 L^3}}{2}
	\paren{3 \zeta - 2 L^2 e^{-i\la}  -
		\zeta e^{-2i\la}} \\
	%
	&+ \xi  \frac{\sqrt{2 L^3}}{2}
	\paren{3 \zeta - 2 L^2 e^{i\la}   -  \zeta e^{2 i\la}}, 
	\end{split} \\
	%
	\begin{split}%\label{def:D2}
	D_2[\zeta](\la,L,\xi,\eta) =& \,
	- {\eta^2}  \frac{L e^{-i\la}}{4}  \paren{
	\zeta + 2 L^2 e^{-i\la}  + 3 \zeta e^{-2 i\la} } 
	\\
	&- {\xi^2} \frac{L e^{i\la}}{4} \paren{\zeta +
	2 L^2 e^{i\la}  + 3 \zeta e^{2 i\la} }
+\eta \xi L \paren{
	3L^2 + 2\zeta\cos \la}.
	\end{split}
	\end{align*}
	Fix $\varrho\geq 0$.
	%
	Then, for $\vabs{\Im \la}\leq \varrho$, the function
	$D_{\geq 3}[\zeta]$ is analytic and satisfies
	\begin{equation}\label{eq:boundD3mes}
	\vabs{D_{\geq 3}[\zeta](\la,L,\eta,\xi)} \leq 
	C \vabs{(\eta,\xi)}^3,
	\end{equation}
	 with $C=C(\varrho)$ a positive constant independent of $\zeta \in [-1,1]$.
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lemma:seriesH1Poi}]
In view of the definition of $D[\zeta]$ in \eqref{def:functionD}, we look for expansions for $r^2$ and $r\cos \tht$ (expressed in Poincar\'e coordinates) in powers of $(\eta,\xi)$.

Let us consider first $r^2$. 
%
Taking into account that $r=L^2(1-e\cos u)$ (see \eqref{eq:rthetaDefinition}) and the expansions in~\eqref{eq:trigoU} we obtain
%\begin{align*}
%r^2 %&= L^4 \claus{ 1-2e\cos u+e^2\cos^2 u} \\ 
%&= L^4 \claus{1 - 2e\cos\ell 
%+ e^2 + e^2 \sin^2\ell + 
%\OO(e\sin\ell,e\cos\ell)^3}.
%\end{align*}
%Since $e\cos\ell$ and $e\sin\ell$ are analytic when $(L,\eta,\xi) \sim (1,0,0)$, the terms of this series are too. Thus, using~\eqref{eq:ePoincare} and~\eqref{eq:eTriglPoincare} we obtain
%\begin{align*}
%r^2 = L^4 &\left\{
%1 - 
%\sqrt{\frac{2}{L}} \paren{e^{-i\la}\eta + e^{i\la} \xi}
%+ \frac{2}{L} \eta \xi 
%\right. \\ &\left. 
%- \frac{1}{2L} \paren{e^{-2i\la}\eta^2 + e^{2i\la} \xi^2 - 2 \eta \xi}
%+ \OO(\eta,\xi)^3 \right\} 
%\end{align*}
%and
\begin{equation}\label{proof:r2Poincare}
\begin{split}
r^2 =& \, L^4 
-L^3 \sqrt{2L} e^{-i\la} \eta
- L^3 \sqrt{2L} e^{i\la}\xi
+ 3 L^3\eta \xi   \\
&- \frac{L^3}{2} e^{-2i\la}\eta^2
- \frac{L^3}{2} e^{2i\la} \xi^2
+\OO(e^{-i\la}\eta, e^{i\la}\xi)^3.
\end{split}
\end{equation}
%This expression is analytic for $(L,\eta,\xi)\sim(1,0,0)$ and, since $\vabs{\Im \la} \leq \varrho$, the terms of order $3$ and higher satisfy estimate \eqref{eq:boundD3mes}.
%
%Now, we consider the term $r\cos \tht$. First, we introduce an expression for the trigonometrics of the true anomaly
%\begin{equation*}
%%\label{eq:trigfDefinition}
%\begin{split}
%\cos f=\frac{\cos u-e}{1-e\cos u}, \hh %\label{eq:cosfDefinition}\\
%\sin f=\frac{\sqrt{1-e^2}\sin u}{1-e\cos u}.
%\end{split}
%\end{equation*}
%
Now, we compute an expansion for $r\cos \tht$.
%
Taking into account \eqref{eq:thetaDefinition} and \eqref{eq:fTrigDefinition},
\begin{align*}
r \cos \tht
&= L^2 \paren{ \cos(g+u) - e\cos g - \left(\sqrt{1-e^2}-1\right)\sin u\sin g }.
\end{align*}
Notice that, since $\la=\ell+g$ and $u=\ell+e\sin u$, we have that $\cos(g+u) = \cos(\la+e\sin u)$ is analytic at $(\eta,\xi)=(0,0)$.
%
Then, using \eqref{eq:ePoincare},
\eqref{eq:gTrigPoincare} and \eqref{eq:trigoU},
we deduce
%
%Considering $\la=\ell+g$ and $e=2\tl{e}\sqrt{\eta \xi}$ (see~\eqref{eq:ePoincare}), we have that
%\begin{align*}
%r\cos \tht 
%&= L^2 \left\{ \cos(\la +u - \ell) - e\cos g + \frac{\eta \xi}{L}\sin u\sin g \right\},
%\end{align*}
%	Moreover, considering~\eqref{eq:uImplicitDefinition}, we have
%	\begin{align*}
%	r\cos \tht 
%	&= L^2 \left\{ \cos \la \cos(e\sin u) 
%	-\sin \la  \sin(e\sin u)
%	- e\cos g 
%	+ \frac{\eta \xi}{L}\sin u\sin g \right\},
%	\end{align*}
%and taking into account $u=\ell+e\sin u$ (see~\eqref{eq:uImplicitDefinition}), \eqref{eq:ePoincare} and~\eqref{eq:gTrigPoincare}  we obtain
%\begin{equation*}%\label{eq:rcosthtPoincare}
%\begin{split}
%r\cos \tht 
%= L^2 &\left\{ \cos \la \cos(e\sin u) 
%-\sin \la  \sin(e\sin u) %\right. \\ &\left.
%- \tl{e}(\eta+\xi) 
%- \frac{i(\eta-\xi)}{4\tl{e}L} e\sin u \right\}.
%\end{split}
%\end{equation*}
%%% AAAAAA
%Then, using again~\eqref{eq:ePoincare}, \eqref{eq:eTriglPoincare} and
%the trigonometric expressions in~\eqref{eq:trigoU} we finally obtain
%\begin{align*}
%r\cos \tht 
%= L^2 &\left\{
%\cos \la  -\tl{e}(\eta+\xi)
%-e\sin\ell\paren{\sin \la +\frac{i}{4\tl{e}L}(\eta-\xi)}
%\right. \\ &\left.
%-e^2\sin^2\ell\paren{\frac{1}{2}\cos \la } 
%-e^2\cos\ell\sin\ell
%\paren{\sin \la +\frac{i}{4\tl{e}L}(\eta-\xi)}
%\right. \\ &\left.
%+ \OO(e\sin\ell,e\cos\ell)^3
%\right\}.
%\end{align*}
%\begin{align*}
%r\cos \tht &= L^2 \cos \la  
%%
%-\sqrt{\frac{L}{2}}(\eta+\xi)
%%
%-i L \sqrt{\frac{L}{2}}\sin \la 
%\paren{e^{-i\la}\eta - e^{i\la}\xi} \\
%%
%&+ \frac{L}{4}
%\paren{e^{-i\la}\eta^2 + e^{i\la}\xi^2 - 2\cos \la \eta\xi} 
%%
%+ \frac{L}{4}\cos \la 
%\paren{e^{-2i\la}\eta^2 + e^{2i\la}\xi^2 - 2\eta\xi} \\
%%
%&- i\frac{L}{2} \sin \la 
%\paren{e^{-2i\la}\eta^2 - e^{2i\la}\xi^2}
%%
%+ \OO(\eta,\xi)^3,
%\end{align*}
%and
\begin{equation}\label{proof:rcosPoincare}
\begin{split}
r\cos \tht =& \,  L^2 \cos \la  
%
- \eta \frac{\sqrt{2 L^3}}{2} \paren{1
+ i e^{-i\la} \sin \la  } 
%
- \xi  \frac{\sqrt{2 L^3}}{2} \paren{ 1 - i e^{i\la} \sin \la  } \\
%
&- \eta \xi {L\cos \la }
%
+ \frac{L}{4} \eta^2 \paren{e^{-i\la} 
+ e^{-2i\la} \cos \la 
-2 i e^{-2i\la} \sin \la } \\ 
%
&+ \xi^2 \frac{L}{4} \paren{e^{i\la}+
 e^{2i\la} \cos \la
+2i e^{2i\la} \sin \la }
%
+ \OO(e^{i\la}\eta, e^{-i\la}\xi)^3.
\end{split}
\end{equation}
Then, joininig the results in~\eqref{proof:r2Poincare} and~\eqref{proof:rcosPoincare}
with the definition of $D[\zeta]$ in~\eqref{def:functionD}, we obtain its expansion in $(\eta,\xi)$.
%
Moreover, since $D[\zeta]$ is analytic for $(L,\eta,\xi)\sim(1,0,0)$ and $\vabs{\Im \la} \leq \varrho$, the terms of order $3$  satisfy the estimate in \eqref{eq:boundD3mes}.
\end{proof}

\begin{remark}\label{remark:seriesH1Poi}
Observe that the Hamiltonian $H^{\Poi} = H_0^{\Poi}+\mu H_1^{\Poi}$ in~\eqref{def:hamiltonianPoincareSplitting} is analytic away from collision with the primaries.	
%
By the decomposition of $\mu H_1^{\Poi}$ in~\eqref{eq:decompositionH1PoiA}, collisions with the primary $S$ are given by the zeroes of the function $D[\mu]$ and collisions with $P$ are given by the zeroes of $D[\mu-1]$.

Since our analysis is performed for $\vabs{(L-1,\eta,\xi)}\leq \e \ll 1$ and $0<\mu\ll 1$, 
%
by Lemma~\ref{lemma:seriesH1Poi}, one has
% we have that
\begin{align*}
	D[\mu] = 1 + \OO(\mu,\e), \qquad
	D[\mu-1] = 2 + 2\cos \la + \OO(\mu,\e).
%	\quad \text{when } \mu,\e \to 0.
\end{align*}
That is, collisions with $S$ are not possible whereas  collisions with $P$ may take place when $\la \sim \pi$.
\end{remark}

%To prove the analyticity of $H^{\Poi}$ (see~\eqref{def:hamiltonianPoincare}), by Lemma~\ref{lemma:seriesH1Poi} and~\eqref{eq:decompositionH1PoiA}, it is necessary to check that the denominators $D[0], D[\mu], D[\mu-1] \neq 0$, which corresponds with the points not at collision with the primaries.
%%
%Indeed, for $\mu, \e>0$ small enough such that $\vabs{(L-1,\eta,\xi)}<\e$,
%by Lemma~\ref{lemma:seriesH1Poi}, we have
%\begin{align*}
%	D[0] = 1 + \OO(\e), \quad
%	D[\mu] = 1 + \OO(\mu,\e), \quad
%	D[\mu-1] = 2 + 2\cos(\la) + \OO(\mu,\e).
%\end{align*}
%Therefore, $\mu H_1^{\Poi}$ is analytic when $\vabs{\la - \pi} \not\sim 0$. 
%%
%However, a complete region of analyticity for this Hamiltonian is not straightforward to define.
%%
%Thus, on this work and~\cite{?},
%to ensure that $\mu H_1^{\Poi}$ is analytic, we use the results on Lemma~\ref{lemma:seriesH1Poi} and check for each individual case that the denominators are not zero.
%
%
%On this work and~\cite{?}, to prove that $H^{\Poi}$ is analytic, we use mainly the results on Lemma~\ref{lemma:seriesH1Poi} and check for each individual case that the denominators $D[0], D[\mu]$ and $D[\mu-1]$ do not approach zero .


%\begin{corollary}\label{corollary:HPoiAnalytic}
%Fix $\varrho \geq 0$.
%%
%There exists $\mu_0 > 0$, 
%such that for $\mu \in (0,\mu_0)$ 
%there exists $\e_0=\e_0(\mu)>0$,
%such that for $\e \in (0,\e_0)$	
%%
%the Hamiltonian 
%$\mu H_1^{\Poi}(\la,L,\eta,\xi;\mu)$ is analytic
%for 
%$\vabs{(L-1,\eta,\xi)}<\e$,
%$\vabs{\Im \la} \leq \varrho$ and
%$\vabs{\la-\pi}>\cttInnPoiA$,
%%
%where $\cttInnPoiA=\cttInnPoiA(\e,\mu)$ is a positive constant.
%\end{corollary}
%\begin{proof}
%To prove the analyticity of $\mu H_1^{\Poi}$, by Lemma~\ref{lemma:seriesH1Poi} and~\eqref{eq:decompositionH1PoiA}, it only remains to see that the denominators $D[0], D[\mu], D[\mu-1]$ are far from zero.
%%
%Indeed, since $\vabs{\Im \la} \leq \varrho$, for $\mu$ small enough we have
%\begin{align*}
%	D[0] = 1 + \OO(\e), \quad
%	D[\mu] = 1 + \OO(\mu,\e), \quad
%	D[\mu-1] = 2 + 2\cos(\la) + \OO(\mu,\e).
%\end{align*}
%Therefore, to confirm the analyticity of $\mu H_1^{\Poi}$ we require $\vabs{\la - \pi} \not\sim 0$, for $\mu$ and $\e$ small enough.
%\end{proof}
%
%On Corollary~\ref{corollary:HPoiAnalytic} we introduce a region of analyticity for the Hamiltonian $H^{\Poi}$ (as given in~\eqref{def:hamiltonianPoincare}).
%%
%However, this region can be difficult to compute.
%%
%On this work and~\cite{?}, to prove that $H^{\Poi}$ is analytic, we use mainly the results on Lemma~\ref{lemma:seriesH1Poi} and check for each individual case that the denominators $D[0], D[\mu]$ and $D[\mu-1]$ do not approach zero (collision with the primaries).





==> Article Inner/proofC-innerDerivation.tex <==
\subsection{Proof of Proposition~\ref{proposition:innerDerivation}}
\label{subsection:proofC-innerDerivation}

To prove Proposition~\ref{proposition:innerDerivation}, we  analyze the Hamiltonian $H^{\Inner}$ which is given (up to a constant) by
\begin{equation*}%\label{proof:hamiltonianInnerA}
% H^{\Inner} = 
\frac{\de^{\frac{4}{3}}}{2 \al_+^2}
\paren{H \circ \phi_{\equi} \circ \phi_{\out} \circ \phi_{\inn}},
\end{equation*}
% where $c=c(\de)$ only depends on $\de$, 
where the changes $\phi_{\equi}$, $\phi_{\out}$ and $\phi_{\inn}$ are defined in~\eqref{def:changeEqui}, \eqref{def:changeOuter} and \eqref{def:changeInner}, and $H=H_0+H_1$ (see \eqref{def:hamiltonianScalingH0} and $H_1$ in~\eqref{def:hamiltonianScalingH1}).

In the rest of the section, when performing changes of coordinates, to simplify notation, we omit the constant terms in the Hamiltonians.
% iterms that are constant or only depending on $\de$ in the equivalences between Hamiltonians.

%The first step is to obtain an expansion of the Hamiltonian $H_1$ with respect to $(x,y)$. 
%
Using the formulas for $H_1^{\Poi}$ in~\eqref{eq:decompositionH1PoiA} and Lemma~\ref{lemma:seriesH1Poi},  
% to analyze $H^{\inn}$.
%
% First, 
we split $H_1^{\Poi}$ into two terms: one for the perturbation coming from the massive primary ($S$) and the other coming from the small primary ($P$),
\begin{align*}
H_1^{\Poi} = H_1^{\Poi,S} + H_1^{\Poi, P},
\end{align*}
which,  recalling that
$\mu = \de^4$, are defined as
\begin{equation}\label{proof:splitH1Poi}
\begin{split}
H_{1}^{\Poi, S} = \frac{1}{\de^4}
\paren{\frac{1}{\sqrt{D[0]}} -\frac{1-\de^4}{ \sqrt{D[\de^4]}}} 
%
\quad \text{ and } \quad
%
H_{1}^{\Poi, P} = - \frac{1}{\sqrt{D[\de^4-1]}}.
\end{split}
\end{equation}
%Accordingly, we split $V$ (see~\eqref{def:potentialV}) as $V=V^S+V^P$ with
%\begin{equation}\label{proof:potentialsSJ}
%	\begin{split}
%	&V^S(\la) = 
%	H_1^{\Poi,S}(\la,1,0,0;0) = 1- \cos \la , \\
%	&V^P(\la) = H_1^{\Poi,P}(\la,1,0,0;0) = -\frac{1}{\sqrt{2+2\cos \la }}.
%	\end{split}
%\end{equation}
%
We also define the Hamiltonian $H^{\equi} = H \circ \phi_{\equi}$, which can be split as
\begin{equation*}%\label{proof:Hequi}
	H^{\equi} = H_{0} + R^{\equi} 
	+ H_1^{\equi,P} + H_1^{\equi,S},
\end{equation*}
with
\begin{equation}\label{proof:H1Requi}
\begin{split}
H_1^{\equi, *}(\la,\La,x,y;\de) =& \,
H_1^{\Poi,*}\circ \phi_{\sca} \circ \phi_{\equi},
\qquad \text{for } {*}=S,P,\\
%
R^{\equi}(\la,\La,x,y;\de) =& 
- V(\la)
+ \frac{1}{\de^4} 
F_{\pend}(\de^2\La + \de^4\LtresLa(\de)) \\
&- 3 \de^2 \La \LtresLa(\de) 
+ \de (x \Ltresy(\de) + y \Ltresx(\de)).
\end{split}
\end{equation}
We recall that  $\phi_{\sca}$ is the scaling given in~\eqref{def:changeScaling}, $V$ is the potential  in~\eqref{def:potentialV},
$F_{\pend}$  is the function ~\eqref{def:Fpend} and
$(\LtresLa,\Ltresx,\Ltresy)$ are introduced in~\eqref{def:pointL3sca}. 

Then, the Hamiltonian $H^{\inn}$ can be written as 
\begin{align}\label{proof:hamiltonianInnerB}
H^{\inn} 
= \frac{\de^{\frac{4}{3}}}{2\al_+^2} 
\paren{
H_0 \circ \Psi
+ R^{\equi} \circ \Psi
+ H_1^{\Poi,P}\circ\Phi 
+ H_1^{\Poi,S}\circ\Phi},
\end{align}
where
\begin{equation*}%\label{proof:changeCoordinatesPhiPsi}
\Psi = \phi_{\out} \circ \phi_{\inn} 
\quad \text{ and } \quad
\Phi = \phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out} \circ \phi_{\Inner}.
\end{equation*}
% Therefore, 
% by \eqref{proof:hamiltonianInnerA} and
% \eqref{proof:H1Requi},
% to prove Proposition~\ref{proposition:innerDerivation}
% we need to compute
% \begin{align}\label{proof:hamiltonianInnerB}
% H^{\inn} 
% = \frac{\de^{\frac{4}{3}}}{2\al_+^2} 
% \paren{
% H_0 \circ \Psi
% + R^{\equi} \circ \Psi
% + H_1^{\Poi,P}\circ\Phi 
% + H_1^{\Poi,S}\circ\Phi}.
% \end{align}
In the following lemmas, we introduce expressions for the changes $\Psi$ and $\Phi$.
% (see~\eqref{proof:changeCoordinatesPhiPsi}).
%

\begin{lemma}\label{lemma:PsiMultipleChanges}
The change of coordinates $\Psi=(\Psi_{\la},\Psi_{\La},\Psi_x,\Psi_y)$	
satisfies
\begin{align*}%\label{proof:changePsi}
\Psi_{\la}(U) &= 
\pi + 3\al_+ \de^{\frac{4}{3}} U^{\frac{2}{3}}
\paren{ 1 + g_{\la}(\de^2 U)}, \\
%%%
\Psi_{\La}(U,W) &= 
-\frac{2\al_+}{3 \de^{\frac{2}{3}} U^{\frac{1}{3}} } 
\paren{ 1 + g_{\La}(\de^2 U)}
%
+ \frac{\al_+ U^{\frac{1}{3}} W}{\de^{\frac{2}{3}}} 
\paren{1+\wt{g}_{\La}(\de^2 U)}, \\
%%%
\Psi_x(X) &= \de^{\frac{1}{3}} \sqrt{2} \al_+ X, 
\\
\Psi_y(Y) &= \de^{\frac{1}{3}} \sqrt{2} \al_+ Y,
\end{align*}
where $g_{\la}(z)$, $g_{\La}(z)$, $\wt{g}_{\La}(z) \sim \OO(z^{\frac{2}{3}})$. 
%
Moreover, taking into account the time-parametrization of the separatrix $(\la_h,\La_h)$ given in~\eqref{eq:separatrixParametrization}, we have that
\begin{equation}\label{proof:separatrixInner}
\begin{split}
\La_h \circ \phi_{\Inner} =
-\frac{2\al_+}{3 \de^{\frac{2}{3}} U^{\frac{1}{3}}}
\paren{ 1 + g_{\La}(\de^2 U)}.
\end{split}
\end{equation}
\end{lemma}

\begin{lemma}\label{lemma:PhiMultipleChanges}
The change of coordinates
$\Phi=  (\Phi_{\la},\Phi_{L},\Phi_{\eta},\Phi_{\xi})$ satisfies
\begin{align*}
\Phi_{\la}(U)&=\Psi_{\la}(U), \quad &
%
\Phi_{L}(U,W) &= 1+\de^2\Psi_{\La}(U,W) + \de^4 \LtresLa(\de), \\
\Phi_{\eta}(X) &= \de \Psi_{x}(X) + \de^4 \Ltresx(\de),
\quad &
\Phi_{\xi}(Y) &= \de \Psi_{y}(Y) + \de^4 \Ltresy(\de),
\end{align*}
where $\Psi=(\Psi_{\la},\Psi_{\La},\Psi_x,\Psi_y)$ is the change of coordinates given in Lemma~\ref{lemma:PsiMultipleChanges}.
\end{lemma}
We omit the proofs of these lemmas  since they  are a straightforward consequence of  Theorem~\ref{theorem:singularities} and the definitions of the changes of coordinates (see \eqref{def:changeScaling}, \eqref{def:changeEqui}, \eqref{def:changeOuter} and \eqref{def:changeInner}).


% Using the formulas provided by these lemmas, one can prove Proposition~\ref{proposition:innerDerivation}.

%%%%%%%
%We apply now the change of coordinates 
%\begin{align*}
%\paren{\phi_{\out}\circ\phi_{\inn} }(U,W,X,Y) 
%= &\left( \la_h(\de^2 U + iA), 
%\h
%\La_h(\de^2 U + iA) - \frac{2 \al^2_+ }{\de^{\frac{4}{3}} 3 \La_h(\de^2 U + iA)}W, \h 
%\right. \\ &\left. \hh
%\de^{\frac{1}{3}} \sqrt{2} \al_+ X, \h
%\de^{\frac{1}{3}} \sqrt{2} \al_+ Y \right),
%\end{align*}
%as defined on~\eqref{def:changeOuter} and~\eqref{def:changeInner}, to  Hamiltonian $H^{\equi}$. 
%%
%Previously, using Theorem~\ref{theorem:singularities}, we have an expression of the parametrization of the separatrix $(\la_h(u),\La_h(u))$ in the inner coordinates
%\begin{equation}\label{proof:separatrixInner}
%\begin{split}
%\la_h(\de^2 U + iA) = 
%\pi + 3\al_+ \de^{\frac{4}{3}} U^{\frac{2}{3}}\left( 1 + g_{\la_h}(\de^2 U)\right), \\
%%
%\La_h(\de^2 U + iA) =
%-\frac{2\al_+}{3} \de^{-\frac{2}{3}} U^{-\frac{1}{3}}\left( 1 + 
%g_{\La_h}(\de^2 U)\right),
%\end{split}
%\end{equation}
%where $g_{\la_h}(x), g_{\La_h}(x) \sim \OO(x^{\frac{2}{3}})$. 
%
%Notice that, since $\vabs{U} \leq \cttInnDerA$, we have $\vabs{g_{\la_h}(\de^2 U)} \leq C(\cttInnDerA)\de^{\frac{4}{3}}$, where $C(\cttInnDerA)$ is a positive constant depending on a power of $\cttInnDerA$.
%
%Analogously, for $\vabs{g_{\La_h}(\de^2 U)}$. 

\begin{proof}[End of the proof of Proposition~\ref{proposition:innerDerivation}]
%
We analyze each component of \eqref{proof:hamiltonianInnerB}.

We denote by $C(\cttInnDerA,\cttInnDerB)>0$ any constant satisfying that there exist
$\cttInnDerC, \cttInnDerAA, \cttInnDerBB>0$
independent of $\cttInnDerA, \cttInnDerB, \de$ such that $C(\cttInnDerA, \cttInnDerB) \leq \cttInnDerC \cttInnDerA^{\cttInnDerAA} \cttInnDerB^{\cttInnDerBB}$.
\begin{enumerate}
	\item We compute the first term of the Hamiltonian $H^{\inn}$ in~\eqref{proof:hamiltonianInnerB}.
	%
	Since $H_{\pend}(\la_h,\La_h)=H_{\pend}(0,0)= -\frac{1}{2}$
	 and taking into account~\eqref{proof:separatrixInner}, we have
\begin{equation*}%\label{proof:innerDerivationResultA}
\begin{split}	
\frac{\de^{\frac{4}{3}}}{2\al_+^2} 
H_0 \circ \Psi 
%
=& \frac{\de^{\frac{4}{3}}}{2\al_+^2} \paren{w -\frac{w^2}{6 \La_h^2(u)} + \frac{xy}{\de^2} } \circ \phi_{\inn}\\
%
=& \, W + XY - 
\frac{3}{4} U^{\frac{2}{3}}  W^2 \left(\frac{1}{1+g_{\La}(\de^2 U)} \right)^2 \\
%
=& \, W + XY - \frac{3}{4} U^{\frac{2}{3}}  W^2
+ \OO \paren{\de^{\frac{4}{3}} 
U^{\frac{2}{3}} W^2}.
\end{split}	
\end{equation*}	
Since $\vabs{U} \leq \cttInnDerA$ and $\vabs{W} \leq \cttInnDerB$, the error term $\OO (\de^{\frac{4}{3}} U^{\frac{2}{3}} W^2)$
 can be bounded by $C(\cttInnDerA,\cttInnDerB) \de^{\frac{4}{3}}$.

For the other terms in \eqref{proof:hamiltonianInnerB}, to simplify the notation, we are not specifying the dependence of the error terms on the variables $(U,W,X,Y)$.
%
Moreover, when referring to error terms of order $\OO(\de^{a})$, we mean that they can be bounded by $C(\cttInnDerA,\cttInnDerB)\de^{a}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item For the second term of the Hamiltonian $H^{\inn}$ in~\eqref{proof:hamiltonianInnerB} (see 
by~\eqref{proof:H1Requi}) we have 
\begin{equation}\label{proof:RequiChange}
\begin{split}
\frac{\de^{\frac{4}{3}}}{2\al_+^2}
R^{\equi} \circ \Psi
%
=& 
-\frac{\de^{\frac{4}{3}}}{2\al_+^2} V(\Psi_{\la})
+ \frac{1}{2\al_+^2\de^{\frac{8}{3}}} 
F_{\pend} \paren{
\de^2 \Psi_{\La} + \de^4 \LtresLa(\de)} \\
%
&- \frac{3 \de^{\frac{10}{3}} \LtresLa(\de)}{2 \al^2_+} \Psi_{\La}
%
+ \frac{\de^{\frac{7}{3}}\Ltresy(\de)}{\sqrt{2} \al_+} \Psi_x 
+ \frac{\de^{\frac{7}{3}}\Ltresx(\de)}{\sqrt{2} \al_+} \Psi_y,
\end{split}
\end{equation}
%\begin{align*}
%\frac{\de^{\frac{4}{3}}}{2\al_+^2}
%R^{\equi} \circ \Psi
%%
%=& \frac{1}{2\al_+^2\de^{\frac{8}{3}}} 
%F_{\pend} \paren{
%\de^2 \La_h(\de^2U + iA)
%-\frac{2 \al^2_+ \de^{\frac{2}{3}}}{3 \La_h(\de^2 U + iA)} W
%+ \de^4 \LtresLa} \\
%%
%&- \de^{\frac{10}{3}} \frac{3 \LtresLa}{2 \al^2_+} \La_h(\de^2 U + iA)
%+ \frac{ \de^{2} \LtresLa W}{ \La_h(\de^2 U + iA)} \\
%&+ \frac{\de^{\frac{8}{3}}}{\sqrt{2} \al_+} 
%\paren{\Ltresy X + \Ltresy Y},
%\end{align*}
where $F_{\pend}(z)=\OO(z^3)$ (see~\eqref{def:Fpend}) and $V(\la)$ is the potential given in \eqref{def:potentialV}.

First we analyze the potential term. 
%
By Lemma~\ref{lemma:PsiMultipleChanges}, we have that
\begin{align*}
-\frac{\de^{\frac{4}{3}}}{2\al_+^2} V(\Psi_{\la}(U))	
%
&= \frac{\de^{\frac{4}{3}}}{2\al_+^2 }
\frac{1}{\sqrt{2+2\cos \Psi_{\la}(U)}}
+ \OO(\de^{\frac{4}{3}}) \\
%
&= \frac{\de^{\frac{4}{3}}}{2\al_+^2 }
\paren{	9 \al^2_+ \de^{\frac{8}{3}} U^{\frac{4}{3}}\left( 1 + g_{\la}(\de^2 U)\right)^2 +
%
\OO\paren{\de^{\frac{16}{3}}U^{\frac{8}{3}}}}^{-\frac{1}{2}} 
+ \OO(\de^{\frac{4}{3}})
\\
&= \frac{1}{3 U^{\frac{2}{3}}} +
\OO(\de^{\frac{4}{3}}).
\end{align*}
Then, since $\cttInnDerA^{-1} \leq \vabs{U} \leq \cttInnDerA$ and $\vabs{(W,X,Y)} \leq \cttInnDerB$, by~\eqref{proof:RequiChange} and Lemma~\ref{lemma:PsiMultipleChanges}, 
\begin{align*}%\label{proof:innerDerivationResultB}
\vabs{\frac{\de^{\frac{4}{3}}}{2\al_+^2}
R^{\equi} \circ \Psi - \frac{1}{3 U^{\frac{2}{3}}}}
\leq
C(\cttInnDerA,\cttInnDerB){\de^{\frac{4}{3}}}.
\end{align*}
%where $C(\cttInnDerA, \cttInnDerB)$ is a positive constant depending on powers of $\cttInnDerA$ and $\cttInnDerB$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item We deal with the third term  of the Hamiltonian $H^{\inn}$ (see~\eqref{proof:splitH1Poi}).
%
%\begin{equation*}%\label{eq:PhiChange}
%\begin{split}
%&\la = \Phi_{\la}(U) = \pi + 3\al_+ \de^{\frac{4}{3}} U^{\frac{2}{3}}
%+ f_{\la}(U;\de),
%\\%[0.5em]
%%
%&L = \Phi_{L}(U,W) = 1 - 
%\al_+ \de^{\frac{4}{3}} \paren{\frac{2}{3} U^{-\frac{1}{3}} 
%	- U^{\frac{1}{3}} W} - f_L(U,W;\de), \\%[0.5em]
%&\eta = \Phi_{\eta}(X) = \sqrt{2}\al_+\de^{\frac{4}{3}} X
%+ f_{\eta}(\de), \\%[0.5em]
%&\xi = \Phi_{\xi}(Y) = \sqrt{2}\al_+ \de^{\frac{4}{3}} Y +
%f_{\xi}(\de),
%\end{split}
%\end{equation*}
%where
%\begin{align*}
%&f_{\la}(U;\de)= 3\al_+ \de^{\frac{4}{3}} U^{\frac{2}{3}}
%g_{\la_h}(\de^2 U) = \OO(\de^{\frac{8}{3}}), \\
%%
%&f_L(U,W;\de)= \al_+ \de^{\frac{4}{3}}\paren{
%	\frac{2}{3} U^{-\frac{1}{3}} g_{\La_h}(\de^2 U)
%	+ U^{\frac{1}{3}}W \frac{g_{\La_h}(\de^2U)}{1+g_{\La_h}(\de^2U)}}
%+ \de^{4} \LtresLa
%= \OO(\de^{\frac{8}{3}}) ,\\
%&f_{\eta}(\de)= \de^4 \Ltresx, \hh
%f_{\xi}(\de)= \de^4 \Ltresy,
%\end{align*} 
%We also have that
%\begin{align*}%\label{eq:PhiChangeLambda}
%\La= \frac{\Phi_L(U,W)-1}{\de^2} =  
%-\frac{\al_+}{\de^{\frac{2}{3}}}
%\paren{\frac{2}{3} U^{-\frac{1}{3}}- U^{\frac{1}{3}} W}
%- \frac{1}{\de^2}f_L(U,W;\de).
%\end{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Now, we compute $H^{\Poi, J}_1 \circ \Phi$, as introduced in equation~\eqref{proof:H1JderivationInner}.
Since
\[ \vabs{\Phi(U,W,X,Y)-(\pi,1,0,0)} 
\leq C(\cttInnDerA, \cttInnDerB) \de^{\frac{4}{3}}
\quad \text{and} \quad 
\vabs{\Im \Phi_{\la}(U)} \leq C(\cttInnDerA) \de^{\frac{4}{3}},
\]
the hypotheses of Lemma~\ref{lemma:seriesH1Poi} hold and therefore:
\begin{equation*}%\label{proof:innerDerivationResultDabans}
\begin{split}
\frac{ \de^{\frac{4}{3}}}{2\al_+^2 }
{H_1^{\Poi,P} \circ \Phi}
%
&= - \frac{\de^{\frac{4}{3}}}{2\al_+^2}
\frac{1}{\sqrt{D[\de^4-1] \circ \Phi }} \\
%
&= - \paren{ \frac{2 \al_+}{\de^{\frac{8}{3}}}	
\paren{D_0+D_1+D_2+D_{\geq 3}}[\de^4-1] \circ \Phi }^{-\frac{1}{2}}.
\end{split}
\end{equation*}
%
We compute every term $D_j[\de^4-1]$, $j=0,1,2, \geq3$.
%
%\paren{ P_0[\de^4-1]+P_1[\de^4-1]+P_2[\de^4-1]+P_3[\de^4-1]}
%where functions $D_i[\de^4-1]$ are defined on Lemma~\ref{lemma:seriesH1Poi}. 
\begin{enumerate}[leftmargin=*, label*=\alph*.]
\item[a)] The term $D_0[\de^4-1]$ satisfies
\begin{equation*}
\begin{split}
D_0[\de^4-1](\la,L;\de) 
=& \, L^4 +2(1-\de^4)L^2\cos \la + (1-\de^4)^2 \\ 
=& \, 2(1+\cos \la)
+ 4(L-1)(1+\cos \la) 
+ 2(L-1)^2 (3+\cos\la) \\
&+ 4(L-1)^3
+(L-1)^4
-2\de^4(1+\cos \la) \\
&-4\de^4(L-1)\cos\la
-2\de^4(L-1)^2\cos\la
+\de^8.
\end{split}
\end{equation*}
Performing the change $\Phi$, by Lemma~\ref{lemma:PhiMultipleChanges}, we have that
\begin{equation*}
%\label{proof:innerDerivationResultD0}
\begin{split}
\frac{2\al_+}{\de^{\frac{8}{3}}} D_0[\de^4-1]\circ \Phi 
&= \frac{2\al_+}{\de^{\frac{8}{3}}} 
\paren{2(1+\cos \Phi_{\la} ) 
+ 4 (\Phi_{L}-1)^2 +
\OO(\de^{\frac{4}{3}})}\\
%
&=  9 U^{\frac{4}{3}} %+ \OO(\de^{\frac{2}{3}}) 
+ 4 U^{\frac{2}{3}} W^2 - \frac{16}{3} W + \frac{16}{9 U^{\frac{2}{3}}}
 + \OO(\de^{\frac{4}{3}}).
\end{split}
\end{equation*}
%
\item[b)] Analgously the term $D_1[\de^4-1]$ satisfies
\begin{equation*}%\label{proofFirstIteration:P1S}
\begin{split}
D_1[\de^4-1] 
=& \, \eta \frac{\sqrt{2 L^3}}{2}  
\left[
(-3- 2 e^{-i\la} + e^{-2i\la})
%
- 4 (L-1) e^{-i\la}
\right. \\ &\left. \qquad \qquad
%
- 2 (L-1)^2 e^{-i\la}
+\de^4 (3- e^{-2i\la})
\right] \\
%
&+ \xi \frac{\sqrt{2 L^3}}{2}  \left[
(-3- 2 e^{i\la} + e^{2i\la})
%
-  4 (L-1) e^{i\la}
\right. \\ &\left. \qquad \qquad \quad
%
- 2 (L-1)^2 e^{i\la}
+\de^4 (3- e^{2i\la}) \right]
\end{split}
\end{equation*}
% Applying the change $\Phi$, by Lemma~\ref{lemma:PhiMultipleChanges}, we have that
and therefore
\begin{equation*}%\label{proof:innerDerivationResultD1}
\begin{split}
\frac{2\al_+}{\de^{\frac{8}{3}}}D_1[\de^4-1]\circ \Phi
%  
=& \frac{2 \al^2_+}{\de^{\frac{4}{3}}}  X
\paren{-4i\paren{\Phi_{\la}-\pi} 
- 4(\Phi_L-1)
 + \OO(\de^{\frac{4}{3}}) }
\\
&+ \frac{2 \al^2_+}{\de^{\frac{4}{3}}} Y
\paren{4i\paren{\Phi_{\la}- \pi} 
	- 4(\Phi_L-1)
	+ \OO(\de^{\frac{4}{3}}) }
\\
=& \, X\paren{-12 i U^{\frac{2}{3}} + 4U^{\frac{1}{3}} - 
	\frac{8}{3 U^{\frac{1}{3}}}} \\
&+ Y\paren{12 i U^{\frac{2}{3}} + 4U^{\frac{1}{3}} - 
\frac{8}{3 U^{\frac{1}{3}}} }
+ \OO(\de^{\frac{4}{3}}).
\end{split}
\end{equation*}
\item[c)] The term $D_2[\de^4-1]$ satisfies
\begin{align*}
D_2[\de^4-1] =& 
%
- \eta^2 \frac{L e^{-i \la}}{4} \paren{
	{-1 + 2 L^2 e^{-i\la} -3 e^{-2i\la} } +
	\de^4 \paren{ 1 + 3 e^{-2i\la}} } \\
%
&- \xi^2 \frac{L e^{-i \la}}{4} \paren{
{-1 + 2 L^2 e^{i\la} -3 e^{2i\la} } +
\de^4 \paren{ 1 + 3 e^{2i\la}} } \\
%
&+ \eta \xi L \paren{ 
3L^2 - 2\cos \la  +
\de^4 2\cos \la }
\end{align*}
and
% Applying the change $\Phi$, by Lemma~\ref{lemma:PhiMultipleChanges}, we have that
\begin{align*}
%\label{proof:innerDerivationResultD2}
&\frac{2\al_+}{\de^{\frac{8}{3}}} D_2[\de^4-1]\circ \Phi
= - 3 X^2  -3 Y^2 + 5 XY + \OO(\de^{\frac{4}{3}}).
\end{align*}
\item[d)] By the estimates of 
$D_{\geq 3}[\de^4-1]$ in~\eqref{eq:boundD3mes} and Lemma~\ref{lemma:PhiMultipleChanges},
\begin{align*}
	%\label{proof:innerDerivationResultD3}
\vabs{\frac{2\al_+}{\de^{\frac{8}{3}}} 
D_3[\de^4-1]\circ \Phi} 
\leq C(\cttInnDerA,\cttInnDerB)
{\de^{\frac{4}{3}}}.
\end{align*}  
\end{enumerate}
Collecting these results, we  conclude that 
% Applying the results in
% \eqref{proof:innerDerivationResultD0},
% \eqref{proof:innerDerivationResultD1},
% \eqref{proof:innerDerivationResultD2} and
% \eqref{proof:innerDerivationResultD3} 
% to equation
% \eqref{proof:innerDerivationResultDabans} we obtain
\begin{equation*}
%\label{proof:innerDerivationResultC}
	\begin{split}
		\frac{ \de^{\frac{4}{3}}}{2\al_+^2 }
		{H_1^{\Poi,P} \circ \Phi}
		%
		&= - \frac{1}{3 U^{\frac{2}{3}}}
		\frac{1}{\sqrt{1+\JJ(U,W,X,Y)}} 
		+ \OO(\de^{\frac{4}{3}}),
	\end{split}
\end{equation*}
where the function $\JJ$ is given in~\eqref{def:hFunction}. %and the terms of higher order in $\de$ can be bounded by a constant $C(\cttInnDerA,\cttInnDerB)$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item 
% It only remains to compute the term $H^{\Poi,S}_1$ of the Hamiltonian~\eqref{proof:hamiltonianInnerB}.
%
Proceeding analogously as for $H^{\Poi,P}_1$, it can be checked that
\begin{align*}
%\label{proof:innerDerivationResultD}
\vabs{\frac{\de^{\frac{4}{3}}}{2\al_+^2}
H^{\Poi,S}_1 \circ \Phi }
\leq
C(\cttInnDerA,\cttInnDerB)\de^{\frac{4}{3}}.
\end{align*}
\end{enumerate}
% Finally, applying~\eqref{proof:innerDerivationResultA},
% \eqref{proof:innerDerivationResultB},
% \eqref{proof:innerDerivationResultC} and
% \eqref{proof:innerDerivationResultD}
% to equation~\eqref{proof:hamiltonianInnerB} we obtain the result.
\end{proof}


==> Article Inner/proofD-innerComputation.tex <==

We split the proof of Theorem~\ref{theorem:innerComputations} into two parts. 
%
In Section~\ref{subsection:innerExistence} we prove the existence of the solutions $\ZuInn$ and $\ZsInn$ and the estimates in~\eqref{result:innerExistence}. 
%
In Section~\ref{subsection:innerDifference}, we 
provide the asymptotic formula for the difference $\Delta \ZInn = \ZuInn-\ZsInn$ given in \eqref{result:innerDifference}.
%
For both parts, we follow the approach given in~\cite{BalSea08}.

Throughout this section, we fix the $\beta_0 \in (0,\frac{\pi}{2})$ appearing in the definition of the domains $\DuInn$ and $\DsInn$ in \eqref{def:domainInnner} and $\EInn$ in~\eqref{def:domainInnnerDiff}.
%
We denote the components of all the functions and operators by a numerical sub-index $f=(f_1,f_2,f_3)^T$, unless stated otherwise.
%
In order to simplify the notation, we denote by $C$ any positive constant independent of $\kappa$.
%
%In order to simplify the notation, we say that $a, b > 0$ satisfy the inequality $a \lesssim b$ if there exists $C>0$, a constant independent of $\kappa$, such that $a \leq C b$.




==> Article Inner/proofD-innerComputationDifference.tex <==
\subsection{Asymptotic formula for the difference}
\label{subsection:innerDifference}

The strategy to prove the second part of Theorem~\ref{theorem:innerComputations} is divided in three steps. 
%
In Section~\ref{subsubsection:innerDiffPreliminaries} we characterize $\DZInn= \ZuInn-\ZsInn$ as a solution of a linear homogeneous equation.
%
In Section~\ref{subsubsection:innerDiffPotential}, we prove that $\DZInn$ is in fact  the unique solution of this linear equation in a suitable Banach space.
% 
Finally, in Section~\ref{subsubsection:innerDiffExponential}, we introduce a  Banach subspace of the previous one (with exponential weights) to obtain
exponentially small estimates for $\DZInn$.

%In this section we prove the second part of Theorem~\ref{theorem:innerComputations}: we provide the asymptotic formula~\eqref{result:innerDifference} for $\Delta \ZInn =\ZuInn-\ZsInn$,
%where $\ZuInn \in \XcalInnUTotal$, $\ZsInn \in \XcalInnSTotal$ are the functions obtained in Proposition~\ref{proposition:innerExistence}. 

\subsubsection{A homogeneous linear equation for \texorpdfstring{$\DZInn$}{the difference}}
\label{subsubsection:innerDiffPreliminaries}
By Theorem~\ref{theorem:innerComputations}, the difference $\DZInn(U) = \ZuInn(U) - \ZsInn(U)$ is well defined for $U \in \EInn$ (see~\eqref{def:domainInnnerDiff}).
%
Since $\ZuInn$, $\ZsInn$ satisfy the same invariance equation~\eqref{eq:invariantEquationInner}, their difference $\DZInn$  satisfies
\begin{equation*}%\label{eq:invariantEquationDiff}
\partial_U \DZInn = 
\AAA \DZInn + R(U)\DZInn,
\end{equation*}
where 
\begin{align}\label{def:operatorRDiff}
R(U)=
\int_0^1 D_Z\RRR[s\ZuInn + (1-s)\ZsInn](U) ds,
\end{align}
and $\AAA$ and $\RRR$ are given in~\eqref{def:matrixAAA} and~\eqref{def:operatorRRRInner}, respectively.
%
We denote by $R_{1}, R_{2}$ and $R_{3}$, the rows of the matrix $R$.

By the method of variation of parameters, there exists $c=(c_w,c_x,c_y)^T \in \complexs^3$ such that
\begin{align*}
\DZInn(U) = e^{\AAA U} \paren{ c
+ \int_{U_0}^{U} e^{-\AAA S} R(S) \DZInn(S) d S}.
\end{align*}
By Proposition~\ref{proposition:innerExistence}, 
$\DZInn = \ZuInn - \ZsInn$ satisfies  $\lim_{\Im U \to -\infty}\DZInn(U) =0$. Therefore $\DZInn$ satisfies
% 
% the integral equation~\eqref{eq:integralEqDifference} can be written as
\begin{equation}\label{eq:differenceMainEq}
\DZInn = \DZo + \II[\DZInn],
\end{equation}
where $\II$ is  the linear operator
\begin{equation}\label{def:operatorEEE}
\II[\varphi](U)=
\begin{pmatrix}
\displaystyle
\int_{-i\infty}^{U}  
\langle R_{1}(S), \varphi(S)\rangle d S \\[1em]
\displaystyle
e^{iU}\int_{-i\infty}^{U}  
e^{-iS} 
\langle R_{2}(S), \varphi(S)\rangle d S \\[1em]
\displaystyle
e^{-iU} \int_{-i\rhoInn}^{U} e^{iS} 
\langle  R_{3}(S), \varphi(S)\rangle d S
\end{pmatrix},
\end{equation}
% 
% %
% % Using this fact, we deduce that $\DZInn$
% % must satisfy
% \begin{equation}\label{eq:integralEqDifference}
% \begin{split}
% &\DWInn(U) =  \int_{-i\infty}^{U}  
% \langle R_{1}(S), \DZInn(S)\rangle d S, \\
% &\DXInn(U) =  e^{iU}\int_{-i\infty}^{U}  
% e^{-iS} 
% \langle R_{2}(S), \DZInn(S)\rangle d S, \\
% &\DYInn(U) = e^{-iU} \paren{ c_y
% + \int_{-i\rhoInn}^{U} e^{iS} 
% \langle  R_{3}(S), \DZInn(S)\rangle d S},
% %\quad c_y = e^{\rhoInn} \DYInn(-i\rhoInn)
% \end{split}
% \end{equation}
% where $c_y = e^{\rhoInn} \DYInn(-i\rhoInn)$.
% %
% %We use this equation to obtain an asymptotic expression for $\DZInn$.
%
and $\DZo$ is the function
\begin{equation*}
%\label{def:initialIterationDiff}
\DZo(U) = (0,0,c_y e^{-iU})^T=(0,0,e^{\rhoInn} \DYInn(-i\rhoInn) e^{-iU})^T.
%\begin{pmatrix}
%0 \\
%0 \\
%c_y e^{-iU}
%\end{pmatrix}.
\end{equation*}

%
%In particular, in Lemma~\ref{lemma:operatorEEexponential}, we analyze how the operator $\EE$ acts on this space.


%To simplify notation, we consider the product space 
%$
%\YcalInn_{\nu_1,\nu_2,\nu_3}= 
%\YcalInn_{\nu_1} \times
%\YcalInn_{\nu_2} \times
%\YcalInn_{\nu_3},
%$
%endowed with the product norm 
%$
%\normInn{\zeta}_{\nu_1,\nu_2,\nu_3}=
%\sum_i \normInn{\zeta_i}_{\nu_i}.
%$

%\begin{proposition}\label{proposition:innerDifference}
%	There exists $\rhoInn>0$ big enough such that for $U \in \EInn$, $\DZInn$ satisfies
%	\begin{align*}
%		\DZInn(U) =  \CInn e^{-iU} \Big((0,0,1)^T + \chi(U) \Big),
%	\end{align*}
%	where $\CInn \in \complexs$ is independent of $\rhoInn$ and there exists $\cttInnDiff>0$ independent of $\kappa$ such that
%	%$\chi$ satisfies %$\normInn{\chi}_{\frac{7}{3},2,1} \leq C$.
%	\[
%	\normInn{\chi_1}_{\frac{7}{3}} \leq \cttInnDiff, \quad
%	\normInn{\chi_2}_{2} \leq \cttInnDiff, \quad
%	\normInn{\chi_3}_{1} \leq \cttInnDiff.
%	\]
%	%Moreover, $\CInn \neq 0$ if and only if $\DZInn \neq 0$.
%\end{proposition}


%Moreover, by Proposition~\ref{proposition:innerExistence}, there exists a constant $\cttInnDiffB>0$ such that
%\[
%\DZInn \in B(\cttInnDiffB) \subset \YcalInn_{\frac{8}{3},\frac{4}{3},\frac{4}{3}}.
%\]

\subsubsection{Characterization of \texorpdfstring{$\DZInn$}{the difference} as a fixed point}
\label{subsubsection:innerDiffPotential}

% We define appropriate Banach spaces to deal with the equation~\eqref{eq:differenceMainEq}.
%
Given $\nu \in \reals$ and $\rhoInn>0$, we define the norm
\begin{align*}
\normInnDiff{\varphi}_{\nu}= \sup_{U \in \EInn} \vabs{U^{\nu} \varphi(U) },	
	%	
	%\normInnD{\zeta}_{\nu}= \sup_{U \in \DdInn} \vabs{U^{\nu} \zeta(U) }, \hh
	%
	%\normInn{\xi}_{\nu}= \sup_{U \in \EInn} \vabs{U^{\nu} \xi(U) },
\end{align*}
where the domain $\EInn$ is given in~\eqref{def:domainInnnerDiff}, 
%
and we introduce the Banach space
\begin{equation*}%\label{def:banachSpacesY}
\begin{split}
		\YcalInn_{\nu}&= 
		\left\{ \varphi: \EInn \to \complexs  \st  
		\varphi \text{ analytic }, 
		\normInnDiff{\varphi}_{\nu} < +\infty \right\}.
	\end{split}
\end{equation*}
Note that  $\YcalInn_{\nu}$ satisfy analogous properties as the ones in Lemma~\ref{lemma:sumNorms}. In this section, 
%
we use this lemma without mentioning it.
%
%Analogous statements to those in Lemma~\ref{lemma:sumNorms} and Remark~\ref{remark:kappaBigEnough} can be obtained for the domain $\EInn$ and the Banach space $\YcalInn_{\nu}$.

We state a technical lemma, whose proof is postponed to Section~\ref{subsubsection:innerTechnicalProofsB}.
\begin{lemma} \label{lemma:operatorEEpotential}
Let $\II$ be the operator defined in~\eqref{def:operatorEEE}. 
%
Then, for $\rhoInn>0$ big enough, 
there exists a constant $\cttInnDiffA>0$ independent of $\kappa$ such that,
for
$\Psi \in \YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$,
\begin{align*}
\normInnDiff{\II_1[\Psi]}_{\frac{8}{3}} 
	&\leq \cttInnDiffA \paren{
	\frac{1}{\rhoInn^2} \normInnDiff{\Psi_1}_{\frac{8}{3}} +
	\normInnDiff{\Psi_2}_{\frac{4}{3}} +
	\normInnDiff{\Psi_3}_{\frac{4}{3}}}, \\
%\label{proof:estimateEE1}\\
%%%%
\normInnDiff{\II_j[\Psi]}_{\frac{4}{3}} 
	&\leq \frac{\cttInnDiffA}{\rhoInn^2} \paren{
	\normInnDiff{\Psi_1}_{\frac{8}{3}} +
	\normInnDiff{\Psi_2}_{\frac{4}{3}} +
	\normInnDiff{\Psi_3}_{\frac{4}{3}} }, \qquad j=2,3.
\end{align*}
\end{lemma}
%
These estimates characterize $\DZInn$ as the unique solution of~\eqref{eq:differenceMainEq} in  $\YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$.

\begin{lemma}\label{lemma:innerExistenceDifference}
%Let $\Delta \ZInn =\ZuInn-\ZsInn$,where $\ZuInn$ and $\ZsInn$ are the functions given in Proposition~\ref{proposition:innerExistence}.
%	
For $\rhoInn>0$ big enough, 
$\DZInn$ is the unique solution of equation~\eqref{eq:differenceMainEq} belonging to
$\YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$.
%
In particular,
\begin{equation*}
\DZInn = \sum_{n \geq 0} \II^n[\DZo].
\end{equation*}
\end{lemma}

\begin{proof}
By Theorem~\ref{theorem:innerComputations}, for $\rhoInn>0$ big enough, $\DZInn$ is a solution of equation~\eqref{eq:differenceMainEq} which satisfies 
$
\DZInn = \ZuInn - \ZsInn \in \YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}.
$
%Moreover, $\DZInn$ belongs to the ball
%\[
%\DZInn \in 
%B_{\YcalInn} = \claus{\zeta \in \YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}
%\st
%\normInnDiff{\zeta_1}_{\frac{8}{3}},
%\normInnDiff{\zeta_2}_{\frac{4}{3}},
%\normInnDiff{\zeta_3}_{\frac{4}{3}} 
%\leq 2\cttInnExistA}.
%\]
Then, it only remains to prove that  equation~\eqref{eq:differenceMainEq} has a unique solution in $\YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$.
To this end, it is enough to show that the operator $\II$ is contractive with a suitable norm in $\YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$.
%
Taking
\[
\normInnDiff{\Psi}_{\times} = \normInnDiff{\Psi_1}_{\frac{8}{3}}
+ \kappa \normInnDiff{\Psi_2}_{\frac{4}{3}}
+ \kappa \normInnDiff{\Psi_3}_{\frac{4}{3}},
\]
Lemma~\ref{lemma:operatorEEpotential} implies
\[
\normInnDiff{\II[\Psi]}_{\times} \leq 
\frac{C}{\kappa} \normInnDiff{\Psi}_{\times}
\]
and, taking $\kappa$ big enough, the result is proven.
%Thus, $\EE$ is contractive in $\YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}}\times \YcalInn_{\frac{4}{3}}$ and has a unique fixed point.
\end{proof}
%%%%%%%%%%%%
%However, operator $\EE$ is not contractive in $B(\cttInnDiffB)$ (see Lemma~\ref{lemma:operatorEEpotential}) and, as a consequence, the fixed point theorem can not be applied.
%%	
%Nonetheless, as done in the proof of Proposition~\ref{proposition:innerExistence}, by way of a Gauss-Seidel argument, we can define a new linear operator with small Lipschitz constant. Let us define
%\begin{equation*} %\label{def:operatorsGaussSeidel}
%{\tEE}[\Psi]= \begin{pmatrix} 
%\EE_1[\Psi_1,\EE_2[\Psi],\EE_3[\Psi]] \\ 
%\EE_2[\Psi] \\
%\EE_3[\Psi] \end{pmatrix}.
%\end{equation*}
%%Let us consider $\Psi \in B(\cttInnDiffB)$.
%%
%Then, by Lemma~\ref{lemma:operatorEEpotential},
%\begin{align*}
%	\normInn{\tEE_1[\Psi]}_{\frac{8}{3}} 
%	\leq C \paren{
%	\frac{1}{\rhoInn^2} \normInn{\Psi_1}_{\frac{8}{3}} +
%	\normInn{\EE_2[\Psi]}_{\frac{4}{3}} +
%	\normInn{\EE_3[\Psi]}_{\frac{4}{3}} }
%	\leq \frac{C}{\rhoInn^2} \normInn{\Psi}_{\frac{8}{3},\frac{4}{3},\frac{4}{3}}.
%\end{align*}
%and, for $\rhoInn>0$ big enough,
%\begin{align*}
%\normInn{\tEE[\Psi]}_{\frac{8}{3},\frac{4}{3},\frac{4}{3}} 
%\leq \frac{C}{\rhoInn^2} \normInn{\Psi}_{\frac{8}{3},\frac{4}{3},\frac{4}{3}}
%\leq \frac{1}{2} \normInn{\Psi}_{\frac{8}{3},\frac{4}{3},\frac{4}{3}}.
%\end{align*}
%Thus, $\Psi=\tEE[\Psi]$ has a fixed point in $B(\cttInnDiffB)$ and, as a result, so does $\Psi=\EE[\Psi]$. 	

\subsubsection{Exponentially small estimates for \texorpdfstring{$\DZInn$}{the difference}}
\label{subsubsection:innerDiffExponential}

Once we have proved that $\DZInn$ is the unique solution of~\eqref{eq:differenceMainEq} in $\YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$, 
%
we use this equation to obtain exponentially small estimates for $\DZInn$. 
%


For any $\nu \in \reals$, we consider the norm
\begin{equation*}
\normInnDiffExp{\varphi}_{\nu} = \sup_{U \in \EInn} \vabs{U^{\nu} e^{i U} \varphi(U)},
\end{equation*}
and the associated Banach space
\begin{equation*}
\ZcalInn_{\nu} = \left\{
\varphi: \EInn \to \complexs \st 
\varphi \text{ analytic, }
\normInnDiffExp{\varphi}_{\nu} < +\infty
\right\}.
\end{equation*}
%
Moreover, for  $\nu_1, \nu_2, \nu_3 \in \reals$, we consider the product space 
\begin{align*}%\label{def:productSpaceDiffExp}
\ZcalInn_{\nu_1,\nu_2,\nu_3}= 
\ZcalInn_{\nu_1} \times
\ZcalInn_{\nu_2} \times
\ZcalInn_{\nu_3},
%
\quad \text{with} \quad
%
\normInnDiffExp{\varphi}_{\nu_1,\nu_2,\nu_3}=
\textstyle\sum_{j=1}^3 \normInnDiffExp{\varphi_j}_{\nu_j}.
\end{align*}

Next lemma, gives some properties of these Banach spaces. It follows the same lines as Lemma~\ref{lemma:sumNorms}.
%
% We use the results in it without mentioning them along the section.

% \textcolor{red}{He afegit aquest lemma. 
% Nomes fa falta posar o el punt 2 o el punt 3, un sobra.
% }


\begin{lemma}\label{lemma:sumNormsExp}
Let $\rhoInn>0$ and $\nu, \eta \in \reals$. The following statements hold:
\begin{enumerate}
\item If $\nu > \eta$, then $\ZcalInn_{\nu} \subset \ZcalInn_{\eta}$ and
$
\normInnDiffExp{\varphi}_{\eta} \leq \left( 
{\rhoInn}{\cos \beta_0}\right)^{\eta-\nu} 
\normInnDiffExp{\varphi}_{\nu}.
$
\item If $\varphi \in \ZcalInn_{\nu}$ and 
$\zeta \in \YcalInn_{\eta}$, then the product
$\varphi \zeta \in \ZcalInn_{\nu+\eta}$ and
$
\normInnDiffExp{\varphi \zeta}_{\nu+\eta} \leq \normInnDiffExp{\varphi}_{\nu} \normInnDiff{\zeta}_{\eta}.
$
\item If $\varphi \in \ZcalInn_{\nu}$ then 
$e^{iU}\varphi \in \YcalInn_{\nu}$ and
$
\normInnDiffSmall{e^{iU} \varphi}_{\nu} = \normInnDiffExp{\varphi}_{\nu}.
$
\end{enumerate}
\end{lemma}


The next lemma analyzes how the operator $\II$ acts on the space $\ZcalInn_{\frac{4}{3},0,0}$. Its proof  is postponed to Section~\ref{subsubsection:innerTechnicalProofsB}.

\begin{lemma} \label{lemma:operatorEEexponential}
%Let $R$ and $\II$ be the operators defined in~\eqref{def:operatorRDiff} and~\eqref{def:operatorEEE}, respectively.
%
Let $\II$ be the operator defined in~\eqref{def:operatorEEE}. For $\rhoInn>0$ big enough, 
there exists a constant $\cttInnDiffB>0$ independent of $\kappa$ such that,
for
$\Psi \in \ZcalInn_{\frac{4}{3},0,0}$,
% we have that 
\begin{align*}
\normInnDiffExp{\II_1[\Psi]}_{\frac{7}{3}} 
\leq \cttInnDiffB \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}, 
\quad
\normInnDiffExp{\II_2[\Psi]}_{2} 
\leq  \cttInnDiffB \normInnDiffExp{\Psi}_{\frac{4}{3},0,0},
\quad
\normInnDiffExp{\II_3[\Psi]}_{0}
\leq \frac{\cttInnDiffB}{\kappa}  \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
%\normInnExp{\langle R_3,\Psi \rangle}_2
%\leq  C \normInnExp{\Psi}_{\frac{4}{3},0,0}.
\end{align*}
Moreover, there exists $\wCInn(\rhoInn) \in \complexs$ (depending on $\Psi$), such that
\begin{equation*}%\label{result:asymptoticsEE3}
	\II_3[\Psi] - e^{-iU}\wCInn(\rhoInn) \in \ZcalInn_{1}.
\end{equation*}
\end{lemma}

%Notice that we have to be more accurate with operator $\EE_3$ to obtain the results in Proposition~\ref{proposition:innerDifference}.
%\begin{lemma}\label{lemma:asymptoticsEE}
%Let $\EE$ be the operator defined in~\eqref{def:operatorEEE}.
%%
%Then, there exists $\rhoInn>0$ big enough, such that 
%for $\Psi \in \ZcalInn_{\frac{4}{3},0,0}$
%we have that
%\begin{align}\label{result:desigualtatEE3}
%	\normInnExp{\EE_3[\Psi]}_{0}
%	\leq \frac{C}{\kappa}  \normInnExp{\Psi}_{\frac{4}{3},0,0}.
%\end{align}
%there exists a constant $\wCInn(\rhoInn)$, where
%\begin{equation}\label{result:asymptoticsEE3}
%\EE_3[\Psi] - e^{-iU}\wCInn(\rhoInn) \in \ZcalInn_{1}.
%\end{equation}
%\end{lemma}

\begin{proof}[End of the proof of the second part of Theorem~\ref{theorem:innerComputations}]

% By Proposition~\ref{proposition:innerExistence}, it only remains to prove the asymptotic formula for $\Delta \ZInn$ given in \eqref{result:innerDifference}.
% 	
Lemma~\ref{lemma:operatorEEexponential} implies that operator $\II: \ZcalInn_{\frac{4}{3},0,0} \to \ZcalInn_{\frac{4}{3},0,0}$ is well defined and contractive. 
%
Indeed, taking $\rhoInn>0$ big enough and $\Psi \in \ZcalInn_{\frac{4}{3},0,0}$, 
\begin{equation}\label{proof:EEcontractive}
\begin{split}
\normInnDiffExp{\II[\Psi]}_{\frac{4}{3},0,0} 
&= \normInnDiffExp{\II_1[\Psi]}_{\frac{4}{3}}
+ \normInnDiffExp{\II_2[\Psi]}_0
+ \normInnDiffExp{\II_3[\Psi]}_0 \\
&\leq
\frac{C}{\rhoInn} \normInnDiffExp{\II_1[\Psi]}_{\frac{7}{3}}+
\frac{C}{\rhoInn^2} \normInnDiffExp{\II_2[\Psi]}_2
+ \normInnDiffExp{\II_3[\Psi]}_0
% \end{align*}
% Applying Lemma~\ref{lemma:operatorEEexponential} we have that, for $\rhoInn>0$ big enough,
% \begin{align}\label{proof:EEcontractive}
% \normInnDiffExp{\II[\Psi]}_{\frac{4}{3},0,0} 
\leq 
%
\frac{C}{\kappa} 
\normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
%\leq \frac{1}{4} \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
\end{split}
\end{equation}
Therefore, since $\DZo=(0,0,c_y e^{-iU})^T \in \ZcalInn_{\frac{4}{3},0,0}$, 
% then
% $\II^n[\DZo] \in \ZcalInn_{\frac{4}{3},0,0} $, for $n\geq 0$.
% Moreover, by
Lemma~\ref{lemma:innerExistenceDifference} and \eqref{proof:EEcontractive} imply that
\begin{equation*}%\label{proof:differenceAsymptoticMainEquation}
\DZInn =(\DWInn,\DXInn,\DYInn)^T = \sum_{n \geq 0} \II^n[\DZo] \in \ZcalInn_{\frac{4}{3},0,0}.
\end{equation*}
Lemma~\ref{lemma:operatorEEexponential} implies 
$
\II:\ZcalInn_{\frac{4}{3},0,0} \to \ZcalInn_{\frac{7}{3},2,0} \subset 
\ZcalInn_{\frac{4}{3},0,0},
$
which allows to give better estimates for $\DZInn$. Indeed,  we have that ${\DZInn - \DZo} = \II[\DZInn] \in \ZcalInn_{\frac{7}{3},2,0}$,  which implies  
\begin{align*}
	\DWInn=\II_1[\DZInn] \in \ZcalInn_{\frac{7}{3}}, \qquad
	\DXInn=\II_2[\DZInn] \in \ZcalInn_{2}, \qquad
% 	\DYInn - c_y e^{-iU} - \wCInn(\rhoInn) e^{-iU} \in \ZcalInn_{1}.
\end{align*}
Moreover, by the second statement in Lemma \ref{lemma:operatorEEexponential}, 
%
there exists $\wCInn(\kappa)$ such that
\[	\DYInn - c_y e^{-iU} - \wCInn(\rhoInn) e^{-iU} \in \ZcalInn_{1}.\]
%Then, by Lemma~\ref{lemma:operatorEEexponential}, there exists a constant $\wCInn(\rhoInn)$ such that
%\begin{align*}
%	\DYInn - c_y e^{-iU} - \wCInn(\rhoInn) e^{-iU} \in \ZcalInn_{1},
%\end{align*}
Calling $\CInn = c_y + \wCInn(\kappa)$ we have that
$
\DYInn(U) - \CInn e^{-iU} \in \ZcalInn_{1},
$
and, therefore $\CInn = \lim_{\Im U \to -\infty}  \DYInn(U)e^{iU}$, which is independent of $\rhoInn$.
%
Then, $\DZInn$ is of the form
\begin{align*}
\DZInn(U) = e^{-iU} \Big((0,0,\CInn)^T + \chi(U) \Big),
\quad \text{with} \quad \chi \in 
\YcalInn_{\frac{7}{3}} \times \YcalInn_{2} \times \YcalInn_{1}.
\end{align*}
%where $\CInn= c_y + \wCInn(\rhoInn)$. 
%
%We observe that, since $\DZInn$ is independent of $\rhoInn$, then the constant $\CInn$ is independent of $\rhoInn$ too.
%%
%Moreover, if $\CInn=0$ implies that $\DYInn \equiv 0$, then $\DZInn$ can be expressed as
%\[
%\DZInn(U) = \CInn e^{-iU} \Big((0,0,1)^T + \chi(U) \Big).
%\]

% \textcolor{red}{Revisar aquest tros:}

Now we prove that, if there exists $U_0 \in \EInn$ such that $\DZInn(U_0) \neq 0$, then $\CInn \neq 0$.
%
This implies  $\DZInn(U) \neq 0$ for all $U \in \EInn$,
since $\DZInn$ is a solution of an homogeneous linear differential equation.
%
Therefore  $c_y \neq 0$. Indeed, $c_y=0$ would imply  $\DZo=0$ and, by Lemma~\ref{lemma:innerExistenceDifference},  one could conclude $\DZInn \equiv 0$.

Thus, it only remains to prove  that $c_y \neq 0$ implies $\CInn\neq 0$. By Lemma~\ref{lemma:innerExistenceDifference},
\begin{align*}
\DZInn - \DZo = \sum_{n\geq 1} \II^n[\DZo].
\end{align*} 
In addition, by the estimate \eqref{proof:EEcontractive},  $\normInnDiffExp{\II_3}_{\frac{4}{3}} \leq \frac{1}{4}$  if  $\rhoInn>0$ is big enough. Since $\DYo=c_y e^{-iU}$, we deduce that
\begin{align*}
\normInnDiffExp{\DYInn - \DYo}_{0} 
\leq \sum_{n\geq 1} \frac{1}{4^n} \normInnDiffExp{\DYo}_{0}
= \frac{1}{3} \vabs{c_y}, 
\end{align*}
and, by the definition of the norm $\normInnDiffExp{\cdot}_0$, for any $U \in \EInn$,
\begin{align*}
\vabs{e^{iU}\DYo(U)} -
	\vabs{e^{iU}\DYInn(U)} \leq 
	 \frac{1}{3} \vabs{c_y}.
\end{align*}
%
%On the other hand, if $\DZInn(U) \neq 0$ for all $U \in \EInn$, then $c_y \neq 0$ (on the contrary, $\DZo \equiv 0$ and by~\eqref{proof:differenceAsymptoticMainEquation}, $\DZInn = 0$).
%
Hence, using that $e^{iU}\DYInn=\CInn+\chi_3(U)$ with $\chi_3 \in \YcalInn_{1}$ and $e^{iU}\DYo(U)=c_y$, we have that for all $U \in \EInn$,
\begin{align*}
\vabs{e^{iU}\DYInn(U)} =
\vabs{\CInn + \chi_3(U)} 
\geq
\vabs{e^{iU}\DYo(U)} - \frac{1}{3} \vabs{c_y}
= \frac{2}{3} \vabs{c_y}.
\end{align*}
%
Finally, taking $\Im(U)\to-\infty$, we obtain that $\vabs{\CInn} \geq \frac{2}{3}\vabs{c_y} > 0$.
%
%Taking $\Im(U)\to-\infty$, we get that $\CInn \geq \frac{2}{3}\vabs{c_y}$ and, since $c_y = e^{\kappa} \DYInn(-i\kappa) \neq 0$ (see~\eqref{eq:integralEqDifference}), we have that $\CInn \neq 0$.
\end{proof}

%Notice that, $c_y = e^{\kappa} \DYInn(-i\kappa) \neq 0$ (see~\eqref{eq:integralEqDifference}).
%%
%Therefore, taking $\Im(U) \to -\infty$, we get that $\CInn \geq \frac{2}{3}\vabs{c_y}> 0$ and thus $\CInn \neq 0$.


==> Article Inner/proofD-innerComputationExistence.tex <==

\subsection{Existence of suitable solutions of the inner equation}
\label{subsection:innerExistence}

From now on we deal only with the analysis for $\ZuInn$. The analysis for $\ZsInn$  is analogous.

%We prove the first part of Theorem~\ref{theorem:innerComputations} through a fixed point argument in suitable Banach spaces. 
%
%We prove the existence of the solution $\ZuInn$ and its estimates in~\eqref{result:innerExistence}. 
%%
%The proof for $\ZsInn$ is analogous.
%Thus, to simplify notation we drop the super-index $\mathrm{u}$. 

\subsubsection{Preliminaries and set up}

The invariance equation~\eqref{eq:invariantEquationInner}, that is $\partial_U \ZuInn = 
\AAA \ZuInn + \RRR[\ZuInn]$,  can be written as $\LL \ZuInn = \RRR[\ZuInn]$
where $\LL$ is  the linear operator
\begin{equation}\label{def:operatorL}
	\LL \varphi =(\partial_U-\AAA)\varphi.
\end{equation}
Notice that if we can construct  a left-inverse of $\LL$ in an appropriate Banach space, we can write~\eqref{eq:invariantEquationInner} as a fixed point equation to be able apply the Banah fixed point theorem.

%We prove the first part of Theorem~\ref{theorem:innerComputations} through a fixed point argument on suitable Banach spaces.

%The function $\ZInn=(\WInn,\XInn,\YInn)$
%satisfies the equation~\eqref{eq:invariantEquationInner} and the asymptotic condition~\eqref{eq:asymptoticConditionsInner}.
%%
%If we define the linear operator
%\begin{equation}\label{def:operatorL}
%	\LL \ZInn=(\partial_U-\AAA)\ZInn ,
%\end{equation}
%Then, the equation~\eqref{eq:invariantEquationInner} can be written as $\LL \ZInn = \RRR[\ZInn]$.

Given $\nu \in \reals$ and $\rhoInn>0$, we define the norm
\begin{align*}
\normInn{\varphi}_{\nu}= \sup_{U \in \DuInn} \vabs{U^{\nu} \varphi(U) },	
%	
%\normInnD{\zeta}_{\nu}= \sup_{U \in \DdInn} \vabs{U^{\nu} \zeta(U) }, \hh
%
%\normInn{\xi}_{\nu}= \sup_{U \in \EInn} \vabs{U^{\nu} \xi(U) },
\end{align*}
where the domain $\DuInn$ is given in~\eqref{def:domainInnner}, 
%
and we introduce the Banach space
\begin{equation*}%\label{def:banachSpacesX}
\begin{split}
	\XcalInn_{\nu}&= 
	\left\{ \varphi: \DuInn \to \complexs  \st  
	\varphi \text{ analytic, } 
	\normInn{\varphi}_{\nu} < +\infty \right\}.
\end{split}
\end{equation*}
Next lemma, proven in~\cite{Bal06}, gives some properties of these Banach spaces.
%
We use this lemma throughout the section  without mentioning it.
%
%We will work with Lemma 4.3 in~\cite{Bal06}.
%
%Its proof follows the same lines as the proof of Lemma 4.3 in~\cite{Bal06}.

\begin{lemma}\label{lemma:sumNorms}
	Let $\rhoInn>0$ and $\nu, \eta \in \reals$. The following statements hold:
	\begin{enumerate}
	\item If $\nu > \eta$, then $\XcalInn_{\nu} \subset \XcalInn_{\eta}$ and
	$
	\normInn{\varphi}_{\eta} \leq \left( 
	{\rhoInn}{\cos \beta_0}
	\right)^{\eta-\nu} 
	\normInn{\varphi}_{\nu}.
	$
	\item If $\varphi \in \XcalInn_{\nu}$ and 
	$\zeta \in \XcalInn_{\eta}$, then the product
	$\varphi \zeta \in \XcalInn_{\nu+\eta}$ and
	$
	\normInn{\varphi \zeta}_{\nu+\eta} \leq \normInn{\varphi}_{\nu} \normInn{\zeta}_{\eta}.
	$
	\end{enumerate}
	%Analogous statements hold for $\XcalInnU$ and $\XcalInnS$.
\end{lemma}

In the following  lemma, we introduce a left-inverse of the operator $\LL$ in~\eqref{def:operatorL}.

\begin{lemma}\label{lemma:Glipschitz}
Consider the operator
\begin{equation*}%\label{def:operatorGG}
	\GG[\varphi](U) = \left(\int_{-\infty}^U \varphi_1(S) dS, 
	\int_{-\infty}^U e^{-i (S-U)} \varphi_2(S) dS , 
	\int_{-\infty}^U e^{i(S-U)} \varphi_3(S) dS \right)^T.
\end{equation*}
Fix $\eta>1$, $\nu>0$ and  $\rhoInn\geq 1$.
%
Then, $\GG: \XcalInn_{\eta} \times \XcalInn_{\nu} \times \XcalInn_{\nu} \to \XcalInn_{\eta-1} \times \XcalInn_{\nu} \times \XcalInn_{\nu}$ is a continuous linear operator and is a left-inverse of $\LL$. 

Moreover, there exist a constant $C>0$ such that
	\begin{enumerate}
	\item If $\varphi \in \XcalInn_{\eta}$, then $\GG_1[\varphi] \in \XcalInn_{\eta-1}$ and
	$
	\normInn{\GG_1[\varphi]}_{\eta-1} \leq C  \normInn{\varphi}_{\eta}.
	$
	\item If $\varphi \in \XcalInn_{\nu}$ and $j=2,3$, then $\GG_j[\varphi] \in \XcalInn_{\nu}$ and
	$
	\normInn{\GG_j[\varphi]}_{\nu} \leq   C \normInn{\varphi}_{\nu}.
	$
	\end{enumerate}
\end{lemma}
\begin{proof}
It follows the same lines as the proof of Lemma 4.6 in~\cite{Bal06}.
\end{proof}
%
Let us then define the fixed point operator 
\begin{equation}\label{def:operatorFF}
\FF= \GG \circ \RRR.
\end{equation}
%where the operators $\RRR$ and $\GG$ are defined on~\eqref{def:operatorRRRInner} and~\eqref{def:operatorGG}, respectively. 
%
A solution of 
$
\ZuInn=\FF[\ZuInn]
$
belonging to $\XcalInn_{\eta} \times \XcalInn_{\nu} \times \XcalInn_{\nu}$
with $\eta,\nu>0$
%
satisfies equation~\eqref{eq:invariantEquationInner} and the asymptotic condition~\eqref{eq:asymptoticConditionsInner}.
% 
Therefore, to prove the first part of Theorem~\ref{theorem:innerComputations} and the asymptotic estimates in \eqref{result:innerExistence}, we look for a fixed point of  the operator $\FF$  in the Banach space
\begin{equation*}%\label{def:banachSpacesXYTotal}
	\XcalInnTotal = \XcalInn_{\frac{8}{3}} \times \XcalInn_{\frac{4}{3}} \times \XcalInn_{\frac{4}{3}}, 
\end{equation*}
endowed with the norm
\[
\normInnTotal{\varphi}= 
\normInn{\varphi_1}_{\frac{8}{3}} + 
\normInn{\varphi_2}_{\frac{4}{3}} + 
\normInn{\varphi_3}_{\frac{4}{3}}.
\] 

\begin{proposition}\label{proposition:innerExistence}	There exists $\rhoInn_0>0$ such that for any $\rhoInn \geq \rhoInn_0$, the fixed point equation $\ZuInn = {\FF}[\ZuInn]$ has a solution $\ZuInn \in \XcalInnTotal$.
%	
Moreover, there exists a constant $\cttInnExistA>0$, independent of $\rhoInn$, such that
\[
\normInnTotal{\ZuInn} \leq \cttInnExistA.
\]
\end{proposition}
%
\begin{remark}\label{remark:kappaBigEnough}
Notice that $\DuInn \subseteq \DuInnR{\rhoInn_0}$ when $\rhoInn\geq\rhoInn_0$ (see~\eqref{def:domainInnner}). 
%
Then, for some $\nu \in \reals$, if $\zeta \in \XcalInn_{\nu}$ (defined for $\rhoInn$) then $\zeta \in \XX_{\nu}$ (defined for $\rhoInn_0$).
%
This allows us to take $\rhoInn$ as big as we need.
\end{remark}

\subsubsection{Proof of Proposition~\ref{proposition:innerExistence}}
%
% We prove Proposition~\ref{proposition:innerExistence} through a fixed point argument.
%
%However, we will see that the Lipschitz constant of $\FF$ is greater than $1$ with the norm in $\XcalInnTotal$.
%%
%Nonetheless, by a Gauss-Seidel scheme, we can modify $\FF$ to define a new operator with a small Lipschitz constant and with the same fixed points.
%
We first state a technical lemma whose proof is postponed until Section~\ref{subsubsection:innerTechnicalProofsA}.
%
For $\varrho>0$, we define the closed ball 
\begin{equation*}%\label{def:ballInner}
B(\varrho) = \claus{\varphi \in \XcalInnTotal \st
\normInnTotal{\varphi}\leq \varrho}.
\end{equation*}

\begin{lemma}\label{lemma:boundsRRR}
Let ${\RRR}$ be the operator defined in~\eqref{def:operatorRRRInner}.
%	
Then, for  $\varrho>0$ and for $\rhoInn>0$ big enough,
there exists a constant $C>0$ 
such that, for any
$\ZInn \in B(\varrho)$, 
\begin{align*}
&\normInn{\RRR_1[\ZInn]}_{\frac{11}{3}} \leq C, \qquad
\normInn{\RRR_j[\ZInn]}_{\frac{4}{3}} \leq C, \qquad
j=2,3,
\end{align*}
	and
	\begin{align*}
	\normInn{\partial_W\RRR_1[\ZInn]}_3 &\leq C, \quad &
	\normInn{\partial_X\RRR_1[\ZInn]}_{\frac{7}{3}} &\leq C, \quad &
	\normInn{\partial_Y\RRR_1[\ZInn]}_{\frac{7}{3}} &\leq C, \\
	\normInn{\partial_W\RRR_j[\ZInn]}_{\frac{2}{3}} &\leq C, \quad &
	\normInn{\partial_X\RRR_j[\ZInn]}_{2} &\leq C , \quad &
	\normInn{\partial_Y\RRR_j[\ZInn]}_{2} &\leq C, \quad j=2,3.
\end{align*} 
\end{lemma}

The next lemma gives properties of the operator $\FF$. 
%
% The first one deals with $\FF[0]$, and it is a direct consequence of Lemmas~\ref{lemma:Glipschitz} and~\ref{lemma:boundsRRR}.
%
% The second lemma is about the Lipschitz constant of $\FF$.
%


\begin{lemma}\label{lemma:firstIterationInner}
	Let ${\FF}$ be the operator defined in~\eqref{def:operatorFF}. 
	Then, for $\rhoInn>0$ big enough, 
	there exists a constant $\cttInnExistB>0$ independent of $\kappa$ such that
	\[
	\normInnTotal{{\FF[0]}} \leq \cttInnExistB.
	\]
% % \end{lemma}
% % 
% % \begin{lemma}\label{lemma:FLipschitzInner}
% Let ${\FF}$ be the operator defined in~\eqref{def:operatorFF}.
%


Moreover, for  $\varrho>0$ and $\rhoInn>0$ big enough, 
there exists a constant $\cttInnExistC>0$ independent of $\kappa$  such that, 
for any $\ZInn=(\WInn,\XInn,\YInn)^T$, $\ZInnB=(\WInnB,\XInnB,\YInnB)^T \in B(\varrho) \subset \XcalInnTotal$, 
% the operator $\FF$ satisfies
	\begin{align*} 
	\normInnSmall{{\FF_1}[\ZInn]-{\FF_1}[\ZInnB]}_{\frac{8}{3}} &\leq \cttInnExistC
	\left( \frac{1}{\rhoInn^2} 
	\normInnSmall{\WInn - \WInnB}_{\frac{8}{3}} 
	+ \normInnSmall{\XInn - \XInnB}_{\frac{4}{3}}
	+ \normInnSmall{\YInn - \YInnB}_{\frac{4}{3}} \right), \\
	%
	%\label{result:F23Lipschitz}
	\normInnSmall{{\FF_j}[\ZInn]-{\FF_j}[\ZInnB]}_{\frac{4}{3}} &\leq \frac{\cttInnExistC}{\rhoInn^2} \normInnTotalSmall{\ZInn - \ZInnB},
	\qquad
	j=2, 3.
	\end{align*}
\end{lemma}

\begin{proof}
%Let ${\RRR}=(\RRR_1,\RRR_2,\RRR_3)$ be the operator defined in~\eqref{def:operatorRRRInner}.	
%	
The estimate for  $\FF[0]$ is a direct consequence of Lemmas~\ref{lemma:Glipschitz} and~\ref{lemma:boundsRRR}.


To estimate the Lipschitz constant, we first estimate each component $\RRR_j[\ZInn]-\RRR_j[\ZInnB]$ separately  for $j=1,2,3$. By the mean value theorem we have
\begin{align*}
\RRR_j[\ZInn]-\RRR_j[\ZInnB] 
&=\boxClaus{\int_0^1 D \RRR_j[s \ZInn + (1-s) \ZInnB]  d s }
(\ZInn - \ZInnB) .
\end{align*}
Then, for $j=2,3$, we have
\begin{align*}
\MoveEqLeft[4]{\normInnSmall{\RRR_1[\ZInn]-\RRR_1[\ZInnB]}_{\frac{11}{3}} \leq
%
\normInnSmall{\WInn - \WInnB}_{\frac{8}{3}}
\sup_{\varphi \in {B(\varrho)}}  \normInn{\partial_W\RRR_1[\varphi]}_{1} }\\
%
&+ \normInnSmall{\XInn - \XInnB}_{\frac{4}{3}}
\sup_{\varphi \in {B(\varrho)}} \normInn{\partial_X{\RRR_1}[\varphi]}_{\frac{7}{3}} 
%
+ \normInnSmall{\YInn - \YInnB}_{\frac{4}{3}} \sup_{\varphi \in {B(\varrho)}} 
\normInn{\partial_Y\RRR_1[\varphi]}_{\frac{7}{3}}, \\
%%%%
\MoveEqLeft[4]{\normInnSmall{\RRR_j[\ZInn]-\RRR_j[\ZInnB]}_{\frac{4}{3}} \leq
%
\normInnSmall{\WInn - \WInnB}_{\frac{8}{3}}
\sup_{\varphi \in {B(\varrho)}} \normInn{\partial_W\RRR_j[\varphi]}_{-\frac{4}{3}} }\\
%
&+ \normInnSmall{\XInn - \XInnB}_{\frac{4}{3}} 
\sup_{\varphi \in {B(\varrho)}} \normInn{\partial_X{\RRR_j}[\varphi]}_{0} 
%
+ \normInnSmall{\YInn - \YInnB}_{\frac{4}{3}}
\sup_{\varphi \in {B(\varrho)} } 
\normInn{\partial_Y \RRR_j[\varphi]}_{0}.
\end{align*}
Applying Lemma~\ref{lemma:boundsRRR}, we obtain
\begin{align*}
\normInnSmall{{\RRR_1}[\ZInn]-{\RRR_1}[\ZInnB]}_{\frac{11}{3}} &\leq C
\left( \frac{1}{\rhoInn^2} \normInnSmall{\WInn - \WInnB}_{\frac{8}{3}} 
+ \normInnSmall{\XInn - \XInnB}_{\frac{4}{3}}
+ \normInnSmall{\YInn - \YInnB}_{\frac{4}{3}} \right),\\
%
\normInnSmall{{\RRR_j}[\ZInn]-{\RRR_j}[\ZInnB]}_{\frac{4}{3}} &\leq \frac{C}{\rhoInn^2} \normInnTotalSmall{\ZInn - \ZInnB},
\quad j=2,3.
\end{align*}
Finally, applying Lemma~\ref{lemma:Glipschitz}, we obtain the estimates in the lemma.
\end{proof}

Lemma~\ref{lemma:firstIterationInner} shows that,
by assuming $\rhoInn>0$ big enough, the operators $\FF_2$ and $\FF_3$ have Lipschitz constant less than $1$.
%
However, this is not the case for $\FF_1$.
%
To overcome this problem, we apply a Gauss-Seidel argument and define a new operator 
\begin{equation*} %\label{def:operatorFGaussSeidel}
\wt{\FF}[\ZInn]=
\wt{\FF}[(\WInn,\XInn,\YInn)]=
\begin{pmatrix} 
\FF_1[\WInn,\FF_2[\ZInn],\FF_3[\ZInn]] \\ 
\FF_2[\ZInn] \\
\FF_3[\ZInn] \end{pmatrix},
\end{equation*}
%where ${\FF}=(\FF_1,\FF_2,\FF_3)$ is the operator defined in~\eqref{def:operatorFF}.
%
which has the same fixed points as $\FF$ and turns out to be contractive in a suitable ball. 
%

\begin{proof}[End of the proof of Proposition \ref{proposition:innerExistence}]
We first obtain an estimate for $\normInnTotalSmall{\wt{\FF}[0]}$. Notice that
\begin{equation*} 
\wt{\FF}[0]= \FF[0]
+ 
\big(\wt \FF[0]-\FF[0]\big)=
\FF[0]
+ 
\big(
\FF_1\left[0,\FF_2[0],\FF_3[0]\right]-\FF_1[0], 0, 0 \big)^T.
\end{equation*} 
%\begin{equation*} 
%\wt{\FF}[0]= \begin{pmatrix} 
%\FF_1[0] \\ 
%\FF_2[0] \\
%\FF_3[0] \end{pmatrix}
%+ 
%\begin{pmatrix} 
%\FF_1[0,\FF_2[0],\FF_3[0]]-\FF_1[0] \\ 
%0\\
%0 \end{pmatrix},
%\end{equation*} 
% and Lemma~\ref{lemma:firstIterationInner} implies that
% \begin{align*}
% \normInnTotalSmall{\paren{0,\FF_2[0],\FF_3[0]}} \leq
% \normInnTotal{\FF[0]} \leq C.
% \end{align*}
Then, by Lemma~\ref{lemma:firstIterationInner}, $(0,\FF_2[0],\FF_3[0])^T\in \XcalInnTotal$ and 
\begin{align*}
\normInnTotalSmall{\wt{\FF}[0]} &\leq
\normInnTotal{\FF[0]} +
\normInn{\FF_1[0,\FF_2[0],\FF_3[0]]-\FF_1[0]}_{\frac{8}{3}} \\
&\leq \normInnTotal{\FF[0]}
+ C \normInn{\FF_2[0]}_{\frac{4}{3}}
+ C \normInn{\FF_3[0]}_{\frac{4}{3}} 
\leq C \normInnTotal{\FF[0]}.
\end{align*}
Thus, we can fix $\varrho>0$ such that
\begin{align*}%\label{eq:fixedpointtilde}
\normInnTotalSmall{\wt{\FF}[0]} \leq \frac{\varrho}{2}. 
\end{align*}
Now, we prove that the operator $\wt{\FF}$ is contractive in $B(\varrho) \subset \XcalInnTotal$. 
%
By Lemma~\ref{lemma:firstIterationInner} and assuming $\rhoInn>0$ big enough, we have that for $\ZInn, \ZInnB \in B(\varrho)$,
\begin{align*}
\normInnSmall{\wt{\FF}_1[\ZInn]-\wt{\FF}_1[\ZInnB]}_{\frac{8}{3}} \leq& 
%
\frac{C}{\rhoInn^2} \normInnSmall{\WInn-\WInnB}_{\frac{8}{3}} +
%
\normInnSmall{\FF_2[\ZInn]-\FF_2[\ZInnB]}_{\frac{4}{3}} +
\normInnSmall{\FF_3[\ZInn]-\FF_3[\ZInnB]}_{\frac{4}{3}} \\
%
%	C \sum_{j=2,3}
%	\normInnSmall{\FF_j[\ZInn]-\FF_j[\ZInnB]}_{\frac{4}{3}} \\
%
\leq& 
\frac{C}{\rhoInn^2} 
\normInnSmall{\WInn-\WInnB}_{\frac{8}{3}} +
\frac{C}{\rhoInn^2}\normInnTotalSmall{\ZInn-\ZInnB}
%
\leq	
\frac{C}{\rhoInn^2}\normInnTotalSmall{\ZInn-\ZInnB}, \\
%%%
\normInnSmall{\wt{\FF}_j[\ZInn]-\wt{\FF}_j[\ZInnB]}_{\frac{4}{3}}  
\leq&
\frac{C}{\rhoInn^2} \normInnTotalSmall{\ZInn-\ZInnB},
\qquad \text{ for } j=2, 3.
\end{align*}
%
Then, there exists $\kappa_0>0$ such that for $\kappa\geq\kappa_0$, the operator
$\wt{\FF}:B(\varrho) \to B(\varrho)$ is well defined and contractive. 
%
Therefore $\wt{\FF}$ has a fixed point 
$\ZuInn \in B(\varrho) \subset \XcalInnTotal$.
\end{proof}


%	Let us consider $\ZInn \in B(\cttInnExistA)$, then applying~\eqref{eq:fixedpointtilde} and~\eqref{eq:fixedpointtilde2} we have that
%	\begin{align*}
%	\normInnTotal{\wt{\FF}[\ZInn]} \leq \normInnTotal{\wt{\FF}[0]} + \normInnTotal{\wt{\FF}[\ZInn]-\wt{\FF}[0]}
%	< \frac{\cttInnExistA}{2}+ \frac{\normInnTotal{\ZInn}}{2} 
%	\leq \cttInnExistA.
%	\end{align*}
%	Therefore, it exists $\ZInn \in B(\cttInnExistA)$ such that $\ZInn = \wt{\FF}[\ZInn]$. %As result, this solution also satisfies that $\ZInn = \FF[\ZInn]$.
%\end{proof}




==> Article Inner/proofD-innerTechnicalProofs.tex <==
% \subsection{\textcolor{red}{Technical Proofs}}
\subsection{Proof of the technical lemmas}
\label{subsection:innerTechnicalProofs}

We devote this section to prove Lemma~\ref{lemma:boundsRRR} of Section~\ref{subsubsection:innerTechnicalProofsA}
and
Lemmas \ref{lemma:operatorEEpotential} and \ref{lemma:operatorEEexponential} 
of Section~\ref{subsubsection:innerTechnicalProofsB}.

%Section~\ref{subsubsection:innerTechnicalProofsA} we prove Lemma~\ref{lemma:boundsRRR} and in Section~\ref{subsubsection:innerTechnicalProofsB} we prove both Lemmas \ref{lemma:operatorEEpotential} and \ref{lemma:operatorEEexponential}.
%\paragraph{Proof of Lemma~\ref{lemma:boundsRRR}}

\subsubsection{Proof of Lemma~\ref{lemma:boundsRRR}}
\label{subsubsection:innerTechnicalProofsA}


Fix $\varrho>0$ and take $\ZInn=(\WInn,\XInn,\YInn)^T \in B(\varrho) \subset \XcalInnTotal$. By the definition \eqref{def:operatorRRRInner} of $\RRR$,
\begin{align}\label{proof:operatorRRRInner}
\RRR[\ZInn](U) = \paren{\frac{f_1(U,\ZInn)}{1+g(U,\ZInn)},\,
 \frac{\wt{f}_2(U,\ZInn)}{1+g(U,\ZInn)}, \,
 \frac{\wt{f}_3(U,\ZInn)}{1+g(U,\ZInn)} },
\end{align}
where
	\begin{equation*}%\label{proof:deff2f3tilde}
	\begin{split}
	\wt{f}_2(U,\ZInn) &= f_2(U,\ZInn) - i{\XInn} g(U,\ZInn), \qquad
	\wt{f}_3(U,\ZInn) = f_3(U,\ZInn) + i{\YInn} g(U,\ZInn), 
	\end{split}
	\end{equation*}
with $g=\partial_W \KK$, $f=(-\partial_U \KK, i\partial_Y \KK,-i\partial_X \KK)^T$ and $\KK$ is the Hamiltonian given in~\eqref{def:hamiltonianK} in terms of the function $\JJ$ (see~\eqref{def:hFunction}).
%
% Therefore, the terms we need to estimate are the first and second derivatives of $\KK$. 

We first estimate $\JJ$ and its derivatives.
For $\rhoInn>0$ big enough, we have 
	\begin{align*}
	& \vabs{\JJ(U,\ZInn)} \leq \frac{C}{U^{2}},\qquad
	%%%%
	\vabs{1+\JJ(U,\ZInn)} \geq 1 - \frac{C}{\rhoInn^2}\geq \frac{1}{2}.
	%%%%
	\end{align*}
Moreover, its  derivatives satisfy
\begin{align*}
	\vabs{\partial_U{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{3}},  &
	%%%%
	\vabs{\partial_W{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{4}{3}}},  &
	%%%%
	\vabs{\partial_X{\JJ}(U,\ZInn)},
	\vabs{\partial_Y{\JJ}(U,\ZInn)}  
	&\leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, 
\end{align*}
and
\begin{align*}
	\vabs{\partial_{U W}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{7}{3}}}, \quad &
	%%%%
	\vabs{\partial_{U X}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{5}{3}}}, 
	\quad &
	%%%% 
	\vabs{\partial_{U Y}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{5}{3}}},
	\\
	%%%% %%%%
	\vabs{\partial^2_{W}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, 
	\quad &
	%%%%
	\vabs{\partial_{W X}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}}, 
	\quad &
	%%%%
	\vabs{\partial_{W Y}{\JJ}(U,\ZInn)}  
	&\leq \frac{C}{\vabs{U}}, 
	\\
	%%%% %%%%
	\vabs{\partial^2_{X}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{4}{3}}},\quad &
	%%%%
	\vabs{\partial_{X Y}{\JJ}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}, 
	\quad &
	%%%%
	\vabs{\partial_{Y}^2{\JJ}(U,\ZInn)}
	&\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}.
\end{align*}
Using these estimates, we obtain the following bounds for $g, f_1,\wt{f}_2$ and $\wt{f}_3$,
\begin{align*}
	\vabs{g(U,\ZInn)} &=
	\vabs{-\frac{3}{2}U^{\frac{2}{3}}\WInn +\frac{1}{6U^{\frac{2}{3}}}
	\frac{\partial_W \JJ}{(1+\JJ)^{\frac{3}{2}}}}
	\leq \frac{C}{\vabs{U}^2},  \\
	%%%%%
	\vabs{f_1(U,\ZInn)} &=
	\vabs{\frac{\WInn^2}{2 U^{\frac{1}{3}}}
		-\frac{2}{9 U^{\frac{5}{3}}}  \frac{\JJ}{\sqrt{1+\JJ}(1+\sqrt{1+\JJ})}
		-\frac{1}{6 U^{\frac{2}{3}}} \frac{\partial_U \JJ}
		{(1+\JJ)^{\frac{3}{2}}}
	} \leq \frac{C}{\vabs{U}^{\frac{11}{3}}}, \\
	%%%%%
	\vabs{\wt{f}_2(U,\ZInn)} &=
	\vabs{\frac{i}{6 U^{\frac{2}{3}}} \frac{\partial_Y \JJ}{(1+\JJ)^{\frac{3}{2}}}
		-i\XInn g(U,\ZInn)}
	\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}, \\
	%%%%%
	\vabs{\wt{f}_3(U,\ZInn)} &=
	\vabs{-\frac{i}{6 U^{\frac{2}{3}}} \frac{\partial_X \JJ}{(1+\JJ)^{\frac{3}{2}}}
		+i\YInn g(U,\ZInn)}
	\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}.
\end{align*}
Analogously, we obtain estimates for the derivatives,
\begin{align*}
	\vabs{\partial_W {g}(U,\ZInn)} 
	&\leq  C \vabs{U}^{\frac{2}{3}}, \quad &
	%%%%%
	\vabs{\partial_X{g}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{5}{3}}},
	\quad & 
	%%%%%
	\vabs{\partial_Y{g}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{5}{3}}}, \\
	%%%%% %%%%%
	\vabs{\partial_W {f_1}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{3}}, 
	\quad &
	%%%%%
	\vabs{\partial_X {f_1}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{7}{3}}}, 
	\quad &
	%%%%%
	\vabs{\partial_Y {f_1}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{7}{3}}}, \\
	%%%%% %%%%
	\vabs{\partial_W {\wt{f}_2}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, 
	\quad &
	%%%%%
	\vabs{\partial_X {\wt{f}_2}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{2}}, 
	\quad &
	%%%%
	\vabs{\partial_Y{\wt{f}_2}(U,\ZInn)}
	&\leq \frac{C}{\vabs{U}^{2}},\\
	%%%% %%%%
	\vabs{\partial_W {\wt{f}_3}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{\frac{2}{3}}},
	\quad &
	%%%%
	\vabs{\partial_X{\wt{f}_3}(U,\ZInn)}
	&\leq \frac{C}{\vabs{U}^{2}},
	\quad &
	%%%%
	\vabs{\partial_Y {\wt{f}_3}(U,\ZInn)} 
	&\leq \frac{C}{\vabs{U}^{2}}.
\end{align*}
Using these results we  estimate the components of $\RRR$ in~\eqref{proof:operatorRRRInner},
\begin{align*}
	&\normInn{\RRR_1[\ZInn]}_{\frac{11}{3}} = 
	\normInn{ \frac{f_1(\cdot,\ZInn)}{1+g(\cdot,\ZInn)} }_{\frac{11}{3}}
	\leq C, 
	&\normInn{\RRR^{\Inn}_j[\ZInn]}_{\frac{4}{3}} = 
	\normInn{ \frac{\wt{f}_j(\cdot,\ZInn)}{1+g(\cdot,\ZInn)} }_{\frac{4}{3}} \leq C,
	%\quad j=2,3.
\end{align*}
for $j=2,3$. Moreover, 
\begin{align*}
	\normInn{\partial_W{\RRR_1}[\ZInn]}_{3} &= 
	\normInn{ 
		\frac{\partial_W f_1}{1+g} - 
		\frac{f_1 \partial_W g}{(1+g)^2} }_3 
	\leq C, &
	%%%%%
	\normInn{\partial_X{\RRR_1}[\ZInn]}_{\frac{7}{3}} &=
	\normInn{ \frac{\partial_X f_1}{1+g} - \frac{f_1 \partial_X g}{(1+g)^2} }_{\frac{7}{3}} 
	\leq C, \\
	%%%%%
	\normInn{\partial_W{\RRR_2}[\ZInn]}_{\frac{2}{3}} &=
	\normInn{\frac{\partial_W \wt{f}_2}{1+g} - \frac{\wt{f}_2 \partial_W g}{(1+g)^2} }_{\frac{2}{3}}  
	\leq C, &
	%%%%%
	\normInn{\partial_X{\RRR_2}[\ZInn]}_{2} &=
	\normInn{ \frac{\partial_X \wt{f}_2}{1+g} - \frac{\tl{f}_2 \partial_X g}{(1+g)^2} }_2 
	\leq C.
	%%%%%
	\end{align*}
Analogously, we obtain the rest of the estimates,
\begin{align*}
	%%%%%
	\normInn{\partial_Y{\RRR_1}[\ZInn]}_{\frac{7}{3}}, \,
	%\leq C, \h
	%%%%%
	\normInn{\partial_Y{\RRR_2}[\ZInn]}_{2}, \,
	%\leq C, \h
	%%%%%
	\normInn{\partial_W{\RRR_3}[\ZInn]}_{\frac{2}{3}}, \,
	%%%%%
	\normInn{\partial_X{\RRR_3}[\ZInn]}_{2}, \,
	%\leq C, \h
	%%%%%
	\normInn{\partial_Y{\RRR^{\Inn}_3}[\ZInn]}_{2} \leq C.
	\end{align*}
\qed

\subsubsection{Proof of Lemmas~\ref{lemma:operatorEEpotential} and \ref{lemma:operatorEEexponential}}
\label{subsubsection:innerTechnicalProofsB}

Let us introduce, for $\rhoInn>0$ and $\al\geq 0$ , the following  linear operators,  
\begin{equation}\label{def:operatorBBB}
\begin{split}
\BB_{\al}[\Psi](U)= e^{i\al U} \int_{-i\infty}^U e^{-i\al S} \Psi(S) dS, 
	\quad
\wt{\BB}[\Psi](U)= e^{-i U} \int_{-i\rhoInn}^U e^{i S} \Psi(S) dS.
\end{split}
\end{equation}

The following lemma is proven in~\cite{Bal06}.

\begin{lemma}\label{lemma:operatorBB}
	Fix $\eta>1$, $\nu>0$, $\al>0$ and $\rhoInn>1$. Then,  the following operators are well defined
	\begin{align*}
		\BB_{0}: \YcalInn_{\eta} \to \YcalInn_{\eta-1}, \qquad
		\BB_{\al}: \YcalInn_{\nu} \to \YcalInn_{\nu}, \qquad
		\wt{\BB}: \YcalInn_{\nu} \to \YcalInn_{\nu}
	\end{align*}
	and there exists a constant $C>0$  such that 
	\begin{align*}
		\normInnDiff{\BB_{0}[\Psi]}_{\eta-1} \leq C \normInnDiff{\Psi}_{\eta}, \hh
		\normInnDiff{\BB_{\al}[\Psi]}_{\nu} \leq C \normInnDiff{\Psi}_{\nu}, \hh
		\normInnDiffSmall{\wt{\BB}[\Psi]}_{\nu} \leq C \normInnDiff{\Psi}_{\nu}.
	\end{align*}
\end{lemma}

It is clear that 
$\II_1[\Psi] = \BB_{0}[\langle R_{1}, \Psi\rangle]$,
$\II_2[\Psi] = \BB_{1}[\langle R_{2}, \Psi\rangle]$ and
$\II_3[\Psi] = \wt{\BB}[\langle R_{3}, \Psi\rangle]$ (see \eqref{def:operatorRDiff} and \eqref{def:operatorEEE}).
Thus, we  use this lemma to prove Lemmas~\ref{lemma:operatorEEpotential} and \ref{lemma:operatorEEexponential}.

\begin{proof}[Proof of Lemma~\ref{lemma:operatorEEpotential}] By the definition of the operator $R$ and Lemma~\ref{lemma:boundsRRR}, we have that
\begin{equation}\label{eq:boundsRDifference}
\begin{aligned}
\normInnDiff{R_{1,1}}_3 &\leq C, 
\quad &
\normInnDiff{R_{1,2}}_{\frac{7}{3}} &\leq C , 
\quad &
\normInnDiff{R_{1,3}}_{\frac{7}{3}} &\leq C , \\
\normInnDiff{R_{j,1}}_{\frac{2}{3}} &\leq C, 
\quad &
\normInnDiff{R_{j,2}}_{2} &\leq C , 
\quad &
\normInnDiff{R_{j,3}}_{2} &\leq C , 
\quad \text{ for } j=2,3.
\end{aligned}
\end{equation}
%for $j=2,3$. 
%
Then, by Lemma~\ref{lemma:operatorBB}, for  $\rhoInn$ big enough and  $\Psi \in \YcalInn_{\frac{8}{3}} \times \YcalInn_{\frac{4}{3}} \times \YcalInn_{\frac{4}{3}}$,  we have that
\begin{equation*}%\label{proofResult:propdiff1}
\begin{split}
\normInnDiff{\II_1[\Psi]}_{\frac{8}{3}} &= 
%
\normInnDiff{\BB_{0}
[\langle R_{1}, \Psi\rangle]}_{\frac{8}{3}}
%
\leq C \normInnDiff{\langle R_{1}, \Psi\rangle}_{\frac{11}{3}}\\
%
 &\leq C \paren{
	\normInnDiff{R_{1,1}}_1 \normInnDiff{\Psi_1}_{\frac{8}{3}} +
	\normInnDiff{R_{1,2}}_{\frac{7}{3}} \normInnDiff{\Psi_2}_{\frac{4}{3}} +
	\normInnDiff{R_{1,3}}_{\frac{7}{3}} \normInnDiff{\Psi_3}_{\frac{4}{3}} }\\
	&\leq 
	C \paren{
	\frac{1}{\rhoInn^2} \normInnDiff{\Psi_1}_{\frac{8}{3}} +
	\normInnDiff{\Psi_2}_{\frac{4}{3}} +
	\normInnDiff{\Psi_3}_{\frac{4}{3}}},
	\end{split}
\end{equation*}
%Then, Lemma~\ref{lemma:operatorBB} implies
%\begin{align*}%\label{proof:estimateEE1}
%	\normInn{\EE_1[\Psi]}_{\frac{8}{3}} &= 
%	\normInn{\BB_{0}^+[\langle R_{1}, \Psi\rangle]}_{\frac{8}{3}}
%	\leq \normInn{\langle R_{1}, \Psi\rangle}_{\frac{11}{3}},
%\end{align*}
which gives the first estimate of the lemma.
%
Analogously, by Lemma~\ref{lemma:operatorBB},
\begin{align*}
\normInnDiff{\II_2[\Psi]}_{\frac{4}{3}} &= 
%
\normInnDiff{\BB_{1}[\langle R_{2}, \Psi\rangle]}_{\frac{4}{3}}
%
\leq C \normInnDiff{
\langle R_{2}, \Psi\rangle}_{\frac{4}{3}},\\
%%
\normInnDiff{\II_3[\Psi]}_{\frac{4}{3}} &=
% 
\normInnDiffSmall{\wt{\BB}[\langle R_{3}, \Psi\rangle]}_{\frac{4}{3}}
%
\leq C \normInnDiff{\langle R_{3}, \Psi\rangle}_{\frac{4}{3}},
\end{align*}
and applying~\eqref{eq:boundsRDifference},
for $j=2,3$, we have
\begin{align*}
\normInnDiff{\langle R_{j}, \Psi\rangle }_{\frac{4}{3}} &\leq
\normInnDiff{R_{j,1}}_{-\frac{4}{3}} \normInnDiff{\Psi_1}_{\frac{8}{3}} 
+
\normInnDiff{R_{j,2}}_{0} \normInnDiff{\Psi_2}_{\frac{4}{3}} 
+
\normInnDiff{R_{j,3}}_{0} \normInnDiff{\Psi_3}_{\frac{4}{3}} \\ 
%
&\leq \frac{C}{\rhoInn^2} \paren{
	\normInnDiff{\Psi_1}_{\frac{8}{3}} +
	\normInnDiff{\Psi_2}_{\frac{4}{3}} +
	\normInnDiff{\Psi_3}_{\frac{4}{3}} },
\end{align*}
which gives the second and third estimates of the lemma.
\end{proof}

%and, by Lemma~\ref{lemma:operatorBB},
%\begin{align*}
%\normInnDiff{\II_2[\Psi]}_{\frac{4}{3}} =& 
%%
%\normInnDiff{\BB_{1}[\langle R_{2}, \Psi\rangle]}_{\frac{4}{3}}
%%
%\leq \normInnDiff{
%\langle R_{2}, \Psi\rangle}_{\frac{4}{3}} 
%%
%\leq \frac{C}{\rhoInn^2}
%\normInnDiff{\Psi}_{\frac{8}{3},\frac{4}{3},\frac{4}{3}}
%\\
%%%
%\normInnDiff{\II_3[\Psi]}_{\frac{4}{3}} =&
%% 
%\normInnDiffSmall{\wt{\BB}[\langle R_{3}, \Psi\rangle]}_{\frac{4}{3}}
%%
%\leq \normInnDiff{\langle R_{3}, \Psi\rangle}_{\frac{4}{3}}
%%
%\leq \frac{C}{\rhoInn^2}
%\normInnDiff{\Psi}_{\frac{8}{3},\frac{4}{3},\frac{4}{3}}.
%\end{align*}

\begin{proof}[Proof of Lemma~\ref{lemma:operatorEEexponential}]
Let us consider $\Psi \in \ZcalInn_{\frac{4}{3},0,0}$ and define
\[
\Phi(U)=e^{i U}R(U)\Psi(U),
\]
in such a way that, by the definition of the operator $\BB_{\al}$ in~\eqref{def:operatorBBB}, 
\begin{equation}\label{proof:integralsPsiToPhi}
\begin{split}
&e^{i U} \II_1[\Psi](U) 
= e^{i U} \int_{-i \infty}^{U} 
e^{-i S} \Phi_1(S) d S 
= \BB_{1}[\Phi_1], \\
%
&e^{i U} \II_2[\Psi](U)
= e^{i2U} \int_{-i\infty}^{U}  
e^{-i2S} 
\Phi_2(S) d S
= \BB_{2}[\Phi_2]  , \\
%
&e^{i U} \II_3[\Psi](U)	= 
\int_{-i\rhoInn}^{U} \Phi_3(S) d S.
\end{split}
\end{equation}
Since $e^{iU} \Psi \in \YcalInn_{\frac{4}{3}}\times \YcalInn_{0} \times \YcalInn_{0}$, by the estimates in~\eqref{eq:boundsRDifference}, we have that, for $j=2,3$,
\begin{equation}\label{proof:estimatesh1h2h3}
\begin{split}
\normInnDiff{\Phi_1}_{\frac{7}{3}}
&\leq \normInnDiff{R_{1,1}}_{1} 
\normInnDiff{e^{iU} \Psi_1}_{\frac{4}{3}} +
\sum_{k=2,3}
\normInnDiff{R_{1,k}}_{\frac{7}{3}} \normInnDiff{e^{iU}\Psi_k}_{0} 
\leq C \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}, \\
%
\normInnDiff{\Phi_j}_{2}
&\leq \normInnDiff{R_{j,1}}_{\frac{2}{3}} \normInnDiff{e^{iU}\Psi_1}_{\frac{4}{3}} +
\sum_{k=2,3}
\normInnDiff{R_{j,k}}_{2} \normInnDiff{e^{iU}\Psi_k}_{0}
\leq C \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
\end{split}
\end{equation}
Therefore, Lemma~\ref{lemma:operatorBB} and  \eqref{proof:integralsPsiToPhi} imply
\begin{equation*}
\begin{split}
\normInnDiffExp{\II_1[\Psi]}_{\frac{7}{3}}
&= \normInnDiff{\BB_{1}[\Phi_1]}_{\frac{7}{3}}
\leq C \normInnDiff{\Phi_1}_{\frac{7}{3}}
\leq C \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}
, \\
%
\normInnDiffExp{\II_2[\Psi]}_{2}
&= \normInnDiff{\BB_{2}[\Phi_2]}_{2}
\leq C \normInnDiff{\Phi_2}_{2}
\leq C\normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
\end{split}
\end{equation*}
Now, we deal with operator $\II_3$. 
%
Notice that, 
by the definition of the operator $\BB_{\al}$ in~\eqref{def:operatorBBB} and \eqref{proof:integralsPsiToPhi}, we have that
\begin{equation*}%\label{proofDiff:decompositionh3}
e^{i U} \II_3[\Psi](U) =
\int_{-i\rhoInn}^{-i\infty} \Phi_3(S) d S +
\int_{-i\infty}^{U} \Phi_3(S) d S 
= -\BB_0[\Phi_3](-i\kappa)
+ \BB_0[\Phi_3](U).
\end{equation*}
%Then, since $\Phi_3 \in \YcalInn_{2}$, we have that
%\begin{align}\label{proof:resultIntegralAsymptotics}
%\vabs{\BB_0[\Phi_3](U)}
%%
%\leq \int_{-i\infty}^0 \vabs{\Phi_3(U+iS)} dS
%%
%\leq \normInnDiff{\Phi_3}_2 
%\int_{-i\infty}^0 \frac{dS}{\vabs{U + iS}^2} dS 
%%
%= \frac{\pi}{2}\frac{\normInnDiff{\Phi_3}_2}{\vabs{U}},
%\end{align}
%and hence
%\begin{equation*}
%\vabs{e^{i U} \II_3[\Psi](U)} \leq
%C \normInnDiff{\Phi_3}_2
%	\paren{ \frac{1}{\rhoInn} + \frac{1}{\vabs{U}}}.
%\end{equation*}
Then, by Lemma~\ref{lemma:operatorBB} and using the estimates~\eqref{proof:estimatesh1h2h3}, we obtain
\begin{align*}
\normInnDiffExp{\II_3[\Psi]}_{0} 
%
&\leq \vabs{\BB_0[\Phi_3](-i\kappa)} + \normInnDiff{\BB_0[\Phi_3]}_0
%
\leq 2 \normInnDiff{\BB_0[\Phi_3]}_0 \\
%
&\leq \frac{C}{\kappa} \normInnDiff{\BB_0[\Phi_3]}_1
%
\leq \frac{C}{\rhoInn} \normInnDiff{\Phi_3}_2
%
\leq \frac{C}{\rhoInn} \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
\end{align*}
Finally, taking $\wCInn(\rhoInn)=-\BB_0[\Phi_3](-i\kappa)$, we conclude
\begin{equation*}
\normInnDiffExp{\II_3[\Psi](U)-e^{-iU}\wCInn(\rhoInn)}_1
%
= \normInnDiff{\BB_0[\Phi_3]}_1
%
\leq C \normInnDiff{\Phi_3}_2 
%
\leq C \normInnDiffExp{\Psi}_{\frac{4}{3},0,0}.
\end{equation*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%CALCULS


%	\begin{align*}
%	&\vabs{\Dx{h}{U}(U,\ZInn)} =
%	\left|
%	-\frac{2^3}{3^3} U^{-\frac{5}{3}} \WInn^2 
%	+\frac{2^6}{3^4} U^{-\frac{7}{3}} \WInn 
%	-\frac{2^5}{3^4} U^{-3} 
%	%
%	+\frac{8i}{9} U^{-\frac{5}{3}} (\XInn-\YInn) 
%	\right. \\ &\phantom{\vabs{\Dx{h}{U}(U,\zeta)} =} \h \left.
%	-\frac{4}{9} U^{-2}\WInn(\XInn+\YInn)  
%	+\frac{40}{3^4} U^{-\frac{8}{3}}(\XInn+\YInn) 
%	%
%	+\frac{4}{9} U^{-\frac{7}{3}}(\XInn^2 + \YInn^2) 
%	\right. \\ &\phantom{\vabs{\Dx{h}{U}(U,\zeta)} =} \h \left.
%	-\frac{40}{3^3} U^{-\frac{7}{3}} \XInn \YInn \right|
%	%
%	\leq \frac{C}{\vabs{U}^{3}}, \\
%	%%%%
%	&\vabs{\Dx{h}{W}(U,\ZInn)} =
%	\vabs{ \frac{8}{9}U^{-\frac{2}{3}} \WInn - \frac{16}{27} U^{-\frac{4}{3}} +\frac{4}{9} U^{-1}(\XInn+\YInn)
%	} \leq \frac{C}{\vabs{U}^{\frac{4}{3}}}, \\
%	%%%%
%	&\vabs{\Dx{h}{X}(U,\ZInn)} =
%	\vabs{ -\frac{4i}{3} U^{-\frac{2}{3}} +\frac{4}{9}U^{-1}\WInn
%		-\frac{8}{27}U^{-\frac{5}{3}}-
%		\frac{2}{3}U^{-\frac{4}{3}}\XInn + \frac{10}{9} U^{-\frac{4}{3}} \YInn
%	} \leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, \\
%	%%%%
%	&\vabs{\Dxy{h}{U}{W}(U,\ZInn)} =
%	\vabs{ -\frac{2^4}{3^3}U^{-\frac{5}{3}} \WInn + 
%		\frac{2^6}{3^4} U^{-\frac{7}{3}} -\frac{4}{9} U^{-2}(\XInn+\YInn)
%	} \leq \frac{C}{\vabs{U}^{\frac{7}{3}}}, \\
%	%%%%
%	&\vabs{\Dxy{h}{U}{X}(U,\ZInn)} =
%	\vabs{\frac{8i}{9} U^{-\frac{5}{3}} 
%		-\frac{4}{9}U^{-2}\WInn
%		+\frac{40}{3^4}U^{-\frac{8}{3}}
%		+\frac{8}{9}U^{-\frac{7}{3}}\XInn 
%		- \frac{40}{3^3} U^{-\frac{7}{3}} \YInn
%	} \leq \frac{C}{\vabs{U}^{\frac{5}{3}}}, \\
%	%	\end{align*}
%	%	\begin{align*}
%	%%%%
%	&\vabs{\Dxx{h}{W}(U,\ZInn)} =
%	\vabs{ \frac{8}{9}U^{-\frac{2}{3}}
%	} \leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, \hh
%	%%%%
%	\vabs{\Dxy{h}{W}{X}(U,\ZInn)} =
%	\vabs{\frac{4}{9} U^{-1}} \leq 
%	\frac{C}{\vabs{U}}, \\
%	%%%%
%	&\vabs{\Dxx{h}{X}(U,\ZInn)} =
%	\vabs{ -\frac{2}{3}U^{-\frac{4}{3}}}
%	\leq \frac{C}{\vabs{U}^{\frac{4}{3}}},\hh
%	%%%%
%	\vabs{\Dxy{h}{X}{Y}(U,\ZInn)} =
%	\vabs{ \frac{10}{9} U^{-\frac{4}{3}}} \leq 
%	\frac{C}{\vabs{U}^{\frac{4}{3}}}, 
%	\end{align*}
%	Analogously, we have
%	\begin{align*}
%	&\vabs{\partial_Y{h}(U,\ZInn)}  
%	\leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, 
%	%%%%
%	&\vabs{\partial_{UY}{h}(U,\ZInn)} 
%	\leq \frac{C}{\vabs{U}^{\frac{5}{3}}}, 
%	%%%%
%	&\vabs{\partial_{WY}{h}(U,\ZInn)}  
%	\leq \frac{C}{\vabs{U}}, 
%	%%%%
%	&\vabs{\partial_{Y^2}{h}(U,\ZInn)}
%	\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}.
%	\end{align*}


%	\begin{align*}
%	&\vabs{g^{\Inn}(U,\ZInn)} =
%	\vabs{\frac{3}{2}U^{\frac{2}{3}}\WInn -\frac{U^{-\frac{2}{3}}}{6}\frac{(\partial_W h)}{(1+h)^{\frac{3}{2}}}}
%	\leq \frac{C}{\vabs{U}^2}, \hh 
%	%
%	\vabs{1+g^{\Inn}(U,\ZInn)} \geq 1-\frac{C}{\rhoInn^2}\geq \frac{1}{2}, \\
%	%
%	&\vabs{\Dx{g^{\Inn}}{W}(U,\ZInn)} =
%	\vabs{\frac{3}{2}U^{\frac{2}{3}}
%		+\frac{U^{-\frac{2}{3}}}{4}\frac{(\partial_W h)^2}{(1+h)^{\frac{5}{2}}}
%		-\frac{U^{-\frac{2}{3}}}{6}\frac{(\partial^2_{W^2} h)}{(1+h)^{\frac{3}{2}}}}
%	\leq  C \vabs{U}^{\frac{2}{3}}, & \\
%	%
%	&\vabs{\Dx{g^{\Inn}}{X}(U,\ZInn)} =
%	\vabs{\frac{U^{-\frac{2}{3}}}{4}\frac{(\partial_W h)(\partial_X h)}{(1+h)^{\frac{5}{2}}}
%		-\frac{U^{-\frac{2}{3}}}{6}\frac{(\partial^2_{WX} h)}{(1+h)^{\frac{3}{2}}}
%	}
%	\leq \frac{C}{\vabs{U}^{\frac{5}{3}}},\hh 
%	%
%	\vabs{\Dx{g^{\Inn}}{Y}(U,\ZInn)} 
%	\leq \frac{C}{\vabs{U}^{\frac{5}{3}}}.
%\end{align*}
%For the bounds of $f^{\Inn}_1=-\partial_U \KK$ we have,
%\begin{align*}
%	&\vabs{f^{\Inn}_1(U,\ZInn)} =
%	\vabs{\frac{1}{2} U^{-\frac{1}{3}} \WInn^2 
%		-\frac{2}{9} U^{-\frac{5}{3}} \frac{h}{\sqrt{1+h}(\sqrt{1+h}+1)}
%		+\frac{1}{6}U^{-\frac{2}{3}} \frac{(\partial_U h)}{(1+h)^{\frac{3}{2}}}
%	} \leq \frac{C}{\vabs{U}^{\frac{11}{3}}}, \\
%	%
%	&\vabs{\Dx{f^{\Inn}_1}{W}(U,\ZInn)} =
%	\vabs{ U^{-\frac{1}{3}}\WInn 
%		+\frac{U^{-\frac{5}{3}}}{9}\frac{(\partial_W h)}{(1+h)^{\frac{3}{2}}}
%		-\frac{U^{-\frac{2}{3}}}{6}\frac{(\partial^2_{UW} h)}{(1+h)^{\frac{3}{2}}}
%		+\frac{U^{-\frac{2}{3}}}{4}
%		\frac{(\partial_W h)(\partial_U h)}{(1+h)^{\frac{5}{2}}}}
%	\leq \frac{C}{\vabs{U}^{3}}, \\
%	%
%	&\vabs{\Dx{f^{\Inn}_1}{X}(U,\ZInn)} =
%	\vabs{
%		\frac{U^{-\frac{5}{3}}}{9} \frac{(\partial_X h)}{(1+h)^{\frac{3}{2}}}-+\frac{U^{-\frac{2}{3}}}{6} \frac{(\partial^2_{UX} h)}{(1+h)^{\frac{3}{2}}}
%		+\frac{U^{-\frac{2}{3}}}{4} \frac{(\partial_{X} h)(\partial_U h)}{(1+h)^{\frac{5}{2}}}
%	} 
%	\leq \frac{C}{\vabs{U}^{\frac{7}{3}}}, \\
%	%
%	&\vabs{\Dx{f^{\Inn}_1}{Y}(U,\ZInn)} \leq \frac{C}{\vabs{U}^{\frac{7}{3}}}.
%\end{align*}
%For the bounds of $\tl{f}^{\Inn}_2$, with $f_2^{\Inner}=i\partial_{Y} \KK$, we obtain,
%\begin{align*}
%	&\vabs{\tl{f}^{\Inn}_2(U,\ZInn)} =
%	\vabs{i\frac{U^{-\frac{2}{3}}}{6} \frac{(\partial_Y h)}{(1+h)^{\frac{3}{2}}}
%		-i\XInn g}
%	\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}, \\
%	%
%	&\vabs{\Dx{\tl{f}^{\Inn}_2}{W}(U,\ZInn)} =
%	\vabs{i\frac{U^{-\frac{2}{3}}}{6} \frac{(\partial^2_{WY} h)}{(1+h)^{\frac{3}{2}}}
%		-i\frac{U^{-\frac{2}{3}}}{4} \frac{(\partial_{W} h)(\partial_{Y} h)}{(1+h)^{\frac{5}{2}}}
%		-i\XInn \partial_w g}
%	\leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, \\
%	%
%	&\vabs{\Dx{\tl{f}^{\Inn}_2}{X}(U,\ZInn)} =
%	\vabs{i\frac{U^{-\frac{2}{3}}}{6} \frac{(\partial^2_{XY} h)}{(1+h)^{\frac{3}{2}}}
%		-i\frac{U^{-\frac{2}{3}}}{4} \frac{(\partial_Y h)(\partial_X h)}{(1+h)^{\frac{5}{2}}}
%		-ig
%		-i \XInn \partial_X g}
%	\leq \frac{C}{\vabs{U}^{2}}, \\
%	%
%	&\vabs{\Dx{\tl{f}^{\Inn}_2}{Y}(U,\ZInn)} =
%	\vabs{i\frac{U^{-\frac{2}{3}}}{6} \frac{(\partial^2_{Y^2} h)}{(1+h)^{\frac{3}{2}}}
%		-i\frac{U^{-\frac{2}{3}}}{4} \frac{(\partial_Y h)^2}{(1+h)^{\frac{5}{2}}}
%		-i\XInn \partial_Y g}
%	\leq \frac{C}{\vabs{U}^{2}}.
%\end{align*}
%Analogously, we obtain the following estimates for $\tl{f}^{\Inn}_3$,
%\begin{align*}
%	\vabs{\tl{f}^{\Inn}_3(U,\ZInn)} 
%	\leq \frac{C}{\vabs{U}^{\frac{4}{3}}}, \h \h
%	%
%	\vabs{\Dx{\tl{f}^{\Inn}_3}{W}(U,\ZInn)} 
%	\leq \frac{C}{\vabs{U}^{\frac{2}{3}}}, \h \h
%	%
%	\vabs{\Dx{\tl{f}^{\Inn}_3}{X}(U,\ZInn)}
%	\leq \frac{C}{\vabs{U}^{2}}, \h \h
%	%
%	\vabs{\Dx{\tl{f}^{\Inn}_3}{Y}(U,\ZInn)} 
%	\leq \frac{C}{\vabs{U}^{2}}.
%\end{align*}
%Therefore, using these results we can bound $\RRR^{\Inn}$. That is, for $i=2,3$, we have
%\begin{align*}
%	&\normInn{\RRR^{\Inn}_1[\ZInn]}_{\frac{11}{3}} = 
%	\sup_{U \in \DInn} \vabs{ 
%		{U}^{\frac{11}{3}}
%		\frac{f^{\Inn}_1}{1+g^{\Inn}} } 
%	\leq C, 
%	&\normInn{\RRR^{\Inn}_i[\ZInn]}_{\frac{4}{3}} = 
%	\sup_{U \in \DInn} \vabs{ 
%		{U}^{\frac{4}{3}}
%		\frac{\tl{f}^{\Inn}_i}{1+g^{\Inn}} } \leq C.
%\end{align*}

%	Moreover, 
%\begin{align*}
%	&\normInn{\Dx{\RRR^{\Inn}_1}{W}[\ZInn]}_{3} = 
%	\sup_{U \in \DInn} \vabs{ 
%		{U}^3 \left(
%		\frac{\partial_W f^{\Inn}_1}{1+g^{\Inn}} - \frac{f^{\Inn}_1 \partial_W g^{\Inn}}{(1+g^{\Inn})^2}\right) } 
%	\leq C, \\
%	%%%%%
%	&\normInn{\Dx{\RRR^{\Inn}_1}{X}[\ZInn]}_{\frac{7}{3}} =
%	\sup_{U \in \DInn} \vabs{ U^{\frac{7}{3}}
%		\left(\frac{\partial_X f^{\Inn}_1}{1+g^{\Inn}} - \frac{f^{\Inn}_1 \partial_X g^{\Inn}}{(1+g^{\Inn})^2}\right) } 
%	\leq C, \\
%	%%%%%
%	&\normInn{\Dx{\RRR^{\Inn}_2}{W}[\ZInn]}_{\frac{2}{3}} =
%	\sup_{U \in \DInn} \vabs{ U^{\frac{2}{3}}
%		\left(\frac{\partial_W \tl{f}^{\Inn}_2}{1+g^{\Inn}} - \frac{\tl{f}^{\Inn}_2 \partial_W g^{\Inn}}{(1+g^{\Inn})^2}\right) }  
%	\leq C, \\
%	%%%%%
%	&\normInn{\Dx{\RRR^{\Inn}_2}{X}[\ZInn]}_{2} =
%	\sup_{U \in \DInn} \vabs{ U^{2}
%		\left(\frac{\partial_X \tl{f}^{\Inn}_2}{1+g^{\Inn}} - \frac{\tl{f}^{\Inn}_2 \partial_X g^{\Inn}}{(1+g^{\Inn})^2}\right) }  
%	\leq C.
%	%%%%%
%	%&\normInn{\Dx{\EE_2}{Y}[\zeta]}_{0} =
%	%\sup_{U \in \DInn} \vabs{
%	%	\frac{\partial_Y \wt{f}_2}{g} - \frac{\wt{f}_2 \partial_Y g}{g^2}} 
%	% \leq \frac{C}{\rhoInn^2}.
%\end{align*}
%Analogously, we can obtain the rest of the bounds:
%\begin{align*}
%	%%%%%
%	\normInn{\Dx{\RRR^{\Inn}_1}{Y}[\ZInn]}_{\frac{7}{3}},
%	%\leq C, \h
%	%%%%%
%	\normInn{\Dx{\RRR^{\Inn}_2}{Y}[\ZInn]}_{2}, 
%	%\leq C, \h
%	%%%%%
%	\normInn{\Dx{\RRR^{\Inn}_3}{W}[\ZInn]}_{\frac{2}{3}}, %\leq C, \h
%	%%%%%
%	\normInn{\Dx{\RRR^{\Inn}_3}{X}[\ZInn]}_{2},
%	%\leq C, \h
%	%%%%%
%	\normInn{\Dx{\RRR^{\Inn}_3}{Y}[\ZInn]}_{2} \leq C.
%\end{align*}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Proof of Lemma~\ref{lemma:firstIterationInner}}
%
%%\begin{proof}%[Proof of Lemma~\ref{lemma:firstIterationInner}]
%	By the definition of operator $\FF$ on~\eqref{def:operatorFF}, we have that
%	\begin{align*}%\label{eq:expressionF0}
%	\FF[0](U) =  
%	\GG \left( 
%	\frac{-\partial_U \KK}
%	{1+ \partial_W{\KK}},
%	\frac{i\partial_Y \KK}
%	{1+ \partial_W{\KK}},
%	\frac{-i\partial_X \KK}
%	{1+ \partial_W{\KK}}
%	\right)(U,0,0,0).
%	\end{align*}
%	where $\KK$ is stated on~\eqref{def:hamiltonianK}.
%	We proceed first by bounding the derivatives of $h(U,0,0,0)$, as defined on~\eqref{def:hFunction}. Then, by inequality~\eqref{eq:UBounds} and assuming $\rhoInn=\rhoInn(\beta_0)>0$ big enough, we have 
%	\begin{align*}
%	&\vabs{h(U,0,0,0)} = 
%	\vabs{1+\frac{16}{81}U^{-2}} \geq 1 - \frac{C}{\rhoInn^2} \geq \frac{1}{2}, \\
%	%
%	&\vabs{1-h(U,0,0,0)} = 
%	\vabs{-\frac{16}{81}U^{-2}} \leq \frac{C}{\vabs{U}^2}, \\
%	%
%	&\vabs{\partial_W h(U,0,0,0)} =
%	\vabs{-\frac{16}{27} U^{-4/3}} \leq \frac{C}{\vabs{U}^{4/3}}, \\
%	%
%	&\vabs{\partial_X h(U,0,0,0)} =
%	\vabs{\frac{4i}{3}U^{-2/3} +\frac{8}{27}U^{-5/3}} \leq \frac{C}{\vabs{U}^{2/3}}, \\
%	%
%	&\vabs{\partial_Y h(U,0,0,0)} =
%	\vabs{-\frac{4i}{3}U^{-2/3} +\frac{8}{27}U^{-5/3}} \leq \frac{C}{\vabs{U}^{2/3}}.
%	\end{align*}
%	Then, we obtain
%	\begin{align*}
%	\vabs{\Dx{\KK}{W}(U,0,0,0)} 
%	%=\vabs{\frac{U^{-2/3}}{6} 
%	%	\frac{\partial_W h(U,0,0,0)}{h(U,0,0,0)^{3/2}}} 
%	\leq \frac{C}{\vabs{U}^{2}}
%	\leq \frac{C}{\rhoInn^2}, 
%	\end{align*}
%	%	\begin{align*}
%	%	\vabs{\KK(U,0,0,0)} \leq \vabs{
%	%		\frac{U^{-2/3}}{3} 
%	%		\frac{(1 -h)}{\sqrt{h}\left(1+\sqrt{h} \right)}}
%	%	\leq \frac{C}{U^{8/3}}
%	%	\end{align*}
%	and,
%	\begin{align*}
%	&\vabs{\Dx{\KK}{U}(U,0,0,0)}  
%	%\leq \vabs{\Dx{}{U} \paren{	
%	%\frac{U^{-2/3}}{3} 
%	%\frac{(1 -h)}{\sqrt{h}\left(1+\sqrt{h} \right)}}}
%	\leq \frac{C}{U^{11/3}} \hh
%	&\vabs{\Dx{\KK}{X}(U,0,0,0)} 
%	%=\vabs{\frac{U^{-2/3}}{6} 
%	%	\frac{\partial_X h(U,0,0,0)}{h(U,0,0,0)^{3/2}}} 
%	\leq\frac{C}{\vabs{U}^{4/3}} , \hh
%	%
%	&\vabs{\Dx{\KK}{Y}(U,0,0,0)} 
%	%=\vabs{\frac{U^{-2/3}}{6} 
%	%	\frac{\partial_Y h(U,0,0,0)}{h(U,0,0,0)^{3/2}}} 
%	\leq \frac{C}{\vabs{U}^{4/3}} .
%	\end{align*}
%	Therefore, for $\rhoInn>0$ big enough such that $\vabs{1+ \partial_W{\KK}} \geq \frac{1}{2}$ and Lemma~\ref{lemma:Glipschitz}, we obtain the statement of the Lemma.

%\subsubsection{Proof of Lemma~\ref{lemma:FLipschitzInner}}
%
%	We have that $\FF = \GG \circ \RRR$, where $\RRR$ and $\GG$ are the operators given in~\eqref{def:operatorRRRInner} and~\eqref{def:operatorGG}, respectively. Operator $\GG$ is characterized on Lemma~\ref{lemma:Glipschitz}. Thus, we focus on bounding each component $\RRR_i[\ZInn]-\RRR_i[\ZInnB]$ separately. Considering $\ZInn, \ZInnB \in B(R_+) \subset \XcalInnTotal$, by the mean value theorem we have
%	\begin{align*}
%	\RRR_i[\ZInn]-\RRR_i[\ZInnB] 
%	&=\int_0^1 \Dx{\RRR_i}{W}[s \ZInn + (1-s) \ZInnB] (\WInn - \WInnB) d s \\
%	&+\int_0^1 \Dx{\RRR_i}{X}[s \ZInn + (1-s) \ZInnB] (\XInn - \XInnB) d s \\
%	&+\int_0^1 \Dx{\RRR_i}{Y}[s \ZInn + (1-s) \ZInnB] (\YInn - \YInnB) d s .
%	\end{align*}
%	Since $\big( s \ZInn + (1-s) \ZInnB\big) \in B(R_+)$ for all $s \in [0,1]$, by Lemma~\ref{lemma:sumNorms}, we have
%	\begin{equation*}
%	\begin{split}
%	\normInn{\RRR_1[\ZInn]-\RRR_1[\ZInnB]}_{\frac{11}{3}} &\leq
%	\sup_{\zeta \in B(R_+)} \left\{ \normInn{\Dx{\RRR_1}{W}[\zeta]}_{1} \right\}
%	\normInn{\WInn - \WInnB}_{\frac{8}{3}}  \\
%	%
%	&+  \sup_{\zeta \in B(R_+)} \left\{ \normInn{\Dx{\RRR_1}{X}[\zeta]}_{\frac{7}{3}} \right\} \normInn{\XInn - \XInnB}_{\frac{4}{3}} \\
%	%
%	&+ \sup_{\zeta \in B(R_+)} \left\{
%	\normInn{\Dx{\RRR_1}{Y}[\zeta]}_{\frac{7}{3}} \right\} \normInn{\YInn - \YInnB}_{\frac{4}{3}}.
%	\end{split}
%	\end{equation*}
%	Then, by taking $\rhoInn(\beta_0)>0$ big enough and  applying Lemmas~\ref{lemma:sumNorms} and~\ref{lemma:boundsRRR} we obtain
%	\begin{align*}
%	\normInn{{\RRR_1}[\ZInn]-{\RRR_1}[\ZInnB]}_{\frac{11}{3}} \leq C
%	\left( \frac{1}{\rhoInn^2} \normInn{\WInn - \WInnB}_{\frac{8}{3}} 
%	+ \normInn{\XInn - \XInnB}_{\frac{4}{3}}
%	+ \normInn{\YInn - \YInnB}_{\frac{4}{3}} \right),
%	\end{align*}
%	and applying Lemma~\ref{lemma:Glipschitz} we obtain~\eqref{result:F1Lipschitz}. Analogously, for $i=2,3$ we have
%	\begin{equation*}
%	\begin{split}
%	\normInn{\RRR_i[\ZInn]-\RRR_i[\ZInnB]}_{\frac{4}{3}} &\leq
%	%
%	\sup_{\zeta \in \BB(b)} \left\{  \normInn{\Dx{\RRR_i}{W}[\zeta]}_{-\frac{4}{3}} \right\} 
%	\normInn{\WInn - \WInnB}_{\frac{8}{3}} \\
%	%
%	&+ \sup_{\zeta \in \BB(b)} \left\{  \normInn{\Dx{\RRR_i}{X}[\zeta]}_{0} \right\}
%	\normInn{\XInn - \XInnB}_{\frac{4}{3}} \\
%	%
%	&+ \sup_{\zeta \in \BB(b)} \left\{  \normInn{\Dx{\RRR_i}{Y}[\zeta]}_{0} \right\}
%	\normInn{\YInn - \YInnB}_{\frac{4}{3}}.
%	\end{split}
%	\end{equation*}
%	Then, by taking $\rhoInn(\beta_0)>0$ big enough, we have
%	\begin{align*}
%	&\normInn{{\RRR_i}[\ZInn]-{\RRR_i}[\ZInnB]}_{\frac{4}{3}} \leq \frac{C}{\rhoInn^2} \normInnTotal{\ZInn - \ZInnB},
%	\end{align*}
%	and applying Lemma~\ref{lemma:Glipschitz} we obtain~\eqref{result:F23Lipschitz}.



==> Article Inner/proofE-lemmaDomainSeparatrix.tex <==
\subsection{Proof of Proposition~\ref{proposition:domainSeparatrix}}
\label{subsection:propZeroes}

For $t \in \reals$, $\La_h(t)$ satisfies $\La_h(t)=0$ if and only if $t=0$ (see Figure~\ref{fig:separatrix}).
%
To prove Proposition~\ref{proposition:domainSeparatrix}, we  follow the same techniques used in the proof of Theorem~\ref{theorem:singularities}.

%\paragraph{Change of variables.}
%
%\paragraph{Classification of zeroes.}
Let us consider $q(t)=\cos(\frac{\la_h(t)}{2})$ as introduced in Theorem~\ref{theorem:singularitiesChangeq}. Then, by~\eqref{eq:equationLahSimplified},
\begin{equation*}
%\label{eq:LahFromq}
\La_h^2(t) = \frac{4}{3 q(t)} 
\big(1-q(t)\big)
\big(q(t)-a_+\big)
\big(q(t)-a_-\big).
\end{equation*}
Let $\La_h(t^*) = 0$ for a given $t^*$. Then, defining $q^*=q(t^*)$, we have three options:
\begin{equation*}%\label{eq:casesZeroes}
q^*=1,a_+,a_-.
% \quad \text{and} \quad
% \vabs{q^*} \to \infty.
\end{equation*}
%\paragraph{Classification of zeroes.}
%These cases have already been examined on Proposition \ref{proposition:singularitiesSeparatrix}.
%
We have seen that 
% $\vabs{q^*} \to \infty$ corresponds to a pole of order $1$,  (see~\eqref{eq:singularitatExpressioInfinit}), and 
$q^*=1$ corresponds to the saddle equilibrium point, namely $\vabs{t^*}\to \infty$, (see~\eqref{proof:classificationSaddle}).
%
Therefore, it cannot lead to zeroes of $\La_h(t)$.
%
On the contrary, $q^*=a_{\pm}$ leads to zeroes of $\La_h(t)$, since we have seen that $q(t)$ is well defined and analytic in a neighborhood of such $t^*$ (see~\eqref{proof:qexpressionZeroes}).

%\paragraph{Computation of visible zeroes.}
To prove Proposition~\ref{proposition:domainSeparatrix} it only remains to compute all possible values of $t^* \in \ol{\Pi_A}$ such that $q^*=q(t^*)$ with $q^*=a_+,a_-$.
%
To do so, we use the techniques and results presented in Section~\ref{subsection:computationSingularities}.

From now on, we consider integration paths $\g:(s_{\ini}, s_{\fin}) \to \mathscr{R}_f$ with initial point $\lim_{s \to s_{\ini}} \g(s) = (a_+,0)$ and endpoint 
$\lim_{s \to s_{\ini}} \proj \g(s) = q^*=a_\pm$.
%
Moreover, we say that a zero $t^*$ of $\La_h$ is \emph{visible} if there exist a path $\g$ such that  $t^* = t^*(\g) \in \ol{\Pi_A}$ and $T[\g](s) \in \Pi_A$ for $s\in[s_{\ini},s_{\fin})$,  (see~\eqref{def:operatorT} and~\eqref{def:operatorSingularities}).
%
% Therefore, we need to compute $t^*(\g)$ for all possible paths and check if they are visible zeroes.

%
First, we recall some of the results obtained in Sections~\ref{subsubsection:pathsB} and~\ref{subsubsection:pathsC}.
\begin{itemize}
\item Consider $q_1 \in (-\infty, a_-) \cup (a_-,-1) \cup (1,+\infty)$. In the proofs of Lemmas~\ref{lemma:caminsPol}, \ref{lemma:caminsNegatius2}, \ref{lemma:caminsBranca2} and
\ref{lemma:caminsBranca1c} we have seen that
\begin{align}\label{proof:integralNotInPiA}
	\vabs{\Im \int_{a_+}^{q_1} \fh d\g} > A.
\end{align}
%
\item Consider $q_1\in(-1,0)$. In the proofs of Lemmas~\ref{lemma:caminsNegatius1} and~\ref{lemma:caminsBranca1c}, we have seen that
\begin{align}\label{proof:integralNotInPiA2}
	\vabs{\Im \int_{a_+}^{q_1} \fh d\g} = A.
\end{align}
\end{itemize}
Now, we classify the paths depending on its endpoint $q^*$.
\begin{enumerate}
\item Consider $q^*=a_-$.
Analogously to the proof of \eqref{proof:integralNotInPiA}, it can be seen that
\[
\vabs{\Im t^*(\g)} = 
\vabs{\Im \int_{a_+}^{a_-} \fh d\g} >A.
\]
Therefore, $q^*=a_-$ does not lead to any visible zero.

\item Consider $q^*=a_+$.
% 
Notice that, by~\eqref{proof:integralNotInPiA} and~\eqref{proof:integralNotInPiA2},
any path crossing $\reals\setminus[0,1]$ leads to non-visible zeroes. 
%
Therefore, we only consider paths $\g$ either crossing $(0,1)$ or not crossing $\reals$.

Since in $(0,1)$ the only singularity of $\fh(q)$ is the branching point $q=a_+$, there exists a homotopic path $\eta=\eta^1 \vee \eta^2 \vee \eta^3$ defined by
\begin{equation*}
\begin{cases}
	\eta^1(q) = (q,0) & 
	\text{ with } q \in (a_+,a_+ + \e], \\
	%
	\proj \eta^2(\phi) = a_+ + \e e^{i\phi} & 
	\text{ with } \phi \in [0, 2\pi k], \\
	%
	\proj \eta^3(q) = q & 
	\text{ with } q \in [a_+ + \e, a_+), 
\end{cases}
\end{equation*}
for some $k \in \integers$ and $\e>0$ small enough. Then,
\begin{equation*}
t^*(\g) = \int_{a_+}^{a_+} \fh d \g = 
\lim_{\e \to 0} \int_{\eta} \fh(q) dq = 0.
\end{equation*}
Therefore, these paths lead to the only visible zero $t^*=0$.
\end{enumerate}
\qed


==> Article Inner/shortcuts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LATEX SPECIFIC SHORTCUTS %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% BASICS %%%
\newcommand{\unstable}{{\mathrm{u}}}
\newcommand{\stable}{{\mathrm{s}}}
\newcommand{\stableun}{^{\mathrm{u},\mathrm{s}}}

%%%% CHANGE VARIABLES %%%
\newcommand{\HInicial}{h}
\newcommand{\rot}{\mathrm{rot}}
\newcommand{\pol}{\mathrm{pol}}
\newcommand{\Del}{\mathrm{Del}}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\sca}{\mathrm{sc}}
\newcommand{\equi}{\mathrm{eq}}
\newcommand{\osc}{\mathrm{osc}}
\newcommand{\pend}{\mathrm{p}}
\newcommand{\lh}{\hat{\lambda}}
\newcommand{\Lh}{\hat{\Lambda}}
\newcommand{\xh}{x}
\newcommand{\xp}{x}
\newcommand{\yh}{y}
\newcommand{\yp}{y}
% L3
\newcommand{\Ltres}{\mathfrak{L}}
\newcommand{\LtresLa}{\mathfrak{L}_{\Lambda}}
\newcommand{\Ltresx}{\mathfrak{L}_x}
\newcommand{\Ltresy}{\mathfrak{L}_y}

%%%% SINGULARITIES %%%
\newcommand{\fh}{\hat{f}}
\newcommand{\vap}{\rho}
\newcommand{\proj}{\mathtt{p}}
\newcommand{\ini}{0}
\newcommand{\fin}{\mathrm{end}}
\newcommand{\argf}{\mathtt{g}}

%%%% INNER SPACE %%%
\newcommand{\inn}{\mathrm{in}}
\newcommand{\Inn}{\mathrm{in}}
\newcommand{\Inner}{{\mathrm{in}}}
\newcommand{\rhoInn}{\kappa}
\newcommand{\CInn}{\Theta}
\newcommand{\wCInn}{\widetilde{\Theta}}
% Domain
\newcommand{\DInn}{\mathcal{D}_{\rhoInn}}
\newcommand{\DInnR}[1]{\mathcal{D}_{#1}}
\newcommand{\DuInn}{\mathcal{D}^{\mathrm{u}}_{\rhoInn}}
\newcommand{\DuInnR}[1]{\mathcal{D}^{\mathrm{u}}_{#1}}
\newcommand{\DsInn}{\mathcal{D}^{\mathrm{s}}_{\rhoInn}}
\newcommand{\DusInn}{\mathcal{D}^{\mathrm{u/s}}_{\rhoInn}}
\newcommand{\DdInn}{\mathcal{D}^{\diamond}_{\rhoInn}}
\newcommand{\DusInnR}[1]{\mathcal{D}^{\mathrm{u/s}}_{\rhoInn_{#1}}}
\newcommand{\EInn}{\mathcal{E}_{\rhoInn}}
\newcommand{\EInnR}[1]{\mathcal{E}_{\rhoInn_{#1}}}
% Domain Outer
\newcommand{\DuInnOut}{{D}^{\mathrm{in,u}}_{\rhoInn}}
\newcommand{\DsInnOut}{{D}^{\mathrm{in,s}}_{\rhoInn}}
\newcommand{\DusInnOut}{{D}^{\mathrm{in,u/s}}_{\rhoInn}}
\newcommand{\DdInnOut}{{D}^{\mathrm{in},\diamond}_{\rhoInn}}
% Banach Spaces
\newcommand{\XcalInn}{\mathcal{X}}
\newcommand{\XcalInnS}{\mathcal{X}^{\mathrm{s}}}
\newcommand{\XcalInnU}{\mathcal{X}^{\mathrm{u}}}
\newcommand{\XcalInnD}{\mathcal{X}^{\diamond}}
\newcommand{\XcalInnUS}{\mathcal{X}^{\mathrm{u/s}}}
\newcommand{\YcalInn}{\mathcal{Y}}
\newcommand{\ZcalInn}{\mathcal{Z}}
\newcommand{\XcalInnTotal}{\mathcal{X}_{\times}}
\newcommand{\XcalInnSTotal}{\mathcal{X}^{\mathrm{s}}_{\times}}
\newcommand{\XcalInnUTotal}{\mathcal{X}^{\mathrm{u}}_{\times}}
\newcommand{\XcalInnDTotal}{\mathcal{X}^{\diamond}_{\times}}
\newcommand{\XcalInnUSTotal}{\mathcal{X}^{\mathrm{u/s}}_{\times}}
\newcommand{\YcalInnTotal}{\mathcal{Y}_{\times}}
% Norms
\newcommand{\normInn}[1]{\left\lVert#1\right\rVert}
\newcommand{\normInnSmall}[1]{\lVert#1\rVert}
\newcommand{\normInnS}[1]{\left\lVert#1\right\rVert^{\mathrm{s}}}
\newcommand{\normInnU}[1]{\left\lVert#1\right\rVert^{\mathrm{u}}}
\newcommand{\normInnD}[1]{\left\lVert#1\right\rVert^{\diamond}}
\newcommand{\normInnUS}[1]{\left\lVert#1\right\rVert^{\mathrm{u/s}}}
\newcommand{\normInnTotal}[1]{\left\lVert#1\right\rVert_{\times}}
\newcommand{\normInnTotalSmall}[1]{\lVert#1\rVert_{\times}}
\newcommand{\normInnUSTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{u/s}}_{\times}}
\newcommand{\normInnDTotal}[1]{\left\lVert#1\right\rVert^{\diamond}_{\times}}
\newcommand{\normInnUTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{u}}_{\times}}
\newcommand{\normInnExp}[1]{\left\lVert#1\right\rVert^{\mathrm{e}}}
% Norms Difference
\newcommand{\normInnDiff}[1]{\left\lVert#1\right\rVert}
\newcommand{\normInnDiffSmall}[1]{\lVert#1\lVert}
\newcommand{\normInnDiffExp}[1]{\left\llbracket#1\right\rrbracket}
% Variables
\newcommand{\ZInn}{Z_0}
\newcommand{\ZInnB}{\widetilde{Z}_0}
\newcommand{\ZInnN}{\widehat{Z}_0}
\newcommand{\ZuInn}{Z^{\mathrm{u}}_0}
\newcommand{\ZuInnN}{\widehat{Z}^{\mathrm{u}}_0}
\newcommand{\ZuInnB}{\widetilde{Z}^{\mathrm{u}}_0}
\newcommand{\ZsInn}{Z^{\mathrm{s}}_0}
\newcommand{\ZsInnN}{\widehat{Z}^{\mathrm{s}}_0}
\newcommand{\ZusInn}{Z^{\mathrm{u,s}}_0}
\newcommand{\ZdInn}{Z^{\diamond}_0}
\newcommand{\ZdInnN}{\widehat{Z}^{\diamond}_0}
\newcommand{\WInn}{W_0}
\newcommand{\WInnB}{\widetilde{W}_0}
\newcommand{\WInnN}{\widehat{W}_0}
\newcommand{\WuInn}{W^{\mathrm{u}}_0}
\newcommand{\WuInnB}{\widetilde{W}^{\mathrm{u}}_0}
\newcommand{\WsInn}{W^{\mathrm{s}}_0}
\newcommand{\WusInn}{W^{\mathrm{u,s}}_0}
\newcommand{\WdInn}{W^{\diamond}_0}
\newcommand{\WdInnN}{\widehat{W}^{\diamond}_0}
\newcommand{\XInn}{X_0}
\newcommand{\XInnB}{\widetilde{X}_0}
\newcommand{\XInnN}{\widehat{X}_0}
\newcommand{\XuInn}{X^{\mathrm{u}}_0}
\newcommand{\XuInnB}{\widetilde{X}^{\mathrm{u}}_0}
\newcommand{\XsInn}{X^{\mathrm{s}}_0}
\newcommand{\XusInn}{X^{\mathrm{u,s}}_0}
\newcommand{\XdInn}{X^{\diamond}_0}
\newcommand{\XdInnN}{\widehat{X}^{\diamond}_0}
\newcommand{\YInn}{Y_0}
\newcommand{\YInnB}{\widetilde{Y}_0}
\newcommand{\YInnN}{\widehat{Y}_0}
\newcommand{\YuInn}{Y^{\mathrm{u}}_0}
\newcommand{\YuInnB}{\widetilde{Y}^{\mathrm{u}}_0}
\newcommand{\YsInn}{Y^{\mathrm{s}}_0}
\newcommand{\YusInn}{Y^{\mathrm{u,s}}_0}
\newcommand{\YdInn}{Y^{\diamond}_0}
\newcommand{\YdInnN}{\widehat{Y}^{\diamond}_0}
% Diference variables
\newcommand{\DZInn}{\Delta Z_0}
\newcommand{\DWInn}{\Delta W_0}
\newcommand{\DXInn}{\Delta X_0}
\newcommand{\DYInn}{\Delta Y_0}
\newcommand{\DZInnN}{\Delta \widehat{Z}_0}
\newcommand{\DWInnN}{\Delta \widehat{W}_0}
\newcommand{\DXInnN}{\Delta \widehat{X}_0}
\newcommand{\DYInnN}{\Delta \widehat{Y}_0}
\newcommand{\DZo}{\Delta Z_{\mathrm{init}}}
\newcommand{\DWo}{\Delta W_{\mathrm{init}}}
\newcommand{\DXo}{\Delta X_{\mathrm{init}}}
\newcommand{\DYo}{\Delta Y_{\mathrm{init}}}
\newcommand{\tDZo}{\widetilde{\Delta Z}_{\mathrm{init}}}
\newcommand{\tDWo}{\widetilde{\Delta W}_{\mathrm{init}}}
\newcommand{\tDXo}{\widetilde{\Delta X}_{\mathrm{init}}}
\newcommand{\tDYo}{\widetilde{\Delta Y}_{\mathrm{init}}}

%%%% OUTER SPACE %%%
\newcommand{\out}{\mathrm{sep}}
% Domain
\newcommand{\DOut}{{D}_{\kappa,\beta}^{\mathrm{sep}}}
\newcommand{\DuOut}{{D}_{\kappa,\beta}^{\mathrm{sep,u}}}
\newcommand{\DsOut}{{D}_{\kappa,\beta}^{\mathrm{sep,s}}}
\newcommand{\DusOut}{{D}_{\kappa,\beta}^{\mathrm{sep,u/s}}}
\newcommand{\DdOut}{{D}_{\kappa,\beta}^{\mathrm{sep,}\diamond}}
% Variables
\newcommand{\zOut}{z}
\newcommand{\zOutB}{\widetilde{z}}
\newcommand{\zuOut}{z^{\mathrm{u}}}
\newcommand{\zuOutB}{\widetilde{z}^{\mathrm{u}}}
\newcommand{\zsOut}{z^{\mathrm{s}}}
\newcommand{\zusOut}{z^{\mathrm{u,s}}}
\newcommand{\zdOut}{z^{\diamond}}
\newcommand{\wOut}{w}
\newcommand{\wOutB}{\widetilde{w}}
\newcommand{\wuOut}{w^{\mathrm{u}}}
\newcommand{\wuOutB}{\widetilde{w}^{\mathrm{u}}}
\newcommand{\wsOut}{w^{\mathrm{s}}}
\newcommand{\wdOut}{w^{\diamond}}
\newcommand{\xOut}{x}
\newcommand{\xOutB}{\widetilde{x}}
\newcommand{\xuOut}{x^{\mathrm{u}}}
\newcommand{\xuOutB}{\widetilde{x}^{\mathrm{u}}}
\newcommand{\xsOut}{x^{\mathrm{s}}}
\newcommand{\xdOut}{x^{\diamond}}
\newcommand{\yOut}{y}
\newcommand{\yOutB}{\widetilde{y}}
\newcommand{\yuOut}{y^{\mathrm{u}}}
\newcommand{\yuOutB}{\widetilde{y}^{\mathrm{u}}}
\newcommand{\ysOut}{y^{\mathrm{s}}}
\newcommand{\ydOut}{y^{\diamond}}
% Stable/ Unstable
\newcommand{\wu}{w^{\mathrm{u}}}
\newcommand{\xu}{x^{\mathrm{u}}}
\newcommand{\yu}{y^{\mathrm{u}}}
\newcommand{\zu}{z^{\mathrm{u}}}
% Diference variables
\newcommand{\dzOut}{\Delta z}
\newcommand{\dwOut}{\Delta w}
\newcommand{\dxOut}{\Delta x}
\newcommand{\dyOut}{\Delta y}
% Change of coordinates
\newcommand{\lauOut}{\lambda^{\mathrm{u}}}
\newcommand{\LauOut}{\Lambda^{\mathrm{u}}}


%%%% CONSTANTS ARTICLE INNER %%%
% Main Results - Reformulation
%\newcommand{\cttInnPoiA}{b_0}
% Main Results - Derivation Inner
\newcommand{\cttInnDerA}{c_1}
\newcommand{\cttInnDerAA}{\gamma_1}
\newcommand{\cttInnDerB}{c_2}
\newcommand{\cttInnDerBB}{\gamma_2}
\newcommand{\cttInnDerC}{b_0}
% Main Results - Analysis Inner
\newcommand{\cttInnExist}{b_1}
\newcommand{\cttInnDiff}{b_2}
% Proof Inner Computation
\newcommand{\cttInnExistA}{b_3}
\newcommand{\cttInnExistB}{b_4}
\newcommand{\cttInnExistC}{b_5}
\newcommand{\cttInnDiffA}{b_6}
\newcommand{\cttInnDiffB}{b_7}

==> Article Inner/singularScaling.tex <==
\paragraph{A singular scaling.}
%\label{subsection:changeCoordinates}
% Let us take into account the two time scales of the system, as given by the eigenvalues in~\eqref{eq:specRot}, by a factor of order $\sqrt{\mu}$.
%
We consider the parameter
\begin{equation*}%\label{def:delta}
	\de= \mu^{\frac{1}{4}}
\end{equation*}
%
and we define the  symplectic scaling 
%
\begin{equation}\label{def:changeScaling}
\phi_{\sca}:
(\la, \La, \xh,  \yh) 
 \mapsto 
(\la,L,\eta,\xi),
\qquad
L = 1 + \de^2 \La , \quad
\eta = \de \xh , \quad
\xi = \de \yh , \quad
\end{equation}
%given by
%\begin{equation*}
%	L = 1 + \de^2 \La , \qquad
%	\eta = \de \xh , \qquad
%	\xi = \de \yh , \qquad
%	t = \de^{-4} \tau,
%\end{equation*}
and the time reparameterization $t = \de^{-2} \tau$. The transformed equations are Hamiltonian with respect to the Hamiltonian
\[
\de^{-4} \paren{ H_0^{\Poi} \circ \phi_{\sca}}+\paren{H_1^{\Poi} \circ \phi_{\sca} }
\]
and the symplectic form $d\la\wedge d\Lambda+idx\wedge dy$.  The Hamiltonian (up to a constant) satisfies
\begin{align*}
\de^{-4} \paren{ H_0^{\Poi} \circ \phi_{\sca}} &=-\frac{3}{2}\La^2 
+ \frac{1}{\de^4} F_{\pend}(\de^2\La)
+ \frac{\xh\yh}{\de^2}, \\
%
\paren{H_1^{\Poi} \circ \phi_{\sca} }&=
V(\la) + \OO(\de),
\end{align*}
with 
\begin{equation}\label{def:Fpend}
\begin{split}
V(\la) &=  H_1^{\Poi}(\la,1,0,0;0),\\
F_{\pend}(z)& = \paren{-\frac{1}{2(1+z)^2}-(1+z)}+\frac{3}{2} + \frac{3}{2}z^2 = \OO(z^3).
\end{split}
\end{equation}
The function $V(\la)$, which we call the potential, has an explicit formula:
\begin{equation}\label{def:potentialV}
V(\la) =  H_1^{\pol}(1,\la;0)
= 1 - \cos \la - \frac{1}{\sqrt{2+2\cos \la}},
\end{equation}
where $H_1^{\pol}$ is defined in~\eqref{def:hamiltonianPolarsSplitting}.
%
Indeed, taking $\de=0$ on the change of coordinates~\eqref{def:changeScaling}, we have that $(\la,L,\eta,\xi)=(\la,1,0,0)$.
%
%These coordinates, on Delaunay variables, correspond with a circular orbit, $e=0$, and with the equivalence of the three anomalies, $\ell=u=f$.
%
These coordinates, correspond with a circular orbit, $e=0$, and applying~\eqref{eq:rthetaDefinition} and \eqref{eq:thetaDefinition}, we obtain that $(r,\tht)=(1,\la)$.
%

We summarize the previous results in the following theorem.

\begin{theorem}\label{theorem:HamiltonianScaling}
The Hamiltonian system given by $h$ in~\eqref{def:hamiltonianInitialNotSplit} expressed in coordinates $(\la,\La,x,y)$
defines a Hamiltonian system with respect to the symplectic form $d\la \wedge d\La + i dx \wedge dy$ 
%
and the Hamiltonian
\begin{equation} \label{def:hamiltonianScaling}
\begin{split}
{H} = 
{H}_{\pend} + 
{H}_{\osc} + 
H_1,
\end{split}
\end{equation}
with 
\begin{align} 
&{H}_{\pend}(\la,\La) = -\frac{3}{2} \La^2  + V(\la), \qquad
% 
{H}_{\osc}(x,y; \de) = \frac{x y}{\de^2}, 
\label{def:HpendHosc}\\
%
&H_1(\la,\La,\xh,\yh;\de) =
\paren{H_1^{\Poi} \circ \phi_{\sca}}  - V(\la) + \frac{1}{\de^4} F_{\pend}(\de^2\La),
\label{def:hamiltonianScalingH1}
\end{align}
and $H_1^{\Poi}$, $F_{\pend}$ and $V$ defined in
\eqref{def:hamiltonianPoincareSplitting},
\eqref{def:Fpend}
and
\eqref{def:potentialV}, respectively.
%
Moreover, the Hamiltonian $H$ is real-analytic\footnote{
	Real-analytic in the sense of $\conj{H(\la,\La,x,y;\de)}= H(\conj{\la},\conj{\La},y,x;\conj{\de}).$} 
away from collision with the primaries. 

Moreover, for $\de > 0$ small enough:
\begin{itemize}
\item The critical point $L_3$ (see~\eqref{def:pointL3}) expressed in  coordinates $(\la,\La,x,y)$ is given by
\begin{equation}\label{def:pointL3sca}
\Ltres(\de)=\paren{0,
	\de^2 \LtresLa(\de),
	\de^3 \Ltresx(\de),
	\de^3 \Ltresy(\de)},
\end{equation}
with $\vabs{\LtresLa(\de)}$, $\vabs{\Ltresx(\de)}$, $\vabs{\Ltresy(\de)} \leq C$, for some constant $C>0$ independent of $\de$.
%
\item The point $\Ltres(\de)$ is a saddle-center equilibrium point and its linear part is
\begin{equation*}
	\begin{pmatrix}
		0 & -3 & 0 & 0 \\
		-\frac{7}{8} & 0 & 0 & 0 \\
		0 & 0 & \frac{i}{\de^2} & 0 \\
		0 & 0 & 0 & -\frac{i}{\de^2}
	\end{pmatrix} + \OO(\de).
\end{equation*}
Therefore, it possesses one-dimensional stable and unstable manifolds and a two- dimensional center manifold.
%\item For $(L,\eta,\xi) \sim (1,0,0)$, $\vabs{\Im \la}<C$ and $\vabs{\la-\pi}>C$
%the Hamiltonian $H$ is real-analytic in the sense of 
%\[
%\conj{H(\la,\La,x,y;\de)}=
%H(\conj{\la},\conj{\La},y,x;\de).
%\]
%%%%%
%	\item Fix $\varrho\geq 0$.
%	%
%	There exists $\nu_0=\nu_0(\de)>0$ (not necessarily small) such that for all $\nu \in (0,\nu_0)$, 
%	the Hamiltonian $H$ is real-analytic in the sense of 
%	\[
%	\conj{H(\la,\La,x,y;\de)}=
%	H(\conj{\la},\conj{\La},y,x;\de),
%	\]
%	for $\vabs{(\La,x,y)}\leq \nu$, 
%	$\vabs{\Im \la}\leq \varrho$ and 
%	$\vabs{\la-\pi}>\cttInnPoiA$
%	where $\cttInnPoiA=\cttInnPoiA(\de,\nu)$ a positive constant.
\end{itemize}
\end{theorem}
%with
%\begin{equation}\label{def:Fpend}
%F_{\pend}(z) = \paren{-\frac{1}{2(1+z)^2}-(1+z)}+\frac{3}{2} + \frac{3}{2}z^2 \sim \OO(z^3).
%\end{equation}
%Notice that $\mathbf{0}$ is saddle-center of this system. 
% specifically a  non-degenerated saddle, as we wanted to obtain.
%Notice that the order of variables for the symplectic form has been altered after this change. See Appendix~\ref{appendixC} for the details.   \\
%
The proof of Theorem~\ref{theorem:HamiltonianScaling} follows from the results obtained through Section~\ref{subsection:reformulation}.


Since the original Hamiltonian is symmetric with respect to the involution ${\Phi}$ in~\eqref{def:involutionCartesians}, the Hamiltonian $H$ is reversible with respect to the involution 
\begin{equation}\label{def:involutionScaling}
	\wt{\Phi}(\la,\La,x,y) = (-\la,\La,y,x).
\end{equation}
From now on, we consider as ``new'' unperturbed Hamiltonian
\begin{equation}\label{def:hamiltonianScalingH0}
{H}_0(\la,\La,\xh,\yh;\de) = {H}_{\pend}(\la,\La) + {H}_{\osc}(\xh,\yh; \de),
\end{equation}
which corresponds to an uncoupled pendulum-like  Hamiltonian ${H}_{\pend}$ and an oscillator ${H}_{\osc}$, and  we refer
to $H_1$ as the perturbation.
%
%Notice that the center possesses a different time scale with respect to the saddle (by a factor ${\de^{-2}}$, see~\eqref{eq:specRot}). 
%
%Thus, $H_0$ has a rapidly rotating term and, as a consequence, the splitting of separatrices phenomenon resulting will be exponentially small.
%


%The remaining part of this work is devoted to study the behavior of the analytical continuation of the  stable and unstable manifolds of $\Ltres(\de)$.

%
%We define as well a new perturbative term
%\begin{equation}\label{def:hamiltonianScalingH1}
%H_1 = H_1^S + H_1^J + R.
%\end{equation}
%To check that this term is small with relation to $\de$, we compute the order of $P^*(\de)$. 
 
%
%Moreover, if we write the differential equations as $\zd = {{F}_{\wt{H}_{0}}(z)}$, then the spectrum of the linear part of the vector field is
%\begin{equation*}
%\mathrm{Spec} \left\{ DF_{\wt{H}_{0}}(\wt{L}_3) \right\} = \left\{ \pm \sqrt{\frac{21}{8}}, \h \pm \frac{i}{\de^2}\right\}.
%\end{equation*}
%Thus, decomposing the hyperbolic and elliptic components, we have that the saddle is given on the projection on variables $(\la,\La)$ and the center on the projection on $(x,y)$. 

%Let us introduce first a result to express the equilibrium point $L_3^{\mu}$ in Poincar\'e coordinates. To simplify notation, we define the parameter $\de:= \mu^{\frac{1}{4}}$.
%\begin{lemma}\label{lemma:puntFixL3}
%	It exists $\de_0>0$, such that for $\de \in (0,\de_0)$, we have that
%	\[
%	\phi_{\Poi}(L_3^{\mu})= (0,1,0,0) +
%	\Big(\de^2 \la^*(\de), \de^4 \La^*(\de), 
%	\de^4 \xi^*(\de), \de^4 \eta^*(\de)\Big),
%	\]
%%	such that
%%	\begin{align*}
%%	& P_{\la}(\de) = \pi + \de^2 \la^*(\de), 
%%	& P_{x}(\de) = \de^3 x^*(\de), \\
%%	& P_{\La}(\de) = \de^2 \La^*(\de), 
%%	& P_{y}(\de) = \de^3 y^*(\de),
%%	\end{align*}
%	with
%	\begin{align*}
%	\vabs{\la^*(\de)} \leq C, \hh 
%	\vabs{\La^*(\de)} \leq C, \hh
%	\vabs{\eta^*(\de)} \leq C, \hh 
%	\vabs{\xi^*(\de)} \leq C.
%	\end{align*}
%%	\begin{align*}
%%	\norm{\la^*}_{\CC^1(0,\de_0)} \leq C, \hh 
%%	\norm{\La^*}_{\CC^1(0,\de_0)} \leq C, \hh
%%	\norm{x^*}_{\CC^1(0,\de_0)} \leq C, \hh 
%%	\norm{y^*}_{\CC^1(0,\de_0)} \leq C.
%%	\end{align*}
%\end{lemma}
%\begin{proof}
%This result is obtained by applying the implicit function theorem on the system given by Hamiltonian~\eqref{def:hamiltonianPoincare}. 
%\end{proof}


==> Article Inner/singularities.tex <==

In this section we analyze the 1-degree of freedom Hamiltonian ${H}_{\pend}(\la,\La)$ introduced in~\eqref{def:HpendHosc},
\begin{equation*}
{H}_{\pend}(\la,\La) = -\frac{3}{2} \La^2  + V(\la), \qquad
V(\la) = 1 - \cos \la - \frac{1}{\sqrt{2+2\cos \la}},
\end{equation*}
and the associated Hamiltonian system
\begin{equation} \label{eq:sistemODEs}
\dot \la= -3\La, \qquad
%
\dot \La=-\sin \la \left(1-\frac{1}{(2+2\cos\la)\efr{3}{2}
}\right),
\end{equation}
This Hamiltonian system has a singularity at $\la=\pi$, which corresponds to the collision with the small primary $P$, and a saddle at $(\la,\La)=(0,0)$ with two homoclinic connections or separatrices, see  Figure~\ref{fig:separatrix}.
%
\begin{figure} 
	\centering
	\begin{overpic}[scale=0.75]{mainSeparatrixPicture.png}
		\put(93,31){{$\pi$}}
		\put(77,29){{$\frac{2}{3}\pi$}}
		\put(49,29){{$0$}}
		\put(17,29){{$-\frac{2}{3}\pi$}}
		\put(-2,31){{ $-\pi$}}
		\put(98,34){{$\la$}}
		\put(5,70){{$\La$}}
	\end{overpic}
	\bigskip
	\caption{Phase portrait of equation~\eqref{eq:sistemODEs}. On blue the two separatrices.}
	\label{fig:separatrix}
\end{figure}
%Then, considering the trigonometric identity $1+\cos(\la)=2\cos^2(\frac{\la}{2})$, these homoclinic orbits satisfy
%\begin{equation}\label{eq:odeSeparatrix}
%	\dot{\la}^2 = 15 - 12\cos^2\paren{\frac{\la}{2}}
%	- \frac{3}{\cos\paren{\frac{\la}{2}}}.
%\end{equation}
From now on, we only consider the separatrix on the right; by symmetry (see \eqref{def:involutionScaling}), the results obtained below are analogous for the separatrix on the left. 
%We are interested in studying the analytic continuation of the time parametrization of this separatrix.
%Let us only consider the separatrix on the right.

We consider the real-analytic time parametrization of the separatrix,
\begin{equation}\label{eq:separatrixParametrization}
\begin{split}
	\s:\reals &\to \torus \times \reals \\
		t &\mapsto \s(t)=(\la_h(t),\La_h(t)),
\end{split}
\end{equation}
with initial condition 
\[
\s(0)=(\la_0,0) 
\quad \text{ where } \quad 
\la_0 \in \left(\frac{2}{3}\pi,\pi\right).
\]
% This parametrization satisfies equation~\eqref{eq:sistemODEs} and the asymptotic condition
% \begin{equation*} \label{eq:conditionSeparatrix}
% 	\lim_{t\to \pm \infty } \s(t) = (0,0).
% \end{equation*}
%We present the first result which deals with the analyticity domain of $\s(t)$.
\begin{theorem}\label{theorem:singularities}
	The real-analytic time parametrization $\s$ in~\eqref{eq:separatrixParametrization} satisfies:
	\begin{itemize}
	\item It extends analytically to the strip
	\begin{equation}\label{def:PiA}
	\Pi_A = \{ t \in \complexs \st  |\Im t|< A \},
	\end{equation}
	where 
	\begin{equation}\label{def:integralA}
	A= \int_0^{a_+} \frac{1}{1-x}\sqrt\frac{x}{3(x+1)(a_+-x)(x-a_-)}  dx
	\approx 0.177744,
	\end{equation}
	with 
	$ %\label{def:apm}
	a_{\pm}=-\frac{1}{2}\pm\frac{\sqrt{2}}{2}.
	$
%	such that $A \in [\frac{3}{50},\frac{3}{10}]$. 
	\item It has only two singularities in $\partial \Pi_A$ at $t=\pm iA$.
	%
	\item There exists $\nu>0$ such that,  for $t \in \complexs$ with $\vabs{t -iA}<\nu$ and $\arg(t -iA) \in (-\frac{3\pi}{2},\frac{\pi}{2})$, $\s(t)=(\la_h(t),\La_h(t))$ can be expressed as
	\begin{equation}\label{eq:homoclinicaSingularities}
	\begin{split}
	&\la_h(t) =  \pi + 3\al_{+} (t- iA)^{\frac{2}{3}} + \OO(t- iA)^{\frac{4}{3}}, \\[0.5em]
	&\La_h(t) =  -\frac{ 2 \al_{+}}{3} \frac{1}{(t- iA)^{\frac{1}{3}}} + 
	\OO(t- iA)^{\frac{1}{3}}, 
	\end{split}
	\end{equation}
with $\al_{+} \in \complexs$ such that $\al_{+}^3=\frac{1}{2}$. 
%


An analogous result holds for $\vabs{t+iA}<\nu$, $\arg(t+iA) \in(-\frac{\pi}{2},\frac{3\pi}{2})$ and $\al_- = \conj{\al_+}$.
\end{itemize}
\end{theorem}

%
% Notice that $A$ is a positive constant that can be computed with any degree of accuracy.
%Using mathematical software. we have obtained $A \approx 0.177744$.
%Moreover, following the same arguments from the proof of Theorem~\ref{theorem:singularities}, see Section~\ref{section:proofA-singularities}, we obtain the next technical result:
%\textcolor{red}{Argumentacio de que $\La_h(u)=0$ nomes per $u=0$ a $\Pi_A$. Per despres poder definir be els dominis outer.}
%

We can also describe the zeroes of $\La_h(t)$ in $\ol{\Pi_A}$. 

% This analysis is not fundamental to analyze the splitting of separatrices. However, since the approach to perform such analysis 

\begin{proposition}\label{proposition:domainSeparatrix}
	Consider the real-analytic time parametrization $\s(t)=(\la_h(t),\La_h(t))$ and the domain $\Pi_A$ defined in~\eqref{eq:separatrixParametrization}
	and \eqref{def:PiA} respectively.
	%
	Then, $\La_h(t)$ has only one zero in $\ol{\Pi_A}$ at $t=0$.
%	\[
%	t=0 \h \text{ and } \h t=\pm B \pm iA,
%	\]
%	where $A$ is the constant given in~\eqref{def:integralA} and
%	%$B$ is a fixed positive real constant.
%	\begin{equation}\label{def:constantB}
%		B= \int_{-1}^{0} \frac{1}{1-x}\sqrt\frac{x}{
%			3(x+1)(x-a_+)(x-a_-)}  dx
%		\approx 0.875896.
%	\end{equation}
\end{proposition}

%Notice that the symmetry of the zeroes of $\La_h(t)$ comes from the real-analyticity of the parametrization $\s(t)$ and the reversibility with respect to the involution $\Phi(\la,\La)=(-\la,\La)$.

We can expand the region of analyticity of the time parametrization $\s$.

\begin{corollary}
% Consider the real-analytic time parametrization $\s(t)$ in~\eqref{eq:separatrixParametrization}.
%
There exists $0<\beta<\frac{\pi}{2}$ such that the real-analytic time parametrization $\s(t)$ extends analytically to
\begin{equation}\label{def:dominiBow}
\begin{split}	
\Pi^{\mathrm{ext}}_{A, \beta} =& \claus{
t \in \complexs \st 
\vabs{\Im t} < \tan \beta \, \Re t + A}
\cup \\
&\claus{
t \in \complexs \st 
\vabs{\Im t} < -\tan \beta \, \Re t + A}.
\end{split}
\end{equation}
(See Figure~\ref{fig:dominiBow}). Moreover, 
\begin{enumerate}
\item $\s$ has only two singularities on $\partial \Pi^{\mathrm{ext}}_{A, \beta}$ at 
$t=\pm iA$.
\item $\La_h$ has only one zero in the closure of  $\Pi^{\mathrm{ext}}_{A, \beta}$ at 
$t=0$.
\end{enumerate}
\end{corollary}	

% \textcolor{red}{Revisar:}

\begin{proof}
By~\cite{Fon95}, there exists $T>0$ such that $\s(t)$ is analytic in
$
\claus{\vabs{\Re t} > T}.
$
%
Moreover, applying Theorem~\ref{theorem:singularities},  $\s(t)$ has two branching points at $t=\pm iA$ and can be expressed as in~\eqref{eq:homoclinicaSingularities} in the domains
\[
\textstyle
D_1= \claus{\vabs{t- iA}<\nu, \,
\arg(t -iA) \in \paren{-\frac{3\pi}{2},\frac{\pi}{2}}}\bigcup \claus{\vabs{t+ iA}<\nu, \, \arg(t +iA) \in \paren{-\frac{\pi}{2},\frac{3\pi}{2}}},
\]
for some $\nu>0$. This implies that the only singularities in $D_1$ are at $t=\pm iA$.
%


Thus, we only need to check Item 1 in
\[
\left(\Pi^{\mathrm{ext}}_{A, \beta} \cap 
\claus{\vabs{\Re t} \leq T}\right)\setminus D_1.
\]
To this end, note that, by Theorem~\ref{theorem:singularities},  $\s(t)$ is analytic in the compact set
$
D_2 = \paren{\ol{\Pi_A} \cap
\claus{\vabs{\Re t} \leq T} }
\setminus D_1
$. Therefore, there exists a cover of $\partial D_2$ by open balls centered in $\partial D_2$ where $\s(t)$ is analytic.
%
Moreover, since $\partial D_2$ is compact, it has a finite subcover.
%
This implies that there exists $\eta>0$ such that we can extend the analyticity domain of $\s(t)$ to
$
\paren{{\Pi_{A+\eta}}\cap
\claus{\vabs{\Re t} \leq T} } \setminus D_1
$.
%
In particular, taking $\beta=\arctan ({\eta}/{T})$,
$\s(t)$ is analytic in 
$
({\Pi_{A,\beta}^{\mathrm{ext}} \cap
	\claus{\vabs{\Re t} \leq T} }) \setminus D_1.
$
% Then, since $D_1$ has only two singularities at $t=\pm iA$ which also belong to $\partial \Pi_{A,\beta}^{\mathrm{ext}}$, we have that $\s(t)$ extends analytically to ${\Pi_{A,\beta}^{\mathrm{ext}} \cap	\claus{\vabs{\Re t} \leq T} }$ and has only the singularities $\pm iA$ in its boundary.


The prove of Item 2 follows the same lines.
\end{proof}

\begin{figure} 
	\centering
	\begin{overpic}[scale=0.65]{dominiBow.png}
		\put(101,27.5){{$\Re t$}}
		\put(45.5,59){{$\Im t$}}
		\put(28,30){{$\beta$}}
		\put(43,45){{$iA$}}
		%\put(40,10){{$-iA$}}
	\end{overpic}
	\bigskip
	\caption{Representation of the domain $\Pi_{A,\beta}^{\mathrm{ext}}$ in~\eqref{def:dominiBow}.}
	\label{fig:dominiBow}
\end{figure}



%The proof of this result is presented in Appendix~\ref{appendixA}. Still, we present here the analysis of the value $A$. Using mathematical software to compute $A$ we obtain:
%\[
%A \approx 0.177744.
%\]
%Moreover, it is possible to analytically bound the value:
%\begin{align*}
%A \leq & \int_0^{a_+} \frac{1}{1-a_+}\sqrt\frac{a_+}{3(0+1)(0-a_-)(a_+-x)} dx \leq \frac{3}{10}.
%% &= \frac{2}{3-\sqrt{2}} \frac{\sqrt{3}}{3} \sqrt{\frac{\sqrt{2}-1}{\sqrt{2}+1}} \int_0^{a_+} \frac{1}{\sqrt{a_+-x}} dx \\
%% &= \frac{2}{3}\frac{\sqrt{3}(\sqrt{2}-1)}{(3-\sqrt{2})} \Big[ -2 \sqrt{a_+-x} \Big]^{x=a_+}_{x=0} 
%% &= \frac{4}{3}\frac{\sqrt{3}(\sqrt{2}-1)}{(3-\sqrt{2})} \sqrt{a_+} 
%% & = \frac{4}{3}\frac{\sqrt{3}(\sqrt{2}-1)}{(3-\sqrt{2})} \sqrt{\frac{\sqrt{2}-1}{2}} 
%% = \frac{2}{3}\sqrt{6}\frac{(\sqrt{2}-1)^{3/2}}{(3-\sqrt{2})} \leq \frac{3}{10}.
%\end{align*}
%And, for the lower bound:
%\begin{align*}
%A \geq & \int_0^{a_+} \frac{1}{1-0}\sqrt\frac{x}{3(a_+ + 1)(a_+ -a_-)(a_+)} dx  \geq \frac{3}{50}.
%% & = \sqrt{\frac{1}{3}\frac{2}{\sqrt{2}+1}\frac{2}{\sqrt{2}-1}\frac{1}{\sqrt{2}}} \int_0^{a_+} \sqrt{x} dx 
%% = \frac{2^{3/4}}{\sqrt{3}} \Big[ \frac{2}{3} t^{3/2}\Big]^{x=a_+}_{x=0}  \\
%% = \frac{2^{7/4}}{3^{3/2}} (a_+)^{3/2} 
%% &= \frac{2^{7/4}}{3^{3/2}} \left(\frac{\sqrt{2}-1}{2}\right)^{3/2} 
%%  = \frac{\sqrt[4]{2}}{3\sqrt{3}} (\sqrt{2}-1)^{\frac{3}{2}} 
%% \geq \frac{3}{50}.
%\end{align*}
%%\end{remark}
%
%%It is worth noticing, that singularities $t^*_{\pm}$ of $\s(t)=(\la(t),\La(t))$ are the only singularities for $\La(t)$ and are zeroes for $\la(t)$.

%% CANVIAR DEFINICIÓ DE ALFA A APPENDIX

%% DEFINICIO INTEGRAL A BEN POSADA.

